Visual Skill Recertification Across Model Changes

Visual skills, programs choosing where a vision-language model looks before clicking, need recertification after model changes. Treating skills as replayable evidence policies, we test replay (the new model re-reads stored views, one request per task) and budgeted re-execution for KEEP/SUSPEND decisions on two desktop grounding benchmarks, with every preregistered maintenance decision frozen before any sealed application was touched. Scope: three models of one provider, two tier changes toward a larger model, one harness, decoding configuration and image contract; cross-family migrations, downgrades and dated snapshots are untested. In this regime skill value changes sign across domains (+10.4 to +17.7 points on ScreenSpot-Pro, -10.4 to 0.0 on our UI-Vision subsample), yet no effect detectably flipped after either model change (post hoc): the comparisons cannot test the case recertification is for. Pooled over skills, replay is close to unbiased where its click agrees with the new model's direct click without drift (partly by that cell's construction; not per skill), and falls short mainly where the old model's zoomed views all missed the target (exploratory). Without flips, fresh-run correction of replay did not pay off: the stratified correction's preregistered equal-budget advantage is not shown beyond the realised pool (two-stage resampling: 16 of 16 intervals against competitors include zero; exploratory), is untested beyond our fixed-count allocation, mostly shrinks once history noise is removed (post hoc), and at exact equal cost does not consistently beat uniform re-evaluation (post hoc). Replay alone scored at least as high as every per-skill, fixed-fraction budgeted policy (post hoc): the old decision reached the sealed-test oracle in 3 of 4 settings while pool estimates transferred imperfectly; in the fourth, replay's pessimism suspended harmful skills.

==> numbers.tex <==
% Generated by research/analysis/export_numbers.py from research/analysis/exports/numbers.json; do not edit by hand.
\makeatletter
\newcommand{\val}[1]{\csname val@#1\endcsname}
\newcommand{\pct}[1]{\csname pct@#1\endcsname}
\newcommand{\ppt}[1]{\csname ppt@#1\endcsname}
\newcommand{\cnt}[1]{\csname cnt@#1\endcsname}
\expandafter\def\csname val@all.records.api-calls\endcsname{133390}
\expandafter\def\csname cnt@all.records.api-calls\endcsname{133{,}390}
\expandafter\def\csname pct@all.records.api-calls\endcsname{13339000.0}
\expandafter\def\csname ppt@all.records.api-calls\endcsname{$+$13339000.0}
\expandafter\def\csname val@all.records.cache-creation-input-tokens\endcsname{733210313}
\expandafter\def\csname cnt@all.records.cache-creation-input-tokens\endcsname{733{,}210{,}313}
\expandafter\def\csname pct@all.records.cache-creation-input-tokens\endcsname{73321031300.0}
\expandafter\def\csname ppt@all.records.cache-creation-input-tokens\endcsname{$+$73321031300.0}
\expandafter\def\csname val@all.records.cache-read-input-tokens\endcsname{4756281777}
\expandafter\def\csname cnt@all.records.cache-read-input-tokens\endcsname{4{,}756{,}281{,}777}
\expandafter\def\csname pct@all.records.cache-read-input-tokens\endcsname{475628177700.0}
\expandafter\def\csname ppt@all.records.cache-read-input-tokens\endcsname{$+$475628177700.0}
\expandafter\def\csname val@all.records.input-tokens\endcsname{256182}
\expandafter\def\csname cnt@all.records.input-tokens\endcsname{256{,}182}
\expandafter\def\csname pct@all.records.input-tokens\endcsname{25618200.0}
\expandafter\def\csname ppt@all.records.input-tokens\endcsname{$+$25618200.0}
\expandafter\def\csname val@all.records.output-tokens\endcsname{23556685}
\expandafter\def\csname cnt@all.records.output-tokens\endcsname{23{,}556{,}685}
\expandafter\def\csname pct@all.records.output-tokens\endcsname{2355668500.0}
\expandafter\def\csname ppt@all.records.output-tokens\endcsname{$+$2355668500.0}
\expandafter\def\csname val@all.records.requests\endcsname{33164}
\expandafter\def\csname cnt@all.records.requests\endcsname{33{,}164}
\expandafter\def\csname pct@all.records.requests\endcsname{3316400.0}
\expandafter\def\csname ppt@all.records.requests\endcsname{$+$3316400.0}
\expandafter\def\csname val@all.records.status.harness-failed\endcsname{6154}
\expandafter\def\csname cnt@all.records.status.harness-failed\endcsname{6{,}154}
\expandafter\def\csname pct@all.records.status.harness-failed\endcsname{615400.0}
\expandafter\def\csname ppt@all.records.status.harness-failed\endcsname{$+$615400.0}
\expandafter\def\csname val@all.records.status.missing-in-journal\endcsname{478}
\expandafter\def\csname cnt@all.records.status.missing-in-journal\endcsname{478}
\expandafter\def\csname pct@all.records.status.missing-in-journal\endcsname{47800.0}
\expandafter\def\csname ppt@all.records.status.missing-in-journal\endcsname{$+$47800.0}
\expandafter\def\csname val@all.records.status.ok\endcsname{26532}
\expandafter\def\csname cnt@all.records.status.ok\endcsname{26{,}532}
\expandafter\def\csname pct@all.records.status.ok\endcsname{2653200.0}
\expandafter\def\csname ppt@all.records.status.ok\endcsname{$+$2653200.0}
\expandafter\def\csname val@all.records.thinking-tokens\endcsname{5662102}
\expandafter\def\csname cnt@all.records.thinking-tokens\endcsname{5{,}662{,}102}
\expandafter\def\csname pct@all.records.thinking-tokens\endcsname{566210200.0}
\expandafter\def\csname ppt@all.records.thinking-tokens\endcsname{$+$566210200.0}
\expandafter\def\csname val@audit.partial-image-reads\endcsname{71}
\expandafter\def\csname cnt@audit.partial-image-reads\endcsname{71}
\expandafter\def\csname pct@audit.partial-image-reads\endcsname{7100.0}
\expandafter\def\csname ppt@audit.partial-image-reads\endcsname{$+$7100.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{7}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{7}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{700.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{$+$700.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{0.429}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{42.9}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{$+$42.9}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{0.429}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{42.9}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{$+$42.9}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{0.036}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{3.6}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{$+$3.6}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{146}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{146}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{14600.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{$+$14600.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{0.890}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{89.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{$+$89.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{0.877}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{87.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{$+$87.7}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0.014}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{1.4}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$+$1.4}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{0.760}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{76.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{$+$76.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.disagree.N\endcsname{33}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.disagree.N\endcsname{33}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.disagree.N\endcsname{3300.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.disagree.N\endcsname{$+$3300.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{0.455}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{45.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{$+$45.5}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{0.424}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{42.4}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{$+$42.4}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0.030}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{3.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{$+$3.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.disagree.share\endcsname{0.172}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.disagree.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.disagree.share\endcsname{17.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.disagree.share\endcsname{$+$17.2}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{6}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{6}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{0.031}
\expandafter\def\csname cnt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{3.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{$+$3.1}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.bias.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.bias.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.bias.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.bias.ci95.1\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.bias.ci95.1\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.bias.ci95.1\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.bias.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.bias.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.bias.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.rho.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.rho.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.rho.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.rho.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.rho.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.rho.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.rho.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.rho.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.rho.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-stable.N\endcsname{38}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-stable.N\endcsname{38}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-stable.N\endcsname{3800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-stable.N\endcsname{$+$3800.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{0.921}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{92.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{$+$92.1}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{0.895}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{89.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{$+$89.5}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.026}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{2.6}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{$+$2.6}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.disagree.N\endcsname{800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.disagree.N\endcsname{$+$800.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.disagree.acc-F\endcsname{0.375}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.disagree.acc-F\endcsname{37.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.disagree.acc-F\endcsname{$+$37.5}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.disagree.acc-R\endcsname{0.375}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.disagree.acc-R\endcsname{37.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.disagree.acc-R\endcsname{$+$37.5}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.tau.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.tau.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.tau.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.tau.ci95.1\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.tau.ci95.1\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.tau.ci95.1\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p1.C.center-d1.tau.mean\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p1.C.center-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.center-d1.tau.mean\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.center-d1.tau.mean\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.bias.ci95.0\endcsname{-0.062}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.bias.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.bias.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.bias.ci95.1\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.bias.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.bias.ci95.1\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.bias.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.bias.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.bias.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.rho.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.rho.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.rho.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.rho.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.rho.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.rho.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.rho.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.rho.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.rho.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-drift.N\endcsname{5}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-drift.N\endcsname{5}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-drift.N\endcsname{500.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-drift.N\endcsname{$+$500.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{0.400}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{40.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{$+$40.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{0.400}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{40.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{$+$40.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-stable.N\endcsname{36}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-stable.N\endcsname{36}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-stable.N\endcsname{3600.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-stable.N\endcsname{$+$3600.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{0.889}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{88.9}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{$+$88.9}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{0.889}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{88.9}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{$+$88.9}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.disagree.acc-F\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.disagree.acc-F\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.disagree.acc-F\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.disagree.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.disagree.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.disagree.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{-0.167}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{$-$16.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{$-$16.7}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.tau.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.tau.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.tau.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.tau.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.tau.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.tau.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p1.C.context-d1.tau.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p1.C.context-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.context-d1.tau.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p1.C.context-d1.tau.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.bias.ci95.0\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.bias.ci95.0\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.bias.ci95.0\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.bias.ci95.1\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.bias.ci95.1\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.bias.ci95.1\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.bias.mean\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.bias.mean\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.bias.mean\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.rho.ci95.0\endcsname{-0.083}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.rho.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.rho.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.rho.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.rho.mean\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.rho.mean\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.rho.mean\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-stable.N\endcsname{37}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-stable.N\endcsname{37}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-stable.N\endcsname{3700.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-stable.N\endcsname{$+$3700.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{0.892}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{89.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{$+$89.2}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{0.811}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{81.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{$+$81.1}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0.081}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{8.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$+$8.1}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.disagree.N\endcsname{8}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.disagree.N\endcsname{8}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.disagree.N\endcsname{800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.disagree.N\endcsname{$+$800.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.disagree.acc-F\endcsname{0.375}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.disagree.acc-F\endcsname{37.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.disagree.acc-F\endcsname{$+$37.5}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.disagree.acc-R\endcsname{0.375}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.disagree.acc-R\endcsname{37.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.disagree.acc-R\endcsname{$+$37.5}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.strata.parse-fail.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.tau.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.tau.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.tau.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.tau.ci95.1\endcsname{0.250}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.tau.ci95.1\endcsname{25.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.tau.ci95.1\endcsname{$+$25.0}
\expandafter\def\csname val@bias.sspro.p1.C.dual-d2.tau.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p1.C.dual-d2.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.dual-d2.tau.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.dual-d2.tau.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.bias.ci95.1\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.bias.ci95.1\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.bias.ci95.1\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.bias.mean\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.bias.mean\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.bias.mean\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.rho.ci95.0\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.rho.ci95.0\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.rho.ci95.0\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.rho.ci95.1\endcsname{0.250}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.rho.ci95.1\endcsname{25.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.rho.ci95.1\endcsname{$+$25.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.rho.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.rho.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.rho.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.agree-stable.N\endcsname{35}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.N\endcsname{35}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.agree-stable.N\endcsname{3500.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.N\endcsname{$+$3500.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{0.857}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{85.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{$+$85.7}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{0.914}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{91.4}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{$+$91.4}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{-0.057}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$5.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$5.7}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.disagree.N\endcsname{11}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.disagree.N\endcsname{11}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.disagree.N\endcsname{1100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.disagree.N\endcsname{$+$1100.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{0.636}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{63.6}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{$+$63.6}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{0.455}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{45.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{$+$45.5}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.182}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{18.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{$+$18.2}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.tau.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.tau.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.tau.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.tau.ci95.1\endcsname{0.271}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.tau.ci95.1\endcsname{27.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.tau.ci95.1\endcsname{$+$27.1}
\expandafter\def\csname val@bias.sspro.p1.C.grid2-d3.tau.mean\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p1.C.grid2-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.grid2-d3.tau.mean\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p1.C.grid2-d3.tau.mean\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.bias.ci95.1\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.bias.ci95.1\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.bias.ci95.1\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.bias.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.bias.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.bias.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.rho.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.rho.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.rho.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.rho.ci95.1\endcsname{0.271}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.rho.ci95.1\endcsname{27.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.rho.ci95.1\endcsname{$+$27.1}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.rho.mean\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.rho.mean\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.rho.mean\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{38}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{38}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{3800.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{$+$3800.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{0.921}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{92.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{$+$92.1}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{0.921}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{92.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{$+$92.1}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.disagree.N\endcsname{7}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.N\endcsname{7}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.disagree.N\endcsname{700.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.N\endcsname{$+$700.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{0.571}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{57.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{$+$57.1}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0.571}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{57.1}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{$+$57.1}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.tau.ci95.0\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.tau.ci95.0\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.tau.ci95.0\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.tau.ci95.1\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.tau.ci95.1\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.tau.ci95.1\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p1.C.zoomclick-d3.tau.mean\endcsname{0.208}
\expandafter\def\csname cnt@bias.sspro.p1.C.zoomclick-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.C.zoomclick-d3.tau.mean\endcsname{20.8}
\expandafter\def\csname ppt@bias.sspro.p1.C.zoomclick-d3.tau.mean\endcsname{$+$20.8}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{0.479}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{47.9}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{$+$47.9}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{0.688}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{68.8}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{$+$68.8}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.center-d1.gain.mean\endcsname{0.208}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.center-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.center-d1.gain.mean\endcsname{20.8}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.center-d1.gain.mean\endcsname{$+$20.8}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.center-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.center-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.center-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.center-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{0.479}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{47.9}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{$+$47.9}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{0.771}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{77.1}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{$+$77.1}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0.458}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{45.8}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{$+$45.8}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.context-d1.gain.mean\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.context-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.context-d1.gain.mean\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.context-d1.gain.mean\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.context-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.context-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.context-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.context-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{0.479}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{47.9}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{$+$47.9}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{0.771}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{77.1}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{$+$77.1}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0.521}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{52.1}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{$+$52.1}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.dual-d2.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.dual-d2.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.dual-d2.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.dual-d2.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{0.479}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{47.9}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{$+$47.9}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{0.771}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{77.1}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{$+$77.1}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0.458}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{45.8}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{$+$45.8}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.grid2-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.grid2-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.grid2-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.grid2-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{0.479}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{47.9}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{$+$47.9}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{0.854}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{85.4}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{$+$85.4}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0.208}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{20.8}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{$+$20.8}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{0.542}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{54.2}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{$+$54.2}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0.375}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{37.5}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{$+$37.5}
\expandafter\def\csname val@bias.sspro.p1.reverse-reader-T.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p1.reverse-reader-T.zoomclick-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p1.reverse-reader-T.zoomclick-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{0.005}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{0.5}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{$+$0.5}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{160}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{160}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{16000.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{$+$16000.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{0.906}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{90.6}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{$+$90.6}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{0.919}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{91.9}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{$+$91.9}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{-0.013}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$-$1.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$-$1.2}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{0.833}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{83.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{$+$83.3}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.disagree.N\endcsname{28}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.disagree.N\endcsname{28}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.disagree.N\endcsname{2800.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.disagree.N\endcsname{$+$2800.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{0.321}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{32.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{$+$32.1}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{0.214}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{21.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{$+$21.4}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0.107}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{10.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{$+$10.7}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.disagree.share\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.disagree.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.disagree.share\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.disagree.share\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{3}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{3}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{300.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{$+$300.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{0.016}
\expandafter\def\csname cnt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{1.6}
\expandafter\def\csname ppt@bias.sspro.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{$+$1.6}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.bias.ci95.1\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.bias.ci95.1\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.bias.ci95.1\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.bias.mean\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.bias.mean\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.bias.mean\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.rho.ci95.0\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.rho.ci95.0\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.rho.ci95.0\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.rho.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.rho.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.rho.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.rho.mean\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.rho.mean\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.rho.mean\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.agree-stable.N\endcsname{42}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.agree-stable.N\endcsname{42}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.agree-stable.N\endcsname{4200.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.agree-stable.N\endcsname{$+$4200.0}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{0.929}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{92.9}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{$+$92.9}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{0.905}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{90.5}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{$+$90.5}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.024}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{2.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{$+$2.4}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.disagree.acc-F\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.disagree.acc-F\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.disagree.acc-F\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.disagree.acc-R\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.disagree.acc-R\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.disagree.acc-R\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.tau.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.tau.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.tau.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.tau.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.tau.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.tau.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.center-d1.tau.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.center-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.center-d1.tau.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.center-d1.tau.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.bias.ci95.1\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.bias.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.bias.ci95.1\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.bias.mean\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.bias.mean\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.bias.mean\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.rho.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.rho.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.rho.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.rho.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.rho.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.rho.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.rho.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.rho.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.rho.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-stable.N\endcsname{40}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-stable.N\endcsname{40}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-stable.N\endcsname{4000.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-stable.N\endcsname{$+$4000.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{0.950}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{95.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{$+$95.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{0.950}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{95.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{$+$95.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.disagree.N\endcsname{7}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.disagree.N\endcsname{7}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.disagree.N\endcsname{700.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.disagree.N\endcsname{$+$700.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.disagree.acc-F\endcsname{0.143}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.disagree.acc-F\endcsname{14.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.disagree.acc-F\endcsname{$+$14.3}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.disagree.acc-R\endcsname{0.143}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.disagree.acc-R\endcsname{14.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.disagree.acc-R\endcsname{$+$14.3}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.tau.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.tau.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.tau.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.tau.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.tau.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.tau.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.context-d1.tau.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.context-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.context-d1.tau.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.context-d1.tau.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.bias.ci95.0\endcsname{-0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.bias.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.bias.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.bias.ci95.1\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.bias.ci95.1\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.bias.ci95.1\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.bias.mean\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.bias.mean\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.bias.mean\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.rho.ci95.0\endcsname{-0.083}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.rho.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.rho.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.rho.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.rho.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.rho.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.rho.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.agree-stable.N\endcsname{39}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.agree-stable.N\endcsname{39}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.agree-stable.N\endcsname{3900.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.agree-stable.N\endcsname{$+$3900.0}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{0.821}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{82.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{$+$82.1}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{0.872}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{87.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{$+$87.2}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{-0.051}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$-$5.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$-$5.1}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.disagree.N\endcsname{9}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.disagree.N\endcsname{9}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.disagree.N\endcsname{900.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.disagree.N\endcsname{$+$900.0}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.disagree.acc-F\endcsname{0.667}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.disagree.acc-F\endcsname{66.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.disagree.acc-F\endcsname{$+$66.7}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.disagree.acc-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.disagree.acc-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.disagree.acc-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.tau.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.tau.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.tau.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.tau.ci95.1\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.tau.ci95.1\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.tau.ci95.1\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p2.C.dual-d2.tau.mean\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.C.dual-d2.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.dual-d2.tau.mean\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.dual-d2.tau.mean\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.bias.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.bias.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.bias.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.bias.ci95.1\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.bias.ci95.1\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.bias.ci95.1\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.bias.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.bias.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.bias.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.rho.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.rho.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.rho.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.rho.ci95.1\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.rho.ci95.1\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.rho.ci95.1\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.rho.mean\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.rho.mean\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.rho.mean\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.agree-stable.N\endcsname{39}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.N\endcsname{39}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.agree-stable.N\endcsname{3900.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.N\endcsname{$+$3900.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{0.923}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{92.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{$+$92.3}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{0.949}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{94.9}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{$+$94.9}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{-0.026}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$2.6}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$2.6}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.parse-fail.N\endcsname{3}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.N\endcsname{3}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.parse-fail.N\endcsname{300.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.N\endcsname{$+$300.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.tau.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.tau.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.tau.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.tau.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.tau.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.tau.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.grid2-d3.tau.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.grid2-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.grid2-d3.tau.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.grid2-d3.tau.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.bias.ci95.1\endcsname{0.188}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.bias.ci95.1\endcsname{18.8}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.bias.ci95.1\endcsname{$+$18.8}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.bias.mean\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.bias.mean\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.bias.mean\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.rho.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.rho.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.rho.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.rho.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.rho.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.rho.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.rho.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.rho.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.rho.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{41}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{41}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{4100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{$+$4100.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{0.927}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{92.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{$+$92.7}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{0.927}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{92.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{$+$92.7}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{0.667}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{66.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{$+$66.7}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.tau.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.tau.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.tau.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.tau.ci95.1\endcsname{0.271}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.tau.ci95.1\endcsname{27.1}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.tau.ci95.1\endcsname{$+$27.1}
\expandafter\def\csname val@bias.sspro.p2.C.zoomclick-d3.tau.mean\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.C.zoomclick-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.C.zoomclick-d3.tau.mean\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.C.zoomclick-d3.tau.mean\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{6}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{6}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{0.016}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{1.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{$+$1.6}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{334}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{334}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{33400.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{$+$33400.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{0.937}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{93.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{$+$93.7}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{0.928}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{92.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{$+$92.8}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0.009}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$+$0.9}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{0.870}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{87.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{$+$87.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.disagree.N\endcsname{41}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.disagree.N\endcsname{41}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.disagree.N\endcsname{4100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.disagree.N\endcsname{$+$4100.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{0.707}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{70.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{$+$70.7}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{0.610}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{61.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{$+$61.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0.098}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{9.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{$+$9.8}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.disagree.share\endcsname{0.107}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.disagree.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.disagree.share\endcsname{10.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.disagree.share\endcsname{$+$10.7}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{3}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{3}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{300.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{$+$300.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{0.008}
\expandafter\def\csname cnt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{0.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{$+$0.8}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.bias.ci95.0\endcsname{-0.010}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.bias.ci95.0\endcsname{$-$1.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.bias.ci95.0\endcsname{$-$1.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.bias.ci95.1\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.bias.ci95.1\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.bias.ci95.1\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.bias.mean\endcsname{0.031}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.bias.mean\endcsname{3.1}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.bias.mean\endcsname{$+$3.1}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.n\endcsname{96}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.n\endcsname{96}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.rho.ci95.0\endcsname{0.052}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.rho.ci95.0\endcsname{5.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.rho.ci95.0\endcsname{$+$5.2}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.rho.ci95.1\endcsname{0.188}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.rho.ci95.1\endcsname{18.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.rho.ci95.1\endcsname{$+$18.8}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.rho.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.rho.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.rho.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-stable.N\endcsname{87}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-stable.N\endcsname{87}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-stable.N\endcsname{8700.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-stable.N\endcsname{$+$8700.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{0.920}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{92.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{$+$92.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{0.908}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{90.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{$+$90.8}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.011}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{1.1}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{$+$1.1}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.disagree.N\endcsname{800.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.disagree.N\endcsname{$+$800.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.disagree.acc-F\endcsname{0.875}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.disagree.acc-F\endcsname{87.5}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.disagree.acc-F\endcsname{$+$87.5}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.disagree.acc-R\endcsname{0.625}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.disagree.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.disagree.acc-R\endcsname{62.5}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.disagree.acc-R\endcsname{$+$62.5}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.250}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{25.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{$+$25.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.tau.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.tau.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.tau.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.tau.ci95.1\endcsname{0.240}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.tau.ci95.1\endcsname{24.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.tau.ci95.1\endcsname{$+$24.0}
\expandafter\def\csname val@bias.sspro.p2.T.center-d1.tau.mean\endcsname{0.156}
\expandafter\def\csname cnt@bias.sspro.p2.T.center-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.center-d1.tau.mean\endcsname{15.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.center-d1.tau.mean\endcsname{$+$15.6}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.bias.ci95.0\endcsname{-0.062}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.bias.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.bias.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.bias.ci95.1\endcsname{0.021}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.bias.ci95.1\endcsname{2.1}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.bias.ci95.1\endcsname{$+$2.1}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.bias.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.bias.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.bias.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.n\endcsname{96}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.n\endcsname{96}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.rho.ci95.0\endcsname{0.073}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.rho.ci95.0\endcsname{7.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.rho.ci95.0\endcsname{$+$7.3}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.rho.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.rho.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.rho.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.rho.mean\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.rho.mean\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.rho.mean\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-stable.N\endcsname{86}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-stable.N\endcsname{86}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-stable.N\endcsname{8600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-stable.N\endcsname{$+$8600.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{0.907}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{90.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{$+$90.7}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{0.930}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{93.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{$+$93.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{-0.023}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{$-$2.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{$-$2.3}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.disagree.N\endcsname{800.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.disagree.N\endcsname{$+$800.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.disagree.acc-F\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.disagree.acc-F\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.disagree.acc-F\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.disagree.acc-R\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.disagree.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.disagree.acc-R\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.disagree.acc-R\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.tau.ci95.0\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.tau.ci95.0\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.tau.ci95.0\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.tau.ci95.1\endcsname{0.208}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.tau.ci95.1\endcsname{20.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.tau.ci95.1\endcsname{$+$20.8}
\expandafter\def\csname val@bias.sspro.p2.T.context-d1.tau.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p2.T.context-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.context-d1.tau.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p2.T.context-d1.tau.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.bias.ci95.1\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.bias.ci95.1\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.bias.ci95.1\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.bias.mean\endcsname{0.052}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.bias.mean\endcsname{5.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.bias.mean\endcsname{$+$5.2}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.n\endcsname{96}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.n\endcsname{96}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.rho.ci95.0\endcsname{0.010}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.rho.ci95.0\endcsname{1.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.rho.ci95.0\endcsname{$+$1.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.rho.ci95.1\endcsname{0.208}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.rho.ci95.1\endcsname{20.8}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.rho.ci95.1\endcsname{$+$20.8}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.rho.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.rho.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.rho.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-stable.N\endcsname{82}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-stable.N\endcsname{82}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-stable.N\endcsname{8200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-stable.N\endcsname{$+$8200.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{0.976}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{97.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{$+$97.6}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{0.927}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{92.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{$+$92.7}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0.049}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{4.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$+$4.9}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.disagree.N\endcsname{12}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.disagree.N\endcsname{12}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.disagree.N\endcsname{1200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.disagree.N\endcsname{$+$1200.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.disagree.acc-F\endcsname{0.583}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.disagree.acc-F\endcsname{58.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.disagree.acc-F\endcsname{$+$58.3}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.disagree.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.disagree.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.disagree.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.tau.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.tau.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.tau.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.tau.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.tau.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.tau.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@bias.sspro.p2.T.dual-d2.tau.mean\endcsname{0.156}
\expandafter\def\csname cnt@bias.sspro.p2.T.dual-d2.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.dual-d2.tau.mean\endcsname{15.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.dual-d2.tau.mean\endcsname{$+$15.6}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.bias.ci95.0\endcsname{-0.010}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.bias.ci95.0\endcsname{$-$1.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.bias.ci95.0\endcsname{$-$1.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.bias.ci95.1\endcsname{0.094}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.bias.ci95.1\endcsname{9.4}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.bias.ci95.1\endcsname{$+$9.4}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.bias.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.bias.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.bias.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.n\endcsname{96}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.n\endcsname{96}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.rho.ci95.0\endcsname{0.052}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.rho.ci95.0\endcsname{5.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.rho.ci95.0\endcsname{$+$5.2}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.rho.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.rho.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.rho.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.rho.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.rho.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.rho.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-stable.N\endcsname{79}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.N\endcsname{79}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-stable.N\endcsname{7900.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.N\endcsname{$+$7900.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{0.949}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{94.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{$+$94.9}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{0.949}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{94.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{$+$94.9}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.disagree.N\endcsname{13}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.disagree.N\endcsname{13}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.disagree.N\endcsname{1300.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.disagree.N\endcsname{$+$1300.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{0.692}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{69.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{$+$69.2}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{0.615}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{61.5}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{$+$61.5}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.077}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{7.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{$+$7.7}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.parse-fail.N\endcsname{3}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.N\endcsname{3}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.parse-fail.N\endcsname{300.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.N\endcsname{$+$300.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.tau.ci95.0\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.tau.ci95.0\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.tau.ci95.0\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.tau.ci95.1\endcsname{0.240}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.tau.ci95.1\endcsname{24.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.tau.ci95.1\endcsname{$+$24.0}
\expandafter\def\csname val@bias.sspro.p2.T.grid2-d3.tau.mean\endcsname{0.146}
\expandafter\def\csname cnt@bias.sspro.p2.T.grid2-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.grid2-d3.tau.mean\endcsname{14.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.grid2-d3.tau.mean\endcsname{$+$14.6}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.bias.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.bias.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.bias.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.bias.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.bias.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.bias.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.bias.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.rho.ci95.0\endcsname{0.094}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.rho.ci95.0\endcsname{9.4}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.rho.ci95.0\endcsname{$+$9.4}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.rho.ci95.1\endcsname{0.219}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.rho.ci95.1\endcsname{21.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.rho.ci95.1\endcsname{$+$21.9}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.rho.mean\endcsname{0.156}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.rho.mean\endcsname{15.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.rho.mean\endcsname{$+$15.6}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{82}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{82}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{8200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{$+$8200.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{0.976}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{97.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{$+$97.6}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{0.976}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{97.6}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{$+$97.6}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.disagree.N\endcsname{12}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.N\endcsname{12}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.disagree.N\endcsname{1200.0}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.N\endcsname{$+$1200.0}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{0.667}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{66.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{$+$66.7}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{0.583}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{58.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{$+$58.3}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.083}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{8.3}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{$+$8.3}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.tau.ci95.0\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.tau.ci95.0\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.tau.ci95.0\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.tau.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.tau.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.tau.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@bias.sspro.p2.T.zoomclick-d3.tau.mean\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.T.zoomclick-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.T.zoomclick-d3.tau.mean\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.T.zoomclick-d3.tau.mean\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{0.854}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{85.4}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{$+$85.4}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{-0.062}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.center-d1.gain.mean\endcsname{0.104}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.center-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.center-d1.gain.mean\endcsname{10.4}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.center-d1.gain.mean\endcsname{$+$10.4}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.center-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.center-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.center-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.center-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{0.875}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{87.5}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{$+$87.5}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0.312}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{31.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{$+$31.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.context-d1.gain.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.context-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.context-d1.gain.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.context-d1.gain.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.context-d1.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.context-d1.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.context-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.context-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{0.938}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{93.8}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{$+$93.8}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{0.062}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{6.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{$+$6.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0.333}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{33.3}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{$+$33.3}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{0.188}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{18.8}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{$+$18.8}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.dual-d2.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.dual-d2.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.dual-d2.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.dual-d2.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{0.875}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{87.5}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{$+$87.5}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0.312}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{31.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{$+$31.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.grid2-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.grid2-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.grid2-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.grid2-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{0.750}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{75.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{$+$75.0}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{0.917}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{91.7}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{$+$91.7}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{0.292}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{29.2}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{$+$29.2}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0.167}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{16.7}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{$+$16.7}
\expandafter\def\csname val@bias.sspro.p2.reverse-reader-T.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname cnt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname pct@bias.sspro.p2.reverse-reader-T.zoomclick-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@bias.sspro.p2.reverse-reader-T.zoomclick-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{36}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{36}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{3600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.N\endcsname{$+$3600.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{0.639}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{63.9}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{$+$63.9}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{-0.111}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{$-$11.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{$-$11.1}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{0.094}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{9.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-drift.share\endcsname{$+$9.4}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{271}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{271}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{27100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.N\endcsname{$+$27100.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{0.838}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{83.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{$+$83.8}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{0.819}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{81.9}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{$+$81.9}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0.018}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{1.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$+$1.8}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{0.706}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{70.6}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.agree-stable.share\endcsname{$+$70.6}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.disagree.N\endcsname{70}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.disagree.N\endcsname{70}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.disagree.N\endcsname{7000.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.disagree.N\endcsname{$+$7000.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{0.471}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{47.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-F\endcsname{$+$47.1}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{0.200}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{20.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.disagree.acc-R\endcsname{$+$20.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0.271}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{27.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{$+$27.1}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.disagree.share\endcsname{0.182}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.disagree.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.disagree.share\endcsname{18.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.disagree.share\endcsname{$+$18.2}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{7}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{7}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{700.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.N\endcsname{$+$700.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{0.714}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{71.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{$+$71.4}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{0.714}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{71.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{$+$71.4}
\expandafter\def\csname val@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{0.018}
\expandafter\def\csname cnt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{1.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.catalog-pooled-strata.parse-fail.share\endcsname{$+$1.8}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.bias.ci95.0\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.bias.ci95.0\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.bias.ci95.0\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.bias.ci95.1\endcsname{0.135}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.bias.ci95.1\endcsname{13.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.bias.ci95.1\endcsname{$+$13.5}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.bias.mean\endcsname{0.073}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.bias.mean\endcsname{7.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.bias.mean\endcsname{$+$7.3}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.rho.ci95.0\endcsname{-0.146}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.rho.ci95.0\endcsname{$-$14.6}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.rho.ci95.0\endcsname{$-$14.6}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.rho.ci95.1\endcsname{0.021}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.rho.ci95.1\endcsname{2.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.rho.ci95.1\endcsname{$+$2.1}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.rho.mean\endcsname{-0.062}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.rho.mean\endcsname{$-$6.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.rho.mean\endcsname{$-$6.2}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-drift.N\endcsname{700.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-drift.N\endcsname{$+$700.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{0.429}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{42.9}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-F\endcsname{$+$42.9}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{0.714}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{71.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-drift.acc-R\endcsname{$+$71.4}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{-0.286}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{$-$28.6}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{$-$28.6}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-stable.N\endcsname{70}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-stable.N\endcsname{70}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-stable.N\endcsname{7000.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-stable.N\endcsname{$+$7000.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{0.843}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{84.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-F\endcsname{$+$84.3}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{0.829}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{82.9}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-stable.acc-R\endcsname{$+$82.9}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.014}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{1.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{$+$1.4}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.disagree.N\endcsname{17}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.disagree.N\endcsname{17}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.disagree.N\endcsname{1700.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.disagree.N\endcsname{$+$1700.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.disagree.acc-F\endcsname{0.588}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.disagree.acc-F\endcsname{58.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.disagree.acc-F\endcsname{$+$58.8}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.disagree.acc-R\endcsname{0.235}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.disagree.acc-R\endcsname{23.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.disagree.acc-R\endcsname{$+$23.5}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.353}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{35.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{$+$35.3}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.tau.ci95.0\endcsname{-0.073}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.tau.ci95.0\endcsname{$-$7.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.tau.ci95.0\endcsname{$-$7.3}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.tau.ci95.1\endcsname{0.094}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.tau.ci95.1\endcsname{9.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.tau.ci95.1\endcsname{$+$9.4}
\expandafter\def\csname val@bias.uiv.p1.C.center-d1.tau.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p1.C.center-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.center-d1.tau.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.center-d1.tau.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.bias.ci95.0\endcsname{-0.073}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.bias.ci95.0\endcsname{$-$7.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.bias.ci95.0\endcsname{$-$7.3}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.bias.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.bias.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.bias.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.bias.mean\endcsname{-0.010}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.bias.mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.bias.mean\endcsname{$-$1.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.rho.ci95.0\endcsname{-0.083}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.rho.ci95.1\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.rho.ci95.1\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.rho.ci95.1\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.rho.mean\endcsname{-0.010}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.rho.mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.rho.mean\endcsname{$-$1.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-drift.N\endcsname{11}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-drift.N\endcsname{11}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-drift.N\endcsname{1100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-drift.N\endcsname{$+$1100.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{0.727}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{72.7}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-F\endcsname{$+$72.7}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{0.818}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{81.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-drift.acc-R\endcsname{$+$81.8}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{-0.091}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{$-$9.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{$-$9.1}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-stable.N\endcsname{73}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-stable.N\endcsname{73}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-stable.N\endcsname{7300.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-stable.N\endcsname{$+$7300.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{0.822}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{82.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-F\endcsname{$+$82.2}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{0.808}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{80.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-stable.acc-R\endcsname{$+$80.8}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.014}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{1.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{$+$1.4}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.disagree.N\endcsname{11}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.disagree.N\endcsname{11}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.disagree.N\endcsname{1100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.disagree.N\endcsname{$+$1100.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.disagree.acc-F\endcsname{0.273}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.disagree.acc-F\endcsname{27.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.disagree.acc-F\endcsname{$+$27.3}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.disagree.acc-R\endcsname{0.364}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.disagree.acc-R\endcsname{36.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.disagree.acc-R\endcsname{$+$36.4}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{-0.091}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{$-$9.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{$-$9.1}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.tau.ci95.0\endcsname{-0.094}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.tau.ci95.0\endcsname{$-$9.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.tau.ci95.0\endcsname{$-$9.4}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.tau.ci95.1\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.tau.ci95.1\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.tau.ci95.1\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.context-d1.tau.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p1.C.context-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.context-d1.tau.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.context-d1.tau.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.bias.ci95.0\endcsname{0.021}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.bias.ci95.0\endcsname{2.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.bias.ci95.0\endcsname{$+$2.1}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.bias.ci95.1\endcsname{0.125}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.bias.ci95.1\endcsname{12.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.bias.ci95.1\endcsname{$+$12.5}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.bias.mean\endcsname{0.073}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.bias.mean\endcsname{7.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.bias.mean\endcsname{$+$7.3}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.rho.ci95.0\endcsname{-0.167}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.rho.ci95.0\endcsname{$-$16.7}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.rho.ci95.0\endcsname{$-$16.7}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.rho.ci95.1\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.rho.ci95.1\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.rho.ci95.1\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.rho.mean\endcsname{-0.073}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.rho.mean\endcsname{$-$7.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.rho.mean\endcsname{$-$7.3}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-drift.N\endcsname{10}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-drift.N\endcsname{10}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-drift.N\endcsname{1000.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-drift.N\endcsname{$+$1000.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{0.600}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{60.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-F\endcsname{$+$60.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{0.600}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{60.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-drift.acc-R\endcsname{$+$60.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-stable.N\endcsname{66}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-stable.N\endcsname{66}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-stable.N\endcsname{6600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-stable.N\endcsname{$+$6600.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{0.864}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{86.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-F\endcsname{$+$86.4}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{0.848}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{84.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-stable.acc-R\endcsname{$+$84.8}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0.015}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{1.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$+$1.5}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.disagree.N\endcsname{20}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.disagree.N\endcsname{20}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.disagree.N\endcsname{2000.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.disagree.N\endcsname{$+$2000.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.disagree.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.disagree.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.disagree.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.disagree.acc-R\endcsname{0.200}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.disagree.acc-R\endcsname{20.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.disagree.acc-R\endcsname{$+$20.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0.300}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{30.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$+$30.0}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.tau.ci95.0\endcsname{-0.083}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.tau.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.tau.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.tau.ci95.1\endcsname{0.073}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.tau.ci95.1\endcsname{7.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.tau.ci95.1\endcsname{$+$7.3}
\expandafter\def\csname val@bias.uiv.p1.C.dual-d2.tau.mean\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.dual-d2.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.dual-d2.tau.mean\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.dual-d2.tau.mean\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.bias.ci95.0\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.bias.ci95.0\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.bias.ci95.0\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.bias.ci95.1\endcsname{0.198}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.bias.ci95.1\endcsname{19.8}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.bias.ci95.1\endcsname{$+$19.8}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.bias.mean\endcsname{0.125}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.bias.mean\endcsname{12.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.bias.mean\endcsname{$+$12.5}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.rho.ci95.0\endcsname{-0.240}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.rho.ci95.0\endcsname{$-$24.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.rho.ci95.0\endcsname{$-$24.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.rho.ci95.1\endcsname{-0.083}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.rho.ci95.1\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.rho.ci95.1\endcsname{$-$8.3}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.rho.mean\endcsname{-0.156}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.rho.mean\endcsname{$-$15.6}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.rho.mean\endcsname{$-$15.6}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-drift.N\endcsname{8}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.N\endcsname{8}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-drift.N\endcsname{800.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.N\endcsname{$+$800.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-F\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-F\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-F\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-R\endcsname{0.875}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-R\endcsname{87.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.acc-R\endcsname{$+$87.5}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{-0.125}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{$-$12.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{$-$12.5}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-stable.N\endcsname{62}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.N\endcsname{62}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-stable.N\endcsname{6200.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.N\endcsname{$+$6200.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{0.823}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{82.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-F\endcsname{$+$82.3}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{0.790}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{79.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.acc-R\endcsname{$+$79.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.032}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{3.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$+$3.2}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.disagree.N\endcsname{22}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.disagree.N\endcsname{22}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.disagree.N\endcsname{2200.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.disagree.N\endcsname{$+$2200.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{0.455}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{45.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-F\endcsname{$+$45.5}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{0.091}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{9.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.disagree.acc-R\endcsname{$+$9.1}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.364}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{36.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{$+$36.4}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.parse-fail.N\endcsname{400.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.N\endcsname{$+$400.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-F\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.tau.ci95.0\endcsname{-0.104}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.tau.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.tau.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.tau.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.tau.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.tau.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@bias.uiv.p1.C.grid2-d3.tau.mean\endcsname{-0.031}
\expandafter\def\csname cnt@bias.uiv.p1.C.grid2-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.grid2-d3.tau.mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.grid2-d3.tau.mean\endcsname{$-$3.1}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.bias.ci95.0\endcsname{-0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.bias.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.bias.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.bias.ci95.1\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.bias.ci95.1\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.bias.ci95.1\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.bias.mean\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.bias.mean\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.bias.mean\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.rho.ci95.0\endcsname{-0.094}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.rho.ci95.0\endcsname{$-$9.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.rho.ci95.0\endcsname{$-$9.4}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.rho.ci95.1\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.rho.ci95.1\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.rho.ci95.1\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.rho.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{6}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{6}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{0.833}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{83.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-F\endcsname{$+$83.3}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{-0.167}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{$-$16.7}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{$-$16.7}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{76}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{76}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{7600.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.N\endcsname{$+$7600.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{0.803}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{80.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{$+$80.3}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{0.816}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{81.6}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{$+$81.6}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{-0.013}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$1.3}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$1.3}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.disagree.N\endcsname{13}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.N\endcsname{13}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.disagree.N\endcsname{1300.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.N\endcsname{$+$1300.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{0.385}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{38.5}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-F\endcsname{$+$38.5}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0.231}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{23.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.acc-R\endcsname{$+$23.1}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.154}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{15.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{$+$15.4}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.tau.ci95.0\endcsname{-0.104}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.tau.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.tau.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.tau.ci95.1\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.tau.ci95.1\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.tau.ci95.1\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p1.C.zoomclick-d3.tau.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p1.C.zoomclick-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.C.zoomclick-d3.tau.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p1.C.zoomclick-d3.tau.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{0.633}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{63.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-direct\endcsname{$+$63.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{0.650}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{65.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{$+$65.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{-0.033}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$-$3.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$-$3.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0.075}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{7.5}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.center-d1.gain.ci95.1\endcsname{$+$7.5}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.center-d1.gain.mean\endcsname{0.017}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.center-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.center-d1.gain.mean\endcsname{1.7}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.center-d1.gain.mean\endcsname{$+$1.7}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.center-d1.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.center-d1.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.center-d1.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.center-d1.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{0.633}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{63.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-direct\endcsname{$+$63.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{0.633}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{63.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{$+$63.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{-0.058}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$-$5.8}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$-$5.8}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0.058}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{5.8}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.context-d1.gain.ci95.1\endcsname{$+$5.8}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.context-d1.gain.mean\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.context-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.context-d1.gain.mean\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.context-d1.gain.mean\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.context-d1.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.context-d1.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.context-d1.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.context-d1.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{0.633}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{63.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{$+$63.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{0.675}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{67.5}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{$+$67.5}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{-0.025}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{$-$2.5}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{$-$2.5}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0.100}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{10.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{$+$10.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.dual-d2.gain.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.dual-d2.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.dual-d2.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.dual-d2.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.dual-d2.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{0.633}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{63.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{$+$63.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{0.658}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{65.8}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{$+$65.8}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0.092}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{9.2}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{$+$9.2}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{0.025}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{2.5}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.grid2-d3.gain.mean\endcsname{$+$2.5}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.grid2-d3.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.grid2-d3.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.grid2-d3.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.grid2-d3.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{0.633}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{63.3}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{$+$63.3}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{0.692}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{69.2}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{$+$69.2}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{0.117}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{11.7}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{$+$11.7}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0.058}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{5.8}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{$+$5.8}
\expandafter\def\csname val@bias.uiv.p1.reverse-reader-T.zoomclick-d3.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p1.reverse-reader-T.zoomclick-d3.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p1.reverse-reader-T.zoomclick-d3.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{9}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{9}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{900.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.N\endcsname{$+$900.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{0.778}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{77.8}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-F\endcsname{$+$77.8}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{0.444}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{44.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.acc-R\endcsname{$+$44.4}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{0.023}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{2.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-drift.share\endcsname{$+$2.3}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{334}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{334}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{33400.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.N\endcsname{$+$33400.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{0.838}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{83.8}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-F\endcsname{$+$83.8}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{0.832}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{83.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.acc-R\endcsname{$+$83.2}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0.006}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0.6}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$+$0.6}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{0.870}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{87.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.agree-stable.share\endcsname{$+$87.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.disagree.N\endcsname{39}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.disagree.N\endcsname{39}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.disagree.N\endcsname{3900.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.disagree.N\endcsname{$+$3900.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{0.462}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{46.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-F\endcsname{$+$46.2}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{0.436}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{43.6}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.disagree.acc-R\endcsname{$+$43.6}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0.026}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{2.6}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{$+$2.6}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.disagree.share\endcsname{0.102}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.disagree.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.disagree.share\endcsname{10.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.disagree.share\endcsname{$+$10.2}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{0.005}
\expandafter\def\csname cnt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{0.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.catalog-pooled-strata.parse-fail.share\endcsname{$+$0.5}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.bias.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.bias.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.bias.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.bias.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.bias.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.bias.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.bias.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.rho.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.rho.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.rho.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.rho.ci95.1\endcsname{0.062}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.rho.ci95.1\endcsname{6.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.rho.ci95.1\endcsname{$+$6.2}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.rho.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.rho.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.rho.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-drift.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-stable.N\endcsname{87}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-stable.N\endcsname{87}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-stable.N\endcsname{8700.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-stable.N\endcsname{$+$8700.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{0.839}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{83.9}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-F\endcsname{$+$83.9}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{0.839}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{83.9}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-stable.acc-R\endcsname{$+$83.9}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.disagree.N\endcsname{8}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.disagree.N\endcsname{800.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.disagree.N\endcsname{$+$800.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.disagree.acc-F\endcsname{0.625}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.disagree.acc-F\endcsname{62.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.disagree.acc-F\endcsname{$+$62.5}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.disagree.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.disagree.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.disagree.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.125}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{12.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.strata.disagree.resid-F-minus-R\endcsname{$+$12.5}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.tau.ci95.0\endcsname{-0.031}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.tau.ci95.0\endcsname{$-$3.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.tau.ci95.0\endcsname{$-$3.1}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.tau.ci95.1\endcsname{0.083}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.tau.ci95.1\endcsname{8.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.tau.ci95.1\endcsname{$+$8.3}
\expandafter\def\csname val@bias.uiv.p2.C.center-d1.tau.mean\endcsname{0.021}
\expandafter\def\csname cnt@bias.uiv.p2.C.center-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.center-d1.tau.mean\endcsname{2.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.center-d1.tau.mean\endcsname{$+$2.1}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.bias.ci95.0\endcsname{-0.052}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.bias.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.bias.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.bias.ci95.1\endcsname{0.031}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.bias.ci95.1\endcsname{3.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.bias.ci95.1\endcsname{$+$3.1}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.bias.mean\endcsname{-0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.bias.mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.bias.mean\endcsname{$-$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.rho.ci95.0\endcsname{-0.083}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.rho.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.rho.ci95.1\endcsname{0.125}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.rho.ci95.1\endcsname{12.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.rho.ci95.1\endcsname{$+$12.5}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.rho.mean\endcsname{0.021}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.rho.mean\endcsname{2.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.rho.mean\endcsname{$+$2.1}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-stable.N\endcsname{84}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-stable.N\endcsname{84}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-stable.N\endcsname{8400.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-stable.N\endcsname{$+$8400.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{0.845}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{84.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-F\endcsname{$+$84.5}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{0.845}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{84.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-stable.acc-R\endcsname{$+$84.5}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.disagree.N\endcsname{10}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.disagree.N\endcsname{10}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.disagree.N\endcsname{1000.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.disagree.N\endcsname{$+$1000.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.disagree.acc-F\endcsname{0.400}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.disagree.acc-F\endcsname{40.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.disagree.acc-F\endcsname{$+$40.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.disagree.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.disagree.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.disagree.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{-0.100}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{$-$10.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.strata.disagree.resid-F-minus-R\endcsname{$-$10.0}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.tau.ci95.0\endcsname{-0.083}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.tau.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.tau.ci95.0\endcsname{$-$8.3}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.tau.ci95.1\endcsname{0.104}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.tau.ci95.1\endcsname{10.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.tau.ci95.1\endcsname{$+$10.4}
\expandafter\def\csname val@bias.uiv.p2.C.context-d1.tau.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.context-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.context-d1.tau.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.context-d1.tau.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.bias.ci95.0\endcsname{-0.052}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.bias.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.bias.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.bias.ci95.1\endcsname{0.083}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.bias.ci95.1\endcsname{8.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.bias.ci95.1\endcsname{$+$8.3}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.bias.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.bias.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.bias.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.rho.ci95.0\endcsname{-0.115}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.rho.ci95.0\endcsname{$-$11.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.rho.ci95.0\endcsname{$-$11.5}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.rho.ci95.1\endcsname{0.062}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.rho.ci95.1\endcsname{6.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.rho.ci95.1\endcsname{$+$6.2}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.rho.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-drift.N\endcsname{4}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-drift.N\endcsname{4}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-drift.N\endcsname{400.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-drift.N\endcsname{$+$400.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-F\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-F\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-F\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-R\endcsname{0.250}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-R\endcsname{25.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-drift.acc-R\endcsname{$+$25.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-stable.N\endcsname{86}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-stable.N\endcsname{86}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-stable.N\endcsname{8600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-stable.N\endcsname{$+$8600.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{0.814}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{81.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-F\endcsname{$+$81.4}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{0.814}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{81.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-stable.acc-R\endcsname{$+$81.4}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.disagree.acc-F\endcsname{0.333}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.disagree.acc-F\endcsname{33.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.disagree.acc-F\endcsname{$+$33.3}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.disagree.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.disagree.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.disagree.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{-0.167}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$-$16.7}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$-$16.7}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.tau.ci95.0\endcsname{-0.073}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.tau.ci95.0\endcsname{$-$7.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.tau.ci95.0\endcsname{$-$7.3}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.tau.ci95.1\endcsname{0.052}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.tau.ci95.1\endcsname{5.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.tau.ci95.1\endcsname{$+$5.2}
\expandafter\def\csname val@bias.uiv.p2.C.dual-d2.tau.mean\endcsname{-0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.dual-d2.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.dual-d2.tau.mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.dual-d2.tau.mean\endcsname{$-$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.bias.ci95.0\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.bias.ci95.0\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.bias.ci95.0\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.bias.ci95.1\endcsname{0.146}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.bias.ci95.1\endcsname{14.6}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.bias.ci95.1\endcsname{$+$14.6}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.bias.mean\endcsname{0.073}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.bias.mean\endcsname{7.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.bias.mean\endcsname{$+$7.3}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.rho.ci95.0\endcsname{-0.146}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.rho.ci95.0\endcsname{$-$14.6}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.rho.ci95.0\endcsname{$-$14.6}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.rho.ci95.1\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.rho.ci95.1\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.rho.ci95.1\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.rho.mean\endcsname{-0.062}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.rho.mean\endcsname{$-$6.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.rho.mean\endcsname{$-$6.2}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.acc-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-drift.resid-F-minus-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-stable.N\endcsname{77}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.N\endcsname{77}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-stable.N\endcsname{7700.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.N\endcsname{$+$7700.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{0.857}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{85.7}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-F\endcsname{$+$85.7}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{0.831}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{83.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.acc-R\endcsname{$+$83.1}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.026}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{2.6}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$+$2.6}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.disagree.N\endcsname{15}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.disagree.N\endcsname{15}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.disagree.N\endcsname{1500.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.disagree.N\endcsname{$+$1500.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{0.467}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{46.7}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-F\endcsname{$+$46.7}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{0.333}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{33.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.disagree.acc-R\endcsname{$+$33.3}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.133}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{13.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{$+$13.3}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.tau.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.tau.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.tau.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.tau.ci95.1\endcsname{0.073}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.tau.ci95.1\endcsname{7.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.tau.ci95.1\endcsname{$+$7.3}
\expandafter\def\csname val@bias.uiv.p2.C.grid2-d3.tau.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.grid2-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.grid2-d3.tau.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.grid2-d3.tau.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.bias.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.bias.ci95.1\endcsname{0.104}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.bias.ci95.1\endcsname{10.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.bias.ci95.1\endcsname{$+$10.4}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.bias.mean\endcsname{0.042}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.bias.mean\endcsname{4.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.bias.mean\endcsname{$+$4.2}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.rho.ci95.0\endcsname{-0.104}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.rho.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.rho.ci95.0\endcsname{$-$10.4}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.rho.ci95.1\endcsname{0.031}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.rho.ci95.1\endcsname{3.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.rho.ci95.1\endcsname{$+$3.1}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.rho.mean\endcsname{-0.031}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.rho.mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.rho.mean\endcsname{$-$3.1}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{85}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{85}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{8500.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.N\endcsname{$+$8500.0}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{0.847}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{84.7}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-F\endcsname{$+$84.7}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{0.824}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{82.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.acc-R\endcsname{$+$82.4}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.024}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{2.4}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{$+$2.4}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.disagree.N\endcsname{11}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.N\endcsname{11}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.disagree.N\endcsname{1100.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.N\endcsname{$+$1100.0}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{0.455}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{45.5}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-F\endcsname{$+$45.5}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0.273}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{27.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.acc-R\endcsname{$+$27.3}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.182}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{18.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{$+$18.2}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.tau.ci95.0\endcsname{-0.052}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.tau.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.tau.ci95.0\endcsname{$-$5.2}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.tau.ci95.1\endcsname{0.073}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.tau.ci95.1\endcsname{7.3}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.tau.ci95.1\endcsname{$+$7.3}
\expandafter\def\csname val@bias.uiv.p2.C.zoomclick-d3.tau.mean\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.C.zoomclick-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.C.zoomclick-d3.tau.mean\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.C.zoomclick-d3.tau.mean\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{11}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{11}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{1100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.N\endcsname{$+$1100.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{0.636}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{63.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-F\endcsname{$+$63.6}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{0.636}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{63.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.acc-R\endcsname{$+$63.6}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{0.019}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{1.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-drift.share\endcsname{$+$1.9}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{512}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{512}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{51200.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.N\endcsname{$+$51200.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{0.859}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{85.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-F\endcsname{$+$85.9}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{0.867}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{86.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.acc-R\endcsname{$+$86.7}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{-0.008}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$-$0.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.resid-F-minus-R\endcsname{$-$0.8}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{0.889}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{88.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.agree-stable.share\endcsname{$+$88.9}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.disagree.N\endcsname{47}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.disagree.N\endcsname{47}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.disagree.N\endcsname{4700.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.disagree.N\endcsname{$+$4700.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{0.426}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{42.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-F\endcsname{$+$42.6}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{0.234}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{23.4}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.disagree.acc-R\endcsname{$+$23.4}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0.191}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{19.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.disagree.resid-F-minus-R\endcsname{$+$19.1}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.disagree.share\endcsname{0.082}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.disagree.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.disagree.share\endcsname{8.2}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.disagree.share\endcsname{$+$8.2}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{6}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{6}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{600.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.N\endcsname{$+$600.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.resid-F-minus-R\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{0.010}
\expandafter\def\csname cnt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{1.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.catalog-pooled-strata.parse-fail.share\endcsname{$+$1.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.bias.ci95.0\endcsname{-0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.bias.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.bias.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.bias.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.bias.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.bias.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.bias.mean\endcsname{-0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.bias.mean\endcsname{$-$0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.bias.mean\endcsname{$-$0.7}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.n\endcsname{144}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.n\endcsname{144}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.n\endcsname{14400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.n\endcsname{$+$14400.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.rho.ci95.0\endcsname{-0.069}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.rho.ci95.0\endcsname{$-$6.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.rho.ci95.0\endcsname{$-$6.9}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.rho.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.rho.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.rho.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.rho.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-drift.N\endcsname{3}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-drift.N\endcsname{3}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-drift.N\endcsname{300.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-drift.N\endcsname{$+$300.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-stable.N\endcsname{128}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-stable.N\endcsname{128}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-stable.N\endcsname{12800.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-stable.N\endcsname{$+$12800.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{0.867}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{86.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-F\endcsname{$+$86.7}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{0.875}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{87.5}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-stable.acc-R\endcsname{$+$87.5}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{-0.008}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{$-$0.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.agree-stable.resid-F-minus-R\endcsname{$-$0.8}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.disagree.N\endcsname{11}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.disagree.N\endcsname{11}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.disagree.N\endcsname{1100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.disagree.N\endcsname{$+$1100.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.disagree.acc-F\endcsname{0.273}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.disagree.acc-F\endcsname{27.3}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.disagree.acc-F\endcsname{$+$27.3}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.disagree.acc-R\endcsname{0.273}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.disagree.acc-R\endcsname{27.3}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.disagree.acc-R\endcsname{$+$27.3}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.disagree.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.tau.ci95.0\endcsname{-0.076}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.tau.ci95.0\endcsname{$-$7.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.tau.ci95.0\endcsname{$-$7.6}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.tau.ci95.1\endcsname{0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.tau.ci95.1\endcsname{0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.tau.ci95.1\endcsname{$+$0.7}
\expandafter\def\csname val@bias.uiv.p2.T.center-d1.tau.mean\endcsname{-0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.center-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.center-d1.tau.mean\endcsname{$-$2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.center-d1.tau.mean\endcsname{$-$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.bias.ci95.1\endcsname{0.062}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.bias.ci95.1\endcsname{6.2}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.bias.ci95.1\endcsname{$+$6.2}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.bias.mean\endcsname{0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.bias.mean\endcsname{2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.bias.mean\endcsname{$+$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.n\endcsname{144}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.n\endcsname{144}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.n\endcsname{14400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.n\endcsname{$+$14400.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.rho.ci95.0\endcsname{-0.076}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.rho.ci95.0\endcsname{$-$7.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.rho.ci95.0\endcsname{$-$7.6}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.rho.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.rho.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.rho.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.rho.mean\endcsname{-0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.rho.mean\endcsname{$-$2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.rho.mean\endcsname{$-$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-drift.N\endcsname{3}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-drift.N\endcsname{3}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-drift.N\endcsname{300.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-drift.N\endcsname{$+$300.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{0.667}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{66.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-F\endcsname{$+$66.7}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{0.667}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{66.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-drift.acc-R\endcsname{$+$66.7}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-stable.N\endcsname{131}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-stable.N\endcsname{131}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-stable.N\endcsname{13100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-stable.N\endcsname{$+$13100.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{0.870}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{87.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-F\endcsname{$+$87.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{0.870}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{87.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-stable.acc-R\endcsname{$+$87.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.agree-stable.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.disagree.N\endcsname{10}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.disagree.N\endcsname{10}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.disagree.N\endcsname{1000.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.disagree.N\endcsname{$+$1000.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.disagree.acc-F\endcsname{0.500}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.disagree.acc-F\endcsname{50.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.disagree.acc-F\endcsname{$+$50.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.disagree.acc-R\endcsname{0.100}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.disagree.acc-R\endcsname{10.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.disagree.acc-R\endcsname{$+$10.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{0.400}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{40.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.strata.disagree.resid-F-minus-R\endcsname{$+$40.0}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.tau.ci95.0\endcsname{-0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.tau.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.tau.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.tau.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.tau.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.tau.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.context-d1.tau.mean\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.context-d1.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.context-d1.tau.mean\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.context-d1.tau.mean\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.bias.ci95.0\endcsname{-0.069}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.bias.ci95.0\endcsname{$-$6.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.bias.ci95.0\endcsname{$-$6.9}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.bias.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.bias.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.bias.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.bias.mean\endcsname{-0.014}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.bias.mean\endcsname{$-$1.4}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.bias.mean\endcsname{$-$1.4}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.n\endcsname{144}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.n\endcsname{144}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.n\endcsname{14400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.n\endcsname{$+$14400.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.rho.ci95.0\endcsname{-0.097}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.rho.ci95.0\endcsname{$-$9.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.rho.ci95.0\endcsname{$-$9.7}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.rho.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.rho.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.rho.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.rho.mean\endcsname{-0.049}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.rho.mean\endcsname{$-$4.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.rho.mean\endcsname{$-$4.9}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-drift.N\endcsname{5}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-drift.N\endcsname{5}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-drift.N\endcsname{500.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-drift.N\endcsname{$+$500.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{0.400}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{40.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-F\endcsname{$+$40.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{0.400}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{40.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-drift.acc-R\endcsname{$+$40.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-stable.N\endcsname{129}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-stable.N\endcsname{129}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-stable.N\endcsname{12900.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-stable.N\endcsname{$+$12900.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{0.829}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{82.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-F\endcsname{$+$82.9}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{0.837}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{83.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-stable.acc-R\endcsname{$+$83.7}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{-0.008}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$-$0.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.agree-stable.resid-F-minus-R\endcsname{$-$0.8}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.disagree.N\endcsname{10}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.disagree.N\endcsname{10}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.disagree.N\endcsname{1000.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.disagree.N\endcsname{$+$1000.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.disagree.acc-F\endcsname{0.300}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.disagree.acc-F\endcsname{30.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.disagree.acc-F\endcsname{$+$30.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.disagree.acc-R\endcsname{0.400}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.disagree.acc-R\endcsname{40.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.disagree.acc-R\endcsname{$+$40.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{-0.100}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$-$10.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.strata.disagree.resid-F-minus-R\endcsname{$-$10.0}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.tau.ci95.0\endcsname{-0.125}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.tau.ci95.0\endcsname{$-$12.5}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.tau.ci95.0\endcsname{$-$12.5}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.tau.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.tau.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.tau.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@bias.uiv.p2.T.dual-d2.tau.mean\endcsname{-0.062}
\expandafter\def\csname cnt@bias.uiv.p2.T.dual-d2.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.dual-d2.tau.mean\endcsname{$-$6.2}
\expandafter\def\csname ppt@bias.uiv.p2.T.dual-d2.tau.mean\endcsname{$-$6.2}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.bias.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.bias.ci95.0\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.bias.ci95.1\endcsname{0.097}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.bias.ci95.1\endcsname{9.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.bias.ci95.1\endcsname{$+$9.7}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.bias.mean\endcsname{0.049}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.bias.mean\endcsname{4.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.bias.mean\endcsname{$+$4.9}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.n\endcsname{144}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.n\endcsname{144}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.n\endcsname{14400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.n\endcsname{$+$14400.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.rho.ci95.0\endcsname{-0.111}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.rho.ci95.0\endcsname{$-$11.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.rho.ci95.0\endcsname{$-$11.1}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.rho.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.rho.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.rho.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.rho.mean\endcsname{-0.056}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.rho.mean\endcsname{$-$5.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.rho.mean\endcsname{$-$5.6}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.agree-stable.N\endcsname{124}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.N\endcsname{124}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.agree-stable.N\endcsname{12400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.N\endcsname{$+$12400.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{0.871}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{87.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-F\endcsname{$+$87.1}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{0.887}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{88.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.acc-R\endcsname{$+$88.7}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{-0.016}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$1.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.agree-stable.resid-F-minus-R\endcsname{$-$1.6}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.disagree.N\endcsname{16}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.disagree.N\endcsname{16}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.disagree.N\endcsname{1600.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.disagree.N\endcsname{$+$1600.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{0.562}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{56.2}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-F\endcsname{$+$56.2}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{0.188}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{18.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.disagree.acc-R\endcsname{$+$18.8}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0.375}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{37.5}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.disagree.resid-F-minus-R\endcsname{$+$37.5}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.parse-fail.N\endcsname{400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.N\endcsname{$+$400.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-F\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.750}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{75.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.strata.parse-fail.resid-F-minus-R\endcsname{$+$75.0}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.tau.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.tau.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.tau.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.tau.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.tau.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.tau.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.grid2-d3.tau.mean\endcsname{-0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.grid2-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.grid2-d3.tau.mean\endcsname{$-$0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.grid2-d3.tau.mean\endcsname{$-$0.7}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.bias.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.bias.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.bias.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.bias.ci95.1\endcsname{0.049}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.bias.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.bias.ci95.1\endcsname{4.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.bias.ci95.1\endcsname{$+$4.9}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.bias.mean\endcsname{0.014}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.bias.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.bias.mean\endcsname{1.4}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.bias.mean\endcsname{$+$1.4}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.n\endcsname{144}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.n\endcsname{144}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.n\endcsname{14400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.n\endcsname{$+$14400.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.rho.ci95.0\endcsname{-0.076}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.rho.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.rho.ci95.0\endcsname{$-$7.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.rho.ci95.0\endcsname{$-$7.6}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.rho.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.rho.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.rho.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.rho.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.rho.mean\endcsname{-0.021}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.rho.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.rho.mean\endcsname{$-$2.1}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-F\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{1.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{100.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.acc-R\endcsname{$+$100.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-drift.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{126}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{126}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{12600.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.N\endcsname{$+$12600.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{0.897}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{89.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-F\endcsname{$+$89.7}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{0.889}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{88.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.acc-R\endcsname{$+$88.9}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.008}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{0.8}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.agree-stable.resid-F-minus-R\endcsname{$+$0.8}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.disagree.N\endcsname{14}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.N\endcsname{14}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.disagree.N\endcsname{1400.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.N\endcsname{$+$1400.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{0.357}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{35.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-F\endcsname{$+$35.7}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{0.286}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{28.6}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.acc-R\endcsname{$+$28.6}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0.071}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{7.1}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.disagree.resid-F-minus-R\endcsname{$+$7.1}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-F\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.acc-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.strata.parse-fail.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.tau.ci95.0\endcsname{-0.049}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.tau.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.tau.ci95.0\endcsname{$-$4.9}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.tau.ci95.0\endcsname{$-$4.9}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.tau.ci95.1\endcsname{0.035}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.tau.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.tau.ci95.1\endcsname{3.5}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.tau.ci95.1\endcsname{$+$3.5}
\expandafter\def\csname val@bias.uiv.p2.T.zoomclick-d3.tau.mean\endcsname{-0.007}
\expandafter\def\csname cnt@bias.uiv.p2.T.zoomclick-d3.tau.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.T.zoomclick-d3.tau.mean\endcsname{$-$0.7}
\expandafter\def\csname ppt@bias.uiv.p2.T.zoomclick-d3.tau.mean\endcsname{$-$0.7}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{0.825}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{82.5}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-direct\endcsname{$+$82.5}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{0.767}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{76.7}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.center-d1.acc-reader-on-packet\endcsname{$+$76.7}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{-0.117}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$-$11.7}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.0\endcsname{$-$11.7}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{-0.008}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.center-d1.gain.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.center-d1.gain.mean\endcsname{-0.058}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.center-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.center-d1.gain.mean\endcsname{$-$5.8}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.center-d1.gain.mean\endcsname{$-$5.8}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.center-d1.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.center-d1.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.center-d1.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.center-d1.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{0.825}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{82.5}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-direct\endcsname{$+$82.5}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{0.767}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{76.7}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.context-d1.acc-reader-on-packet\endcsname{$+$76.7}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{-0.117}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$-$11.7}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.0\endcsname{$-$11.7}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{-0.008}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.context-d1.gain.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.context-d1.gain.mean\endcsname{-0.058}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.context-d1.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.context-d1.gain.mean\endcsname{$-$5.8}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.context-d1.gain.mean\endcsname{$-$5.8}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.context-d1.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.context-d1.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.context-d1.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.context-d1.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{0.825}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{82.5}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-direct\endcsname{$+$82.5}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{0.783}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{78.3}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.dual-d2.acc-reader-on-packet\endcsname{$+$78.3}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{-0.100}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{$-$10.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.0\endcsname{$-$10.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0.008}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{0.8}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.dual-d2.gain.ci95.1\endcsname{$+$0.8}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{-0.042}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{$-$4.2}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.dual-d2.gain.mean\endcsname{$-$4.2}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.dual-d2.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.dual-d2.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.dual-d2.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.dual-d2.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{0.825}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{82.5}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-direct\endcsname{$+$82.5}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{0.792}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{79.2}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.grid2-d3.acc-reader-on-packet\endcsname{$+$79.2}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{-0.092}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$-$9.2}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.0\endcsname{$-$9.2}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0.017}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{1.7}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.ci95.1\endcsname{$+$1.7}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{-0.033}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{$-$3.3}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.grid2-d3.gain.mean\endcsname{$-$3.3}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.grid2-d3.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.grid2-d3.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.grid2-d3.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.grid2-d3.n\endcsname{$+$12000.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{0.825}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{82.5}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-direct\endcsname{$+$82.5}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{0.775}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{1}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{77.5}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.acc-reader-on-packet\endcsname{$+$77.5}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{-0.100}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{$-$10.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.0\endcsname{$-$10.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{-0.008}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{-0.050}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{0}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{$-$5.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.gain.mean\endcsname{$-$5.0}
\expandafter\def\csname val@bias.uiv.p2.reverse-reader-T.zoomclick-d3.n\endcsname{120}
\expandafter\def\csname cnt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.n\endcsname{120}
\expandafter\def\csname pct@bias.uiv.p2.reverse-reader-T.zoomclick-d3.n\endcsname{12000.0}
\expandafter\def\csname ppt@bias.uiv.p2.reverse-reader-T.zoomclick-d3.n\endcsname{$+$12000.0}
\expandafter\def\csname val@census.sspro.applications\endcsname{26}
\expandafter\def\csname cnt@census.sspro.applications\endcsname{26}
\expandafter\def\csname pct@census.sspro.applications\endcsname{2600.0}
\expandafter\def\csname ppt@census.sspro.applications\endcsname{$+$2600.0}
\expandafter\def\csname val@census.sspro.median-target-short-side-px\endcsname{8.119}
\expandafter\def\csname cnt@census.sspro.median-target-short-side-px\endcsname{8}
\expandafter\def\csname pct@census.sspro.median-target-short-side-px\endcsname{811.9}
\expandafter\def\csname ppt@census.sspro.median-target-short-side-px\endcsname{$+$811.9}
\expandafter\def\csname val@census.sspro.median-target-side-text\endcsname{8.1}
\expandafter\def\csname val@census.sspro.n-target-sizes\endcsname{176}
\expandafter\def\csname cnt@census.sspro.n-target-sizes\endcsname{176}
\expandafter\def\csname pct@census.sspro.n-target-sizes\endcsname{17600.0}
\expandafter\def\csname ppt@census.sspro.n-target-sizes\endcsname{$+$17600.0}
\expandafter\def\csname val@census.sspro.tasks\endcsname{1581}
\expandafter\def\csname cnt@census.sspro.tasks\endcsname{1{,}581}
\expandafter\def\csname pct@census.sspro.tasks\endcsname{158100.0}
\expandafter\def\csname ppt@census.sspro.tasks\endcsname{$+$158100.0}
\expandafter\def\csname val@census.uiv.applications\endcsname{83}
\expandafter\def\csname cnt@census.uiv.applications\endcsname{83}
\expandafter\def\csname pct@census.uiv.applications\endcsname{8300.0}
\expandafter\def\csname ppt@census.uiv.applications\endcsname{$+$8300.0}
\expandafter\def\csname val@census.uiv.median-target-short-side-px\endcsname{15.650}
\expandafter\def\csname cnt@census.uiv.median-target-short-side-px\endcsname{16}
\expandafter\def\csname pct@census.uiv.median-target-short-side-px\endcsname{1565.0}
\expandafter\def\csname ppt@census.uiv.median-target-short-side-px\endcsname{$+$1565.0}
\expandafter\def\csname val@census.uiv.median-target-side-text\endcsname{15.6}
\expandafter\def\csname val@census.uiv.n-target-sizes\endcsname{304}
\expandafter\def\csname cnt@census.uiv.n-target-sizes\endcsname{304}
\expandafter\def\csname pct@census.uiv.n-target-sizes\endcsname{30400.0}
\expandafter\def\csname ppt@census.uiv.n-target-sizes\endcsname{$+$30400.0}
\expandafter\def\csname val@census.uiv.roots-kept\endcsname{1561}
\expandafter\def\csname cnt@census.uiv.roots-kept\endcsname{1{,}561}
\expandafter\def\csname pct@census.uiv.roots-kept\endcsname{156100.0}
\expandafter\def\csname ppt@census.uiv.roots-kept\endcsname{$+$156100.0}
\expandafter\def\csname val@census.uiv.screenshots\endcsname{1164}
\expandafter\def\csname cnt@census.uiv.screenshots\endcsname{1{,}164}
\expandafter\def\csname pct@census.uiv.screenshots\endcsname{116400.0}
\expandafter\def\csname ppt@census.uiv.screenshots\endcsname{$+$116400.0}
\expandafter\def\csname val@d020.n-C\endcsname{16}
\expandafter\def\csname cnt@d020.n-C\endcsname{16}
\expandafter\def\csname pct@d020.n-C\endcsname{1600.0}
\expandafter\def\csname ppt@d020.n-C\endcsname{$+$1600.0}
\expandafter\def\csname val@d020.n-T\endcsname{14}
\expandafter\def\csname cnt@d020.n-T\endcsname{14}
\expandafter\def\csname pct@d020.n-T\endcsname{1400.0}
\expandafter\def\csname ppt@d020.n-T\endcsname{$+$1400.0}
\expandafter\def\csname val@d020.n-total\endcsname{30}
\expandafter\def\csname cnt@d020.n-total\endcsname{30}
\expandafter\def\csname pct@d020.n-total\endcsname{3000.0}
\expandafter\def\csname ppt@d020.n-total\endcsname{$+$3000.0}
\expandafter\def\csname val@d020.sensitivity.max-abs-change\endcsname{0.007}
\expandafter\def\csname cnt@d020.sensitivity.max-abs-change\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.max-abs-change\endcsname{0.7}
\expandafter\def\csname ppt@d020.sensitivity.max-abs-change\endcsname{$+$0.7}
\expandafter\def\csname val@d020.sensitivity.n-excluded-pairs\endcsname{12}
\expandafter\def\csname cnt@d020.sensitivity.n-excluded-pairs\endcsname{12}
\expandafter\def\csname pct@d020.sensitivity.n-excluded-pairs\endcsname{1200.0}
\expandafter\def\csname ppt@d020.sensitivity.n-excluded-pairs\endcsname{$+$1200.0}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-generic-ppi-source.base\endcsname{0.013}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-generic-ppi-source.base\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-generic-ppi-source.base\endcsname{1.3}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-generic-ppi-source.base\endcsname{$+$1.3}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-generic-ppi-source.excluding\endcsname{0.008}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-generic-ppi-source.excluding\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-generic-ppi-source.excluding\endcsname{0.8}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-generic-ppi-source.excluding\endcsname{$+$0.8}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-replay-only.base\endcsname{-0.030}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-replay-only.base\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-replay-only.base\endcsname{$-$3.0}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-replay-only.base\endcsname{$-$3.0}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-replay-only.excluding\endcsname{-0.028}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-replay-only.excluding\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-replay-only.excluding\endcsname{$-$2.8}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-replay-only.excluding\endcsname{$-$2.8}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-replay-ppi-uniform.base\endcsname{0.001}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-replay-ppi-uniform.base\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-replay-ppi-uniform.base\endcsname{0.1}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-replay-ppi-uniform.base\endcsname{$+$0.1}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-replay-ppi-uniform.excluding\endcsname{-0.001}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-replay-ppi-uniform.excluding\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-replay-ppi-uniform.excluding\endcsname{$-$0.1}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-replay-ppi-uniform.excluding\endcsname{$-$0.1}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-uniform-fresh.base\endcsname{0.007}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-uniform-fresh.base\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-uniform-fresh.base\endcsname{0.7}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-uniform-fresh.base\endcsname{$+$0.7}
\expandafter\def\csname val@d020.sensitivity.rcr-minus-uniform-fresh.excluding\endcsname{0.007}
\expandafter\def\csname cnt@d020.sensitivity.rcr-minus-uniform-fresh.excluding\endcsname{0}
\expandafter\def\csname pct@d020.sensitivity.rcr-minus-uniform-fresh.excluding\endcsname{0.7}
\expandafter\def\csname ppt@d020.sensitivity.rcr-minus-uniform-fresh.excluding\endcsname{$+$0.7}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.1.agreement\endcsname{0.930}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.1.agreement\endcsname{93.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.1.agreement\endcsname{$+$93.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.1.rmse\endcsname{0.138}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.1.rmse\endcsname{13.8}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.1.rmse\endcsname{$+$13.8}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.25.agreement\endcsname{0.950}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.25.agreement\endcsname{95.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.25.agreement\endcsname{$+$95.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.25.rmse\endcsname{0.082}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.25.rmse\endcsname{8.2}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.25.rmse\endcsname{$+$8.2}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.5.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.5.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.5.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@0.5.rmse\endcsname{0.044}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@0.5.rmse\endcsname{4.4}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@0.5.rmse\endcsname{$+$4.4}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.old-source.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.old-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.old-source.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.old-source.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.old-source.rmse\endcsname{0.045}
\expandafter\def\csname cnt@expl.sspro.p1.e1.old-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.old-source.rmse\endcsname{4.5}
\expandafter\def\csname ppt@expl.sspro.p1.e1.old-source.rmse\endcsname{$+$4.5}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{100}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{100}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{10000.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{$+$10000.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.25.agreement\endcsname{0.990}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.25.agreement\endcsname{99.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.25.agreement\endcsname{$+$99.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.25.rmse\endcsname{0.077}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.25.rmse\endcsname{7.7}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.25.rmse\endcsname{$+$7.7}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.5.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.5.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.5.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@0.5.rmse\endcsname{0.039}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@0.5.rmse\endcsname{3.9}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@0.5.rmse\endcsname{$+$3.9}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.rcr-stratified@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.rcr-stratified@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-only.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-only.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-only.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-only.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-only.rmse\endcsname{0.041}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-only.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-only.rmse\endcsname{4.1}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-only.rmse\endcsname{$+$4.1}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{0.920}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{92.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{$+$92.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{0.120}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{12.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{$+$12.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{0.940}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{94.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{$+$94.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{0.066}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{6.6}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{$+$6.6}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{0.038}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{3.8}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{$+$3.8}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.1.agreement\endcsname{0.910}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.1.agreement\endcsname{91.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.1.agreement\endcsname{$+$91.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.1.rmse\endcsname{0.209}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.1.rmse\endcsname{20.9}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.1.rmse\endcsname{$+$20.9}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.25.agreement\endcsname{0.940}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.25.agreement\endcsname{94.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.25.agreement\endcsname{$+$94.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.25.rmse\endcsname{0.122}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.25.rmse\endcsname{12.2}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.25.rmse\endcsname{$+$12.2}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.5.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.5.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.5.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@0.5.rmse\endcsname{0.065}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@0.5.rmse\endcsname{6.5}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@0.5.rmse\endcsname{$+$6.5}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e1.uniform-fresh@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1.uniform-fresh@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.ci95.1\endcsname{0.060}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.ci95.1\endcsname{6.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.ci95.1\endcsname{$+$6.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.delta-eta2\endcsname{0.002}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.delta-eta2\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.delta-eta2\endcsname{0.2}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.delta-eta2\endcsname{$+$0.2}
\expandafter\def\csname val@expl.sspro.p1.e10.C.n-flagged\endcsname{10}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.n-flagged\endcsname{10}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.n-flagged\endcsname{1000.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.n-flagged\endcsname{$+$1000.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.perm-null-mean\endcsname{0.015}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.perm-null-mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.perm-null-mean\endcsname{1.5}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.perm-null-mean\endcsname{$+$1.5}
\expandafter\def\csname val@expl.sspro.p1.e10.C.perm-p\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.perm-p\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.perm-p\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.perm-p\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.perm-p-rowwise\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.perm-p-rowwise\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.perm-p-rowwise\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.perm-p-rowwise\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.share-in-disagree\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.share-in-disagree\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.share-in-disagree\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.share-in-disagree\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e10.C.share-outside-agree-stable\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e10.C.share-outside-agree-stable\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e10.C.share-outside-agree-stable\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e10.C.share-outside-agree-stable\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1eq.generic-ppi-source.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.generic-ppi-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.generic-ppi-source.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.generic-ppi-source.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1eq.generic-ppi-source.rmse\endcsname{0.033}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.generic-ppi-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.generic-ppi-source.rmse\endcsname{3.3}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.generic-ppi-source.rmse\endcsname{$+$3.3}
\expandafter\def\csname val@expl.sspro.p1.e1eq.rcr-stratified.agreement\endcsname{0.990}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.rcr-stratified.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.rcr-stratified.agreement\endcsname{99.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.rcr-stratified.agreement\endcsname{$+$99.0}
\expandafter\def\csname val@expl.sspro.p1.e1eq.rcr-stratified.rmse\endcsname{0.077}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.rcr-stratified.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.rcr-stratified.rmse\endcsname{7.7}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.rcr-stratified.rmse\endcsname{$+$7.7}
\expandafter\def\csname val@expl.sspro.p1.e1eq.replay-ppi-uniform.agreement\endcsname{0.940}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.replay-ppi-uniform.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.replay-ppi-uniform.agreement\endcsname{94.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.replay-ppi-uniform.agreement\endcsname{$+$94.0}
\expandafter\def\csname val@expl.sspro.p1.e1eq.replay-ppi-uniform.rmse\endcsname{0.066}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.replay-ppi-uniform.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.replay-ppi-uniform.rmse\endcsname{6.6}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.replay-ppi-uniform.rmse\endcsname{$+$6.6}
\expandafter\def\csname val@expl.sspro.p1.e1eq.uniform-fresh.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.uniform-fresh.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.uniform-fresh.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.uniform-fresh.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e1eq.uniform-fresh.rmse\endcsname{0.050}
\expandafter\def\csname cnt@expl.sspro.p1.e1eq.uniform-fresh.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e1eq.uniform-fresh.rmse\endcsname{5.0}
\expandafter\def\csname ppt@expl.sspro.p1.e1eq.uniform-fresh.rmse\endcsname{$+$5.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{0.010}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{1.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{$+$1.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{-0.005}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.5}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.5}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{3}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{3}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{300.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{$+$300.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{3}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{3}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{300.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{$+$300.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-only.max\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-only.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-only.max\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-only.max\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-only.min\endcsname{-0.025}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-only.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-only.min\endcsname{$-$2.5}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-only.min\endcsname{$-$2.5}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-only.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-only.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-only.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-only.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-only.n-negative\endcsname{5}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-only.n-negative\endcsname{5}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-only.n-negative\endcsname{500.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-only.n-negative\endcsname{$+$500.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.006}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.6}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{$+$0.6}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{-0.003}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.3}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.3}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{2}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{2}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{200.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{$+$200.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{4}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{4}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{400.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{$+$400.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-uniform-fresh.max\endcsname{0.017}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-uniform-fresh.max\endcsname{1.7}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.max\endcsname{$+$1.7}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-uniform-fresh.min\endcsname{-0.011}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-uniform-fresh.min\endcsname{$-$1.1}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.min\endcsname{$-$1.1}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{2}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{2}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{200.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{$+$200.0}
\expandafter\def\csname val@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{4}
\expandafter\def\csname cnt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{4}
\expandafter\def\csname pct@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{400.0}
\expandafter\def\csname ppt@expl.sspro.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{$+$400.0}
\expandafter\def\csname val@expl.sspro.p1.e3.C.ci95.0\endcsname{-0.204}
\expandafter\def\csname cnt@expl.sspro.p1.e3.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e3.C.ci95.0\endcsname{$-$20.4}
\expandafter\def\csname ppt@expl.sspro.p1.e3.C.ci95.0\endcsname{$-$20.4}
\expandafter\def\csname val@expl.sspro.p1.e3.C.ci95.1\endcsname{0.227}
\expandafter\def\csname cnt@expl.sspro.p1.e3.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e3.C.ci95.1\endcsname{22.7}
\expandafter\def\csname ppt@expl.sspro.p1.e3.C.ci95.1\endcsname{$+$22.7}
\expandafter\def\csname val@expl.sspro.p1.e3.C.gap\endcsname{0.017}
\expandafter\def\csname cnt@expl.sspro.p1.e3.C.gap\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e3.C.gap\endcsname{1.7}
\expandafter\def\csname ppt@expl.sspro.p1.e3.C.gap\endcsname{$+$1.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.covered.N\endcsname{151}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.covered.N\endcsname{151}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.covered.N\endcsname{15100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.covered.N\endcsname{$+$15100.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.covered.acc-F\endcsname{0.927}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.covered.acc-F\endcsname{92.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.covered.acc-F\endcsname{$+$92.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.covered.acc-R\endcsname{0.947}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.covered.acc-R\endcsname{94.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.covered.acc-R\endcsname{$+$94.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.covered.resid-F-minus-R\endcsname{-0.020}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.covered.resid-F-minus-R\endcsname{$-$2.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.covered.resid-F-minus-R\endcsname{$-$2.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.covered.share\endcsname{0.863}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.covered.share\endcsname{86.3}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.covered.share\endcsname{$+$86.3}
\expandafter\def\csname val@expl.sspro.p1.e5.C.missed.N\endcsname{24}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.missed.N\endcsname{24}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.missed.N\endcsname{2400.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.missed.N\endcsname{$+$2400.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.missed.acc-F\endcsname{0.208}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.missed.acc-F\endcsname{20.8}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.missed.acc-F\endcsname{$+$20.8}
\expandafter\def\csname val@expl.sspro.p1.e5.C.missed.acc-R\endcsname{0.083}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.missed.acc-R\endcsname{8.3}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.missed.acc-R\endcsname{$+$8.3}
\expandafter\def\csname val@expl.sspro.p1.e5.C.missed.resid-F-minus-R\endcsname{0.125}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.missed.resid-F-minus-R\endcsname{12.5}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.missed.resid-F-minus-R\endcsname{$+$12.5}
\expandafter\def\csname val@expl.sspro.p1.e5.C.missed.share\endcsname{0.137}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.missed.share\endcsname{13.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.missed.share\endcsname{$+$13.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.missed.share-of-replay-errors\endcsname{0.733}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.missed.share-of-replay-errors\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.missed.share-of-replay-errors\endcsname{73.3}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.missed.share-of-replay-errors\endcsname{$+$73.3}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.covered.N\endcsname{76}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.covered.N\endcsname{76}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.covered.N\endcsname{7600.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.covered.N\endcsname{$+$7600.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.covered.acc-F\endcsname{0.895}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.covered.acc-F\endcsname{89.5}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.covered.acc-F\endcsname{$+$89.5}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.covered.acc-R\endcsname{0.908}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.covered.acc-R\endcsname{90.8}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.covered.acc-R\endcsname{$+$90.8}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{-0.013}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$1.3}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$1.3}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.covered.share\endcsname{0.864}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.covered.share\endcsname{86.4}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.covered.share\endcsname{$+$86.4}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.missed.N\endcsname{12}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.missed.N\endcsname{12}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.missed.N\endcsname{1200.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.missed.N\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.missed.acc-F\endcsname{0.250}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.missed.acc-F\endcsname{25.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.missed.acc-F\endcsname{$+$25.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.missed.acc-R\endcsname{0.167}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.missed.acc-R\endcsname{16.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.missed.acc-R\endcsname{$+$16.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0.083}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{8.3}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{$+$8.3}
\expandafter\def\csname val@expl.sspro.p1.e5.C.multi-view.missed.share\endcsname{0.136}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.multi-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.multi-view.missed.share\endcsname{13.6}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.multi-view.missed.share\endcsname{$+$13.6}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.covered.N\endcsname{75}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.covered.N\endcsname{75}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.covered.N\endcsname{7500.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.covered.N\endcsname{$+$7500.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.covered.acc-F\endcsname{0.960}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.covered.acc-F\endcsname{96.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.covered.acc-F\endcsname{$+$96.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.covered.acc-R\endcsname{0.987}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.covered.acc-R\endcsname{98.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.covered.acc-R\endcsname{$+$98.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{-0.027}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{$-$2.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{$-$2.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.covered.share\endcsname{0.862}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.covered.share\endcsname{86.2}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.covered.share\endcsname{$+$86.2}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.missed.N\endcsname{12}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.missed.N\endcsname{12}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.missed.N\endcsname{1200.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.missed.N\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.missed.acc-F\endcsname{0.167}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.missed.acc-F\endcsname{16.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.missed.acc-F\endcsname{$+$16.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{0.167}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{16.7}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{$+$16.7}
\expandafter\def\csname val@expl.sspro.p1.e5.C.single-view.missed.share\endcsname{0.138}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.single-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.single-view.missed.share\endcsname{13.8}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.single-view.missed.share\endcsname{$+$13.8}
\expandafter\def\csname val@expl.sspro.p1.e5.C.strata.agree-drift.missed-share\endcsname{0.200}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.strata.agree-drift.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.strata.agree-drift.missed-share\endcsname{20.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.strata.agree-drift.missed-share\endcsname{$+$20.0}
\expandafter\def\csname val@expl.sspro.p1.e5.C.strata.agree-stable.missed-share\endcsname{0.103}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.strata.agree-stable.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.strata.agree-stable.missed-share\endcsname{10.3}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.strata.agree-stable.missed-share\endcsname{$+$10.3}
\expandafter\def\csname val@expl.sspro.p1.e5.C.strata.disagree.missed-share\endcsname{0.304}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.strata.disagree.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.strata.disagree.missed-share\endcsname{30.4}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.strata.disagree.missed-share\endcsname{$+$30.4}
\expandafter\def\csname val@expl.sspro.p1.e5.C.strata.parse-fail.missed-share\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p1.e5.C.strata.parse-fail.missed-share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e5.C.strata.parse-fail.missed-share\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.C.strata.parse-fail.missed-share\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p1.e5.T.covered.N\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e5.T.covered.N\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.T.covered.N\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.T.covered.N\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e5.T.missed.N\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p1.e5.T.missed.N\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e5.T.missed.N\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e5.T.missed.N\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e6.histories\endcsname{20}
\expandafter\def\csname cnt@expl.sspro.p1.e6.histories\endcsname{20}
\expandafter\def\csname pct@expl.sspro.p1.e6.histories\endcsname{2000.0}
\expandafter\def\csname ppt@expl.sspro.p1.e6.histories\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{-0.007}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$0.7}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$0.7}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0.021}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{2.1}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{$+$2.1}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{0.003}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{0.3}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{$+$0.3}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0.354}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{35.4}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{$+$35.4}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-only.mean\endcsname{-0.002}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-only.mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-only.mean\endcsname{$-$0.2}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-only.p-le0\endcsname{0.853}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-only.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-only.p-le0\endcsname{85.3}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-only.p-le0\endcsname{$+$85.3}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{-0.009}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$0.9}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$0.9}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0.019}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{1.9}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{$+$1.9}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.002}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.2}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{$+$0.2}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0.415}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{41.5}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{$+$41.5}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{-0.017}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0.018}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{1.8}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{$+$1.8}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{0.505}
\expandafter\def\csname cnt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{50.5}
\expandafter\def\csname ppt@expl.sspro.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{$+$50.5}
\expandafter\def\csname val@expl.sspro.p1.e6.reps\endcsname{1000}
\expandafter\def\csname cnt@expl.sspro.p1.e6.reps\endcsname{1{,}000}
\expandafter\def\csname pct@expl.sspro.p1.e6.reps\endcsname{100000.0}
\expandafter\def\csname ppt@expl.sspro.p1.e6.reps\endcsname{$+$100000.0}
\expandafter\def\csname val@expl.sspro.p1.e8.C.direct-in-zoomed.n\endcsname{165}
\expandafter\def\csname cnt@expl.sspro.p1.e8.C.direct-in-zoomed.n\endcsname{165}
\expandafter\def\csname pct@expl.sspro.p1.e8.C.direct-in-zoomed.n\endcsname{16500.0}
\expandafter\def\csname ppt@expl.sspro.p1.e8.C.direct-in-zoomed.n\endcsname{$+$16500.0}
\expandafter\def\csname val@expl.sspro.p1.e8.C.direct-in-zoomed.resid\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e8.C.direct-in-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e8.C.direct-in-zoomed.resid\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e8.C.direct-in-zoomed.resid\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e8.C.direct-outside-zoomed.n\endcsname{10}
\expandafter\def\csname cnt@expl.sspro.p1.e8.C.direct-outside-zoomed.n\endcsname{10}
\expandafter\def\csname pct@expl.sspro.p1.e8.C.direct-outside-zoomed.n\endcsname{1000.0}
\expandafter\def\csname ppt@expl.sspro.p1.e8.C.direct-outside-zoomed.n\endcsname{$+$1000.0}
\expandafter\def\csname val@expl.sspro.p1.e8.C.direct-outside-zoomed.resid\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e8.C.direct-outside-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e8.C.direct-outside-zoomed.resid\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e8.C.direct-outside-zoomed.resid\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e8.C.eta2-agree-stable-vs-other\endcsname{0.012}
\expandafter\def\csname cnt@expl.sspro.p1.e8.C.eta2-agree-stable-vs-other\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e8.C.eta2-agree-stable-vs-other\endcsname{1.2}
\expandafter\def\csname ppt@expl.sspro.p1.e8.C.eta2-agree-stable-vs-other\endcsname{$+$1.2}
\expandafter\def\csname val@expl.sspro.p1.e8.C.eta2-direct-in-zoomed\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p1.e8.C.eta2-direct-in-zoomed\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e8.C.eta2-direct-in-zoomed\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p1.e8.C.eta2-direct-in-zoomed\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p1.e9.mean\endcsname{-0.026}
\expandafter\def\csname cnt@expl.sspro.p1.e9.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p1.e9.mean\endcsname{$-$2.6}
\expandafter\def\csname ppt@expl.sspro.p1.e9.mean\endcsname{$-$2.6}
\expandafter\def\csname val@expl.sspro.p1.e9.n\endcsname{4}
\expandafter\def\csname cnt@expl.sspro.p1.e9.n\endcsname{4}
\expandafter\def\csname pct@expl.sspro.p1.e9.n\endcsname{400.0}
\expandafter\def\csname ppt@expl.sspro.p1.e9.n\endcsname{$+$400.0}
\expandafter\def\csname val@expl.sspro.p1.e9.n-negative\endcsname{3}
\expandafter\def\csname cnt@expl.sspro.p1.e9.n-negative\endcsname{3}
\expandafter\def\csname pct@expl.sspro.p1.e9.n-negative\endcsname{300.0}
\expandafter\def\csname ppt@expl.sspro.p1.e9.n-negative\endcsname{$+$300.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.1.agreement\endcsname{0.920}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.1.agreement\endcsname{92.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.1.agreement\endcsname{$+$92.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.1.rmse\endcsname{0.131}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.1.rmse\endcsname{13.1}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.1.rmse\endcsname{$+$13.1}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.25.agreement\endcsname{0.890}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.25.agreement\endcsname{89.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.25.agreement\endcsname{$+$89.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.25.rmse\endcsname{0.087}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.25.rmse\endcsname{8.7}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.25.rmse\endcsname{$+$8.7}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.5.agreement\endcsname{0.960}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.5.agreement\endcsname{96.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.5.agreement\endcsname{$+$96.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@0.5.rmse\endcsname{0.049}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@0.5.rmse\endcsname{4.9}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@0.5.rmse\endcsname{$+$4.9}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.old-source.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.old-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.old-source.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.old-source.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.old-source.rmse\endcsname{0.048}
\expandafter\def\csname cnt@expl.sspro.p2.e1.old-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.old-source.rmse\endcsname{4.8}
\expandafter\def\csname ppt@expl.sspro.p2.e1.old-source.rmse\endcsname{$+$4.8}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.1.agreement\endcsname{0.912}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.1.agreement\endcsname{91.2}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.1.agreement\endcsname{$+$91.2}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{20}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{20}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{2000.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.1.rmse\endcsname{0.111}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.1.rmse\endcsname{11.1}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.1.rmse\endcsname{$+$11.1}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.25.agreement\endcsname{0.940}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.25.agreement\endcsname{94.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.25.agreement\endcsname{$+$94.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.25.rmse\endcsname{0.052}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.25.rmse\endcsname{5.2}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.25.rmse\endcsname{$+$5.2}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.5.agreement\endcsname{0.980}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.5.agreement\endcsname{98.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.5.agreement\endcsname{$+$98.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@0.5.rmse\endcsname{0.035}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@0.5.rmse\endcsname{3.5}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@0.5.rmse\endcsname{$+$3.5}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.rcr-stratified@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.rcr-stratified@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-only.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-only.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-only.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-only.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-only.rmse\endcsname{0.036}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-only.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-only.rmse\endcsname{3.6}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-only.rmse\endcsname{$+$3.6}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{0.910}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{91.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{$+$91.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{0.124}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{12.4}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{$+$12.4}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{0.890}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{89.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{$+$89.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{0.080}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{8.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{$+$8.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{0.950}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{95.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{$+$95.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{0.049}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{4.9}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{$+$4.9}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.1.agreement\endcsname{0.930}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.1.agreement\endcsname{93.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.1.agreement\endcsname{$+$93.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.1.rmse\endcsname{0.155}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.1.rmse\endcsname{15.5}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.1.rmse\endcsname{$+$15.5}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.25.agreement\endcsname{0.910}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.25.agreement\endcsname{91.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.25.agreement\endcsname{$+$91.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.25.rmse\endcsname{0.114}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.25.rmse\endcsname{11.4}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.25.rmse\endcsname{$+$11.4}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.5.agreement\endcsname{0.980}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.5.agreement\endcsname{98.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.5.agreement\endcsname{$+$98.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@0.5.rmse\endcsname{0.051}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@0.5.rmse\endcsname{5.1}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@0.5.rmse\endcsname{$+$5.1}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e1.uniform-fresh@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e1.uniform-fresh@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e10.C.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e10.C.ci95.1\endcsname{0.236}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.ci95.1\endcsname{23.6}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.ci95.1\endcsname{$+$23.6}
\expandafter\def\csname val@expl.sspro.p2.e10.C.delta-eta2\endcsname{0.010}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.delta-eta2\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.delta-eta2\endcsname{1.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.delta-eta2\endcsname{$+$1.0}
\expandafter\def\csname val@expl.sspro.p2.e10.C.n-flagged\endcsname{21}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.n-flagged\endcsname{21}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.n-flagged\endcsname{2100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.n-flagged\endcsname{$+$2100.0}
\expandafter\def\csname val@expl.sspro.p2.e10.C.perm-null-mean\endcsname{0.015}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.perm-null-mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.perm-null-mean\endcsname{1.5}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.perm-null-mean\endcsname{$+$1.5}
\expandafter\def\csname val@expl.sspro.p2.e10.C.perm-p\endcsname{0.716}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.perm-p\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.perm-p\endcsname{71.6}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.perm-p\endcsname{$+$71.6}
\expandafter\def\csname val@expl.sspro.p2.e10.C.perm-p-rowwise\endcsname{0.673}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.perm-p-rowwise\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.perm-p-rowwise\endcsname{67.3}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.perm-p-rowwise\endcsname{$+$67.3}
\expandafter\def\csname val@expl.sspro.p2.e10.C.share-in-disagree\endcsname{0.905}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.share-in-disagree\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.share-in-disagree\endcsname{90.5}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.share-in-disagree\endcsname{$+$90.5}
\expandafter\def\csname val@expl.sspro.p2.e10.C.share-outside-agree-stable\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.C.share-outside-agree-stable\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.C.share-outside-agree-stable\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.C.share-outside-agree-stable\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e10.T.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e10.T.ci95.1\endcsname{0.055}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.ci95.1\endcsname{5.5}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.ci95.1\endcsname{$+$5.5}
\expandafter\def\csname val@expl.sspro.p2.e10.T.delta-eta2\endcsname{0.001}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.delta-eta2\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.delta-eta2\endcsname{0.1}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.delta-eta2\endcsname{$+$0.1}
\expandafter\def\csname val@expl.sspro.p2.e10.T.n-flagged\endcsname{17}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.n-flagged\endcsname{17}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.n-flagged\endcsname{1700.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.n-flagged\endcsname{$+$1700.0}
\expandafter\def\csname val@expl.sspro.p2.e10.T.perm-null-mean\endcsname{0.006}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.perm-null-mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.perm-null-mean\endcsname{0.6}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.perm-null-mean\endcsname{$+$0.6}
\expandafter\def\csname val@expl.sspro.p2.e10.T.perm-p\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.perm-p\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.perm-p\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.perm-p\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e10.T.perm-p-rowwise\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.perm-p-rowwise\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.perm-p-rowwise\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.perm-p-rowwise\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e10.T.share-in-disagree\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.share-in-disagree\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.share-in-disagree\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.share-in-disagree\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e10.T.share-outside-agree-stable\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e10.T.share-outside-agree-stable\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e10.T.share-outside-agree-stable\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e10.T.share-outside-agree-stable\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e1eq.generic-ppi-source.agreement\endcsname{0.969}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.generic-ppi-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.generic-ppi-source.agreement\endcsname{96.9}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.generic-ppi-source.agreement\endcsname{$+$96.9}
\expandafter\def\csname val@expl.sspro.p2.e1eq.generic-ppi-source.rmse\endcsname{0.037}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.generic-ppi-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.generic-ppi-source.rmse\endcsname{3.7}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.generic-ppi-source.rmse\endcsname{$+$3.7}
\expandafter\def\csname val@expl.sspro.p2.e1eq.rcr-stratified.agreement\endcsname{0.940}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.rcr-stratified.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.rcr-stratified.agreement\endcsname{94.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.rcr-stratified.agreement\endcsname{$+$94.0}
\expandafter\def\csname val@expl.sspro.p2.e1eq.rcr-stratified.rmse\endcsname{0.052}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.rcr-stratified.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.rcr-stratified.rmse\endcsname{5.2}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.rcr-stratified.rmse\endcsname{$+$5.2}
\expandafter\def\csname val@expl.sspro.p2.e1eq.replay-ppi-uniform.agreement\endcsname{0.890}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.replay-ppi-uniform.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.replay-ppi-uniform.agreement\endcsname{89.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.replay-ppi-uniform.agreement\endcsname{$+$89.0}
\expandafter\def\csname val@expl.sspro.p2.e1eq.replay-ppi-uniform.rmse\endcsname{0.080}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.replay-ppi-uniform.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.replay-ppi-uniform.rmse\endcsname{8.0}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.replay-ppi-uniform.rmse\endcsname{$+$8.0}
\expandafter\def\csname val@expl.sspro.p2.e1eq.uniform-fresh.agreement\endcsname{0.985}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.uniform-fresh.agreement\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.uniform-fresh.agreement\endcsname{98.5}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.uniform-fresh.agreement\endcsname{$+$98.5}
\expandafter\def\csname val@expl.sspro.p2.e1eq.uniform-fresh.rmse\endcsname{0.039}
\expandafter\def\csname cnt@expl.sspro.p2.e1eq.uniform-fresh.rmse\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e1eq.uniform-fresh.rmse\endcsname{3.9}
\expandafter\def\csname ppt@expl.sspro.p2.e1eq.uniform-fresh.rmse\endcsname{$+$3.9}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{0.007}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{0.7}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{$+$0.7}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{-0.005}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.5}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.5}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{2}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{2}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{200.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{$+$200.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{4}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{4}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{400.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{$+$400.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-only.max\endcsname{-0.014}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-only.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-only.max\endcsname{$-$1.4}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-only.max\endcsname{$-$1.4}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-only.min\endcsname{-0.018}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-only.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-only.min\endcsname{$-$1.8}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-only.min\endcsname{$-$1.8}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-only.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-only.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-only.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-only.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-only.n-negative\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-only.n-negative\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-only.n-negative\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-only.n-negative\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-only.n-positive\endcsname{0}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-only.n-positive\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-only.n-positive\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-only.n-positive\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.002}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.2}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{$+$0.2}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{-0.008}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.8}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.8}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{5}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{5}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{500.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{$+$500.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{1}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-uniform-fresh.max\endcsname{0.008}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.max\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-uniform-fresh.max\endcsname{0.8}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.max\endcsname{$+$0.8}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-uniform-fresh.min\endcsname{-0.006}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.min\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-uniform-fresh.min\endcsname{$-$0.6}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.min\endcsname{$-$0.6}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{5}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{5}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{500.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{$+$500.0}
\expandafter\def\csname val@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{1}
\expandafter\def\csname cnt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e3.C.ci95.0\endcsname{0.040}
\expandafter\def\csname cnt@expl.sspro.p2.e3.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e3.C.ci95.0\endcsname{4.0}
\expandafter\def\csname ppt@expl.sspro.p2.e3.C.ci95.0\endcsname{$+$4.0}
\expandafter\def\csname val@expl.sspro.p2.e3.C.ci95.1\endcsname{1.022}
\expandafter\def\csname cnt@expl.sspro.p2.e3.C.ci95.1\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e3.C.ci95.1\endcsname{102.2}
\expandafter\def\csname ppt@expl.sspro.p2.e3.C.ci95.1\endcsname{$+$102.2}
\expandafter\def\csname val@expl.sspro.p2.e3.C.gap\endcsname{0.120}
\expandafter\def\csname cnt@expl.sspro.p2.e3.C.gap\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e3.C.gap\endcsname{12.0}
\expandafter\def\csname ppt@expl.sspro.p2.e3.C.gap\endcsname{$+$12.0}
\expandafter\def\csname val@expl.sspro.p2.e3.T.ci95.0\endcsname{0.029}
\expandafter\def\csname cnt@expl.sspro.p2.e3.T.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e3.T.ci95.0\endcsname{2.9}
\expandafter\def\csname ppt@expl.sspro.p2.e3.T.ci95.0\endcsname{$+$2.9}
\expandafter\def\csname val@expl.sspro.p2.e3.T.ci95.1\endcsname{0.178}
\expandafter\def\csname cnt@expl.sspro.p2.e3.T.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e3.T.ci95.1\endcsname{17.8}
\expandafter\def\csname ppt@expl.sspro.p2.e3.T.ci95.1\endcsname{$+$17.8}
\expandafter\def\csname val@expl.sspro.p2.e3.T.gap\endcsname{0.089}
\expandafter\def\csname cnt@expl.sspro.p2.e3.T.gap\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e3.T.gap\endcsname{8.9}
\expandafter\def\csname ppt@expl.sspro.p2.e3.T.gap\endcsname{$+$8.9}
\expandafter\def\csname val@expl.sspro.p2.e4.center-d1.diff.ci95.0\endcsname{-0.062}
\expandafter\def\csname cnt@expl.sspro.p2.e4.center-d1.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.center-d1.diff.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname ppt@expl.sspro.p2.e4.center-d1.diff.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname val@expl.sspro.p2.e4.center-d1.diff.ci95.1\endcsname{0.146}
\expandafter\def\csname cnt@expl.sspro.p2.e4.center-d1.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.center-d1.diff.ci95.1\endcsname{14.6}
\expandafter\def\csname ppt@expl.sspro.p2.e4.center-d1.diff.ci95.1\endcsname{$+$14.6}
\expandafter\def\csname val@expl.sspro.p2.e4.center-d1.diff.mean\endcsname{0.042}
\expandafter\def\csname cnt@expl.sspro.p2.e4.center-d1.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.center-d1.diff.mean\endcsname{4.2}
\expandafter\def\csname ppt@expl.sspro.p2.e4.center-d1.diff.mean\endcsname{$+$4.2}
\expandafter\def\csname val@expl.sspro.p2.e4.center-d1.n\endcsname{48}
\expandafter\def\csname cnt@expl.sspro.p2.e4.center-d1.n\endcsname{48}
\expandafter\def\csname pct@expl.sspro.p2.e4.center-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.center-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@expl.sspro.p2.e4.context-d1.diff.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e4.context-d1.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.context-d1.diff.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.context-d1.diff.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e4.context-d1.diff.ci95.1\endcsname{0.125}
\expandafter\def\csname cnt@expl.sspro.p2.e4.context-d1.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.context-d1.diff.ci95.1\endcsname{12.5}
\expandafter\def\csname ppt@expl.sspro.p2.e4.context-d1.diff.ci95.1\endcsname{$+$12.5}
\expandafter\def\csname val@expl.sspro.p2.e4.context-d1.diff.mean\endcsname{0.062}
\expandafter\def\csname cnt@expl.sspro.p2.e4.context-d1.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.context-d1.diff.mean\endcsname{6.2}
\expandafter\def\csname ppt@expl.sspro.p2.e4.context-d1.diff.mean\endcsname{$+$6.2}
\expandafter\def\csname val@expl.sspro.p2.e4.context-d1.n\endcsname{48}
\expandafter\def\csname cnt@expl.sspro.p2.e4.context-d1.n\endcsname{48}
\expandafter\def\csname pct@expl.sspro.p2.e4.context-d1.n\endcsname{4800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.context-d1.n\endcsname{$+$4800.0}
\expandafter\def\csname val@expl.sspro.p2.e4.dual-d2.diff.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@expl.sspro.p2.e4.dual-d2.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.dual-d2.diff.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@expl.sspro.p2.e4.dual-d2.diff.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@expl.sspro.p2.e4.dual-d2.diff.ci95.1\endcsname{0.167}
\expandafter\def\csname cnt@expl.sspro.p2.e4.dual-d2.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.dual-d2.diff.ci95.1\endcsname{16.7}
\expandafter\def\csname ppt@expl.sspro.p2.e4.dual-d2.diff.ci95.1\endcsname{$+$16.7}
\expandafter\def\csname val@expl.sspro.p2.e4.dual-d2.diff.mean\endcsname{0.104}
\expandafter\def\csname cnt@expl.sspro.p2.e4.dual-d2.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.dual-d2.diff.mean\endcsname{10.4}
\expandafter\def\csname ppt@expl.sspro.p2.e4.dual-d2.diff.mean\endcsname{$+$10.4}
\expandafter\def\csname val@expl.sspro.p2.e4.dual-d2.n\endcsname{48}
\expandafter\def\csname cnt@expl.sspro.p2.e4.dual-d2.n\endcsname{48}
\expandafter\def\csname pct@expl.sspro.p2.e4.dual-d2.n\endcsname{4800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.dual-d2.n\endcsname{$+$4800.0}
\expandafter\def\csname val@expl.sspro.p2.e4.grid2-d3.diff.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e4.grid2-d3.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.grid2-d3.diff.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.grid2-d3.diff.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e4.grid2-d3.diff.ci95.1\endcsname{0.125}
\expandafter\def\csname cnt@expl.sspro.p2.e4.grid2-d3.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.grid2-d3.diff.ci95.1\endcsname{12.5}
\expandafter\def\csname ppt@expl.sspro.p2.e4.grid2-d3.diff.ci95.1\endcsname{$+$12.5}
\expandafter\def\csname val@expl.sspro.p2.e4.grid2-d3.diff.mean\endcsname{0.062}
\expandafter\def\csname cnt@expl.sspro.p2.e4.grid2-d3.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.grid2-d3.diff.mean\endcsname{6.2}
\expandafter\def\csname ppt@expl.sspro.p2.e4.grid2-d3.diff.mean\endcsname{$+$6.2}
\expandafter\def\csname val@expl.sspro.p2.e4.grid2-d3.n\endcsname{48}
\expandafter\def\csname cnt@expl.sspro.p2.e4.grid2-d3.n\endcsname{48}
\expandafter\def\csname pct@expl.sspro.p2.e4.grid2-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.grid2-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e4.zoomclick-d3.diff.mean\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e4.zoomclick-d3.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e4.zoomclick-d3.diff.mean\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.zoomclick-d3.diff.mean\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e4.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname cnt@expl.sspro.p2.e4.zoomclick-d3.n\endcsname{48}
\expandafter\def\csname pct@expl.sspro.p2.e4.zoomclick-d3.n\endcsname{4800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e4.zoomclick-d3.n\endcsname{$+$4800.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.covered.N\endcsname{163}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.covered.N\endcsname{163}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.covered.N\endcsname{16300.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.covered.N\endcsname{$+$16300.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.covered.acc-F\endcsname{0.908}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.covered.acc-F\endcsname{90.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.covered.acc-F\endcsname{$+$90.8}
\expandafter\def\csname val@expl.sspro.p2.e5.C.covered.acc-R\endcsname{0.939}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.covered.acc-R\endcsname{93.9}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.covered.acc-R\endcsname{$+$93.9}
\expandafter\def\csname val@expl.sspro.p2.e5.C.covered.resid-F-minus-R\endcsname{-0.031}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.covered.resid-F-minus-R\endcsname{$-$3.1}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.covered.resid-F-minus-R\endcsname{$-$3.1}
\expandafter\def\csname val@expl.sspro.p2.e5.C.covered.share\endcsname{0.858}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.covered.share\endcsname{85.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.covered.share\endcsname{$+$85.8}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.N\endcsname{27}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.N\endcsname{27}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.N\endcsname{2700.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.N\endcsname{$+$2700.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.acc-F\endcsname{0.296}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.acc-F\endcsname{29.6}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.acc-F\endcsname{$+$29.6}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.acc-R\endcsname{0.037}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.acc-R\endcsname{3.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.acc-R\endcsname{$+$3.7}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.resid-F-minus-R\endcsname{0.259}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.resid-F-minus-R\endcsname{25.9}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.resid-F-minus-R\endcsname{$+$25.9}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.share\endcsname{0.142}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.share\endcsname{14.2}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.share\endcsname{$+$14.2}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.share-of-net-residual\endcsname{3.500}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.share-of-net-residual\endcsname{4}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.share-of-net-residual\endcsname{350.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.share-of-net-residual\endcsname{$+$350.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.missed.share-of-replay-errors\endcsname{0.722}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.missed.share-of-replay-errors\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.missed.share-of-replay-errors\endcsname{72.2}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.missed.share-of-replay-errors\endcsname{$+$72.2}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.covered.N\endcsname{81}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.covered.N\endcsname{81}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.covered.N\endcsname{8100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.covered.N\endcsname{$+$8100.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.covered.acc-F\endcsname{0.877}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.covered.acc-F\endcsname{87.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.covered.acc-F\endcsname{$+$87.7}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.covered.acc-R\endcsname{0.938}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.covered.acc-R\endcsname{93.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.covered.acc-R\endcsname{$+$93.8}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{-0.062}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$6.2}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$6.2}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.covered.share\endcsname{0.844}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.covered.share\endcsname{84.4}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.covered.share\endcsname{$+$84.4}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.missed.N\endcsname{15}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.missed.N\endcsname{15}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.missed.N\endcsname{1500.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.missed.N\endcsname{$+$1500.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.missed.acc-F\endcsname{0.467}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.missed.acc-F\endcsname{46.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.missed.acc-F\endcsname{$+$46.7}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.missed.acc-R\endcsname{0.067}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.missed.acc-R\endcsname{6.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.missed.acc-R\endcsname{$+$6.7}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0.400}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{40.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{$+$40.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.multi-view.missed.share\endcsname{0.156}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.multi-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.multi-view.missed.share\endcsname{15.6}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.multi-view.missed.share\endcsname{$+$15.6}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.covered.N\endcsname{82}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.covered.N\endcsname{82}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.covered.N\endcsname{8200.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.covered.N\endcsname{$+$8200.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.covered.acc-F\endcsname{0.939}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.covered.acc-F\endcsname{93.9}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.covered.acc-F\endcsname{$+$93.9}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.covered.acc-R\endcsname{0.939}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.covered.acc-R\endcsname{93.9}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.covered.acc-R\endcsname{$+$93.9}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.covered.share\endcsname{0.872}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.covered.share\endcsname{87.2}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.covered.share\endcsname{$+$87.2}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.missed.N\endcsname{12}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.missed.N\endcsname{12}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.missed.N\endcsname{1200.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.missed.N\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.missed.acc-F\endcsname{0.083}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.missed.acc-F\endcsname{8.3}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.missed.acc-F\endcsname{$+$8.3}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{0.083}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{8.3}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{$+$8.3}
\expandafter\def\csname val@expl.sspro.p2.e5.C.single-view.missed.share\endcsname{0.128}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.single-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.single-view.missed.share\endcsname{12.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.single-view.missed.share\endcsname{$+$12.8}
\expandafter\def\csname val@expl.sspro.p2.e5.C.strata.agree-drift.missed-share\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.strata.agree-drift.missed-share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.strata.agree-drift.missed-share\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.strata.agree-drift.missed-share\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.strata.agree-stable.missed-share\endcsname{0.050}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.strata.agree-stable.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.strata.agree-stable.missed-share\endcsname{5.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.strata.agree-stable.missed-share\endcsname{$+$5.0}
\expandafter\def\csname val@expl.sspro.p2.e5.C.strata.disagree.missed-share\endcsname{0.607}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.strata.disagree.missed-share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.strata.disagree.missed-share\endcsname{60.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.strata.disagree.missed-share\endcsname{$+$60.7}
\expandafter\def\csname val@expl.sspro.p2.e5.C.strata.parse-fail.missed-share\endcsname{1.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.C.strata.parse-fail.missed-share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.C.strata.parse-fail.missed-share\endcsname{100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.C.strata.parse-fail.missed-share\endcsname{$+$100.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.covered.N\endcsname{361}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.covered.N\endcsname{361}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.covered.N\endcsname{36100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.covered.N\endcsname{$+$36100.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.covered.acc-F\endcsname{0.936}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.covered.acc-F\endcsname{93.6}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.covered.acc-F\endcsname{$+$93.6}
\expandafter\def\csname val@expl.sspro.p2.e5.T.covered.acc-R\endcsname{0.931}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.covered.acc-R\endcsname{93.1}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.covered.acc-R\endcsname{$+$93.1}
\expandafter\def\csname val@expl.sspro.p2.e5.T.covered.resid-F-minus-R\endcsname{0.006}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.covered.resid-F-minus-R\endcsname{0.6}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.covered.resid-F-minus-R\endcsname{$+$0.6}
\expandafter\def\csname val@expl.sspro.p2.e5.T.covered.share\endcsname{0.963}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.covered.share\endcsname{96.3}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.covered.share\endcsname{$+$96.3}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.N\endcsname{14}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.N\endcsname{14}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.N\endcsname{1400.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.N\endcsname{$+$1400.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.acc-F\endcsname{0.286}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.acc-F\endcsname{28.6}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.acc-F\endcsname{$+$28.6}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.resid-F-minus-R\endcsname{0.286}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.resid-F-minus-R\endcsname{28.6}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.resid-F-minus-R\endcsname{$+$28.6}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.share\endcsname{0.037}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.share\endcsname{3.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.share\endcsname{$+$3.7}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.share-of-net-residual\endcsname{0.667}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.share-of-net-residual\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.share-of-net-residual\endcsname{66.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.share-of-net-residual\endcsname{$+$66.7}
\expandafter\def\csname val@expl.sspro.p2.e5.T.missed.share-of-replay-errors\endcsname{0.359}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.missed.share-of-replay-errors\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.missed.share-of-replay-errors\endcsname{35.9}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.missed.share-of-replay-errors\endcsname{$+$35.9}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.covered.N\endcsname{184}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.covered.N\endcsname{184}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.covered.N\endcsname{18400.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.covered.N\endcsname{$+$18400.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.covered.acc-F\endcsname{0.935}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.covered.acc-F\endcsname{93.5}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.covered.acc-F\endcsname{$+$93.5}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.covered.acc-R\endcsname{0.924}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.covered.acc-R\endcsname{92.4}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.covered.acc-R\endcsname{$+$92.4}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{0.011}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{1.1}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{$+$1.1}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.covered.share\endcsname{0.968}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.covered.share\endcsname{96.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.covered.share\endcsname{$+$96.8}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.missed.N\endcsname{6}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.missed.N\endcsname{6}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.missed.N\endcsname{600.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.missed.N\endcsname{$+$600.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.missed.acc-F\endcsname{0.167}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.missed.acc-F\endcsname{16.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.missed.acc-F\endcsname{$+$16.7}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{0.167}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{16.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{$+$16.7}
\expandafter\def\csname val@expl.sspro.p2.e5.T.multi-view.missed.share\endcsname{0.032}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.multi-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.multi-view.missed.share\endcsname{3.2}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.multi-view.missed.share\endcsname{$+$3.2}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.covered.N\endcsname{177}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.covered.N\endcsname{177}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.covered.N\endcsname{17700.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.covered.N\endcsname{$+$17700.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.covered.acc-F\endcsname{0.938}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.covered.acc-F\endcsname{93.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.covered.acc-F\endcsname{$+$93.8}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.covered.acc-R\endcsname{0.938}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.covered.acc-R\endcsname{93.8}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.covered.acc-R\endcsname{$+$93.8}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.covered.share\endcsname{0.957}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.covered.share\endcsname{95.7}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.covered.share\endcsname{$+$95.7}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.missed.N\endcsname{8}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.missed.N\endcsname{8}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.missed.N\endcsname{800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.missed.N\endcsname{$+$800.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.missed.acc-F\endcsname{0.375}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.missed.acc-F\endcsname{37.5}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.missed.acc-F\endcsname{$+$37.5}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{0.375}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{37.5}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{$+$37.5}
\expandafter\def\csname val@expl.sspro.p2.e5.T.single-view.missed.share\endcsname{0.043}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.single-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.single-view.missed.share\endcsname{4.3}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.single-view.missed.share\endcsname{$+$4.3}
\expandafter\def\csname val@expl.sspro.p2.e5.T.strata.agree-drift.missed-share\endcsname{0.000}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.strata.agree-drift.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.strata.agree-drift.missed-share\endcsname{0.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.strata.agree-drift.missed-share\endcsname{0.0}
\expandafter\def\csname val@expl.sspro.p2.e5.T.strata.agree-stable.missed-share\endcsname{0.012}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.strata.agree-stable.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.strata.agree-stable.missed-share\endcsname{1.2}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.strata.agree-stable.missed-share\endcsname{$+$1.2}
\expandafter\def\csname val@expl.sspro.p2.e5.T.strata.disagree.missed-share\endcsname{0.270}
\expandafter\def\csname cnt@expl.sspro.p2.e5.T.strata.disagree.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e5.T.strata.disagree.missed-share\endcsname{27.0}
\expandafter\def\csname ppt@expl.sspro.p2.e5.T.strata.disagree.missed-share\endcsname{$+$27.0}
\expandafter\def\csname val@expl.sspro.p2.e6.histories\endcsname{20}
\expandafter\def\csname cnt@expl.sspro.p2.e6.histories\endcsname{20}
\expandafter\def\csname pct@expl.sspro.p2.e6.histories\endcsname{2000.0}
\expandafter\def\csname ppt@expl.sspro.p2.e6.histories\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{-0.021}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$2.1}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0.015}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{1.5}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{$+$1.5}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{-0.001}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{$-$0.1}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{$-$0.1}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0.579}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{57.9}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{$+$57.9}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{-0.036}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$3.6}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$3.6}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{0.032}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{3.2}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{$+$3.2}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-only.mean\endcsname{-0.008}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-only.mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-only.mean\endcsname{$-$0.8}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-only.p-le0\endcsname{0.808}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-only.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-only.p-le0\endcsname{80.8}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-only.p-le0\endcsname{$+$80.8}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{-0.016}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$1.6}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$1.6}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{-0.001}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{$-$0.1}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{$-$0.1}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0.583}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{58.3}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{$+$58.3}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{-0.026}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$2.6}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$2.6}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0.009}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0.9}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{$+$0.9}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{-0.004}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{$-$0.4}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{$-$0.4}
\expandafter\def\csname val@expl.sspro.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{0.696}
\expandafter\def\csname cnt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.sspro.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{69.6}
\expandafter\def\csname ppt@expl.sspro.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{$+$69.6}
\expandafter\def\csname val@expl.sspro.p2.e6.reps\endcsname{1000}
\expandafter\def\csname cnt@expl.sspro.p2.e6.reps\endcsname{1{,}000}
\expandafter\def\csname pct@expl.sspro.p2.e6.reps\endcsname{100000.0}
\expandafter\def\csname ppt@expl.sspro.p2.e6.reps\endcsname{$+$100000.0}
\expandafter\def\csname val@expl.sspro.p2.e8.C.direct-in-zoomed.n\endcsname{169}
\expandafter\def\csname cnt@expl.sspro.p2.e8.C.direct-in-zoomed.n\endcsname{169}
\expandafter\def\csname pct@expl.sspro.p2.e8.C.direct-in-zoomed.n\endcsname{16900.0}
\expandafter\def\csname ppt@expl.sspro.p2.e8.C.direct-in-zoomed.n\endcsname{$+$16900.0}
\expandafter\def\csname val@expl.sspro.p2.e8.C.direct-in-zoomed.resid\endcsname{-0.012}
\expandafter\def\csname cnt@expl.sspro.p2.e8.C.direct-in-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.C.direct-in-zoomed.resid\endcsname{$-$1.2}
\expandafter\def\csname ppt@expl.sspro.p2.e8.C.direct-in-zoomed.resid\endcsname{$-$1.2}
\expandafter\def\csname val@expl.sspro.p2.e8.C.direct-outside-zoomed.n\endcsname{21}
\expandafter\def\csname cnt@expl.sspro.p2.e8.C.direct-outside-zoomed.n\endcsname{21}
\expandafter\def\csname pct@expl.sspro.p2.e8.C.direct-outside-zoomed.n\endcsname{2100.0}
\expandafter\def\csname ppt@expl.sspro.p2.e8.C.direct-outside-zoomed.n\endcsname{$+$2100.0}
\expandafter\def\csname val@expl.sspro.p2.e8.C.direct-outside-zoomed.resid\endcsname{0.190}
\expandafter\def\csname cnt@expl.sspro.p2.e8.C.direct-outside-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.C.direct-outside-zoomed.resid\endcsname{19.0}
\expandafter\def\csname ppt@expl.sspro.p2.e8.C.direct-outside-zoomed.resid\endcsname{$+$19.0}
\expandafter\def\csname val@expl.sspro.p2.e8.C.eta2-agree-stable-vs-other\endcsname{0.034}
\expandafter\def\csname cnt@expl.sspro.p2.e8.C.eta2-agree-stable-vs-other\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.C.eta2-agree-stable-vs-other\endcsname{3.4}
\expandafter\def\csname ppt@expl.sspro.p2.e8.C.eta2-agree-stable-vs-other\endcsname{$+$3.4}
\expandafter\def\csname val@expl.sspro.p2.e8.C.eta2-direct-in-zoomed\endcsname{0.048}
\expandafter\def\csname cnt@expl.sspro.p2.e8.C.eta2-direct-in-zoomed\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.C.eta2-direct-in-zoomed\endcsname{4.8}
\expandafter\def\csname ppt@expl.sspro.p2.e8.C.eta2-direct-in-zoomed\endcsname{$+$4.8}
\expandafter\def\csname val@expl.sspro.p2.e8.T.direct-in-zoomed.n\endcsname{358}
\expandafter\def\csname cnt@expl.sspro.p2.e8.T.direct-in-zoomed.n\endcsname{358}
\expandafter\def\csname pct@expl.sspro.p2.e8.T.direct-in-zoomed.n\endcsname{35800.0}
\expandafter\def\csname ppt@expl.sspro.p2.e8.T.direct-in-zoomed.n\endcsname{$+$35800.0}
\expandafter\def\csname val@expl.sspro.p2.e8.T.direct-in-zoomed.resid\endcsname{0.014}
\expandafter\def\csname cnt@expl.sspro.p2.e8.T.direct-in-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.T.direct-in-zoomed.resid\endcsname{1.4}
\expandafter\def\csname ppt@expl.sspro.p2.e8.T.direct-in-zoomed.resid\endcsname{$+$1.4}
\expandafter\def\csname val@expl.sspro.p2.e8.T.direct-outside-zoomed.n\endcsname{17}
\expandafter\def\csname cnt@expl.sspro.p2.e8.T.direct-outside-zoomed.n\endcsname{17}
\expandafter\def\csname pct@expl.sspro.p2.e8.T.direct-outside-zoomed.n\endcsname{1700.0}
\expandafter\def\csname ppt@expl.sspro.p2.e8.T.direct-outside-zoomed.n\endcsname{$+$1700.0}
\expandafter\def\csname val@expl.sspro.p2.e8.T.direct-outside-zoomed.resid\endcsname{0.059}
\expandafter\def\csname cnt@expl.sspro.p2.e8.T.direct-outside-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.T.direct-outside-zoomed.resid\endcsname{5.9}
\expandafter\def\csname ppt@expl.sspro.p2.e8.T.direct-outside-zoomed.resid\endcsname{$+$5.9}
\expandafter\def\csname val@expl.sspro.p2.e8.T.eta2-agree-stable-vs-other\endcsname{0.007}
\expandafter\def\csname cnt@expl.sspro.p2.e8.T.eta2-agree-stable-vs-other\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.T.eta2-agree-stable-vs-other\endcsname{0.7}
\expandafter\def\csname ppt@expl.sspro.p2.e8.T.eta2-agree-stable-vs-other\endcsname{$+$0.7}
\expandafter\def\csname val@expl.sspro.p2.e8.T.eta2-direct-in-zoomed\endcsname{0.001}
\expandafter\def\csname cnt@expl.sspro.p2.e8.T.eta2-direct-in-zoomed\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e8.T.eta2-direct-in-zoomed\endcsname{0.1}
\expandafter\def\csname ppt@expl.sspro.p2.e8.T.eta2-direct-in-zoomed\endcsname{$+$0.1}
\expandafter\def\csname val@expl.sspro.p2.e9.mean\endcsname{-0.021}
\expandafter\def\csname cnt@expl.sspro.p2.e9.mean\endcsname{0}
\expandafter\def\csname pct@expl.sspro.p2.e9.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@expl.sspro.p2.e9.mean\endcsname{$-$2.1}
\expandafter\def\csname val@expl.sspro.p2.e9.n\endcsname{4}
\expandafter\def\csname cnt@expl.sspro.p2.e9.n\endcsname{4}
\expandafter\def\csname pct@expl.sspro.p2.e9.n\endcsname{400.0}
\expandafter\def\csname ppt@expl.sspro.p2.e9.n\endcsname{$+$400.0}
\expandafter\def\csname val@expl.sspro.p2.e9.n-negative\endcsname{3}
\expandafter\def\csname cnt@expl.sspro.p2.e9.n-negative\endcsname{3}
\expandafter\def\csname pct@expl.sspro.p2.e9.n-negative\endcsname{300.0}
\expandafter\def\csname ppt@expl.sspro.p2.e9.n-negative\endcsname{$+$300.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.1.agreement\endcsname{0.470}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.1.agreement\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.1.agreement\endcsname{47.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.1.agreement\endcsname{$+$47.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.1.rmse\endcsname{0.123}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.1.rmse\endcsname{12.3}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.1.rmse\endcsname{$+$12.3}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.25.agreement\endcsname{0.580}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.25.agreement\endcsname{58.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.25.agreement\endcsname{$+$58.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.25.rmse\endcsname{0.080}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.25.rmse\endcsname{8.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.25.rmse\endcsname{$+$8.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.5.agreement\endcsname{0.610}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.5.agreement\endcsname{61.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.5.agreement\endcsname{$+$61.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@0.5.rmse\endcsname{0.045}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@0.5.rmse\endcsname{4.5}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@0.5.rmse\endcsname{$+$4.5}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.old-source.agreement\endcsname{0.600}
\expandafter\def\csname cnt@expl.uiv.p1.e1.old-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.old-source.agreement\endcsname{60.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.old-source.agreement\endcsname{$+$60.0}
\expandafter\def\csname val@expl.uiv.p1.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.old-source.rmse\endcsname{0.077}
\expandafter\def\csname cnt@expl.uiv.p1.e1.old-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.old-source.rmse\endcsname{7.7}
\expandafter\def\csname ppt@expl.uiv.p1.e1.old-source.rmse\endcsname{$+$7.7}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.1.agreement\endcsname{0.650}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.1.agreement\endcsname{65.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.1.agreement\endcsname{$+$65.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.1.rmse\endcsname{0.067}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.1.rmse\endcsname{6.7}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.1.rmse\endcsname{$+$6.7}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.25.agreement\endcsname{0.720}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.25.agreement\endcsname{72.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.25.agreement\endcsname{$+$72.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.25.rmse\endcsname{0.048}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.25.rmse\endcsname{4.8}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.25.rmse\endcsname{$+$4.8}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.5.agreement\endcsname{0.790}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.5.agreement\endcsname{79.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.5.agreement\endcsname{$+$79.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@0.5.rmse\endcsname{0.026}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@0.5.rmse\endcsname{2.6}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@0.5.rmse\endcsname{$+$2.6}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.rcr-stratified@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.rcr-stratified@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-only.agreement\endcsname{0.600}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-only.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-only.agreement\endcsname{60.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-only.agreement\endcsname{$+$60.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-only.rmse\endcsname{0.073}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-only.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-only.rmse\endcsname{7.3}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-only.rmse\endcsname{$+$7.3}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{0.700}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{70.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.1.agreement\endcsname{$+$70.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{0.098}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{9.8}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.1.rmse\endcsname{$+$9.8}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{0.600}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{60.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.25.agreement\endcsname{$+$60.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{0.063}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{6.3}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.25.rmse\endcsname{$+$6.3}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{0.700}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{70.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.5.agreement\endcsname{$+$70.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{0.033}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{3.3}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@0.5.rmse\endcsname{$+$3.3}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.1.agreement\endcsname{0.560}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.1.agreement\endcsname{56.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.1.agreement\endcsname{$+$56.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.1.rmse\endcsname{0.103}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.1.rmse\endcsname{10.3}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.1.rmse\endcsname{$+$10.3}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.25.agreement\endcsname{0.640}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.25.agreement\endcsname{64.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.25.agreement\endcsname{$+$64.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.25.rmse\endcsname{0.057}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.25.rmse\endcsname{5.7}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.25.rmse\endcsname{$+$5.7}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.5.agreement\endcsname{0.680}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.5.agreement\endcsname{68.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.5.agreement\endcsname{$+$68.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@0.5.rmse\endcsname{0.038}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@0.5.rmse\endcsname{3.8}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@0.5.rmse\endcsname{$+$3.8}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e1.uniform-fresh@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p1.e1.uniform-fresh@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e10.C.ci95.0\endcsname{0.001}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.ci95.0\endcsname{0.1}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.ci95.0\endcsname{$+$0.1}
\expandafter\def\csname val@expl.uiv.p1.e10.C.ci95.1\endcsname{0.236}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.ci95.1\endcsname{23.6}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.ci95.1\endcsname{$+$23.6}
\expandafter\def\csname val@expl.uiv.p1.e10.C.delta-eta2\endcsname{0.070}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.delta-eta2\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.delta-eta2\endcsname{7.0}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.delta-eta2\endcsname{$+$7.0}
\expandafter\def\csname val@expl.uiv.p1.e10.C.n-flagged\endcsname{45}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.n-flagged\endcsname{45}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.n-flagged\endcsname{4500.0}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.n-flagged\endcsname{$+$4500.0}
\expandafter\def\csname val@expl.uiv.p1.e10.C.perm-null-mean\endcsname{0.018}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.perm-null-mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.perm-null-mean\endcsname{1.8}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.perm-null-mean\endcsname{$+$1.8}
\expandafter\def\csname val@expl.uiv.p1.e10.C.perm-p\endcsname{0.030}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.perm-p\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.perm-p\endcsname{3.0}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.perm-p\endcsname{$+$3.0}
\expandafter\def\csname val@expl.uiv.p1.e10.C.perm-p-rowwise\endcsname{0.003}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.perm-p-rowwise\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.perm-p-rowwise\endcsname{0.3}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.perm-p-rowwise\endcsname{$+$0.3}
\expandafter\def\csname val@expl.uiv.p1.e10.C.share-in-disagree\endcsname{0.756}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.share-in-disagree\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.share-in-disagree\endcsname{75.6}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.share-in-disagree\endcsname{$+$75.6}
\expandafter\def\csname val@expl.uiv.p1.e10.C.share-outside-agree-stable\endcsname{0.956}
\expandafter\def\csname cnt@expl.uiv.p1.e10.C.share-outside-agree-stable\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e10.C.share-outside-agree-stable\endcsname{95.6}
\expandafter\def\csname ppt@expl.uiv.p1.e10.C.share-outside-agree-stable\endcsname{$+$95.6}
\expandafter\def\csname val@expl.uiv.p1.e1eq.generic-ppi-source.agreement\endcsname{0.702}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.generic-ppi-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.generic-ppi-source.agreement\endcsname{70.2}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.generic-ppi-source.agreement\endcsname{$+$70.2}
\expandafter\def\csname val@expl.uiv.p1.e1eq.generic-ppi-source.rmse\endcsname{0.034}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.generic-ppi-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.generic-ppi-source.rmse\endcsname{3.4}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.generic-ppi-source.rmse\endcsname{$+$3.4}
\expandafter\def\csname val@expl.uiv.p1.e1eq.rcr-stratified.agreement\endcsname{0.720}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.rcr-stratified.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.rcr-stratified.agreement\endcsname{72.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.rcr-stratified.agreement\endcsname{$+$72.0}
\expandafter\def\csname val@expl.uiv.p1.e1eq.rcr-stratified.rmse\endcsname{0.048}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.rcr-stratified.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.rcr-stratified.rmse\endcsname{4.8}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.rcr-stratified.rmse\endcsname{$+$4.8}
\expandafter\def\csname val@expl.uiv.p1.e1eq.replay-ppi-uniform.agreement\endcsname{0.600}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.replay-ppi-uniform.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.replay-ppi-uniform.agreement\endcsname{60.0}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.replay-ppi-uniform.agreement\endcsname{$+$60.0}
\expandafter\def\csname val@expl.uiv.p1.e1eq.replay-ppi-uniform.rmse\endcsname{0.063}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.replay-ppi-uniform.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.replay-ppi-uniform.rmse\endcsname{6.3}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.replay-ppi-uniform.rmse\endcsname{$+$6.3}
\expandafter\def\csname val@expl.uiv.p1.e1eq.uniform-fresh.agreement\endcsname{0.756}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.uniform-fresh.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.uniform-fresh.agreement\endcsname{75.6}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.uniform-fresh.agreement\endcsname{$+$75.6}
\expandafter\def\csname val@expl.uiv.p1.e1eq.uniform-fresh.rmse\endcsname{0.029}
\expandafter\def\csname cnt@expl.uiv.p1.e1eq.uniform-fresh.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e1eq.uniform-fresh.rmse\endcsname{2.9}
\expandafter\def\csname ppt@expl.uiv.p1.e1eq.uniform-fresh.rmse\endcsname{$+$2.9}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{0.024}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{2.4}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.max\endcsname{$+$2.4}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{-0.003}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.3}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.3}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{2}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{2}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{$+$200.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{10}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{10}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{1000.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{$+$1000.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-only.max\endcsname{-0.013}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-only.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-only.max\endcsname{$-$1.3}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-only.max\endcsname{$-$1.3}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-only.min\endcsname{-0.044}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-only.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-only.min\endcsname{$-$4.4}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-only.min\endcsname{$-$4.4}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-only.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-only.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-only.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-only.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-only.n-negative\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-only.n-negative\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-only.n-negative\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-only.n-negative\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-only.n-positive\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.024}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{2.4}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.max\endcsname{$+$2.4}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{-0.007}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.7}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.7}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{4}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{4}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{400.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{$+$400.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{8}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{8}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{800.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{$+$800.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-uniform-fresh.max\endcsname{0.033}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-uniform-fresh.max\endcsname{3.3}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.max\endcsname{$+$3.3}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-uniform-fresh.min\endcsname{0.004}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-uniform-fresh.min\endcsname{0.4}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.min\endcsname{$+$0.4}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-negative\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e2.rcr-minus-uniform-fresh.n-positive\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p1.e3.C.ci95.0\endcsname{0.101}
\expandafter\def\csname cnt@expl.uiv.p1.e3.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e3.C.ci95.0\endcsname{10.1}
\expandafter\def\csname ppt@expl.uiv.p1.e3.C.ci95.0\endcsname{$+$10.1}
\expandafter\def\csname val@expl.uiv.p1.e3.C.ci95.1\endcsname{0.449}
\expandafter\def\csname cnt@expl.uiv.p1.e3.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e3.C.ci95.1\endcsname{44.9}
\expandafter\def\csname ppt@expl.uiv.p1.e3.C.ci95.1\endcsname{$+$44.9}
\expandafter\def\csname val@expl.uiv.p1.e3.C.gap\endcsname{0.253}
\expandafter\def\csname cnt@expl.uiv.p1.e3.C.gap\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e3.C.gap\endcsname{25.3}
\expandafter\def\csname ppt@expl.uiv.p1.e3.C.gap\endcsname{$+$25.3}
\expandafter\def\csname val@expl.uiv.p1.e5.C.covered.N\endcsname{297}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.covered.N\endcsname{297}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.covered.N\endcsname{29700.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.covered.N\endcsname{$+$29700.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.covered.acc-F\endcsname{0.835}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.covered.acc-F\endcsname{83.5}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.covered.acc-F\endcsname{$+$83.5}
\expandafter\def\csname val@expl.uiv.p1.e5.C.covered.acc-R\endcsname{0.832}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.covered.acc-R\endcsname{83.2}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.covered.acc-R\endcsname{$+$83.2}
\expandafter\def\csname val@expl.uiv.p1.e5.C.covered.resid-F-minus-R\endcsname{0.003}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.covered.resid-F-minus-R\endcsname{0.3}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.covered.resid-F-minus-R\endcsname{$+$0.3}
\expandafter\def\csname val@expl.uiv.p1.e5.C.covered.share\endcsname{0.816}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.covered.share\endcsname{81.6}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.covered.share\endcsname{$+$81.6}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.N\endcsname{67}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.N\endcsname{67}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.N\endcsname{6700.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.N\endcsname{$+$6700.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.acc-F\endcsname{0.448}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.acc-F\endcsname{44.8}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.acc-F\endcsname{$+$44.8}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.acc-R\endcsname{0.075}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.acc-R\endcsname{7.5}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.acc-R\endcsname{$+$7.5}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.resid-F-minus-R\endcsname{0.373}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.resid-F-minus-R\endcsname{37.3}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.resid-F-minus-R\endcsname{$+$37.3}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.share\endcsname{0.184}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.share\endcsname{18.4}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.share\endcsname{$+$18.4}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.share-of-net-residual\endcsname{0.962}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.share-of-net-residual\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.share-of-net-residual\endcsname{96.2}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.share-of-net-residual\endcsname{$+$96.2}
\expandafter\def\csname val@expl.uiv.p1.e5.C.missed.share-of-replay-errors\endcsname{0.554}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.missed.share-of-replay-errors\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.missed.share-of-replay-errors\endcsname{55.4}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.missed.share-of-replay-errors\endcsname{$+$55.4}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.covered.N\endcsname{155}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.covered.N\endcsname{155}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.covered.N\endcsname{15500.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.covered.N\endcsname{$+$15500.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.covered.acc-F\endcsname{0.832}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.covered.acc-F\endcsname{83.2}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.covered.acc-F\endcsname{$+$83.2}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.covered.acc-R\endcsname{0.839}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.covered.acc-R\endcsname{83.9}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.covered.acc-R\endcsname{$+$83.9}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{-0.006}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$0.6}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$0.6}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.covered.share\endcsname{0.829}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.covered.share\endcsname{82.9}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.covered.share\endcsname{$+$82.9}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.missed.N\endcsname{32}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.missed.N\endcsname{32}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.missed.N\endcsname{3200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.missed.N\endcsname{$+$3200.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.missed.acc-F\endcsname{0.438}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.missed.acc-F\endcsname{43.8}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.missed.acc-F\endcsname{$+$43.8}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.missed.acc-R\endcsname{0.156}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.missed.acc-R\endcsname{15.6}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.missed.acc-R\endcsname{$+$15.6}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0.281}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{28.1}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.missed.resid-F-minus-R\endcsname{$+$28.1}
\expandafter\def\csname val@expl.uiv.p1.e5.C.multi-view.missed.share\endcsname{0.171}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.multi-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.multi-view.missed.share\endcsname{17.1}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.multi-view.missed.share\endcsname{$+$17.1}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.covered.N\endcsname{142}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.covered.N\endcsname{142}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.covered.N\endcsname{14200.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.covered.N\endcsname{$+$14200.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.covered.acc-F\endcsname{0.838}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.covered.acc-F\endcsname{83.8}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.covered.acc-F\endcsname{$+$83.8}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.covered.acc-R\endcsname{0.824}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.covered.acc-R\endcsname{82.4}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.covered.acc-R\endcsname{$+$82.4}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{0.014}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{1.4}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.covered.resid-F-minus-R\endcsname{$+$1.4}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.covered.share\endcsname{0.802}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.covered.share\endcsname{80.2}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.covered.share\endcsname{$+$80.2}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.missed.N\endcsname{35}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.missed.N\endcsname{35}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.missed.N\endcsname{3500.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.missed.N\endcsname{$+$3500.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.missed.acc-F\endcsname{0.457}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.missed.acc-F\endcsname{45.7}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.missed.acc-F\endcsname{$+$45.7}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{0.457}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{45.7}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.missed.resid-F-minus-R\endcsname{$+$45.7}
\expandafter\def\csname val@expl.uiv.p1.e5.C.single-view.missed.share\endcsname{0.198}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.single-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.single-view.missed.share\endcsname{19.8}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.single-view.missed.share\endcsname{$+$19.8}
\expandafter\def\csname val@expl.uiv.p1.e5.C.strata.agree-drift.missed-share\endcsname{0.409}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.strata.agree-drift.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.strata.agree-drift.missed-share\endcsname{40.9}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.strata.agree-drift.missed-share\endcsname{$+$40.9}
\expandafter\def\csname val@expl.uiv.p1.e5.C.strata.agree-stable.missed-share\endcsname{0.081}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.strata.agree-stable.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.strata.agree-stable.missed-share\endcsname{8.1}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.strata.agree-stable.missed-share\endcsname{$+$8.1}
\expandafter\def\csname val@expl.uiv.p1.e5.C.strata.disagree.missed-share\endcsname{0.493}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.strata.disagree.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.strata.disagree.missed-share\endcsname{49.3}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.strata.disagree.missed-share\endcsname{$+$49.3}
\expandafter\def\csname val@expl.uiv.p1.e5.C.strata.parse-fail.missed-share\endcsname{0.750}
\expandafter\def\csname cnt@expl.uiv.p1.e5.C.strata.parse-fail.missed-share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e5.C.strata.parse-fail.missed-share\endcsname{75.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.C.strata.parse-fail.missed-share\endcsname{$+$75.0}
\expandafter\def\csname val@expl.uiv.p1.e5.T.covered.N\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e5.T.covered.N\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.T.covered.N\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.T.covered.N\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e5.T.missed.N\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p1.e5.T.missed.N\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e5.T.missed.N\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p1.e5.T.missed.N\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p1.e6.histories\endcsname{20}
\expandafter\def\csname cnt@expl.uiv.p1.e6.histories\endcsname{20}
\expandafter\def\csname pct@expl.uiv.p1.e6.histories\endcsname{2000.0}
\expandafter\def\csname ppt@expl.uiv.p1.e6.histories\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{-0.018}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$1.8}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$1.8}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0.020}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{2.0}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{$+$2.0}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{0.001}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{0.1}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.mean\endcsname{$+$0.1}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0.442}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{44.2}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{$+$44.2}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{-0.062}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$6.2}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{0.009}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{0.9}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-only.ci95.1\endcsname{$+$0.9}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-only.mean\endcsname{-0.023}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-only.mean\endcsname{$-$2.3}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-only.mean\endcsname{$-$2.3}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-only.p-le0\endcsname{0.944}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-only.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-only.p-le0\endcsname{94.4}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-only.p-le0\endcsname{$+$94.4}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{-0.014}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$1.4}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$1.4}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0.017}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{1.7}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{$+$1.7}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.001}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.1}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{$+$0.1}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0.446}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{44.6}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{$+$44.6}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{-0.005}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$0.5}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$0.5}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0.030}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{3.0}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{$+$3.0}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{0.010}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{1.0}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.mean\endcsname{$+$1.0}
\expandafter\def\csname val@expl.uiv.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{0.105}
\expandafter\def\csname cnt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{10.5}
\expandafter\def\csname ppt@expl.uiv.p1.e6.rcr-minus-uniform-fresh.p-le0\endcsname{$+$10.5}
\expandafter\def\csname val@expl.uiv.p1.e6.reps\endcsname{1000}
\expandafter\def\csname cnt@expl.uiv.p1.e6.reps\endcsname{1{,}000}
\expandafter\def\csname pct@expl.uiv.p1.e6.reps\endcsname{100000.0}
\expandafter\def\csname ppt@expl.uiv.p1.e6.reps\endcsname{$+$100000.0}
\expandafter\def\csname val@expl.uiv.p1.e8.C.direct-in-zoomed.n\endcsname{319}
\expandafter\def\csname cnt@expl.uiv.p1.e8.C.direct-in-zoomed.n\endcsname{319}
\expandafter\def\csname pct@expl.uiv.p1.e8.C.direct-in-zoomed.n\endcsname{31900.0}
\expandafter\def\csname ppt@expl.uiv.p1.e8.C.direct-in-zoomed.n\endcsname{$+$31900.0}
\expandafter\def\csname val@expl.uiv.p1.e8.C.direct-in-zoomed.resid\endcsname{0.019}
\expandafter\def\csname cnt@expl.uiv.p1.e8.C.direct-in-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e8.C.direct-in-zoomed.resid\endcsname{1.9}
\expandafter\def\csname ppt@expl.uiv.p1.e8.C.direct-in-zoomed.resid\endcsname{$+$1.9}
\expandafter\def\csname val@expl.uiv.p1.e8.C.direct-outside-zoomed.n\endcsname{45}
\expandafter\def\csname cnt@expl.uiv.p1.e8.C.direct-outside-zoomed.n\endcsname{45}
\expandafter\def\csname pct@expl.uiv.p1.e8.C.direct-outside-zoomed.n\endcsname{4500.0}
\expandafter\def\csname ppt@expl.uiv.p1.e8.C.direct-outside-zoomed.n\endcsname{$+$4500.0}
\expandafter\def\csname val@expl.uiv.p1.e8.C.direct-outside-zoomed.resid\endcsname{0.444}
\expandafter\def\csname cnt@expl.uiv.p1.e8.C.direct-outside-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e8.C.direct-outside-zoomed.resid\endcsname{44.4}
\expandafter\def\csname ppt@expl.uiv.p1.e8.C.direct-outside-zoomed.resid\endcsname{$+$44.4}
\expandafter\def\csname val@expl.uiv.p1.e8.C.eta2-agree-stable-vs-other\endcsname{0.074}
\expandafter\def\csname cnt@expl.uiv.p1.e8.C.eta2-agree-stable-vs-other\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e8.C.eta2-agree-stable-vs-other\endcsname{7.4}
\expandafter\def\csname ppt@expl.uiv.p1.e8.C.eta2-agree-stable-vs-other\endcsname{$+$7.4}
\expandafter\def\csname val@expl.uiv.p1.e8.C.eta2-direct-in-zoomed\endcsname{0.178}
\expandafter\def\csname cnt@expl.uiv.p1.e8.C.eta2-direct-in-zoomed\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e8.C.eta2-direct-in-zoomed\endcsname{17.8}
\expandafter\def\csname ppt@expl.uiv.p1.e8.C.eta2-direct-in-zoomed\endcsname{$+$17.8}
\expandafter\def\csname val@expl.uiv.p1.e9.mean\endcsname{-0.065}
\expandafter\def\csname cnt@expl.uiv.p1.e9.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p1.e9.mean\endcsname{$-$6.5}
\expandafter\def\csname ppt@expl.uiv.p1.e9.mean\endcsname{$-$6.5}
\expandafter\def\csname val@expl.uiv.p1.e9.n\endcsname{4}
\expandafter\def\csname cnt@expl.uiv.p1.e9.n\endcsname{4}
\expandafter\def\csname pct@expl.uiv.p1.e9.n\endcsname{400.0}
\expandafter\def\csname ppt@expl.uiv.p1.e9.n\endcsname{$+$400.0}
\expandafter\def\csname val@expl.uiv.p1.e9.n-negative\endcsname{3}
\expandafter\def\csname cnt@expl.uiv.p1.e9.n-negative\endcsname{3}
\expandafter\def\csname pct@expl.uiv.p1.e9.n-negative\endcsname{300.0}
\expandafter\def\csname ppt@expl.uiv.p1.e9.n-negative\endcsname{$+$300.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.1.agreement\endcsname{0.550}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.1.agreement\endcsname{55.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.1.agreement\endcsname{$+$55.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.1.rmse\endcsname{0.111}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.1.rmse\endcsname{11.1}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.1.rmse\endcsname{$+$11.1}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.25.agreement\endcsname{0.510}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.25.agreement\endcsname{51.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.25.agreement\endcsname{$+$51.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.25.rmse\endcsname{0.065}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.25.rmse\endcsname{6.5}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.25.rmse\endcsname{$+$6.5}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.5.agreement\endcsname{0.710}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.5.agreement\endcsname{71.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.5.agreement\endcsname{$+$71.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@0.5.rmse\endcsname{0.032}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@0.5.rmse\endcsname{3.2}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@0.5.rmse\endcsname{$+$3.2}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.generic-ppi-source@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.old-source.agreement\endcsname{0.200}
\expandafter\def\csname cnt@expl.uiv.p2.e1.old-source.agreement\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.old-source.agreement\endcsname{20.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.old-source.agreement\endcsname{$+$20.0}
\expandafter\def\csname val@expl.uiv.p2.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.old-source.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.old-source.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.old-source.rmse\endcsname{0.028}
\expandafter\def\csname cnt@expl.uiv.p2.e1.old-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.old-source.rmse\endcsname{2.8}
\expandafter\def\csname ppt@expl.uiv.p2.e1.old-source.rmse\endcsname{$+$2.8}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.1.agreement\endcsname{0.480}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.1.agreement\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.1.agreement\endcsname{48.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.1.agreement\endcsname{$+$48.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.1.rmse\endcsname{0.097}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.1.rmse\endcsname{9.7}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.1.rmse\endcsname{$+$9.7}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.25.agreement\endcsname{0.530}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.25.agreement\endcsname{53.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.25.agreement\endcsname{$+$53.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.25.rmse\endcsname{0.046}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.25.rmse\endcsname{4.6}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.25.rmse\endcsname{$+$4.6}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.5.agreement\endcsname{0.550}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.5.agreement\endcsname{55.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.5.agreement\endcsname{$+$55.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@0.5.rmse\endcsname{0.028}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@0.5.rmse\endcsname{2.8}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@0.5.rmse\endcsname{$+$2.8}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.rcr-stratified@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.rcr-stratified@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.rcr-stratified@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-only.agreement\endcsname{0.600}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-only.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-only.agreement\endcsname{60.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-only.agreement\endcsname{$+$60.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-only.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-only.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-only.rmse\endcsname{0.038}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-only.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-only.rmse\endcsname{3.8}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-only.rmse\endcsname{$+$3.8}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{0.580}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{58.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.1.agreement\endcsname{$+$58.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{0.108}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{10.8}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.1.rmse\endcsname{$+$10.8}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{0.530}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{53.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.25.agreement\endcsname{$+$53.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{0.062}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{6.2}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.25.rmse\endcsname{$+$6.2}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{0.650}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{65.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.5.agreement\endcsname{$+$65.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{0.030}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{3.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@0.5.rmse\endcsname{$+$3.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.replay-ppi-uniform@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.1.agreement\endcsname{0.680}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.1.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.1.agreement\endcsname{68.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.1.agreement\endcsname{$+$68.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.1.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.1.rmse\endcsname{0.096}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.1.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.1.rmse\endcsname{9.6}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.1.rmse\endcsname{$+$9.6}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.25.agreement\endcsname{0.620}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.25.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.25.agreement\endcsname{62.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.25.agreement\endcsname{$+$62.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.25.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.25.rmse\endcsname{0.057}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.25.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.25.rmse\endcsname{5.7}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.25.rmse\endcsname{$+$5.7}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.5.agreement\endcsname{0.760}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.5.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.5.agreement\endcsname{76.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.5.agreement\endcsname{$+$76.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.5.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@0.5.rmse\endcsname{0.028}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@0.5.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@0.5.rmse\endcsname{2.8}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@0.5.rmse\endcsname{$+$2.8}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@1.0.agreement\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@1.0.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@1.0.agreement\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@1.0.agreement\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@1.0.n-infeasible\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e1.uniform-fresh@1.0.rmse\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e1.uniform-fresh@1.0.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1.uniform-fresh@1.0.rmse\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e10.C.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e10.C.ci95.1\endcsname{0.203}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.ci95.1\endcsname{20.3}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.ci95.1\endcsname{$+$20.3}
\expandafter\def\csname val@expl.uiv.p2.e10.C.delta-eta2\endcsname{0.020}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.delta-eta2\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.delta-eta2\endcsname{2.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.delta-eta2\endcsname{$+$2.0}
\expandafter\def\csname val@expl.uiv.p2.e10.C.n-flagged\endcsname{20}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.n-flagged\endcsname{20}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.n-flagged\endcsname{2000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.n-flagged\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.uiv.p2.e10.C.perm-null-mean\endcsname{0.029}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.perm-null-mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.perm-null-mean\endcsname{2.9}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.perm-null-mean\endcsname{$+$2.9}
\expandafter\def\csname val@expl.uiv.p2.e10.C.perm-p\endcsname{0.827}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.perm-p\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.perm-p\endcsname{82.7}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.perm-p\endcsname{$+$82.7}
\expandafter\def\csname val@expl.uiv.p2.e10.C.perm-p-rowwise\endcsname{0.223}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.perm-p-rowwise\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.perm-p-rowwise\endcsname{22.3}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.perm-p-rowwise\endcsname{$+$22.3}
\expandafter\def\csname val@expl.uiv.p2.e10.C.share-in-disagree\endcsname{0.850}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.share-in-disagree\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.share-in-disagree\endcsname{85.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.share-in-disagree\endcsname{$+$85.0}
\expandafter\def\csname val@expl.uiv.p2.e10.C.share-outside-agree-stable\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p2.e10.C.share-outside-agree-stable\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e10.C.share-outside-agree-stable\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.C.share-outside-agree-stable\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e10.T.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.ci95.0\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e10.T.ci95.1\endcsname{0.108}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.ci95.1\endcsname{10.8}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.ci95.1\endcsname{$+$10.8}
\expandafter\def\csname val@expl.uiv.p2.e10.T.delta-eta2\endcsname{0.020}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.delta-eta2\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.delta-eta2\endcsname{2.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.delta-eta2\endcsname{$+$2.0}
\expandafter\def\csname val@expl.uiv.p2.e10.T.n-flagged\endcsname{19}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.n-flagged\endcsname{19}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.n-flagged\endcsname{1900.0}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.n-flagged\endcsname{$+$1900.0}
\expandafter\def\csname val@expl.uiv.p2.e10.T.perm-null-mean\endcsname{0.007}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.perm-null-mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.perm-null-mean\endcsname{0.7}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.perm-null-mean\endcsname{$+$0.7}
\expandafter\def\csname val@expl.uiv.p2.e10.T.perm-p\endcsname{0.168}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.perm-p\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.perm-p\endcsname{16.8}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.perm-p\endcsname{$+$16.8}
\expandafter\def\csname val@expl.uiv.p2.e10.T.perm-p-rowwise\endcsname{0.196}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.perm-p-rowwise\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.perm-p-rowwise\endcsname{19.6}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.perm-p-rowwise\endcsname{$+$19.6}
\expandafter\def\csname val@expl.uiv.p2.e10.T.share-in-disagree\endcsname{0.789}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.share-in-disagree\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.share-in-disagree\endcsname{78.9}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.share-in-disagree\endcsname{$+$78.9}
\expandafter\def\csname val@expl.uiv.p2.e10.T.share-outside-agree-stable\endcsname{0.947}
\expandafter\def\csname cnt@expl.uiv.p2.e10.T.share-outside-agree-stable\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e10.T.share-outside-agree-stable\endcsname{94.7}
\expandafter\def\csname ppt@expl.uiv.p2.e10.T.share-outside-agree-stable\endcsname{$+$94.7}
\expandafter\def\csname val@expl.uiv.p2.e1eq.generic-ppi-source.agreement\endcsname{0.785}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.generic-ppi-source.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.generic-ppi-source.agreement\endcsname{78.5}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.generic-ppi-source.agreement\endcsname{$+$78.5}
\expandafter\def\csname val@expl.uiv.p2.e1eq.generic-ppi-source.rmse\endcsname{0.024}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.generic-ppi-source.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.generic-ppi-source.rmse\endcsname{2.4}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.generic-ppi-source.rmse\endcsname{$+$2.4}
\expandafter\def\csname val@expl.uiv.p2.e1eq.rcr-stratified.agreement\endcsname{0.530}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.rcr-stratified.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.rcr-stratified.agreement\endcsname{53.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.rcr-stratified.agreement\endcsname{$+$53.0}
\expandafter\def\csname val@expl.uiv.p2.e1eq.rcr-stratified.rmse\endcsname{0.046}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.rcr-stratified.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.rcr-stratified.rmse\endcsname{4.6}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.rcr-stratified.rmse\endcsname{$+$4.6}
\expandafter\def\csname val@expl.uiv.p2.e1eq.replay-ppi-uniform.agreement\endcsname{0.530}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.replay-ppi-uniform.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.replay-ppi-uniform.agreement\endcsname{53.0}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.replay-ppi-uniform.agreement\endcsname{$+$53.0}
\expandafter\def\csname val@expl.uiv.p2.e1eq.replay-ppi-uniform.rmse\endcsname{0.062}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.replay-ppi-uniform.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.replay-ppi-uniform.rmse\endcsname{6.2}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.replay-ppi-uniform.rmse\endcsname{$+$6.2}
\expandafter\def\csname val@expl.uiv.p2.e1eq.uniform-fresh.agreement\endcsname{0.822}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.uniform-fresh.agreement\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.uniform-fresh.agreement\endcsname{82.2}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.uniform-fresh.agreement\endcsname{$+$82.2}
\expandafter\def\csname val@expl.uiv.p2.e1eq.uniform-fresh.rmse\endcsname{0.021}
\expandafter\def\csname cnt@expl.uiv.p2.e1eq.uniform-fresh.rmse\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e1eq.uniform-fresh.rmse\endcsname{2.1}
\expandafter\def\csname ppt@expl.uiv.p2.e1eq.uniform-fresh.rmse\endcsname{$+$2.1}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{0.006}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{0.6}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.max\endcsname{$+$0.6}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{-0.004}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.4}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.min\endcsname{$-$0.4}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{7}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{7}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{700.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-negative\endcsname{$+$700.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{5}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{5}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{500.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-generic-ppi-source.n-positive\endcsname{$+$500.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-only.max\endcsname{0.006}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-only.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-only.max\endcsname{0.6}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-only.max\endcsname{$+$0.6}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-only.min\endcsname{-0.010}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-only.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-only.min\endcsname{$-$1.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-only.min\endcsname{$-$1.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-only.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-only.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-only.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-only.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-only.n-negative\endcsname{10}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-only.n-negative\endcsname{10}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-only.n-negative\endcsname{1000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-only.n-negative\endcsname{$+$1000.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-only.n-positive\endcsname{2}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-only.n-positive\endcsname{2}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-only.n-positive\endcsname{200.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-only.n-positive\endcsname{$+$200.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.004}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{0.4}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.max\endcsname{$+$0.4}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{-0.005}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.5}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.min\endcsname{$-$0.5}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{3}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{3}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{300.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-negative\endcsname{$+$300.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{9}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{9}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{900.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-replay-ppi-uniform.n-positive\endcsname{$+$900.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-uniform-fresh.max\endcsname{0.010}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.max\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-uniform-fresh.max\endcsname{1.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.max\endcsname{$+$1.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-uniform-fresh.min\endcsname{-0.001}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.min\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-uniform-fresh.min\endcsname{$-$0.1}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.min\endcsname{$-$0.1}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n\endcsname{12}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n\endcsname{12}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n\endcsname{1200.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n\endcsname{$+$1200.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{1}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-negative\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{11}
\expandafter\def\csname cnt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{11}
\expandafter\def\csname pct@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{1100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e2.rcr-minus-uniform-fresh.n-positive\endcsname{$+$1100.0}
\expandafter\def\csname val@expl.uiv.p2.e3.C.ci95.0\endcsname{-0.156}
\expandafter\def\csname cnt@expl.uiv.p2.e3.C.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e3.C.ci95.0\endcsname{$-$15.6}
\expandafter\def\csname ppt@expl.uiv.p2.e3.C.ci95.0\endcsname{$-$15.6}
\expandafter\def\csname val@expl.uiv.p2.e3.C.ci95.1\endcsname{0.259}
\expandafter\def\csname cnt@expl.uiv.p2.e3.C.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e3.C.ci95.1\endcsname{25.9}
\expandafter\def\csname ppt@expl.uiv.p2.e3.C.ci95.1\endcsname{$+$25.9}
\expandafter\def\csname val@expl.uiv.p2.e3.C.gap\endcsname{0.020}
\expandafter\def\csname cnt@expl.uiv.p2.e3.C.gap\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e3.C.gap\endcsname{2.0}
\expandafter\def\csname ppt@expl.uiv.p2.e3.C.gap\endcsname{$+$2.0}
\expandafter\def\csname val@expl.uiv.p2.e3.T.ci95.0\endcsname{0.042}
\expandafter\def\csname cnt@expl.uiv.p2.e3.T.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e3.T.ci95.0\endcsname{4.2}
\expandafter\def\csname ppt@expl.uiv.p2.e3.T.ci95.0\endcsname{$+$4.2}
\expandafter\def\csname val@expl.uiv.p2.e3.T.ci95.1\endcsname{0.415}
\expandafter\def\csname cnt@expl.uiv.p2.e3.T.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e3.T.ci95.1\endcsname{41.5}
\expandafter\def\csname ppt@expl.uiv.p2.e3.T.ci95.1\endcsname{$+$41.5}
\expandafter\def\csname val@expl.uiv.p2.e3.T.gap\endcsname{0.199}
\expandafter\def\csname cnt@expl.uiv.p2.e3.T.gap\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e3.T.gap\endcsname{19.9}
\expandafter\def\csname ppt@expl.uiv.p2.e3.T.gap\endcsname{$+$19.9}
\expandafter\def\csname val@expl.uiv.p2.e4.center-d1.diff.ci95.0\endcsname{-0.050}
\expandafter\def\csname cnt@expl.uiv.p2.e4.center-d1.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.center-d1.diff.ci95.0\endcsname{$-$5.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.center-d1.diff.ci95.0\endcsname{$-$5.0}
\expandafter\def\csname val@expl.uiv.p2.e4.center-d1.diff.ci95.1\endcsname{0.033}
\expandafter\def\csname cnt@expl.uiv.p2.e4.center-d1.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.center-d1.diff.ci95.1\endcsname{3.3}
\expandafter\def\csname ppt@expl.uiv.p2.e4.center-d1.diff.ci95.1\endcsname{$+$3.3}
\expandafter\def\csname val@expl.uiv.p2.e4.center-d1.diff.mean\endcsname{-0.008}
\expandafter\def\csname cnt@expl.uiv.p2.e4.center-d1.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.center-d1.diff.mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@expl.uiv.p2.e4.center-d1.diff.mean\endcsname{$-$0.8}
\expandafter\def\csname val@expl.uiv.p2.e4.center-d1.n\endcsname{120}
\expandafter\def\csname cnt@expl.uiv.p2.e4.center-d1.n\endcsname{120}
\expandafter\def\csname pct@expl.uiv.p2.e4.center-d1.n\endcsname{12000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.center-d1.n\endcsname{$+$12000.0}
\expandafter\def\csname val@expl.uiv.p2.e4.context-d1.diff.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@expl.uiv.p2.e4.context-d1.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.context-d1.diff.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@expl.uiv.p2.e4.context-d1.diff.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@expl.uiv.p2.e4.context-d1.diff.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@expl.uiv.p2.e4.context-d1.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.context-d1.diff.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@expl.uiv.p2.e4.context-d1.diff.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@expl.uiv.p2.e4.context-d1.diff.mean\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e4.context-d1.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.context-d1.diff.mean\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.context-d1.diff.mean\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e4.context-d1.n\endcsname{120}
\expandafter\def\csname cnt@expl.uiv.p2.e4.context-d1.n\endcsname{120}
\expandafter\def\csname pct@expl.uiv.p2.e4.context-d1.n\endcsname{12000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.context-d1.n\endcsname{$+$12000.0}
\expandafter\def\csname val@expl.uiv.p2.e4.dual-d2.diff.ci95.0\endcsname{0.008}
\expandafter\def\csname cnt@expl.uiv.p2.e4.dual-d2.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.dual-d2.diff.ci95.0\endcsname{0.8}
\expandafter\def\csname ppt@expl.uiv.p2.e4.dual-d2.diff.ci95.0\endcsname{$+$0.8}
\expandafter\def\csname val@expl.uiv.p2.e4.dual-d2.diff.ci95.1\endcsname{0.117}
\expandafter\def\csname cnt@expl.uiv.p2.e4.dual-d2.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.dual-d2.diff.ci95.1\endcsname{11.7}
\expandafter\def\csname ppt@expl.uiv.p2.e4.dual-d2.diff.ci95.1\endcsname{$+$11.7}
\expandafter\def\csname val@expl.uiv.p2.e4.dual-d2.diff.mean\endcsname{0.058}
\expandafter\def\csname cnt@expl.uiv.p2.e4.dual-d2.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.dual-d2.diff.mean\endcsname{5.8}
\expandafter\def\csname ppt@expl.uiv.p2.e4.dual-d2.diff.mean\endcsname{$+$5.8}
\expandafter\def\csname val@expl.uiv.p2.e4.dual-d2.n\endcsname{120}
\expandafter\def\csname cnt@expl.uiv.p2.e4.dual-d2.n\endcsname{120}
\expandafter\def\csname pct@expl.uiv.p2.e4.dual-d2.n\endcsname{12000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.dual-d2.n\endcsname{$+$12000.0}
\expandafter\def\csname val@expl.uiv.p2.e4.grid2-d3.diff.ci95.0\endcsname{-0.017}
\expandafter\def\csname cnt@expl.uiv.p2.e4.grid2-d3.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.grid2-d3.diff.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname ppt@expl.uiv.p2.e4.grid2-d3.diff.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname val@expl.uiv.p2.e4.grid2-d3.diff.ci95.1\endcsname{0.100}
\expandafter\def\csname cnt@expl.uiv.p2.e4.grid2-d3.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.grid2-d3.diff.ci95.1\endcsname{10.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.grid2-d3.diff.ci95.1\endcsname{$+$10.0}
\expandafter\def\csname val@expl.uiv.p2.e4.grid2-d3.diff.mean\endcsname{0.042}
\expandafter\def\csname cnt@expl.uiv.p2.e4.grid2-d3.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.grid2-d3.diff.mean\endcsname{4.2}
\expandafter\def\csname ppt@expl.uiv.p2.e4.grid2-d3.diff.mean\endcsname{$+$4.2}
\expandafter\def\csname val@expl.uiv.p2.e4.grid2-d3.n\endcsname{120}
\expandafter\def\csname cnt@expl.uiv.p2.e4.grid2-d3.n\endcsname{120}
\expandafter\def\csname pct@expl.uiv.p2.e4.grid2-d3.n\endcsname{12000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.grid2-d3.n\endcsname{$+$12000.0}
\expandafter\def\csname val@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{-0.058}
\expandafter\def\csname cnt@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{$-$5.8}
\expandafter\def\csname ppt@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.0\endcsname{$-$5.8}
\expandafter\def\csname val@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{0.042}
\expandafter\def\csname cnt@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{4.2}
\expandafter\def\csname ppt@expl.uiv.p2.e4.zoomclick-d3.diff.ci95.1\endcsname{$+$4.2}
\expandafter\def\csname val@expl.uiv.p2.e4.zoomclick-d3.diff.mean\endcsname{-0.008}
\expandafter\def\csname cnt@expl.uiv.p2.e4.zoomclick-d3.diff.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e4.zoomclick-d3.diff.mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@expl.uiv.p2.e4.zoomclick-d3.diff.mean\endcsname{$-$0.8}
\expandafter\def\csname val@expl.uiv.p2.e4.zoomclick-d3.n\endcsname{120}
\expandafter\def\csname cnt@expl.uiv.p2.e4.zoomclick-d3.n\endcsname{120}
\expandafter\def\csname pct@expl.uiv.p2.e4.zoomclick-d3.n\endcsname{12000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e4.zoomclick-d3.n\endcsname{$+$12000.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.covered.N\endcsname{345}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.covered.N\endcsname{345}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.covered.N\endcsname{34500.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.covered.N\endcsname{$+$34500.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.covered.acc-F\endcsname{0.846}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.covered.acc-F\endcsname{84.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.covered.acc-F\endcsname{$+$84.6}
\expandafter\def\csname val@expl.uiv.p2.e5.C.covered.acc-R\endcsname{0.855}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.covered.acc-R\endcsname{85.5}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.covered.acc-R\endcsname{$+$85.5}
\expandafter\def\csname val@expl.uiv.p2.e5.C.covered.resid-F-minus-R\endcsname{-0.009}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.covered.resid-F-minus-R\endcsname{$-$0.9}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.covered.resid-F-minus-R\endcsname{$-$0.9}
\expandafter\def\csname val@expl.uiv.p2.e5.C.covered.share\endcsname{0.908}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.covered.share\endcsname{90.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.covered.share\endcsname{$+$90.8}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.N\endcsname{35}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.N\endcsname{35}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.N\endcsname{3500.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.N\endcsname{$+$3500.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.acc-F\endcsname{0.314}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.acc-F\endcsname{31.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.acc-F\endcsname{$+$31.4}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.acc-R\endcsname{0.086}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.acc-R\endcsname{8.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.acc-R\endcsname{$+$8.6}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.resid-F-minus-R\endcsname{0.229}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.resid-F-minus-R\endcsname{22.9}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.resid-F-minus-R\endcsname{$+$22.9}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.share\endcsname{0.092}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.share\endcsname{9.2}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.share\endcsname{$+$9.2}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.share-of-net-residual\endcsname{1.600}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.share-of-net-residual\endcsname{2}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.share-of-net-residual\endcsname{160.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.share-of-net-residual\endcsname{$+$160.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.missed.share-of-replay-errors\endcsname{0.390}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.missed.share-of-replay-errors\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.missed.share-of-replay-errors\endcsname{39.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.missed.share-of-replay-errors\endcsname{$+$39.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.covered.N\endcsname{174}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.covered.N\endcsname{174}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.covered.N\endcsname{17400.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.covered.N\endcsname{$+$17400.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.covered.acc-F\endcsname{0.845}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.covered.acc-F\endcsname{84.5}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.covered.acc-F\endcsname{$+$84.5}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.covered.acc-R\endcsname{0.856}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.covered.acc-R\endcsname{85.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.covered.acc-R\endcsname{$+$85.6}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{-0.011}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$1.1}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.covered.resid-F-minus-R\endcsname{$-$1.1}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.covered.share\endcsname{0.906}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.covered.share\endcsname{90.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.covered.share\endcsname{$+$90.6}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.missed.N\endcsname{18}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.missed.N\endcsname{18}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.missed.N\endcsname{1800.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.missed.N\endcsname{$+$1800.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.missed.acc-F\endcsname{0.278}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.missed.acc-F\endcsname{27.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.missed.acc-F\endcsname{$+$27.8}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.missed.acc-R\endcsname{0.167}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.missed.acc-R\endcsname{16.7}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.missed.acc-R\endcsname{$+$16.7}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0.111}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{11.1}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.missed.resid-F-minus-R\endcsname{$+$11.1}
\expandafter\def\csname val@expl.uiv.p2.e5.C.multi-view.missed.share\endcsname{0.094}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.multi-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.multi-view.missed.share\endcsname{9.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.multi-view.missed.share\endcsname{$+$9.4}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.covered.N\endcsname{171}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.covered.N\endcsname{171}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.covered.N\endcsname{17100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.covered.N\endcsname{$+$17100.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.covered.acc-F\endcsname{0.848}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.covered.acc-F\endcsname{84.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.covered.acc-F\endcsname{$+$84.8}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.covered.acc-R\endcsname{0.854}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.covered.acc-R\endcsname{85.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.covered.acc-R\endcsname{$+$85.4}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{-0.006}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{$-$0.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.covered.resid-F-minus-R\endcsname{$-$0.6}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.covered.share\endcsname{0.910}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.covered.share\endcsname{91.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.covered.share\endcsname{$+$91.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.missed.N\endcsname{17}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.missed.N\endcsname{17}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.missed.N\endcsname{1700.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.missed.N\endcsname{$+$1700.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.missed.acc-F\endcsname{0.353}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.missed.acc-F\endcsname{35.3}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.missed.acc-F\endcsname{$+$35.3}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.missed.acc-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.missed.acc-R\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{0.353}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{35.3}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.missed.resid-F-minus-R\endcsname{$+$35.3}
\expandafter\def\csname val@expl.uiv.p2.e5.C.single-view.missed.share\endcsname{0.090}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.single-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.single-view.missed.share\endcsname{9.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.single-view.missed.share\endcsname{$+$9.0}
\expandafter\def\csname val@expl.uiv.p2.e5.C.strata.agree-drift.missed-share\endcsname{0.625}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.strata.agree-drift.missed-share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.strata.agree-drift.missed-share\endcsname{62.5}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.strata.agree-drift.missed-share\endcsname{$+$62.5}
\expandafter\def\csname val@expl.uiv.p2.e5.C.strata.agree-stable.missed-share\endcsname{0.048}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.strata.agree-stable.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.strata.agree-stable.missed-share\endcsname{4.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.strata.agree-stable.missed-share\endcsname{$+$4.8}
\expandafter\def\csname val@expl.uiv.p2.e5.C.strata.disagree.missed-share\endcsname{0.368}
\expandafter\def\csname cnt@expl.uiv.p2.e5.C.strata.disagree.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.C.strata.disagree.missed-share\endcsname{36.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.C.strata.disagree.missed-share\endcsname{$+$36.8}
\expandafter\def\csname val@expl.uiv.p2.e5.T.covered.N\endcsname{521}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.covered.N\endcsname{521}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.covered.N\endcsname{52100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.covered.N\endcsname{$+$52100.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.covered.acc-F\endcsname{0.877}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.covered.acc-F\endcsname{87.7}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.covered.acc-F\endcsname{$+$87.7}
\expandafter\def\csname val@expl.uiv.p2.e5.T.covered.acc-R\endcsname{0.877}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.covered.acc-R\endcsname{87.7}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.covered.acc-R\endcsname{$+$87.7}
\expandafter\def\csname val@expl.uiv.p2.e5.T.covered.resid-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.covered.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.covered.resid-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.covered.share\endcsname{0.920}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.covered.share\endcsname{92.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.covered.share\endcsname{$+$92.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.N\endcsname{45}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.N\endcsname{45}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.N\endcsname{4500.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.N\endcsname{$+$4500.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.acc-F\endcsname{0.222}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.acc-F\endcsname{22.2}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.acc-F\endcsname{$+$22.2}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.acc-R\endcsname{0.089}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.acc-R\endcsname{8.9}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.acc-R\endcsname{$+$8.9}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.resid-F-minus-R\endcsname{0.133}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.resid-F-minus-R\endcsname{13.3}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.resid-F-minus-R\endcsname{$+$13.3}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.share\endcsname{0.080}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.share\endcsname{8.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.share\endcsname{$+$8.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.share-of-net-residual\endcsname{1.000}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.share-of-net-residual\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.share-of-net-residual\endcsname{100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.share-of-net-residual\endcsname{$+$100.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.missed.share-of-replay-errors\endcsname{0.390}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.missed.share-of-replay-errors\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.missed.share-of-replay-errors\endcsname{39.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.missed.share-of-replay-errors\endcsname{$+$39.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.covered.N\endcsname{260}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.covered.N\endcsname{260}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.covered.N\endcsname{26000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.covered.N\endcsname{$+$26000.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.covered.acc-F\endcsname{0.877}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.covered.acc-F\endcsname{87.7}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.covered.acc-F\endcsname{$+$87.7}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.covered.acc-R\endcsname{0.873}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.covered.acc-R\endcsname{87.3}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.covered.acc-R\endcsname{$+$87.3}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{0.004}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{0.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.covered.resid-F-minus-R\endcsname{$+$0.4}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.covered.share\endcsname{0.915}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.covered.share\endcsname{91.5}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.covered.share\endcsname{$+$91.5}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.missed.N\endcsname{24}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.missed.N\endcsname{24}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.missed.N\endcsname{2400.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.missed.N\endcsname{$+$2400.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.missed.acc-F\endcsname{0.208}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.missed.acc-F\endcsname{20.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.missed.acc-F\endcsname{$+$20.8}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.missed.acc-R\endcsname{0.125}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.missed.acc-R\endcsname{12.5}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.missed.acc-R\endcsname{$+$12.5}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{0.083}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{8.3}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.missed.resid-F-minus-R\endcsname{$+$8.3}
\expandafter\def\csname val@expl.uiv.p2.e5.T.multi-view.missed.share\endcsname{0.085}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.multi-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.multi-view.missed.share\endcsname{8.5}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.multi-view.missed.share\endcsname{$+$8.5}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.covered.N\endcsname{261}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.covered.N\endcsname{261}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.covered.N\endcsname{26100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.covered.N\endcsname{$+$26100.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.covered.acc-F\endcsname{0.877}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.covered.acc-F\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.covered.acc-F\endcsname{87.7}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.covered.acc-F\endcsname{$+$87.7}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.covered.acc-R\endcsname{0.881}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.covered.acc-R\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.covered.acc-R\endcsname{88.1}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.covered.acc-R\endcsname{$+$88.1}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{-0.004}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{$-$0.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.covered.resid-F-minus-R\endcsname{$-$0.4}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.covered.share\endcsname{0.926}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.covered.share\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.covered.share\endcsname{92.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.covered.share\endcsname{$+$92.6}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.missed.N\endcsname{21}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.missed.N\endcsname{21}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.missed.N\endcsname{2100.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.missed.N\endcsname{$+$2100.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.missed.acc-F\endcsname{0.238}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.missed.acc-F\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.missed.acc-F\endcsname{23.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.missed.acc-F\endcsname{$+$23.8}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.missed.acc-R\endcsname{0.048}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.missed.acc-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.missed.acc-R\endcsname{4.8}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.missed.acc-R\endcsname{$+$4.8}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{0.190}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{19.0}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.missed.resid-F-minus-R\endcsname{$+$19.0}
\expandafter\def\csname val@expl.uiv.p2.e5.T.single-view.missed.share\endcsname{0.074}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.single-view.missed.share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.single-view.missed.share\endcsname{7.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.single-view.missed.share\endcsname{$+$7.4}
\expandafter\def\csname val@expl.uiv.p2.e5.T.strata.agree-drift.missed-share\endcsname{0.444}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.strata.agree-drift.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.strata.agree-drift.missed-share\endcsname{44.4}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.strata.agree-drift.missed-share\endcsname{$+$44.4}
\expandafter\def\csname val@expl.uiv.p2.e5.T.strata.agree-stable.missed-share\endcsname{0.049}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.strata.agree-stable.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.strata.agree-stable.missed-share\endcsname{4.9}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.strata.agree-stable.missed-share\endcsname{$+$4.9}
\expandafter\def\csname val@expl.uiv.p2.e5.T.strata.disagree.missed-share\endcsname{0.356}
\expandafter\def\csname cnt@expl.uiv.p2.e5.T.strata.disagree.missed-share\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e5.T.strata.disagree.missed-share\endcsname{35.6}
\expandafter\def\csname ppt@expl.uiv.p2.e5.T.strata.disagree.missed-share\endcsname{$+$35.6}
\expandafter\def\csname val@expl.uiv.p2.e6.histories\endcsname{20}
\expandafter\def\csname cnt@expl.uiv.p2.e6.histories\endcsname{20}
\expandafter\def\csname pct@expl.uiv.p2.e6.histories\endcsname{2000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e6.histories\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{-0.007}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$0.7}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.0\endcsname{$-$0.7}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0.009}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{0.9}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.ci95.1\endcsname{$+$0.9}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{0.001}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{0.1}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.mean\endcsname{$+$0.1}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0.422}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{42.2}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-generic-ppi-source.p-le0\endcsname{$+$42.2}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{-0.020}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$2.0}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.0\endcsname{$-$2.0}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{0.016}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{1.6}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-only.ci95.1\endcsname{$+$1.6}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-only.mean\endcsname{-0.002}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-only.mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-only.mean\endcsname{$-$0.2}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-only.p-le0\endcsname{0.595}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-only.p-le0\endcsname{1}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-only.p-le0\endcsname{59.5}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-only.p-le0\endcsname{$+$59.5}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{-0.007}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$0.7}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.0\endcsname{$-$0.7}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0.008}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{0.8}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.ci95.1\endcsname{$+$0.8}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.mean\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0.459}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{45.9}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-replay-ppi-uniform.p-le0\endcsname{$+$45.9}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{-0.003}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$0.3}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.0\endcsname{$-$0.3}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{0.003}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{0.3}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.mean\endcsname{$+$0.3}
\expandafter\def\csname val@expl.uiv.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{0.195}
\expandafter\def\csname cnt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{19.5}
\expandafter\def\csname ppt@expl.uiv.p2.e6.rcr-minus-uniform-fresh.p-le0\endcsname{$+$19.5}
\expandafter\def\csname val@expl.uiv.p2.e6.reps\endcsname{1000}
\expandafter\def\csname cnt@expl.uiv.p2.e6.reps\endcsname{1{,}000}
\expandafter\def\csname pct@expl.uiv.p2.e6.reps\endcsname{100000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e6.reps\endcsname{$+$100000.0}
\expandafter\def\csname val@expl.uiv.p2.e8.C.direct-in-zoomed.n\endcsname{360}
\expandafter\def\csname cnt@expl.uiv.p2.e8.C.direct-in-zoomed.n\endcsname{360}
\expandafter\def\csname pct@expl.uiv.p2.e8.C.direct-in-zoomed.n\endcsname{36000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e8.C.direct-in-zoomed.n\endcsname{$+$36000.0}
\expandafter\def\csname val@expl.uiv.p2.e8.C.direct-in-zoomed.resid\endcsname{0.006}
\expandafter\def\csname cnt@expl.uiv.p2.e8.C.direct-in-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.C.direct-in-zoomed.resid\endcsname{0.6}
\expandafter\def\csname ppt@expl.uiv.p2.e8.C.direct-in-zoomed.resid\endcsname{$+$0.6}
\expandafter\def\csname val@expl.uiv.p2.e8.C.direct-outside-zoomed.n\endcsname{20}
\expandafter\def\csname cnt@expl.uiv.p2.e8.C.direct-outside-zoomed.n\endcsname{20}
\expandafter\def\csname pct@expl.uiv.p2.e8.C.direct-outside-zoomed.n\endcsname{2000.0}
\expandafter\def\csname ppt@expl.uiv.p2.e8.C.direct-outside-zoomed.n\endcsname{$+$2000.0}
\expandafter\def\csname val@expl.uiv.p2.e8.C.direct-outside-zoomed.resid\endcsname{0.150}
\expandafter\def\csname cnt@expl.uiv.p2.e8.C.direct-outside-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.C.direct-outside-zoomed.resid\endcsname{15.0}
\expandafter\def\csname ppt@expl.uiv.p2.e8.C.direct-outside-zoomed.resid\endcsname{$+$15.0}
\expandafter\def\csname val@expl.uiv.p2.e8.C.eta2-agree-stable-vs-other\endcsname{0.004}
\expandafter\def\csname cnt@expl.uiv.p2.e8.C.eta2-agree-stable-vs-other\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.C.eta2-agree-stable-vs-other\endcsname{0.4}
\expandafter\def\csname ppt@expl.uiv.p2.e8.C.eta2-agree-stable-vs-other\endcsname{$+$0.4}
\expandafter\def\csname val@expl.uiv.p2.e8.C.eta2-direct-in-zoomed\endcsname{0.011}
\expandafter\def\csname cnt@expl.uiv.p2.e8.C.eta2-direct-in-zoomed\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.C.eta2-direct-in-zoomed\endcsname{1.1}
\expandafter\def\csname ppt@expl.uiv.p2.e8.C.eta2-direct-in-zoomed\endcsname{$+$1.1}
\expandafter\def\csname val@expl.uiv.p2.e8.T.direct-in-zoomed.n\endcsname{547}
\expandafter\def\csname cnt@expl.uiv.p2.e8.T.direct-in-zoomed.n\endcsname{547}
\expandafter\def\csname pct@expl.uiv.p2.e8.T.direct-in-zoomed.n\endcsname{54700.0}
\expandafter\def\csname ppt@expl.uiv.p2.e8.T.direct-in-zoomed.n\endcsname{$+$54700.0}
\expandafter\def\csname val@expl.uiv.p2.e8.T.direct-in-zoomed.resid\endcsname{0.000}
\expandafter\def\csname cnt@expl.uiv.p2.e8.T.direct-in-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.T.direct-in-zoomed.resid\endcsname{0.0}
\expandafter\def\csname ppt@expl.uiv.p2.e8.T.direct-in-zoomed.resid\endcsname{0.0}
\expandafter\def\csname val@expl.uiv.p2.e8.T.direct-outside-zoomed.n\endcsname{19}
\expandafter\def\csname cnt@expl.uiv.p2.e8.T.direct-outside-zoomed.n\endcsname{19}
\expandafter\def\csname pct@expl.uiv.p2.e8.T.direct-outside-zoomed.n\endcsname{1900.0}
\expandafter\def\csname ppt@expl.uiv.p2.e8.T.direct-outside-zoomed.n\endcsname{$+$1900.0}
\expandafter\def\csname val@expl.uiv.p2.e8.T.direct-outside-zoomed.resid\endcsname{0.316}
\expandafter\def\csname cnt@expl.uiv.p2.e8.T.direct-outside-zoomed.resid\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.T.direct-outside-zoomed.resid\endcsname{31.6}
\expandafter\def\csname ppt@expl.uiv.p2.e8.T.direct-outside-zoomed.resid\endcsname{$+$31.6}
\expandafter\def\csname val@expl.uiv.p2.e8.T.eta2-agree-stable-vs-other\endcsname{0.051}
\expandafter\def\csname cnt@expl.uiv.p2.e8.T.eta2-agree-stable-vs-other\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.T.eta2-agree-stable-vs-other\endcsname{5.1}
\expandafter\def\csname ppt@expl.uiv.p2.e8.T.eta2-agree-stable-vs-other\endcsname{$+$5.1}
\expandafter\def\csname val@expl.uiv.p2.e8.T.eta2-direct-in-zoomed\endcsname{0.051}
\expandafter\def\csname cnt@expl.uiv.p2.e8.T.eta2-direct-in-zoomed\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e8.T.eta2-direct-in-zoomed\endcsname{5.1}
\expandafter\def\csname ppt@expl.uiv.p2.e8.T.eta2-direct-in-zoomed\endcsname{$+$5.1}
\expandafter\def\csname val@expl.uiv.p2.e9.mean\endcsname{-0.021}
\expandafter\def\csname cnt@expl.uiv.p2.e9.mean\endcsname{0}
\expandafter\def\csname pct@expl.uiv.p2.e9.mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@expl.uiv.p2.e9.mean\endcsname{$-$2.1}
\expandafter\def\csname val@expl.uiv.p2.e9.n\endcsname{4}
\expandafter\def\csname cnt@expl.uiv.p2.e9.n\endcsname{4}
\expandafter\def\csname pct@expl.uiv.p2.e9.n\endcsname{400.0}
\expandafter\def\csname ppt@expl.uiv.p2.e9.n\endcsname{$+$400.0}
\expandafter\def\csname val@expl.uiv.p2.e9.n-negative\endcsname{3}
\expandafter\def\csname cnt@expl.uiv.p2.e9.n-negative\endcsname{3}
\expandafter\def\csname pct@expl.uiv.p2.e9.n-negative\endcsname{300.0}
\expandafter\def\csname ppt@expl.uiv.p2.e9.n-negative\endcsname{$+$300.0}
\expandafter\def\csname val@holm.family-size\endcsname{8}
\expandafter\def\csname cnt@holm.family-size\endcsname{8}
\expandafter\def\csname pct@holm.family-size\endcsname{800.0}
\expandafter\def\csname ppt@holm.family-size\endcsname{$+$800.0}
\expandafter\def\csname val@holm.n-marginal\endcsname{3}
\expandafter\def\csname cnt@holm.n-marginal\endcsname{3}
\expandafter\def\csname pct@holm.n-marginal\endcsname{300.0}
\expandafter\def\csname ppt@holm.n-marginal\endcsname{$+$300.0}
\expandafter\def\csname val@holm.n-rejected\endcsname{7}
\expandafter\def\csname cnt@holm.n-rejected\endcsname{7}
\expandafter\def\csname pct@holm.n-rejected\endcsname{700.0}
\expandafter\def\csname ppt@holm.n-rejected\endcsname{$+$700.0}
\expandafter\def\csname val@holm.sspro.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{0.021}
\expandafter\def\csname cnt@holm.sspro.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{2.1}
\expandafter\def\csname ppt@holm.sspro.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{$+$2.1}
\expandafter\def\csname val@holm.sspro.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0.004}
\expandafter\def\csname cnt@holm.sspro.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0.4}
\expandafter\def\csname ppt@holm.sspro.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{$+$0.4}
\expandafter\def\csname val@holm.sspro.p1.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname cnt@holm.sspro.p1.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname pct@holm.sspro.p1.rcr-vs-generic-ppi-source.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.sspro.p1.rcr-vs-generic-ppi-source.reject\endcsname{$+$100.0}
\expandafter\def\csname val@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0.049}
\expandafter\def\csname cnt@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{4.9}
\expandafter\def\csname ppt@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{$+$4.9}
\expandafter\def\csname val@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0.014}
\expandafter\def\csname cnt@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{1.4}
\expandafter\def\csname ppt@holm.sspro.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{$+$1.4}
\expandafter\def\csname val@holm.sspro.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{1}
\expandafter\def\csname cnt@holm.sspro.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{1}
\expandafter\def\csname pct@holm.sspro.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.sspro.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{$+$100.0}
\expandafter\def\csname val@holm.sspro.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{0.002}
\expandafter\def\csname cnt@holm.sspro.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{0.2}
\expandafter\def\csname ppt@holm.sspro.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{$+$0.2}
\expandafter\def\csname val@holm.sspro.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{0.000}
\expandafter\def\csname cnt@holm.sspro.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{0.0}
\expandafter\def\csname ppt@holm.sspro.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{0.0}
\expandafter\def\csname val@holm.sspro.p2.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname cnt@holm.sspro.p2.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname pct@holm.sspro.p2.rcr-vs-generic-ppi-source.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.sspro.p2.rcr-vs-generic-ppi-source.reject\endcsname{$+$100.0}
\expandafter\def\csname val@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0.002}
\expandafter\def\csname cnt@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0.2}
\expandafter\def\csname ppt@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{$+$0.2}
\expandafter\def\csname val@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0.000}
\expandafter\def\csname cnt@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0.0}
\expandafter\def\csname ppt@holm.sspro.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0.0}
\expandafter\def\csname val@holm.sspro.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{1}
\expandafter\def\csname cnt@holm.sspro.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{1}
\expandafter\def\csname pct@holm.sspro.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.sspro.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{$+$100.0}
\expandafter\def\csname val@holm.uiv.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{0.002}
\expandafter\def\csname cnt@holm.uiv.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{0.2}
\expandafter\def\csname ppt@holm.uiv.p1.rcr-vs-generic-ppi-source.p-holm\endcsname{$+$0.2}
\expandafter\def\csname val@holm.uiv.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0.000}
\expandafter\def\csname cnt@holm.uiv.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0.0}
\expandafter\def\csname ppt@holm.uiv.p1.rcr-vs-generic-ppi-source.p-raw\endcsname{0.0}
\expandafter\def\csname val@holm.uiv.p1.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname cnt@holm.uiv.p1.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname pct@holm.uiv.p1.rcr-vs-generic-ppi-source.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.uiv.p1.rcr-vs-generic-ppi-source.reject\endcsname{$+$100.0}
\expandafter\def\csname val@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0.165}
\expandafter\def\csname cnt@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{16.5}
\expandafter\def\csname ppt@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-holm\endcsname{$+$16.5}
\expandafter\def\csname val@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0.165}
\expandafter\def\csname cnt@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{16.5}
\expandafter\def\csname ppt@holm.uiv.p1.rcr-vs-replay-ppi-uniform.p-raw\endcsname{$+$16.5}
\expandafter\def\csname val@holm.uiv.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{0}
\expandafter\def\csname cnt@holm.uiv.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{0.0}
\expandafter\def\csname ppt@holm.uiv.p1.rcr-vs-replay-ppi-uniform.reject\endcsname{0.0}
\expandafter\def\csname val@holm.uiv.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{0.049}
\expandafter\def\csname cnt@holm.uiv.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{4.9}
\expandafter\def\csname ppt@holm.uiv.p2.rcr-vs-generic-ppi-source.p-holm\endcsname{$+$4.9}
\expandafter\def\csname val@holm.uiv.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{0.012}
\expandafter\def\csname cnt@holm.uiv.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{1.2}
\expandafter\def\csname ppt@holm.uiv.p2.rcr-vs-generic-ppi-source.p-raw\endcsname{$+$1.2}
\expandafter\def\csname val@holm.uiv.p2.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname cnt@holm.uiv.p2.rcr-vs-generic-ppi-source.reject\endcsname{1}
\expandafter\def\csname pct@holm.uiv.p2.rcr-vs-generic-ppi-source.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.uiv.p2.rcr-vs-generic-ppi-source.reject\endcsname{$+$100.0}
\expandafter\def\csname val@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0.049}
\expandafter\def\csname cnt@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{4.9}
\expandafter\def\csname ppt@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-holm\endcsname{$+$4.9}
\expandafter\def\csname val@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0.013}
\expandafter\def\csname cnt@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{0}
\expandafter\def\csname pct@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{1.3}
\expandafter\def\csname ppt@holm.uiv.p2.rcr-vs-replay-ppi-uniform.p-raw\endcsname{$+$1.3}
\expandafter\def\csname val@holm.uiv.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{1}
\expandafter\def\csname cnt@holm.uiv.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{1}
\expandafter\def\csname pct@holm.uiv.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{100.0}
\expandafter\def\csname ppt@holm.uiv.p2.rcr-vs-replay-ppi-uniform.reject\endcsname{$+$100.0}
\expandafter\def\csname val@overlap.pilot-uiv.A.apps\endcsname{4}
\expandafter\def\csname cnt@overlap.pilot-uiv.A.apps\endcsname{4}
\expandafter\def\csname pct@overlap.pilot-uiv.A.apps\endcsname{400.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.A.apps\endcsname{$+$400.0}
\expandafter\def\csname val@overlap.pilot-uiv.A.n\endcsname{32}
\expandafter\def\csname cnt@overlap.pilot-uiv.A.n\endcsname{32}
\expandafter\def\csname pct@overlap.pilot-uiv.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@overlap.pilot-uiv.A.of\endcsname{64}
\expandafter\def\csname cnt@overlap.pilot-uiv.A.of\endcsname{64}
\expandafter\def\csname pct@overlap.pilot-uiv.A.of\endcsname{6400.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.A.of\endcsname{$+$6400.0}
\expandafter\def\csname val@overlap.pilot-uiv.A.of-apps\endcsname{8}
\expandafter\def\csname cnt@overlap.pilot-uiv.A.of-apps\endcsname{8}
\expandafter\def\csname pct@overlap.pilot-uiv.A.of-apps\endcsname{800.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.A.of-apps\endcsname{$+$800.0}
\expandafter\def\csname val@overlap.pilot-uiv.C.apps\endcsname{4}
\expandafter\def\csname cnt@overlap.pilot-uiv.C.apps\endcsname{4}
\expandafter\def\csname pct@overlap.pilot-uiv.C.apps\endcsname{400.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.C.apps\endcsname{$+$400.0}
\expandafter\def\csname val@overlap.pilot-uiv.C.n\endcsname{32}
\expandafter\def\csname cnt@overlap.pilot-uiv.C.n\endcsname{32}
\expandafter\def\csname pct@overlap.pilot-uiv.C.n\endcsname{3200.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.C.n\endcsname{$+$3200.0}
\expandafter\def\csname val@overlap.pilot-uiv.C.of\endcsname{96}
\expandafter\def\csname cnt@overlap.pilot-uiv.C.of\endcsname{96}
\expandafter\def\csname pct@overlap.pilot-uiv.C.of\endcsname{9600.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.C.of\endcsname{$+$9600.0}
\expandafter\def\csname val@overlap.pilot-uiv.C.of-apps\endcsname{12}
\expandafter\def\csname cnt@overlap.pilot-uiv.C.of-apps\endcsname{12}
\expandafter\def\csname pct@overlap.pilot-uiv.C.of-apps\endcsname{1200.0}
\expandafter\def\csname ppt@overlap.pilot-uiv.C.of-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{0.594}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{59.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{$+$59.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{0.906}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{90.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{0.812}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{81.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{0.875}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{87.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{0.906}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{90.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{0.750}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{75.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{-0.031}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{$-$3.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{$-$3.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{2.031}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{203.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{$+$203.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{0.125}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{12.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{$+$12.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{25}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{25}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{2500.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{$+$2500.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{0.960}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{96.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{$+$96.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{0.960}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{96.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{$+$96.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-srcfail.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.N\endcsname{4}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.N\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.N\endcsname{400.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.N\endcsname{$+$400.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-F\endcsname{0.250}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-F\endcsname{25.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-F\endcsname{$+$25.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-R\endcsname{0.750}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-R\endcsname{75.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.mean-R\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree-stable.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{0.219}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{21.9}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{$+$21.9}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{0.094}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{9.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{0.594}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{59.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{$+$59.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{0.812}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{81.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{0.812}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{81.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{0.844}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{84.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{$+$84.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{0.906}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{90.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{0.031}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{3.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{$+$3.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{0.031}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{3.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{$+$3.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{27}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{27}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{2700.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{$+$2700.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{0.889}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{88.9}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{$+$88.9}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{0.926}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{92.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{$+$92.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{0.189}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{18.9}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{$+$18.9}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.N\endcsname{2}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.N\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree-stable.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.parse-fail.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{0.219}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{21.9}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{$+$21.9}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{0.062}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{6.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{$+$6.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{0.594}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{59.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{$+$59.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{0.875}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{87.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{0.875}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{87.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{0.812}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{81.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{0.719}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{71.9}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{$+$71.9}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{3.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{3}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{300.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{3.031}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{3}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{303.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{$+$303.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{0.094}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{9.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-F\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-F\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-F\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-srcfail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{24}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{24}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{2400.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{$+$2400.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{0.917}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{91.7}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{$+$91.7}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{0.917}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{91.7}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{$+$91.7}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{0.408}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{40.8}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{$+$40.8}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.N\endcsname{1}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.N\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-srcfail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.N\endcsname{3}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.N\endcsname{3}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.N\endcsname{300.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.N\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-F\endcsname{0.667}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-F\endcsname{66.7}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-F\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.sd-resid\endcsname{0.471}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.sd-resid\endcsname{47.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree-stable.sd-resid\endcsname{$+$47.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{0.188}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{18.8}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{$+$18.8}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{0.094}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{9.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{0.594}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{59.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{$+$59.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{0.875}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{87.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{0.906}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{90.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{0.844}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{84.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{$+$84.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{0.094}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{9.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{4.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{400.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{$+$400.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{3.938}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{393.8}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{$+$393.8}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{25}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{25}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{2500.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{$+$2500.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{0.920}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{92.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{$+$92.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{0.920}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{92.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{$+$92.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.N\endcsname{3}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.N\endcsname{3}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.N\endcsname{300.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.N\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-R\endcsname{0.667}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-R\endcsname{66.7}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.mean-R\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.sd-resid\endcsname{0.471}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.sd-resid\endcsname{47.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree-stable.sd-resid\endcsname{$+$47.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.N\endcsname{400.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.N\endcsname{$+$400.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.parse-fail.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{0.188}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{18.8}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{$+$18.8}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{0.094}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{9.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-source\endcsname{0.594}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-source\endcsname{59.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-source\endcsname{$+$59.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-target\endcsname{0.781}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-target\endcsname{78.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-direct-target\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-replay\endcsname{0.875}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-replay\endcsname{87.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-replay\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-source-natural\endcsname{0.812}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-source-natural\endcsname{81.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-source-natural\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-target-natural\endcsname{0.906}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-target-natural\endcsname{90.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.acc-target-natural\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-R\endcsname{0.906}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-R\endcsname{90.6}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-R\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-S\endcsname{0.844}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-S\endcsname{84.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.agreement-F-S\endcsname{$+$84.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.bias-F-minus-R\endcsname{0.031}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.bias-F-minus-R\endcsname{3.1}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.bias-F-minus-R\endcsname{$+$3.1}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-source-natural\endcsname{3.875}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-source-natural\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-source-natural\endcsname{387.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-source-natural\endcsname{$+$387.5}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-target-natural\endcsname{3.812}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-target-natural\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-target-natural\endcsname{381.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.mean-requests-target-natural\endcsname{$+$381.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.rho-replay\endcsname{0.094}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.rho-replay\endcsname{9.4}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.rho-replay\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.N\endcsname{26}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.N\endcsname{26}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.N\endcsname{2600.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.N\endcsname{$+$2600.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-F\endcsname{0.962}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-F\endcsname{96.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-F\endcsname{$+$96.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-R\endcsname{0.962}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-R\endcsname{96.2}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.mean-R\endcsname{$+$96.2}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.N\endcsname{2}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.N\endcsname{2}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-srcfail.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.N\endcsname{4}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.N\endcsname{4}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.N\endcsname{400.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.N\endcsname{$+$400.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-F\endcsname{0.750}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-F\endcsname{75.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-F\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-R\endcsname{0.750}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-R\endcsname{75.0}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.mean-R\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.sd-resid\endcsname{0.707}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.sd-resid\endcsname{1}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.sd-resid\endcsname{70.7}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.strata.disagree-stable.sd-resid\endcsname{$+$70.7}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-source\endcsname{0.219}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-source\endcsname{21.9}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-source\endcsname{$+$21.9}
\expandafter\def\csname val@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-target\endcsname{0.125}
\expandafter\def\csname cnt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-target\endcsname{12.5}
\expandafter\def\csname ppt@pilot.sspro.pilot-haiku-to-sonnet.per-skill.zoomclick-d3.A.tau-target\endcsname{$+$12.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.full-recert\endcsname{0.837}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.full-recert\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.full-recert\endcsname{83.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.full-recert\endcsname{$+$83.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.1\endcsname{0.823}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.1\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.1\endcsname{82.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.1\endcsname{$+$82.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.25\endcsname{0.831}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.25\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.25\endcsname{83.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.25\endcsname{$+$83.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.5\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.5\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.5\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@0.5\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@1.0\endcsname{0.837}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@1.0\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@1.0\endcsname{83.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.generic-ppi-source@1.0\endcsname{$+$83.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.keep-all\endcsname{0.806}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.keep-all\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.keep-all\endcsname{80.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.keep-all\endcsname{$+$80.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.old-decision\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.old-decision\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.old-decision\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.old-decision\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.oracle-dep\endcsname{0.837}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.oracle-dep\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.oracle-dep\endcsname{83.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.oracle-dep\endcsname{$+$83.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.25\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.25\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.25\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.25\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.5\endcsname{0.834}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.5\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.5\endcsname{83.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@0.5\endcsname{$+$83.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@1.0\endcsname{0.837}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@1.0\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@1.0\endcsname{83.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.rcr-stratified@1.0\endcsname{$+$83.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-only\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-only\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-only\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-only\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.1\endcsname{0.824}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.1\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.1\endcsname{82.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.1\endcsname{$+$82.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.25\endcsname{0.829}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.25\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.25\endcsname{82.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.25\endcsname{$+$82.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.5\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.5\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.5\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@0.5\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@1.0\endcsname{0.837}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@1.0\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@1.0\endcsname{83.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.replay-ppi-uniform@1.0\endcsname{$+$83.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.suspend-all\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.suspend-all\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.suspend-all\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.suspend-all\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.1\endcsname{0.820}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.1\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.1\endcsname{82.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.1\endcsname{$+$82.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.25\endcsname{0.831}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.25\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.25\endcsname{83.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.25\endcsname{$+$83.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.5\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.5\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.5\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@0.5\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@1.0\endcsname{0.837}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@1.0\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@1.0\endcsname{83.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.catalog.uniform-fresh@1.0\endcsname{$+$83.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{0.688}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{68.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-source\endcsname{$+$68.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{0.906}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{90.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-direct-target\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{0.750}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{75.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-replay\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{0.656}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{65.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-source-natural\endcsname{$+$65.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{0.844}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{84.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.acc-target-natural\endcsname{$+$84.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{0.906}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{90.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-R\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{0.812}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{81.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.agreement-F-S\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{0.094}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{9.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.bias-F-minus-R\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{2.281}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{228.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-source-natural\endcsname{$+$228.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{-0.156}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{$-$15.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.rho-replay\endcsname{$-$15.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{25}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{25}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{2500.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.N\endcsname{$+$2500.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{0.880}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{88.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-F\endcsname{$+$88.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{0.880}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{88.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.mean-R\endcsname{$+$88.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-F\endcsname{0.667}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-F\endcsname{66.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-F\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-R\endcsname{0.167}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-R\endcsname{16.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.mean-R\endcsname{$+$16.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.strata.disagree.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{-0.031}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{-0.062}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{$-$6.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.A.tau-target\endcsname{$-$6.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-source\endcsname{0.729}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-source\endcsname{72.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-source\endcsname{$+$72.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-target\endcsname{0.854}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-target\endcsname{85.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-direct-target\endcsname{$+$85.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-replay\endcsname{0.812}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-replay\endcsname{81.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-replay\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-source-natural\endcsname{0.667}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-source-natural\endcsname{66.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-source-natural\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-target-natural\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-target-natural\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.acc-target-natural\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-R\endcsname{0.854}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-R\endcsname{85.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-R\endcsname{$+$85.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-S\endcsname{0.792}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-S\endcsname{79.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.agreement-F-S\endcsname{$+$79.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.bias-F-minus-R\endcsname{0.021}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.bias-F-minus-R\endcsname{2.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.bias-F-minus-R\endcsname{$+$2.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-source-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-source-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-source-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.n\endcsname{48}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.n\endcsname{48}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.n\endcsname{4800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.n\endcsname{$+$4800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.rho-replay\endcsname{-0.042}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.rho-replay\endcsname{$-$4.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.rho-replay\endcsname{$-$4.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.N\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.N\endcsname{38}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.N\endcsname{38}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.N\endcsname{3800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.N\endcsname{$+$3800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-F\endcsname{0.921}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-F\endcsname{92.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-F\endcsname{$+$92.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-R\endcsname{0.947}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-R\endcsname{94.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.mean-R\endcsname{$+$94.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.sd-resid\endcsname{0.280}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.sd-resid\endcsname{28.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.agree-stable.sd-resid\endcsname{$+$28.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.N\endcsname{8}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.N\endcsname{8}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.N\endcsname{800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.N\endcsname{$+$800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-R\endcsname{0.250}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-R\endcsname{25.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.mean-R\endcsname{$+$25.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.sd-resid\endcsname{0.661}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.sd-resid\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.sd-resid\endcsname{66.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.disagree.sd-resid\endcsname{$+$66.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.N\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.N\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.N\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-F\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-F\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-F\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-source\endcsname{-0.062}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-source\endcsname{$-$6.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-source\endcsname{$-$6.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-target\endcsname{-0.021}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-target\endcsname{$-$2.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.C.tau-target\endcsname{$-$2.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-source\endcsname{0.639}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-source\endcsname{63.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-source\endcsname{$+$63.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-target\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-target\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-direct-target\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-replay\endcsname{0.750}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-replay\endcsname{75.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-replay\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-source-natural\endcsname{0.625}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-source-natural\endcsname{62.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-source-natural\endcsname{$+$62.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-target-natural\endcsname{0.819}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-target-natural\endcsname{81.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.acc-target-natural\endcsname{$+$81.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-R\endcsname{0.847}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-R\endcsname{84.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-R\endcsname{$+$84.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-S\endcsname{0.778}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-S\endcsname{77.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.agreement-F-S\endcsname{$+$77.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.bias-F-minus-R\endcsname{0.069}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.bias-F-minus-R\endcsname{6.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.bias-F-minus-R\endcsname{$+$6.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-source-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-source-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-source-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.n\endcsname{72}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.n\endcsname{72}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.n\endcsname{7200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.n\endcsname{$+$7200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.rho-replay\endcsname{-0.083}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.rho-replay\endcsname{$-$8.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.rho-replay\endcsname{$-$8.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.N\endcsname{700.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.N\endcsname{$+$700.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-F\endcsname{0.857}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-F\endcsname{85.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-F\endcsname{$+$85.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.sd-resid\endcsname{0.350}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.sd-resid\endcsname{35.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-drift.sd-resid\endcsname{$+$35.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.N\endcsname{49}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.N\endcsname{49}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.N\endcsname{4900.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.N\endcsname{$+$4900.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-F\endcsname{0.898}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-F\endcsname{89.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-F\endcsname{$+$89.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-R\endcsname{0.898}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-R\endcsname{89.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.mean-R\endcsname{$+$89.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.N\endcsname{14}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.N\endcsname{14}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.N\endcsname{1400.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.N\endcsname{$+$1400.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-R\endcsname{0.214}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-R\endcsname{21.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.mean-R\endcsname{$+$21.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.sd-resid\endcsname{0.700}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.sd-resid\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.sd-resid\endcsname{70.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.disagree.sd-resid\endcsname{$+$70.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.strata.parse-fail.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-source\endcsname{-0.014}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-source\endcsname{$-$1.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-source\endcsname{$-$1.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-target\endcsname{-0.014}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-target\endcsname{$-$1.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.center-d1.V.tau-target\endcsname{$-$1.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{0.688}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{68.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-source\endcsname{$+$68.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{0.906}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{90.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-direct-target\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{0.719}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{71.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-replay\endcsname{$+$71.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{0.656}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{65.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-source-natural\endcsname{$+$65.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{0.781}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{78.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.acc-target-natural\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{0.875}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{87.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-R\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{0.812}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{81.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.agreement-F-S\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{0.062}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{6.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.bias-F-minus-R\endcsname{$+$6.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{2.531}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{253.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-source-natural\endcsname{$+$253.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{-0.188}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{$-$18.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.rho-replay\endcsname{$-$18.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{23}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{23}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{2300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.N\endcsname{$+$2300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{0.870}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{87.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-F\endcsname{$+$87.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{0.870}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{87.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.mean-R\endcsname{$+$87.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.N\endcsname{7}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.N\endcsname{7}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.N\endcsname{700.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.N\endcsname{$+$700.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-F\endcsname{0.429}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-F\endcsname{42.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-F\endcsname{$+$42.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-R\endcsname{0.143}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-R\endcsname{14.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.mean-R\endcsname{$+$14.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.sd-resid\endcsname{0.700}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.sd-resid\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.sd-resid\endcsname{70.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.strata.disagree.sd-resid\endcsname{$+$70.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{-0.031}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{-0.125}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{$-$12.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.A.tau-target\endcsname{$-$12.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-source\endcsname{0.729}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-source\endcsname{72.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-source\endcsname{$+$72.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-target\endcsname{0.854}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-target\endcsname{85.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-direct-target\endcsname{$+$85.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-replay\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-replay\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-replay\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-source-natural\endcsname{0.646}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-source-natural\endcsname{64.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-source-natural\endcsname{$+$64.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-target-natural\endcsname{0.896}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-target-natural\endcsname{89.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.acc-target-natural\endcsname{$+$89.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-R\endcsname{0.938}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-R\endcsname{93.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-R\endcsname{$+$93.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-S\endcsname{0.750}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-S\endcsname{75.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.agreement-F-S\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.bias-F-minus-R\endcsname{0.062}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.bias-F-minus-R\endcsname{6.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.bias-F-minus-R\endcsname{$+$6.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-source-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-source-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-source-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.n\endcsname{48}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.n\endcsname{48}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.n\endcsname{4800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.n\endcsname{$+$4800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.rho-replay\endcsname{-0.021}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.rho-replay\endcsname{$-$2.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.rho-replay\endcsname{$-$2.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.N\endcsname{700.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.N\endcsname{$+$700.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-F\endcsname{0.714}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-F\endcsname{71.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-F\endcsname{$+$71.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-R\endcsname{0.714}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-R\endcsname{71.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.mean-R\endcsname{$+$71.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.N\endcsname{35}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.N\endcsname{35}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.N\endcsname{3500.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.N\endcsname{$+$3500.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-F\endcsname{0.943}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-F\endcsname{94.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-F\endcsname{$+$94.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-R\endcsname{0.943}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-R\endcsname{94.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.mean-R\endcsname{$+$94.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.N\endcsname{6}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.N\endcsname{6}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.N\endcsname{600.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.N\endcsname{$+$600.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-F\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-F\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-F\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-R\endcsname{0.333}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-R\endcsname{33.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.mean-R\endcsname{$+$33.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.strata.disagree.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-source\endcsname{-0.083}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-source\endcsname{$-$8.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-source\endcsname{$-$8.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-target\endcsname{0.042}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-target\endcsname{4.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.C.tau-target\endcsname{$+$4.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-source\endcsname{0.639}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-source\endcsname{63.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-source\endcsname{$+$63.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-target\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-target\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-direct-target\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-replay\endcsname{0.764}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-replay\endcsname{76.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-replay\endcsname{$+$76.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-source-natural\endcsname{0.667}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-source-natural\endcsname{66.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-source-natural\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-target-natural\endcsname{0.847}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-target-natural\endcsname{84.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.acc-target-natural\endcsname{$+$84.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-R\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-R\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-R\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-S\endcsname{0.764}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-S\endcsname{76.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.agreement-F-S\endcsname{$+$76.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.bias-F-minus-R\endcsname{0.083}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.bias-F-minus-R\endcsname{8.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.bias-F-minus-R\endcsname{$+$8.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-source-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-source-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-source-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-source-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-target-natural\endcsname{2.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-target-natural\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-target-natural\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.mean-requests-target-natural\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.n\endcsname{72}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.n\endcsname{72}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.n\endcsname{7200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.n\endcsname{$+$7200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.rho-replay\endcsname{-0.069}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.rho-replay\endcsname{$-$6.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.rho-replay\endcsname{$-$6.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.N\endcsname{6}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.N\endcsname{6}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.N\endcsname{600.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.N\endcsname{$+$600.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-F\endcsname{0.667}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-F\endcsname{66.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-F\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-R\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-R\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.mean-R\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.sd-resid\endcsname{0.373}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.sd-resid\endcsname{37.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-drift.sd-resid\endcsname{$+$37.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.N\endcsname{50}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.N\endcsname{50}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.N\endcsname{5000.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.N\endcsname{$+$5000.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-F\endcsname{0.980}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-F\endcsname{98.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-F\endcsname{$+$98.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-R\endcsname{0.940}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-R\endcsname{94.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.mean-R\endcsname{$+$94.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.sd-resid\endcsname{0.196}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.sd-resid\endcsname{19.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.agree-stable.sd-resid\endcsname{$+$19.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.N\endcsname{14}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.N\endcsname{14}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.N\endcsname{1400.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.N\endcsname{$+$1400.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-R\endcsname{0.214}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-R\endcsname{21.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.mean-R\endcsname{$+$21.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.sd-resid\endcsname{0.700}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.sd-resid\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.sd-resid\endcsname{70.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.disagree.sd-resid\endcsname{$+$70.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.strata.parse-fail.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-source\endcsname{0.028}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-source\endcsname{2.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-source\endcsname{$+$2.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-target\endcsname{0.014}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-target\endcsname{1.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.context-d1.V.tau-target\endcsname{$+$1.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{0.688}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{68.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-source\endcsname{$+$68.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{0.906}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{90.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-direct-target\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{0.688}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{68.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-replay\endcsname{$+$68.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{0.656}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{65.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-source-natural\endcsname{$+$65.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{0.781}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{78.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.acc-target-natural\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{0.844}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{84.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-R\endcsname{$+$84.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{0.812}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{81.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.agreement-F-S\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{0.094}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{9.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.bias-F-minus-R\endcsname{$+$9.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{3.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-source-natural\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{3.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.mean-requests-target-natural\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{-0.219}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{$-$21.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.rho-replay\endcsname{$-$21.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-drift.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{23}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{23}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{2300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.N\endcsname{$+$2300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{0.870}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{87.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-F\endcsname{$+$87.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{0.870}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{87.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.mean-R\endcsname{$+$87.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.agree-stable.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.N\endcsname{7}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.N\endcsname{7}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.N\endcsname{700.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.N\endcsname{$+$700.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-F\endcsname{0.571}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-F\endcsname{57.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-F\endcsname{$+$57.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.sd-resid\endcsname{0.495}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.sd-resid\endcsname{49.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.strata.disagree.sd-resid\endcsname{$+$49.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{-0.031}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{-0.125}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{$-$12.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.A.tau-target\endcsname{$-$12.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-source\endcsname{0.729}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-source\endcsname{72.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-source\endcsname{$+$72.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-target\endcsname{0.854}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-target\endcsname{85.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-direct-target\endcsname{$+$85.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-replay\endcsname{0.750}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-replay\endcsname{75.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-replay\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-source-natural\endcsname{0.583}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-source-natural\endcsname{58.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-source-natural\endcsname{$+$58.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-target-natural\endcsname{0.812}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-target-natural\endcsname{81.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.acc-target-natural\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-R\endcsname{0.896}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-R\endcsname{89.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-R\endcsname{$+$89.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-S\endcsname{0.771}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-S\endcsname{77.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.agreement-F-S\endcsname{$+$77.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.bias-F-minus-R\endcsname{0.062}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.bias-F-minus-R\endcsname{6.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.bias-F-minus-R\endcsname{$+$6.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-source-natural\endcsname{3.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-source-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-source-natural\endcsname{300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-source-natural\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-target-natural\endcsname{3.042}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-target-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-target-natural\endcsname{304.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.mean-requests-target-natural\endcsname{$+$304.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.n\endcsname{48}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.n\endcsname{48}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.n\endcsname{4800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.n\endcsname{$+$4800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.rho-replay\endcsname{-0.104}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.rho-replay\endcsname{$-$10.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.rho-replay\endcsname{$-$10.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.N\endcsname{9}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.N\endcsname{9}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.N\endcsname{900.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.N\endcsname{$+$900.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-F\endcsname{0.778}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-F\endcsname{77.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-F\endcsname{$+$77.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-R\endcsname{0.778}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-R\endcsname{77.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.mean-R\endcsname{$+$77.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.N\endcsname{34}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.N\endcsname{34}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.N\endcsname{3400.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.N\endcsname{$+$3400.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-F\endcsname{0.882}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-F\endcsname{88.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-F\endcsname{$+$88.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-R\endcsname{0.853}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-R\endcsname{85.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.mean-R\endcsname{$+$85.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.sd-resid\endcsname{0.296}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.sd-resid\endcsname{29.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.agree-stable.sd-resid\endcsname{$+$29.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.N\endcsname{5}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.N\endcsname{5}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.N\endcsname{500.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.N\endcsname{$+$500.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-F\endcsname{0.400}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-F\endcsname{40.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-F\endcsname{$+$40.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.sd-resid\endcsname{0.490}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.sd-resid\endcsname{49.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.strata.disagree.sd-resid\endcsname{$+$49.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-source\endcsname{-0.146}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-source\endcsname{$-$14.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-source\endcsname{$-$14.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-target\endcsname{-0.042}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-target\endcsname{$-$4.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.C.tau-target\endcsname{$-$4.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-source\endcsname{0.639}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-source\endcsname{63.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-source\endcsname{$+$63.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-target\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-target\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-direct-target\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-replay\endcsname{0.722}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-replay\endcsname{72.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-replay\endcsname{$+$72.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-source-natural\endcsname{0.597}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-source-natural\endcsname{59.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-source-natural\endcsname{$+$59.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-target-natural\endcsname{0.819}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-target-natural\endcsname{81.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.acc-target-natural\endcsname{$+$81.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-R\endcsname{0.764}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-R\endcsname{76.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-R\endcsname{$+$76.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-S\endcsname{0.694}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-S\endcsname{69.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.agreement-F-S\endcsname{$+$69.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.bias-F-minus-R\endcsname{0.097}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.bias-F-minus-R\endcsname{9.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.bias-F-minus-R\endcsname{$+$9.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-source-natural\endcsname{3.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-source-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-source-natural\endcsname{300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-source-natural\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-target-natural\endcsname{3.014}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-target-natural\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-target-natural\endcsname{301.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.mean-requests-target-natural\endcsname{$+$301.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.n\endcsname{72}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.n\endcsname{72}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.n\endcsname{7200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.n\endcsname{$+$7200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.rho-replay\endcsname{-0.111}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.rho-replay\endcsname{$-$11.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.rho-replay\endcsname{$-$11.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.N\endcsname{7}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.N\endcsname{700.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.N\endcsname{$+$700.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-F\endcsname{0.714}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-F\endcsname{71.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-F\endcsname{$+$71.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-R\endcsname{0.857}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-R\endcsname{85.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.mean-R\endcsname{$+$85.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.sd-resid\endcsname{0.350}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.sd-resid\endcsname{35.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-drift.sd-resid\endcsname{$+$35.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.N\endcsname{48}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.N\endcsname{48}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.N\endcsname{4800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.N\endcsname{$+$4800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-F\endcsname{0.875}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-F\endcsname{87.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-F\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-R\endcsname{0.917}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-R\endcsname{91.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.mean-R\endcsname{$+$91.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.sd-resid\endcsname{0.351}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.sd-resid\endcsname{35.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.agree-stable.sd-resid\endcsname{$+$35.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.N\endcsname{15}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.N\endcsname{15}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.N\endcsname{1500.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.N\endcsname{$+$1500.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-F\endcsname{0.667}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-F\endcsname{66.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-F\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-R\endcsname{0.133}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-R\endcsname{13.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.mean-R\endcsname{$+$13.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.sd-resid\endcsname{0.499}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.sd-resid\endcsname{49.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.disagree.sd-resid\endcsname{$+$49.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.strata.parse-fail.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-source\endcsname{-0.042}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-source\endcsname{$-$4.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-source\endcsname{$-$4.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-target\endcsname{-0.014}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-target\endcsname{$-$1.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.dual-d2.V.tau-target\endcsname{$-$1.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{0.688}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{68.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-source\endcsname{$+$68.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{0.906}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{90.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-direct-target\endcsname{$+$90.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{0.719}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{71.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-replay\endcsname{$+$71.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{0.656}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{65.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-source-natural\endcsname{$+$65.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{0.781}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{78.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.acc-target-natural\endcsname{$+$78.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{0.875}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{87.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-R\endcsname{$+$87.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{0.812}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{81.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.agreement-F-S\endcsname{$+$81.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{0.062}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{6.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.bias-F-minus-R\endcsname{$+$6.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{3.875}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{387.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-source-natural\endcsname{$+$387.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{3.562}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{356.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.mean-requests-target-natural\endcsname{$+$356.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{32}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{32}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{3200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.n\endcsname{$+$3200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{-0.188}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{$-$18.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.rho-replay\endcsname{$-$18.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-drift.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{23}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{23}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{2300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.N\endcsname{$+$2300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{0.826}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{82.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-F\endcsname{$+$82.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{0.870}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{87.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.mean-R\endcsname{$+$87.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{0.204}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{20.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.agree-stable.sd-resid\endcsname{$+$20.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.N\endcsname{7}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.N\endcsname{7}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.N\endcsname{700.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.N\endcsname{$+$700.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-F\endcsname{0.571}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-F\endcsname{57.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-F\endcsname{$+$57.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-R\endcsname{0.143}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-R\endcsname{14.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.mean-R\endcsname{$+$14.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.sd-resid\endcsname{0.495}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.sd-resid\endcsname{49.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.strata.disagree.sd-resid\endcsname{$+$49.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{-0.031}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-source\endcsname{$-$3.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{-0.125}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{$-$12.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.A.tau-target\endcsname{$-$12.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-source\endcsname{0.729}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-source\endcsname{72.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-source\endcsname{$+$72.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-target\endcsname{0.854}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-target\endcsname{85.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-direct-target\endcsname{$+$85.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-replay\endcsname{0.708}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-replay\endcsname{70.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-replay\endcsname{$+$70.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-source-natural\endcsname{0.583}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-source-natural\endcsname{58.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-source-natural\endcsname{$+$58.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-target-natural\endcsname{0.708}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-target-natural\endcsname{70.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.acc-target-natural\endcsname{$+$70.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-R\endcsname{0.792}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-R\endcsname{79.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-R\endcsname{$+$79.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-S\endcsname{0.750}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-S\endcsname{75.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.agreement-F-S\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.bias-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.bias-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.bias-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-source-natural\endcsname{3.958}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-source-natural\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-source-natural\endcsname{395.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-source-natural\endcsname{$+$395.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-target-natural\endcsname{3.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-target-natural\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-target-natural\endcsname{383.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.mean-requests-target-natural\endcsname{$+$383.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.n\endcsname{48}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.n\endcsname{48}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.n\endcsname{4800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.n\endcsname{$+$4800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.rho-replay\endcsname{-0.146}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.rho-replay\endcsname{$-$14.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.rho-replay\endcsname{$-$14.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.N\endcsname{3}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.N\endcsname{3}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.N\endcsname{300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.N\endcsname{$+$300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-F\endcsname{0.667}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-F\endcsname{66.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-F\endcsname{$+$66.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-R\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-R\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.mean-R\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.sd-resid\endcsname{0.471}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.sd-resid\endcsname{47.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-drift.sd-resid\endcsname{$+$47.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.N\endcsname{33}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.N\endcsname{33}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.N\endcsname{3300.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.N\endcsname{$+$3300.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-F\endcsname{0.788}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-F\endcsname{78.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-F\endcsname{$+$78.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-R\endcsname{0.909}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-R\endcsname{90.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.mean-R\endcsname{$+$90.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.sd-resid\endcsname{0.326}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.sd-resid\endcsname{32.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.agree-stable.sd-resid\endcsname{$+$32.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.N\endcsname{10}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.N\endcsname{10}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.N\endcsname{1000.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.N\endcsname{$+$1000.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-F\endcsname{0.400}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-F\endcsname{40.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-F\endcsname{$+$40.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-R\endcsname{0.100}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-R\endcsname{10.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.mean-R\endcsname{$+$10.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.sd-resid\endcsname{0.458}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.sd-resid\endcsname{45.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.disagree.sd-resid\endcsname{$+$45.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.N\endcsname{2}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.N\endcsname{200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.N\endcsname{$+$200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-F\endcsname{1.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-F\endcsname{100.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-F\endcsname{$+$100.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.sd-resid\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.sd-resid\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.strata.parse-fail.sd-resid\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-source\endcsname{-0.146}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-source\endcsname{$-$14.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-source\endcsname{$-$14.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-target\endcsname{-0.146}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-target\endcsname{$-$14.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.C.tau-target\endcsname{$-$14.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-source\endcsname{0.639}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-source\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-source\endcsname{63.9}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-source\endcsname{$+$63.9}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-target\endcsname{0.833}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-target\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-target\endcsname{83.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-direct-target\endcsname{$+$83.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-replay\endcsname{0.736}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-replay\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-replay\endcsname{73.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-replay\endcsname{$+$73.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-source-natural\endcsname{0.611}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-source-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-source-natural\endcsname{61.1}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-source-natural\endcsname{$+$61.1}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-target-natural\endcsname{0.736}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-target-natural\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-target-natural\endcsname{73.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.acc-target-natural\endcsname{$+$73.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-R\endcsname{0.778}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-R\endcsname{77.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-R\endcsname{$+$77.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-S\endcsname{0.764}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-S\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-S\endcsname{76.4}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.agreement-F-S\endcsname{$+$76.4}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.bias-F-minus-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.bias-F-minus-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.bias-F-minus-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.bias-F-minus-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-source-natural\endcsname{3.958}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-source-natural\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-source-natural\endcsname{395.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-source-natural\endcsname{$+$395.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-target-natural\endcsname{3.722}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-target-natural\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-target-natural\endcsname{372.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.mean-requests-target-natural\endcsname{$+$372.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.n\endcsname{72}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.n\endcsname{72}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.n\endcsname{7200.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.n\endcsname{$+$7200.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.rho-replay\endcsname{-0.097}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.rho-replay\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.rho-replay\endcsname{$-$9.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.rho-replay\endcsname{$-$9.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.N\endcsname{4}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.N\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.N\endcsname{400.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.N\endcsname{$+$400.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-R\endcsname{0.750}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-R\endcsname{75.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.mean-R\endcsname{$+$75.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.sd-resid\endcsname{0.433}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.sd-resid\endcsname{43.3}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-drift.sd-resid\endcsname{$+$43.3}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.N\endcsname{48}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.N\endcsname{48}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.N\endcsname{4800.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.N\endcsname{$+$4800.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-F\endcsname{0.896}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-F\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-F\endcsname{89.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-F\endcsname{$+$89.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-R\endcsname{0.938}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-R\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-R\endcsname{93.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.mean-R\endcsname{$+$93.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.sd-resid\endcsname{0.286}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.sd-resid\endcsname{28.6}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.agree-stable.sd-resid\endcsname{$+$28.6}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.N\endcsname{16}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.N\endcsname{16}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.N\endcsname{1600.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.N\endcsname{$+$1600.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-F\endcsname{0.375}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-F\endcsname{37.5}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-F\endcsname{$+$37.5}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-R\endcsname{0.312}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-R\endcsname{31.2}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.mean-R\endcsname{$+$31.2}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.sd-resid\endcsname{0.747}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.sd-resid\endcsname{1}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.sd-resid\endcsname{74.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.disagree.sd-resid\endcsname{$+$74.7}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.N\endcsname{4}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.N\endcsname{400.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.N\endcsname{$+$400.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-F\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-F\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-F\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-F\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-R\endcsname{0.000}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-R\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.mean-R\endcsname{0.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.sd-resid\endcsname{0.500}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.sd-resid\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.sd-resid\endcsname{50.0}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.strata.parse-fail.sd-resid\endcsname{$+$50.0}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-source\endcsname{-0.028}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-source\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-source\endcsname{$-$2.8}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-source\endcsname{$-$2.8}
\expandafter\def\csname val@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-target\endcsname{-0.097}
\expandafter\def\csname cnt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-target\endcsname{0}
\expandafter\def\csname pct@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-target\endcsname{$-$9.7}
\expandafter\def\csname ppt@pilot.uiv.pilot-haiku-to-sonnet.per-skill.grid2-d3.V.tau-target\endcsname{$-$9.7}
\expandafter\def\csname val@plan.agree-cut\endcsname{0.020}
\expandafter\def\csname cnt@plan.agree-cut\endcsname{0}
\expandafter\def\csname pct@plan.agree-cut\endcsname{2.0}
\expandafter\def\csname ppt@plan.agree-cut\endcsname{$+$2.0}
\expandafter\def\csname val@plan.bootstrap-B\endcsname{4000}
\expandafter\def\csname cnt@plan.bootstrap-B\endcsname{4{,}000}
\expandafter\def\csname pct@plan.bootstrap-B\endcsname{400000.0}
\expandafter\def\csname ppt@plan.bootstrap-B\endcsname{$+$400000.0}
\expandafter\def\csname val@plan.drift-cut\endcsname{0.100}
\expandafter\def\csname cnt@plan.drift-cut\endcsname{0}
\expandafter\def\csname pct@plan.drift-cut\endcsname{10.0}
\expandafter\def\csname ppt@plan.drift-cut\endcsname{$+$10.0}
\expandafter\def\csname val@plan.n-catalog-skills\endcsname{4}
\expandafter\def\csname cnt@plan.n-catalog-skills\endcsname{4}
\expandafter\def\csname pct@plan.n-catalog-skills\endcsname{400.0}
\expandafter\def\csname ppt@plan.n-catalog-skills\endcsname{$+$400.0}
\expandafter\def\csname val@plan.n-histories\endcsname{20}
\expandafter\def\csname cnt@plan.n-histories\endcsname{20}
\expandafter\def\csname pct@plan.n-histories\endcsname{2000.0}
\expandafter\def\csname ppt@plan.n-histories\endcsname{$+$2000.0}
\expandafter\def\csname val@plan.n-skills\endcsname{5}
\expandafter\def\csname cnt@plan.n-skills\endcsname{5}
\expandafter\def\csname pct@plan.n-skills\endcsname{500.0}
\expandafter\def\csname ppt@plan.n-skills\endcsname{$+$500.0}
\expandafter\def\csname val@plan.primary-fraction\endcsname{0.250}
\expandafter\def\csname cnt@plan.primary-fraction\endcsname{0}
\expandafter\def\csname pct@plan.primary-fraction\endcsname{25.0}
\expandafter\def\csname ppt@plan.primary-fraction\endcsname{$+$25.0}
\expandafter\def\csname val@plan.sigma-default\endcsname{0.500}
\expandafter\def\csname cnt@plan.sigma-default\endcsname{0}
\expandafter\def\csname pct@plan.sigma-default\endcsname{50.0}
\expandafter\def\csname ppt@plan.sigma-default\endcsname{$+$50.0}
\expandafter\def\csname val@plan.sigma-floor\endcsname{0.100}
\expandafter\def\csname cnt@plan.sigma-floor\endcsname{0}
\expandafter\def\csname pct@plan.sigma-floor\endcsname{10.0}
\expandafter\def\csname ppt@plan.sigma-floor\endcsname{$+$10.0}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:haiku->sonnet.center-d1\endcsname{{'agree\_stable': 0.0, 'parse\_fail': 0.4714045207910317, 'disagree': 0.816496580927726}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:haiku->sonnet.context-d1\endcsname{{'agree\_stable': 0.19230769230769232, 'disagree': 0.4330127018922193, 'agree\_drift': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:haiku->sonnet.dual-d2\endcsname{{'agree\_stable': 0.41573970964154905, 'disagree': 0.4330127018922193, 'agree\_drift': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:haiku->sonnet.grid2-d3\endcsname{{'agree\_stable': 0.19595917942265426, 'disagree': 0.4330127018922193, 'parse\_fail': 0.4714045207910317}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:haiku->sonnet.zoomclick-d3\endcsname{{'agree\_stable': 0.0, 'disagree': 0.7453559924999299, 'agree\_drift': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:sonnet->opus.center-d1\endcsname{{'agree\_stable': 0.0, 'disagree': 0.0, 'parse\_fail': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:sonnet->opus.context-d1\endcsname{{'agree\_stable': 0.0, 'disagree': 0.0, 'agree\_drift': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:sonnet->opus.dual-d2\endcsname{{'agree\_stable': 0.18885257457751056, 'disagree': 0.0, 'agree\_drift': 0.0}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:sonnet->opus.grid2-d3\endcsname{{'agree\_stable': 0.18246560765962694, 'disagree': 0.4714045207910317}}
\expandafter\def\csname val@plan.sigma-h.main-sspro-v1:sonnet->opus.zoomclick-d3\endcsname{{'agree\_stable': 0.17950549357115014, 'disagree': 0.0}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:haiku->sonnet.center-d1\endcsname{{'agree\_stable': 0.1373351620873625, 'disagree': 0.49690399499995325, 'agree\_drift': 0.5, 'parse\_fail': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:haiku->sonnet.context-d1\endcsname{{'agree\_stable': 0.0, 'disagree': 0.458257569495584}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:haiku->sonnet.dual-d2\endcsname{{'agree\_stable': 0.20203050891044216, 'disagree': 0.6400954789890507, 'agree\_drift': 0.0}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:haiku->sonnet.grid2-d3\endcsname{{'agree\_stable': 0.21081851067789195, 'agree\_drift': 0.0, 'disagree': 0.4979295977319692, 'parse\_fail': 0.4714045207910317}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:haiku->sonnet.zoomclick-d3\endcsname{{'agree\_stable': 0.0, 'disagree': 0.7216878364870322, 'agree\_drift': 0.0}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:sonnet->opus.center-d1\endcsname{{'agree\_stable': 0.18719327529067273, 'agree\_drift': 0.0, 'disagree': 0.3499271061118826}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:sonnet->opus.context-d1\endcsname{{'agree\_stable': 0.13243211584099399, 'agree\_drift': 0.0, 'disagree': 0.4898979485566356}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:sonnet->opus.dual-d2\endcsname{{'agree\_stable': 0.13481684980149108, 'disagree': 0.4714045207910317, 'agree\_drift': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:sonnet->opus.grid2-d3\endcsname{{'agree\_stable': 0.0, 'disagree': 0.51425947722658, 'parse\_fail': 0.5}}
\expandafter\def\csname val@plan.sigma-h.main-uiv-v1:sonnet->opus.zoomclick-d3\endcsname{{'agree\_stable': 0.18719327529067273, 'agree\_drift': 0.5, 'disagree': 0.5994789404140899}}
\expandafter\def\csname val@sspro.p1.catalog.best-single@0.1.mean-over-histories\endcsname{0.836}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@0.1.mean-over-histories\endcsname{83.6}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@0.1.mean-over-histories\endcsname{$+$83.6}
\expandafter\def\csname val@sspro.p1.catalog.best-single@0.1.sd-over-histories\endcsname{0.034}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@0.1.sd-over-histories\endcsname{3.4}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@0.1.sd-over-histories\endcsname{$+$3.4}
\expandafter\def\csname val@sspro.p1.catalog.best-single@0.25.mean-over-histories\endcsname{0.853}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@0.25.mean-over-histories\endcsname{85.3}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@0.25.mean-over-histories\endcsname{$+$85.3}
\expandafter\def\csname val@sspro.p1.catalog.best-single@0.25.sd-over-histories\endcsname{0.016}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@0.25.sd-over-histories\endcsname{1.6}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@0.25.sd-over-histories\endcsname{$+$1.6}
\expandafter\def\csname val@sspro.p1.catalog.best-single@0.5.mean-over-histories\endcsname{0.851}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@0.5.mean-over-histories\endcsname{85.1}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@0.5.mean-over-histories\endcsname{$+$85.1}
\expandafter\def\csname val@sspro.p1.catalog.best-single@0.5.sd-over-histories\endcsname{0.015}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@0.5.sd-over-histories\endcsname{1.5}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@0.5.sd-over-histories\endcsname{$+$1.5}
\expandafter\def\csname val@sspro.p1.catalog.best-single@1.0.mean-over-histories\endcsname{0.844}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@1.0.mean-over-histories\endcsname{84.4}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@1.0.mean-over-histories\endcsname{$+$84.4}
\expandafter\def\csname val@sspro.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.full-recert.score\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.full-recert.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.full-recert.score\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.full-recert.score\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{0.849}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{84.9}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{$+$84.9}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0.017}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{1.7}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{$+$1.7}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{0.852}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{85.2}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{$+$85.2}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0.014}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{1.4}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{$+$1.4}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.keep-all.score\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.keep-all.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.keep-all.score\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.keep-all.score\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.old-decision.score\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.old-decision.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.old-decision.score\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.old-decision.score\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.oracle-on-T.score\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.oracle-on-T.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.oracle-on-T.score\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.oracle-on-T.score\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{0.740}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{74.0}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{$+$74.0}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{0.858}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{85.8}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{$+$85.8}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0.008}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0.8}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{$+$0.8}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.replay-only.score\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-only.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.replay-only.score\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-only.score\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{0.847}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{84.7}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{$+$84.7}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0.018}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{1.8}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{$+$1.8}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{0.849}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{84.9}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{$+$84.9}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0.016}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{1.6}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{$+$1.6}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.suspend-all.score\endcsname{0.740}
\expandafter\def\csname cnt@sspro.p1.catalog.suspend-all.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.suspend-all.score\endcsname{74.0}
\expandafter\def\csname ppt@sspro.p1.catalog.suspend-all.score\endcsname{$+$74.0}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{0.848}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{84.8}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{$+$84.8}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0.029}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{2.9}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{$+$2.9}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0.022}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{2.2}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{$+$2.2}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{-0.018}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$1.8}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$1.8}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{0.030}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{3.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{$+$3.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{-0.015}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$1.5}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$1.5}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.mean\endcsname{0.004}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.mean\endcsname{0.4}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.mean\endcsname{$+$0.4}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{0.375}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{37.5}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{$+$37.5}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0.117}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{11.7}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{$+$11.7}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{-0.004}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$-$0.4}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$-$0.4}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{-0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{-0.003}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{-0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$-$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{0.981}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{98.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{$+$98.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.001}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{$+$0.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0.013}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{1.3}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{$+$1.3}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0.006}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0.6}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{$+$0.6}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.004}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.4}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{$+$0.4}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{-0.004}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{-0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{-0.003}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.mean\endcsname{-0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.mean\endcsname{$-$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{0.981}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{98.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{$+$98.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{-0.004}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{-0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{-0.003}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.mean\endcsname{-0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.mean\endcsname{$-$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{0.981}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{98.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{$+$98.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.001}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{$+$0.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0.018}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{1.8}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{$+$1.8}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.009}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.9}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{$+$0.9}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0.014}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{1.4}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{$+$1.4}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{0.018}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{1.8}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{$+$1.8}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0.238}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{23.8}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{$+$23.8}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{0.031}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{3.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{$+$3.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{0.118}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{11.8}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{$+$11.8}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0.006}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0.6}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{$+$0.6}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0.001}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0.1}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{$+$0.1}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0.015}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{1.5}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{$+$1.5}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.007}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.7}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{$+$0.7}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{61.688}
\expandafter\def\csname cnt@sspro.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{62}
\expandafter\def\csname pct@sspro.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{6168.8}
\expandafter\def\csname ppt@sspro.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{$+$6168.8}
\expandafter\def\csname val@sspro.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{80.900}
\expandafter\def\csname cnt@sspro.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{81}
\expandafter\def\csname pct@sspro.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{8090.0}
\expandafter\def\csname ppt@sspro.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{$+$8090.0}
\expandafter\def\csname val@sspro.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{113.750}
\expandafter\def\csname cnt@sspro.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{114}
\expandafter\def\csname pct@sspro.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{11375.0}
\expandafter\def\csname ppt@sspro.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{$+$11375.0}
\expandafter\def\csname val@sspro.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{180}
\expandafter\def\csname pct@sspro.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.cost.full-recert.mean-requests-per-skill\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.cost.full-recert.mean-requests-per-skill\endcsname{180}
\expandafter\def\csname pct@sspro.p1.cost.full-recert.mean-requests-per-skill\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.cost.full-recert.mean-requests-per-skill\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{61.688}
\expandafter\def\csname cnt@sspro.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{62}
\expandafter\def\csname pct@sspro.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{6168.8}
\expandafter\def\csname ppt@sspro.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{$+$6168.8}
\expandafter\def\csname val@sspro.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{80.900}
\expandafter\def\csname cnt@sspro.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{81}
\expandafter\def\csname pct@sspro.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{8090.0}
\expandafter\def\csname ppt@sspro.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{$+$8090.0}
\expandafter\def\csname val@sspro.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{113.750}
\expandafter\def\csname cnt@sspro.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{114}
\expandafter\def\csname pct@sspro.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{11375.0}
\expandafter\def\csname ppt@sspro.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{$+$11375.0}
\expandafter\def\csname val@sspro.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{180}
\expandafter\def\csname pct@sspro.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{1}
\expandafter\def\csname pct@sspro.p1.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{96}
\expandafter\def\csname pct@sspro.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{128.887}
\expandafter\def\csname cnt@sspro.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{129}
\expandafter\def\csname pct@sspro.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{12888.7}
\expandafter\def\csname ppt@sspro.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{$+$12888.7}
\expandafter\def\csname val@sspro.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{161.750}
\expandafter\def\csname cnt@sspro.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{162}
\expandafter\def\csname pct@sspro.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{16175.0}
\expandafter\def\csname ppt@sspro.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{$+$16175.0}
\expandafter\def\csname val@sspro.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{227.500}
\expandafter\def\csname cnt@sspro.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{228}
\expandafter\def\csname pct@sspro.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{22750.0}
\expandafter\def\csname ppt@sspro.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{$+$22750.0}
\expandafter\def\csname val@sspro.p1.cost.replay-only.mean-requests-per-skill\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p1.cost.replay-only.mean-requests-per-skill\endcsname{96}
\expandafter\def\csname pct@sspro.p1.cost.replay-only.mean-requests-per-skill\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.cost.replay-only.mean-requests-per-skill\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{109.688}
\expandafter\def\csname cnt@sspro.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{110}
\expandafter\def\csname pct@sspro.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{10968.8}
\expandafter\def\csname ppt@sspro.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{$+$10968.8}
\expandafter\def\csname val@sspro.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{128.900}
\expandafter\def\csname cnt@sspro.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{129}
\expandafter\def\csname pct@sspro.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{12890.0}
\expandafter\def\csname ppt@sspro.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{$+$12890.0}
\expandafter\def\csname val@sspro.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{161.750}
\expandafter\def\csname cnt@sspro.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{162}
\expandafter\def\csname pct@sspro.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{16175.0}
\expandafter\def\csname ppt@sspro.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{$+$16175.0}
\expandafter\def\csname val@sspro.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{227.500}
\expandafter\def\csname cnt@sspro.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{228}
\expandafter\def\csname pct@sspro.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{22750.0}
\expandafter\def\csname ppt@sspro.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{$+$22750.0}
\expandafter\def\csname val@sspro.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{61.688}
\expandafter\def\csname cnt@sspro.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{62}
\expandafter\def\csname pct@sspro.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{6168.8}
\expandafter\def\csname ppt@sspro.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{$+$6168.8}
\expandafter\def\csname val@sspro.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{80.900}
\expandafter\def\csname cnt@sspro.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{81}
\expandafter\def\csname pct@sspro.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{8090.0}
\expandafter\def\csname ppt@sspro.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{$+$8090.0}
\expandafter\def\csname val@sspro.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{113.750}
\expandafter\def\csname cnt@sspro.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{114}
\expandafter\def\csname pct@sspro.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{11375.0}
\expandafter\def\csname ppt@sspro.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{$+$11375.0}
\expandafter\def\csname val@sspro.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{180}
\expandafter\def\csname pct@sspro.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.1.center-d1\endcsname{0.750}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.1.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.1.center-d1\endcsname{75.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.1.center-d1\endcsname{$+$75.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.1.direct\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.1.direct\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.1.direct\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.1.direct\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.1.dual-d2\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.1.dual-d2\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.1.dual-d2\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.1.dual-d2\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.1.grid2-d3\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.1.grid2-d3\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.1.grid2-d3\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.1.grid2-d3\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.25.center-d1\endcsname{0.700}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.25.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.25.center-d1\endcsname{70.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.25.center-d1\endcsname{$+$70.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.25.dual-d2\endcsname{0.200}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.25.dual-d2\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.25.dual-d2\endcsname{20.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.25.dual-d2\endcsname{$+$20.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.25.grid2-d3\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.25.grid2-d3\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.25.grid2-d3\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.25.grid2-d3\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.5.center-d1\endcsname{0.800}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.5.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.5.center-d1\endcsname{80.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.5.center-d1\endcsname{$+$80.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.5.dual-d2\endcsname{0.150}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.5.dual-d2\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.5.dual-d2\endcsname{15.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.5.dual-d2\endcsname{$+$15.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@0.5.grid2-d3\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@0.5.grid2-d3\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.best-single@0.5.grid2-d3\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@0.5.grid2-d3\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p1.decide.best-single@1.0.center-d1\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.best-single@1.0.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.best-single@1.0.center-d1\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.best-single@1.0.center-d1\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.153}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{15.3}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$15.3}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.134}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{13.4}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$13.4}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{10600.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$10600.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.185}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{18.5}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$18.5}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.128}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{12.8}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$12.8}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.130}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{13.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$13.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.203}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{20.3}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$20.3}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.163}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{16.2}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$16.2}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.086}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{8.6}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$8.6}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.188}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{18.8}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$18.8}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.087}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{8.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$8.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.183}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{18.3}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$18.3}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.158}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{15.8}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$15.8}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.120}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{12.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$12.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.183}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{18.3}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$18.3}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.035}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{3.5}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$3.5}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.174}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{17.4}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$17.4}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.028}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.8}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.8}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.177}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{17.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$17.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.022}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.2}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.2}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.169}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{16.9}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$16.9}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.cost.full-recert-fresh\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.cost.full-recert-fresh\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget-tau.old-source\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.no-budget-tau.old-source\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.no-budget-tau.old-source\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.center-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p1.decide.center-d1.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.sigma-used.disagree\endcsname{0.816}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.sigma-used.disagree\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.sigma-used.disagree\endcsname{81.6}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.sigma-used.disagree\endcsname{$+$81.6}
\expandafter\def\csname val@sspro.p1.decide.center-d1.sigma-used.parse-fail\endcsname{0.471}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.sigma-used.parse-fail\endcsname{47.1}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.sigma-used.parse-fail\endcsname{$+$47.1}
\expandafter\def\csname val@sspro.p1.decide.center-d1.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.strata-N.agree-drift\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.strata-N.agree-drift\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.strata-N.agree-stable\endcsname{38}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.strata-N.agree-stable\endcsname{38}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.strata-N.agree-stable\endcsname{3800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.strata-N.agree-stable\endcsname{$+$3800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.strata-N.disagree\endcsname{8}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.strata-N.disagree\endcsname{8}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.strata-N.disagree\endcsname{800.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.strata-N.disagree\endcsname{$+$800.0}
\expandafter\def\csname val@sspro.p1.decide.center-d1.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname cnt@sspro.p1.decide.center-d1.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.center-d1.strata-N.parse-fail\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.center-d1.strata-N.parse-fail\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.143}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{14.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$14.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.143}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{14.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$14.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{10600.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$10600.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.135}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{13.5}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$13.5}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.099}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{9.9}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$9.9}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.070}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{7.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$7.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.203}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{20.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$20.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.121}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{12.1}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$12.1}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.077}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{7.7}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$7.7}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.097}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{9.7}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$9.7}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.037}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{3.7}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$3.7}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.113}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{11.2}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$11.2}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.048}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{4.8}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.8}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.083}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{8.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$8.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.109}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{10.9}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$10.9}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.102}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.043}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.108}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{10.8}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.8}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.033}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{3.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.106}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{10.6}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$10.6}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.cost.full-recert-fresh\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.cost.full-recert-fresh\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget-tau.old-source\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.no-budget-tau.old-source\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.no-budget-tau.old-source\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.context-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p1.decide.context-d1.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.sigma-used.agree-stable\endcsname{0.192}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.sigma-used.agree-stable\endcsname{19.2}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.sigma-used.agree-stable\endcsname{$+$19.2}
\expandafter\def\csname val@sspro.p1.decide.context-d1.sigma-used.disagree\endcsname{0.433}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.sigma-used.disagree\endcsname{43.3}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.sigma-used.disagree\endcsname{$+$43.3}
\expandafter\def\csname val@sspro.p1.decide.context-d1.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.strata-N.agree-drift\endcsname{5}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.strata-N.agree-drift\endcsname{5}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.strata-N.agree-drift\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.strata-N.agree-drift\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.strata-N.agree-stable\endcsname{36}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.strata-N.agree-stable\endcsname{36}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.strata-N.agree-stable\endcsname{3600.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.strata-N.agree-stable\endcsname{$+$3600.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.strata-N.disagree\endcsname{6}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.strata-N.disagree\endcsname{6}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.strata-N.disagree\endcsname{600.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.strata-N.disagree\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.p1.decide.context-d1.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname cnt@sspro.p1.decide.context-d1.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.context-d1.strata-N.parse-fail\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.context-d1.strata-N.parse-fail\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{63.100}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{6310.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$6310.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.142}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{14.2}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$14.2}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.173}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{17.3}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$17.3}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111.100}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{11110.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$11110.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.103}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.136}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{13.6}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$13.6}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{63.100}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{6310.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$6310.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.120}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{12.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$12.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.204}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{20.4}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$20.4}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{84.350}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{8435.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$8435.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.142}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{14.2}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$14.2}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.111}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{11.1}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$11.1}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{132.150}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{13215.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$13215.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.151}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{15.1}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$15.1}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.121}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{12.1}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$12.1}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132.350}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{13235.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$13235.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.089}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{8.9}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$8.9}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{84.350}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{8435.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$8435.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.138}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{13.8}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$13.8}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.113}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{11.3}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$11.3}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{120.550}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{121}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{12055.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$12055.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.137}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{13.7}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$13.7}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.059}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{5.9}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$5.9}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{168.300}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{16830.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$16830.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.135}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{13.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$13.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.069}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{6.9}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$6.9}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168.550}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{169}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{16855.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$16855.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.129}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{12.9}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$12.9}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.055}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{5.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$5.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{120.550}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{121}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{12055.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$12055.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.129}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{12.9}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$12.9}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.059}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{5.9}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$5.9}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{193.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{193}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{19300.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$19300.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{241.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{241}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{24100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$24100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{241.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{241}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{24100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$24100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{193.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{193}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{19300.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$19300.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{145}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{145}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{14500.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{$+$14500.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{0.416}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{41.6}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{$+$41.6}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.sigma-used.disagree\endcsname{0.433}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.sigma-used.disagree\endcsname{43.3}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.sigma-used.disagree\endcsname{$+$43.3}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.strata-N.agree-drift\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.strata-N.agree-drift\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.strata-N.agree-stable\endcsname{37}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.strata-N.agree-stable\endcsname{37}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.strata-N.agree-stable\endcsname{3700.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.strata-N.agree-stable\endcsname{$+$3700.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.strata-N.disagree\endcsname{8}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.strata-N.disagree\endcsname{8}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.strata-N.disagree\endcsname{800.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.strata-N.disagree\endcsname{$+$800.0}
\expandafter\def\csname val@sspro.p1.decide.dual-d2.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname cnt@sspro.p1.decide.dual-d2.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname pct@sspro.p1.decide.dual-d2.strata-N.parse-fail\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p1.decide.dual-d2.strata-N.parse-fail\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{67.650}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{68}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{6765.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$6765.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.155}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{15.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$15.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.145}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{14.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$14.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{115.650}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{116}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{11565.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$11565.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.155}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{15.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$15.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.145}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{14.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$14.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{67.650}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{68}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{6765.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$6765.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.110}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{11.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$11.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.205}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{20.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$20.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{95.250}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{95}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{9525.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$9525.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.129}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{12.9}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$12.9}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.072}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{7.2}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$7.2}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{143.400}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{143}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{14340.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$14340.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.138}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{13.8}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$13.8}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.073}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{7.3}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$7.3}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{143.250}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{143}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{14325.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$14325.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.129}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{12.9}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$12.9}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.072}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{7.2}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$7.2}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{95.250}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{95}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{9525.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$9525.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.121}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{12.1}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$12.1}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.141}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{14.1}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$14.1}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{142.450}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{142}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{14245.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$14245.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{190.700}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{191}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{19070.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$19070.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.140}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{14.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$14.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{190.450}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{190}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{19045.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$19045.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{142.450}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{142}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{14245.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$14245.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.148}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{14.8}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$14.8}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.074}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{7.4}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$7.4}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{237.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{237}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{23700.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$23700.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{285.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{285}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{28500.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$28500.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{285.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{285}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{28500.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$28500.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{237.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{237}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{23700.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$23700.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{189}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{189}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{18900.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{$+$18900.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{0.196}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{19.6}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{$+$19.6}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.sigma-used.disagree\endcsname{0.433}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.sigma-used.disagree\endcsname{43.3}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.sigma-used.disagree\endcsname{$+$43.3}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{0.471}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{47.1}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{$+$47.1}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{35}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{35}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{3500.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{$+$3500.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.strata-N.disagree\endcsname{11}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.strata-N.disagree\endcsname{11}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.strata-N.disagree\endcsname{1100.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.strata-N.disagree\endcsname{$+$1100.0}
\expandafter\def\csname val@sspro.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname cnt@sspro.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname pct@sspro.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{63.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{6300.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$6300.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.187}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{18.7}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$18.7}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{11100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$11100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.187}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{18.7}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$18.7}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{63.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{6300.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$6300.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.160}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{16.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$16.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.215}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{21.5}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$21.5}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{84.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{8400.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$8400.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.196}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{19.6}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$19.6}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.040}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{4.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$4.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{132.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{13200.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$13200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{13200.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$13200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.196}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{19.6}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$19.6}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.040}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{4.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{84.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{8400.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$8400.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.188}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{18.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$18.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.120}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{12.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$12.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.204}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{20.4}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$20.4}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.022}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{2.2}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$2.2}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.204}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{20.4}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$20.4}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.022}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.2}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.2}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.068}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{6.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$6.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{144}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{144}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{0.250}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{25.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{$+$25.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{0.745}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{74.5}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{$+$74.5}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{2}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{2}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{38}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{38}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{3800.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{$+$3800.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{7}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{7}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{700.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{$+$700.0}
\expandafter\def\csname val@sspro.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname cnt@sspro.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname pct@sspro.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.bracket-costs.0\endcsname{113.750}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.bracket-costs.0\endcsname{114}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.bracket-costs.0\endcsname{11375.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.bracket-costs.0\endcsname{$+$11375.0}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.bracket-costs.1\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.bracket-costs.1\endcsname{180}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.bracket-costs.1\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.bracket-costs.1\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{-0.022}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$2.2}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$2.2}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{-0.018}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$1.8}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$1.8}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.mean\endcsname{0.009}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.mean\endcsname{0.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.mean\endcsname{$+$0.9}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{0.332}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{33.2}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{$+$33.2}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.135}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{13.5}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{$+$13.5}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{0.849}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{84.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{$+$84.9}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.status\endcsname{ok}
\expandafter\def\csname val@sspro.p1.equal-cost.best-single.weight\endcsname{0.230}
\expandafter\def\csname cnt@sspro.p1.equal-cost.best-single.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.best-single.weight\endcsname{23.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.best-single.weight\endcsname{$+$23.0}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{113.750}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{114}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{11375.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{$+$11375.0}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{180}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{-0.004}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{-0.000}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{-0.003}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{-0.002}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{$-$0.2}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0.981}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{98.1}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{$+$98.1}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.status\endcsname{ok}
\expandafter\def\csname val@sspro.p1.equal-cost.generic-ppi-source.weight\endcsname{0.230}
\expandafter\def\csname cnt@sspro.p1.equal-cost.generic-ppi-source.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.generic-ppi-source.weight\endcsname{23.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.generic-ppi-source.weight\endcsname{$+$23.0}
\expandafter\def\csname val@sspro.p1.equal-cost.rcr-cost\endcsname{128.887}
\expandafter\def\csname cnt@sspro.p1.equal-cost.rcr-cost\endcsname{129}
\expandafter\def\csname pct@sspro.p1.equal-cost.rcr-cost\endcsname{12888.7}
\expandafter\def\csname ppt@sspro.p1.equal-cost.rcr-cost\endcsname{$+$12888.7}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{109.688}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{110}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{10968.8}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{$+$10968.8}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{128.900}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{129}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{12890.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{$+$12890.0}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.001}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.1}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{$+$0.1}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0.018}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{1.8}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{$+$1.8}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.009}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{$+$0.9}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0.014}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{1.4}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{$+$1.4}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{0.849}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{84.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{$+$84.9}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.status\endcsname{ok}
\expandafter\def\csname val@sspro.p1.equal-cost.replay-ppi-uniform.weight\endcsname{0.999}
\expandafter\def\csname cnt@sspro.p1.equal-cost.replay-ppi-uniform.weight\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.replay-ppi-uniform.weight\endcsname{99.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.replay-ppi-uniform.weight\endcsname{$+$99.9}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{113.750}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{114}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{11375.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{$+$11375.0}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{179.500}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{180}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{17950.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{$+$17950.0}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{-0.004}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{-0.000}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{-0.003}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{-0.002}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{$-$0.2}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{0.981}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{98.1}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{$+$98.1}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{0.859}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{85.9}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{$+$85.9}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.status\endcsname{ok}
\expandafter\def\csname val@sspro.p1.equal-cost.uniform-fresh.weight\endcsname{0.230}
\expandafter\def\csname cnt@sspro.p1.equal-cost.uniform-fresh.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p1.equal-cost.uniform-fresh.weight\endcsname{23.0}
\expandafter\def\csname ppt@sspro.p1.equal-cost.uniform-fresh.weight\endcsname{$+$23.0}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.acc-macro\endcsname{0.844}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.acc-macro\endcsname{84.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.acc-macro\endcsname{$+$84.4}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.mean-requests\endcsname{2.000}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.mean-requests\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.mean-requests\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.n\endcsname{96}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0.219}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{21.9}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{$+$21.9}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.004}
\expandafter\def\csname cnt@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$0.4}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.acc-macro\endcsname{0.854}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.acc-macro\endcsname{85.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.acc-macro\endcsname{$+$85.4}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.mean-requests\endcsname{2.000}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.mean-requests\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.mean-requests\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.n\endcsname{96}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0.260}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{26.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{$+$26.0}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{0.031}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{3.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{$+$3.1}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0.115}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{11.5}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{$+$11.5}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.011}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{1.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{$+$1.1}
\expandafter\def\csname val@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.004}
\expandafter\def\csname cnt@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$0.4}
\expandafter\def\csname val@sspro.p1.execution-layer.direct\endcsname{0.740}
\expandafter\def\csname cnt@sspro.p1.execution-layer.direct\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.direct\endcsname{74.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.direct\endcsname{$+$74.0}
\expandafter\def\csname val@sspro.p1.execution-layer.direct-sc3\endcsname{0.729}
\expandafter\def\csname cnt@sspro.p1.execution-layer.direct-sc3\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.direct-sc3\endcsname{72.9}
\expandafter\def\csname ppt@sspro.p1.execution-layer.direct-sc3\endcsname{$+$72.9}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.acc-macro\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.acc-macro\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.acc-macro\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.mean-requests\endcsname{3.021}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.mean-requests\endcsname{3}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.mean-requests\endcsname{302.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.mean-requests\endcsname{$+$302.1}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.n\endcsname{96}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{0.302}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{30.2}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{$+$30.2}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{0.031}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{3.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{$+$3.1}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0.020}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{2.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{$+$2.0}
\expandafter\def\csname val@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.013}
\expandafter\def\csname cnt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1.3}
\expandafter\def\csname ppt@sspro.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$1.3}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.acc-macro\endcsname{0.854}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.acc-macro\endcsname{85.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.acc-macro\endcsname{$+$85.4}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.mean-requests\endcsname{3.844}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.mean-requests\endcsname{4}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.mean-requests\endcsname{384.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.mean-requests\endcsname{$+$384.4}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.n\endcsname{96}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{0.115}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{11.5}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{$+$11.5}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.025}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{2.5}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{$+$2.5}
\expandafter\def\csname val@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.015}
\expandafter\def\csname cnt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1.5}
\expandafter\def\csname ppt@sspro.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$1.5}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{0.917}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{91.7}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{$+$91.7}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{2.979}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{3}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{297.9}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{$+$297.9}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{0.094}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{9.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{$+$9.4}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0.292}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{29.2}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{$+$29.2}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{0.177}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{17.7}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{$+$17.7}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{0.007}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{0.7}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{$+$0.7}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{0.004}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{0.4}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{$+$0.4}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.006}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.6}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{$+$0.6}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname cnt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname pct@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname val@sspro.p1.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p1.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p1.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p1.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p1.n-cal-apps\endcsname{6}
\expandafter\def\csname cnt@sspro.p1.n-cal-apps\endcsname{6}
\expandafter\def\csname pct@sspro.p1.n-cal-apps\endcsname{600.0}
\expandafter\def\csname ppt@sspro.p1.n-cal-apps\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.p1.n-test\endcsname{96}
\expandafter\def\csname cnt@sspro.p1.n-test\endcsname{96}
\expandafter\def\csname pct@sspro.p1.n-test\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p1.n-test\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p1.n-test-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p1.n-test-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p1.n-test-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p1.n-test-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p1.primary.best-single.cost\endcsname{80.900}
\expandafter\def\csname cnt@sspro.p1.primary.best-single.cost\endcsname{81}
\expandafter\def\csname pct@sspro.p1.primary.best-single.cost\endcsname{8090.0}
\expandafter\def\csname ppt@sspro.p1.primary.best-single.cost\endcsname{$+$8090.0}
\expandafter\def\csname val@sspro.p1.primary.best-single.cost-fraction-of-full\endcsname{0.451}
\expandafter\def\csname cnt@sspro.p1.primary.best-single.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.best-single.cost-fraction-of-full\endcsname{45.1}
\expandafter\def\csname ppt@sspro.p1.primary.best-single.cost-fraction-of-full\endcsname{$+$45.1}
\expandafter\def\csname val@sspro.p1.primary.best-single.score\endcsname{0.853}
\expandafter\def\csname cnt@sspro.p1.primary.best-single.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.best-single.score\endcsname{85.3}
\expandafter\def\csname ppt@sspro.p1.primary.best-single.score\endcsname{$+$85.3}
\expandafter\def\csname val@sspro.p1.primary.best-single.vs-full-recert\endcsname{-0.006}
\expandafter\def\csname cnt@sspro.p1.primary.best-single.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.best-single.vs-full-recert\endcsname{$-$0.6}
\expandafter\def\csname ppt@sspro.p1.primary.best-single.vs-full-recert\endcsname{$-$0.6}
\expandafter\def\csname val@sspro.p1.primary.best-single.vs-suspend-all\endcsname{0.114}
\expandafter\def\csname cnt@sspro.p1.primary.best-single.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.best-single.vs-suspend-all\endcsname{11.4}
\expandafter\def\csname ppt@sspro.p1.primary.best-single.vs-suspend-all\endcsname{$+$11.4}
\expandafter\def\csname val@sspro.p1.primary.generic-ppi-source.cost\endcsname{80.900}
\expandafter\def\csname cnt@sspro.p1.primary.generic-ppi-source.cost\endcsname{81}
\expandafter\def\csname pct@sspro.p1.primary.generic-ppi-source.cost\endcsname{8090.0}
\expandafter\def\csname ppt@sspro.p1.primary.generic-ppi-source.cost\endcsname{$+$8090.0}
\expandafter\def\csname val@sspro.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0.451}
\expandafter\def\csname cnt@sspro.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{45.1}
\expandafter\def\csname ppt@sspro.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{$+$45.1}
\expandafter\def\csname val@sspro.p1.primary.generic-ppi-source.score\endcsname{0.852}
\expandafter\def\csname cnt@sspro.p1.primary.generic-ppi-source.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.generic-ppi-source.score\endcsname{85.2}
\expandafter\def\csname ppt@sspro.p1.primary.generic-ppi-source.score\endcsname{$+$85.2}
\expandafter\def\csname val@sspro.p1.primary.generic-ppi-source.vs-full-recert\endcsname{-0.008}
\expandafter\def\csname cnt@sspro.p1.primary.generic-ppi-source.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.generic-ppi-source.vs-full-recert\endcsname{$-$0.8}
\expandafter\def\csname ppt@sspro.p1.primary.generic-ppi-source.vs-full-recert\endcsname{$-$0.8}
\expandafter\def\csname val@sspro.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{0.112}
\expandafter\def\csname cnt@sspro.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{11.2}
\expandafter\def\csname ppt@sspro.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{$+$11.2}
\expandafter\def\csname val@sspro.p1.primary.rcr-stratified.cost\endcsname{128.887}
\expandafter\def\csname cnt@sspro.p1.primary.rcr-stratified.cost\endcsname{129}
\expandafter\def\csname pct@sspro.p1.primary.rcr-stratified.cost\endcsname{12888.7}
\expandafter\def\csname ppt@sspro.p1.primary.rcr-stratified.cost\endcsname{$+$12888.7}
\expandafter\def\csname val@sspro.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{0.718}
\expandafter\def\csname cnt@sspro.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{71.8}
\expandafter\def\csname ppt@sspro.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{$+$71.8}
\expandafter\def\csname val@sspro.p1.primary.rcr-stratified.score\endcsname{0.858}
\expandafter\def\csname cnt@sspro.p1.primary.rcr-stratified.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.rcr-stratified.score\endcsname{85.8}
\expandafter\def\csname ppt@sspro.p1.primary.rcr-stratified.score\endcsname{$+$85.8}
\expandafter\def\csname val@sspro.p1.primary.rcr-stratified.vs-full-recert\endcsname{-0.002}
\expandafter\def\csname cnt@sspro.p1.primary.rcr-stratified.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.rcr-stratified.vs-full-recert\endcsname{$-$0.2}
\expandafter\def\csname ppt@sspro.p1.primary.rcr-stratified.vs-full-recert\endcsname{$-$0.2}
\expandafter\def\csname val@sspro.p1.primary.rcr-stratified.vs-suspend-all\endcsname{0.118}
\expandafter\def\csname cnt@sspro.p1.primary.rcr-stratified.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.rcr-stratified.vs-suspend-all\endcsname{11.8}
\expandafter\def\csname ppt@sspro.p1.primary.rcr-stratified.vs-suspend-all\endcsname{$+$11.8}
\expandafter\def\csname val@sspro.p1.primary.replay-ppi-uniform.cost\endcsname{128.900}
\expandafter\def\csname cnt@sspro.p1.primary.replay-ppi-uniform.cost\endcsname{129}
\expandafter\def\csname pct@sspro.p1.primary.replay-ppi-uniform.cost\endcsname{12890.0}
\expandafter\def\csname ppt@sspro.p1.primary.replay-ppi-uniform.cost\endcsname{$+$12890.0}
\expandafter\def\csname val@sspro.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{0.718}
\expandafter\def\csname cnt@sspro.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{71.8}
\expandafter\def\csname ppt@sspro.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{$+$71.8}
\expandafter\def\csname val@sspro.p1.primary.replay-ppi-uniform.score\endcsname{0.849}
\expandafter\def\csname cnt@sspro.p1.primary.replay-ppi-uniform.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.replay-ppi-uniform.score\endcsname{84.9}
\expandafter\def\csname ppt@sspro.p1.primary.replay-ppi-uniform.score\endcsname{$+$84.9}
\expandafter\def\csname val@sspro.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{-0.011}
\expandafter\def\csname cnt@sspro.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{$-$1.1}
\expandafter\def\csname ppt@sspro.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{$-$1.1}
\expandafter\def\csname val@sspro.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{0.109}
\expandafter\def\csname cnt@sspro.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{10.9}
\expandafter\def\csname ppt@sspro.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{$+$10.9}
\expandafter\def\csname val@sspro.p1.primary.uniform-fresh.cost\endcsname{80.900}
\expandafter\def\csname cnt@sspro.p1.primary.uniform-fresh.cost\endcsname{81}
\expandafter\def\csname pct@sspro.p1.primary.uniform-fresh.cost\endcsname{8090.0}
\expandafter\def\csname ppt@sspro.p1.primary.uniform-fresh.cost\endcsname{$+$8090.0}
\expandafter\def\csname val@sspro.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{0.451}
\expandafter\def\csname cnt@sspro.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{45.1}
\expandafter\def\csname ppt@sspro.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{$+$45.1}
\expandafter\def\csname val@sspro.p1.primary.uniform-fresh.score\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p1.primary.uniform-fresh.score\endcsname{1}
\expandafter\def\csname pct@sspro.p1.primary.uniform-fresh.score\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p1.primary.uniform-fresh.score\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p1.primary.uniform-fresh.vs-full-recert\endcsname{-0.009}
\expandafter\def\csname cnt@sspro.p1.primary.uniform-fresh.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.uniform-fresh.vs-full-recert\endcsname{$-$0.9}
\expandafter\def\csname ppt@sspro.p1.primary.uniform-fresh.vs-full-recert\endcsname{$-$0.9}
\expandafter\def\csname val@sspro.p1.primary.uniform-fresh.vs-suspend-all\endcsname{0.111}
\expandafter\def\csname cnt@sspro.p1.primary.uniform-fresh.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p1.primary.uniform-fresh.vs-suspend-all\endcsname{11.1}
\expandafter\def\csname ppt@sspro.p1.primary.uniform-fresh.vs-suspend-all\endcsname{$+$11.1}
\expandafter\def\csname val@sspro.p2.catalog.best-single@0.1.mean-over-histories\endcsname{0.908}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@0.1.mean-over-histories\endcsname{90.8}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@0.1.mean-over-histories\endcsname{$+$90.8}
\expandafter\def\csname val@sspro.p2.catalog.best-single@0.1.sd-over-histories\endcsname{0.034}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@0.1.sd-over-histories\endcsname{3.4}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@0.1.sd-over-histories\endcsname{$+$3.4}
\expandafter\def\csname val@sspro.p2.catalog.best-single@0.25.mean-over-histories\endcsname{0.913}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@0.25.mean-over-histories\endcsname{91.3}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@0.25.mean-over-histories\endcsname{$+$91.3}
\expandafter\def\csname val@sspro.p2.catalog.best-single@0.25.sd-over-histories\endcsname{0.008}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@0.25.sd-over-histories\endcsname{0.8}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@0.25.sd-over-histories\endcsname{$+$0.8}
\expandafter\def\csname val@sspro.p2.catalog.best-single@0.5.mean-over-histories\endcsname{0.907}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@0.5.mean-over-histories\endcsname{90.7}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@0.5.mean-over-histories\endcsname{$+$90.7}
\expandafter\def\csname val@sspro.p2.catalog.best-single@0.5.sd-over-histories\endcsname{0.013}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@0.5.sd-over-histories\endcsname{1.3}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@0.5.sd-over-histories\endcsname{$+$1.3}
\expandafter\def\csname val@sspro.p2.catalog.best-single@1.0.mean-over-histories\endcsname{0.917}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@1.0.mean-over-histories\endcsname{91.7}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@1.0.mean-over-histories\endcsname{$+$91.7}
\expandafter\def\csname val@sspro.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.catalog.full-recert.score\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.full-recert.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.full-recert.score\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.full-recert.score\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{0.895}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{89.5}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{$+$89.5}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0.018}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{1.8}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{$+$1.8}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0.019}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{1.9}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{$+$1.9}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{0.898}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{89.8}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{$+$89.8}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.016}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{1.6}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{$+$1.6}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.catalog.keep-all.score\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.keep-all.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.keep-all.score\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.keep-all.score\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.old-decision.score\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.old-decision.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.old-decision.score\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.old-decision.score\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.oracle-on-T.score\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.oracle-on-T.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.oracle-on-T.score\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.oracle-on-T.score\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{0.856}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{85.6}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{$+$85.6}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.019}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{1.9}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{$+$1.9}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{0.895}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{89.5}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{$+$89.5}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0.018}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{1.8}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{$+$1.8}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{0.902}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{90.2}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{$+$90.2}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.012}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{1.2}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{$+$1.2}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.catalog.replay-only.score\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-only.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.replay-only.score\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-only.score\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{0.889}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{88.9}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{$+$88.9}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0.019}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{1.9}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{$+$1.9}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0.023}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{2.3}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{$+$2.3}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{0.896}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{89.6}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{$+$89.6}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.017}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{1.7}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{$+$1.7}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.catalog.suspend-all.score\endcsname{0.760}
\expandafter\def\csname cnt@sspro.p2.catalog.suspend-all.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.suspend-all.score\endcsname{76.0}
\expandafter\def\csname ppt@sspro.p2.catalog.suspend-all.score\endcsname{$+$76.0}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{0.895}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{89.5}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{$+$89.5}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0.020}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{2.0}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{$+$2.0}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{0.891}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{89.1}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{$+$89.1}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0.025}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{2.5}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{$+$2.5}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{0.902}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{90.2}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{$+$90.2}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.012}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{1.2}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{$+$1.2}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@sspro.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{-0.028}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{-0.009}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{$-$0.9}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{$-$0.9}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{-0.027}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$2.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$2.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.mean\endcsname{-0.018}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.mean\endcsname{$-$1.8}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.mean\endcsname{$-$1.8}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0.963}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{96.3}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{$+$96.3}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{-0.017}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$-$1.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$-$1.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{-0.016}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$-$1.6}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$-$1.6}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{-0.011}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$-$1.1}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$-$1.1}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.703}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{70.3}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{$+$70.3}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.005}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.5}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{$+$0.5}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.006}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.6}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{$+$0.6}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{-0.017}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{-0.016}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$-$1.6}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$-$1.6}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.mean\endcsname{-0.011}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.mean\endcsname{$-$1.1}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.mean\endcsname{$-$1.1}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.703}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{70.3}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{$+$70.3}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{-0.017}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$1.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{-0.016}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$1.6}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$1.6}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.mean\endcsname{-0.011}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.mean\endcsname{$-$1.1}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.mean\endcsname{$-$1.1}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0.703}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{70.3}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{$+$70.3}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.005}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.5}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{$+$0.5}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.006}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.6}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{$+$0.6}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{0.072}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{7.2}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{$+$7.2}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0.209}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{20.9}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{$+$20.9}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{0.081}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{8.1}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{$+$8.1}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{0.134}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{13.4}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{$+$13.4}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0.005}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0.5}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{$+$0.5}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.002}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.2}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{$+$0.2}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.004}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.4}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{$+$0.4}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{61.650}
\expandafter\def\csname cnt@sspro.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{62}
\expandafter\def\csname pct@sspro.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{6165.0}
\expandafter\def\csname ppt@sspro.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{$+$6165.0}
\expandafter\def\csname val@sspro.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{80.787}
\expandafter\def\csname cnt@sspro.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{81}
\expandafter\def\csname pct@sspro.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{8078.7}
\expandafter\def\csname ppt@sspro.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{$+$8078.7}
\expandafter\def\csname val@sspro.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{113.588}
\expandafter\def\csname cnt@sspro.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{114}
\expandafter\def\csname pct@sspro.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{11358.8}
\expandafter\def\csname ppt@sspro.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{$+$11358.8}
\expandafter\def\csname val@sspro.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{179}
\expandafter\def\csname pct@sspro.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.cost.full-recert.mean-requests-per-skill\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.cost.full-recert.mean-requests-per-skill\endcsname{179}
\expandafter\def\csname pct@sspro.p2.cost.full-recert.mean-requests-per-skill\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.cost.full-recert.mean-requests-per-skill\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{61.650}
\expandafter\def\csname cnt@sspro.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{62}
\expandafter\def\csname pct@sspro.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{6165.0}
\expandafter\def\csname ppt@sspro.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{$+$6165.0}
\expandafter\def\csname val@sspro.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{80.787}
\expandafter\def\csname cnt@sspro.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{81}
\expandafter\def\csname pct@sspro.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{8078.7}
\expandafter\def\csname ppt@sspro.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{$+$8078.7}
\expandafter\def\csname val@sspro.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{113.588}
\expandafter\def\csname cnt@sspro.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{114}
\expandafter\def\csname pct@sspro.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{11358.8}
\expandafter\def\csname ppt@sspro.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{$+$11358.8}
\expandafter\def\csname val@sspro.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{179}
\expandafter\def\csname pct@sspro.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{1}
\expandafter\def\csname pct@sspro.p2.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.cost.rcr-infeasible-histories@0.1.mean-requests-per-skill\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{104.750}
\expandafter\def\csname cnt@sspro.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{105}
\expandafter\def\csname pct@sspro.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{10475.0}
\expandafter\def\csname ppt@sspro.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{$+$10475.0}
\expandafter\def\csname val@sspro.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{128.900}
\expandafter\def\csname cnt@sspro.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{129}
\expandafter\def\csname pct@sspro.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{12890.0}
\expandafter\def\csname ppt@sspro.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{$+$12890.0}
\expandafter\def\csname val@sspro.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{161.725}
\expandafter\def\csname cnt@sspro.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{162}
\expandafter\def\csname pct@sspro.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{16172.5}
\expandafter\def\csname ppt@sspro.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{$+$16172.5}
\expandafter\def\csname val@sspro.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{227.000}
\expandafter\def\csname cnt@sspro.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{227}
\expandafter\def\csname pct@sspro.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{22700.0}
\expandafter\def\csname ppt@sspro.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{$+$22700.0}
\expandafter\def\csname val@sspro.p2.cost.replay-only.mean-requests-per-skill\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p2.cost.replay-only.mean-requests-per-skill\endcsname{96}
\expandafter\def\csname pct@sspro.p2.cost.replay-only.mean-requests-per-skill\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.cost.replay-only.mean-requests-per-skill\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{109.650}
\expandafter\def\csname cnt@sspro.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{110}
\expandafter\def\csname pct@sspro.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{10965.0}
\expandafter\def\csname ppt@sspro.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{$+$10965.0}
\expandafter\def\csname val@sspro.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{128.787}
\expandafter\def\csname cnt@sspro.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{129}
\expandafter\def\csname pct@sspro.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{12878.8}
\expandafter\def\csname ppt@sspro.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{$+$12878.8}
\expandafter\def\csname val@sspro.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{161.588}
\expandafter\def\csname cnt@sspro.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{162}
\expandafter\def\csname pct@sspro.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{16158.8}
\expandafter\def\csname ppt@sspro.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{$+$16158.8}
\expandafter\def\csname val@sspro.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{227.000}
\expandafter\def\csname cnt@sspro.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{227}
\expandafter\def\csname pct@sspro.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{22700.0}
\expandafter\def\csname ppt@sspro.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{$+$22700.0}
\expandafter\def\csname val@sspro.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{61.650}
\expandafter\def\csname cnt@sspro.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{62}
\expandafter\def\csname pct@sspro.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{6165.0}
\expandafter\def\csname ppt@sspro.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{$+$6165.0}
\expandafter\def\csname val@sspro.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{80.787}
\expandafter\def\csname cnt@sspro.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{81}
\expandafter\def\csname pct@sspro.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{8078.7}
\expandafter\def\csname ppt@sspro.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{$+$8078.7}
\expandafter\def\csname val@sspro.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{113.588}
\expandafter\def\csname cnt@sspro.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{114}
\expandafter\def\csname pct@sspro.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{11358.8}
\expandafter\def\csname ppt@sspro.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{$+$11358.8}
\expandafter\def\csname val@sspro.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{179}
\expandafter\def\csname pct@sspro.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.1.center-d1\endcsname{0.700}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.1.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.1.center-d1\endcsname{70.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.1.center-d1\endcsname{$+$70.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.1.direct\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.1.direct\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.1.direct\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.1.direct\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.1.dual-d2\endcsname{0.200}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.1.dual-d2\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.1.dual-d2\endcsname{20.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.1.dual-d2\endcsname{$+$20.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.1.grid2-d3\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.1.grid2-d3\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.1.grid2-d3\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.1.grid2-d3\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.25.center-d1\endcsname{0.550}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.25.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.25.center-d1\endcsname{55.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.25.center-d1\endcsname{$+$55.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.25.context-d1\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.25.context-d1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.25.context-d1\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.25.context-d1\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.25.dual-d2\endcsname{0.200}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.25.dual-d2\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.25.dual-d2\endcsname{20.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.25.dual-d2\endcsname{$+$20.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.25.grid2-d3\endcsname{0.200}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.25.grid2-d3\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.25.grid2-d3\endcsname{20.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.25.grid2-d3\endcsname{$+$20.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.5.center-d1\endcsname{0.600}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.5.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.5.center-d1\endcsname{60.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.5.center-d1\endcsname{$+$60.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.5.context-d1\endcsname{0.250}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.5.context-d1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.5.context-d1\endcsname{25.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.5.context-d1\endcsname{$+$25.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@0.5.grid2-d3\endcsname{0.150}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@0.5.grid2-d3\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.best-single@0.5.grid2-d3\endcsname{15.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@0.5.grid2-d3\endcsname{$+$15.0}
\expandafter\def\csname val@sspro.p2.decide.best-single@1.0.center-d1\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.best-single@1.0.center-d1\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.best-single@1.0.center-d1\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.best-single@1.0.center-d1\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.103}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{10.3}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$10.3}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{106.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{106}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{10600.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$10600.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.127}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{12.7}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$12.7}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{10600.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$10600.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.093}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{9.3}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$9.3}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.044}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{4.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.090}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{9.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$9.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.118}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{11.8}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$11.8}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.033}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{3.3}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$3.3}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.113}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{11.3}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$11.3}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.033}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{3.3}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.3}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.079}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{7.9}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$7.9}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.072}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{7.2}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$7.2}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.106}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{10.6}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$10.6}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.101}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{10.1}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$10.1}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.021}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.1}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.1}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.110}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{11.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$11.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.038}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.8}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.8}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.cost.full-recert-fresh\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.cost.full-recert-fresh\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget-tau.old-source\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.no-budget-tau.old-source\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.no-budget-tau.old-source\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{0.083}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{8.3}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{$+$8.3}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.center-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p2.decide.center-d1.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.sigma-used.disagree\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.sigma-used.disagree\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.sigma-used.disagree\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.strata-N.agree-stable\endcsname{42}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.strata-N.agree-stable\endcsname{42}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.strata-N.agree-stable\endcsname{4200.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.strata-N.agree-stable\endcsname{$+$4200.0}
\expandafter\def\csname val@sspro.p2.decide.center-d1.strata-N.disagree\endcsname{6}
\expandafter\def\csname cnt@sspro.p2.decide.center-d1.strata-N.disagree\endcsname{6}
\expandafter\def\csname pct@sspro.p2.decide.center-d1.strata-N.disagree\endcsname{600.0}
\expandafter\def\csname ppt@sspro.p2.decide.center-d1.strata-N.disagree\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.101}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{10.1}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$10.1}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.117}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{11.7}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$11.7}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{106.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{106}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{10600.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$10600.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{106}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{10600.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$10600.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.063}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{6.3}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.3}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{58}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{5800.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$5800.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.090}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{9.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$9.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.148}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{14.8}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$14.8}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.070}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{7.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$7.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.115}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{11.5}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$11.5}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.031}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{3.1}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$3.1}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.096}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{9.6}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$9.6}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{72}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{7200.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$7200.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.071}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{7.1}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$7.1}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.088}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{8.8}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$8.8}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.051}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{5.1}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$5.1}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.106}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{10.6}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$10.6}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.102}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.034}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{3.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{96}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.108}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{10.8}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$10.8}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.044}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{4.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$4.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.cost.full-recert-fresh\endcsname{96}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.cost.full-recert-fresh\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.cost.full-recert-fresh\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget-tau.old-source\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.no-budget-tau.old-source\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.no-budget-tau.old-source\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.context-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p2.decide.context-d1.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.sigma-used.disagree\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.sigma-used.disagree\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.sigma-used.disagree\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.strata-N.agree-drift\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.strata-N.agree-drift\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.strata-N.agree-stable\endcsname{40}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.strata-N.agree-stable\endcsname{40}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.strata-N.agree-stable\endcsname{4000.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.strata-N.agree-stable\endcsname{$+$4000.0}
\expandafter\def\csname val@sspro.p2.decide.context-d1.strata-N.disagree\endcsname{7}
\expandafter\def\csname cnt@sspro.p2.decide.context-d1.strata-N.disagree\endcsname{7}
\expandafter\def\csname pct@sspro.p2.decide.context-d1.strata-N.disagree\endcsname{700.0}
\expandafter\def\csname ppt@sspro.p2.decide.context-d1.strata-N.disagree\endcsname{$+$700.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{63.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{6300.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$6300.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.042}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{4.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$4.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.200}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{20.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$20.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{111.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{111}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{11100.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$11100.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.030}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{3.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$3.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.187}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{18.7}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$18.7}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{11100.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$11100.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.042}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{4.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$4.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.219}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{21.9}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$21.9}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{63.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{6300.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$6300.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.060}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{6.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$6.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.191}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{19.1}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$19.1}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{84.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{8400.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$8400.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.033}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{3.3}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$3.3}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.131}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{13.1}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$13.1}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{132.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{13200.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$13200.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.067}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{6.7}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$6.7}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.089}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{8.9}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$8.9}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{13200.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$13200.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.029}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{2.9}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$2.9}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.130}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{13.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$13.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{84.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{8400.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$8400.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.033}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{3.3}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$3.3}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.152}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{15.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$15.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.048}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{4.8}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$4.8}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.072}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{7.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$7.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.071}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{7.1}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$7.1}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.058}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{5.8}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$5.8}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.088}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{8.8}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$8.8}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.054}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{5.4}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$5.4}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.061}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{6.1}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$6.1}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.063}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{6.3}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$6.3}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.063}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{6.3}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$6.3}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.063}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{6.3}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$6.3}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{144}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{0.042}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{4.2}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{$+$4.2}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{0.189}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{18.9}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{$+$18.9}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.sigma-used.disagree\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.sigma-used.disagree\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.sigma-used.disagree\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.strata-N.agree-stable\endcsname{39}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.strata-N.agree-stable\endcsname{39}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.strata-N.agree-stable\endcsname{3900.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.strata-N.agree-stable\endcsname{$+$3900.0}
\expandafter\def\csname val@sspro.p2.decide.dual-d2.strata-N.disagree\endcsname{9}
\expandafter\def\csname cnt@sspro.p2.decide.dual-d2.strata-N.disagree\endcsname{9}
\expandafter\def\csname pct@sspro.p2.decide.dual-d2.strata-N.disagree\endcsname{900.0}
\expandafter\def\csname ppt@sspro.p2.decide.dual-d2.strata-N.disagree\endcsname{$+$900.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{67.600}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{68}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{6760.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$6760.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.103}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.102}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{115.600}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{116}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{11560.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$11560.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.103}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.102}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{67.600}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{68}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{6760.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$6760.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.090}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{9.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$9.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.134}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{13.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$13.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{95.150}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{95}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{9515.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$9515.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.117}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{11.7}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$11.7}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.080}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{8.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$8.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{143.600}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{14360.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$14360.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.111}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{11.1}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$11.1}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.041}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{4.1}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$4.1}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{143.150}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{143}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{14315.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$14315.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.117}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{11.7}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$11.7}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.080}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{8.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$8.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{95.150}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{95}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{9515.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$9515.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.079}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{7.9}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$7.9}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{142.350}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{142}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{14235.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$14235.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.102}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{190.900}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{191}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{19090.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$19090.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.109}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{10.9}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$10.9}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.025}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.5}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.5}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{190.350}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{190}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{19035.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$19035.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.102}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{10.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.045}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{4.5}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.5}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{142.350}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{142}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{14235.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$14235.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.106}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{10.6}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$10.6}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.050}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{5.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$5.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{236.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{236}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{23600.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$23600.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{284.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{284}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{28400.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$28400.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{284.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{284}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{28400.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$28400.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{236.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{236}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{23600.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$23600.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{188}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{188}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{18800.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{$+$18800.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{0.182}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{18.2}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{$+$18.2}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.sigma-used.disagree\endcsname{0.471}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.sigma-used.disagree\endcsname{47.1}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.sigma-used.disagree\endcsname{$+$47.1}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{39}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{39}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{3900.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{$+$3900.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.strata-N.disagree\endcsname{6}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.strata-N.disagree\endcsname{6}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.strata-N.disagree\endcsname{600.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.strata-N.disagree\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{3}
\expandafter\def\csname cnt@sspro.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{3}
\expandafter\def\csname pct@sspro.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{300.0}
\expandafter\def\csname ppt@sspro.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{$+$300.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{5}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{500.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{$+$500.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{63.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{6300.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$6300.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.165}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{16.5}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$16.5}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.136}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{13.6}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$13.6}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{111.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{111}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{11100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$11100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.172}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{17.2}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$17.2}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.044}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{4.4}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$4.4}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{111}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{11100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$11100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.164}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{16.4}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$16.4}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.111}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{11.1}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$11.1}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{63.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{63}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{6300.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$6300.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.140}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{14.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$14.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.169}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{16.9}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$16.9}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{12}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{84.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{8400.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$8400.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.085}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{8.5}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$8.5}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{132.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{13200.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$13200.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.173}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{17.3}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$17.3}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.030}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{3.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$3.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{132}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{13200.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$13200.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.175}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{17.5}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$17.5}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.066}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{6.6}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.6}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{84.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{84}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{8400.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$8400.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.133}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{13.3}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$13.3}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.116}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{11.6}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$11.6}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{24}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{2400.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{$+$2400.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.165}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{16.5}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$16.5}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.036}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{3.6}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$3.6}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.173}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{17.3}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$17.3}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.030}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{3.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$3.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{168}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.173}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{17.3}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$17.3}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{120.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{120}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{12000.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$12000.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.056}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{5.6}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$5.6}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.cost.direct-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.cost.direct-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.cost.direct-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{144}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{144}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{14400.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{$+$14400.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.cost.replay-all\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.cost.replay-all\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.cost.replay-all\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0.180}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{18.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{$+$18.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{0.100}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{10.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{$+$10.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{41}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{41}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{4100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{$+$4100.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{6}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{6}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{600.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.p2.decide.zoomclick-d3.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname cnt@sspro.p2.decide.zoomclick-d3.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname pct@sspro.p2.decide.zoomclick-d3.strata-N.parse-fail\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.decide.zoomclick-d3.strata-N.parse-fail\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.bracket-costs.0\endcsname{113.588}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.bracket-costs.0\endcsname{114}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.bracket-costs.0\endcsname{11358.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.bracket-costs.0\endcsname{$+$11358.8}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.bracket-costs.1\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.bracket-costs.1\endcsname{179}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.bracket-costs.1\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.bracket-costs.1\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{-0.029}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$2.9}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$2.9}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{-0.001}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{$-$0.1}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{$-$0.1}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{-0.027}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$2.7}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$2.7}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.mean\endcsname{-0.015}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.mean\endcsname{$-$1.5}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.mean\endcsname{$-$1.5}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{0.981}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{98.1}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{$+$98.1}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.733}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{73.3}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{$+$73.3}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{0.909}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{90.9}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{$+$90.9}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.status\endcsname{ok}
\expandafter\def\csname val@sspro.p2.equal-cost.best-single.weight\endcsname{0.234}
\expandafter\def\csname cnt@sspro.p2.equal-cost.best-single.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.best-single.weight\endcsname{23.4}
\expandafter\def\csname ppt@sspro.p2.equal-cost.best-single.weight\endcsname{$+$23.4}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{113.588}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{114}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{11358.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{$+$11358.8}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{179}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{-0.008}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$-$0.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$-$0.8}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{-0.003}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{$-$0.3}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{$-$0.3}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{-0.008}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{-0.005}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{$-$0.5}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{$-$0.5}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.001}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.1}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{$+$0.1}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{0.900}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{90.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{$+$90.0}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.status\endcsname{ok}
\expandafter\def\csname val@sspro.p2.equal-cost.generic-ppi-source.weight\endcsname{0.234}
\expandafter\def\csname cnt@sspro.p2.equal-cost.generic-ppi-source.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.generic-ppi-source.weight\endcsname{23.4}
\expandafter\def\csname ppt@sspro.p2.equal-cost.generic-ppi-source.weight\endcsname{$+$23.4}
\expandafter\def\csname val@sspro.p2.equal-cost.rcr-cost\endcsname{128.900}
\expandafter\def\csname cnt@sspro.p2.equal-cost.rcr-cost\endcsname{129}
\expandafter\def\csname pct@sspro.p2.equal-cost.rcr-cost\endcsname{12890.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.rcr-cost\endcsname{$+$12890.0}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{128.787}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{129}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{12878.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{$+$12878.8}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{161.588}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{162}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{16158.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{$+$16158.8}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.005}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.5}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{$+$0.5}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.006}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.6}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{$+$0.6}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.010}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{1.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{$+$1.0}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.status\endcsname{ok}
\expandafter\def\csname val@sspro.p2.equal-cost.replay-ppi-uniform.weight\endcsname{0.003}
\expandafter\def\csname cnt@sspro.p2.equal-cost.replay-ppi-uniform.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.replay-ppi-uniform.weight\endcsname{0.3}
\expandafter\def\csname ppt@sspro.p2.equal-cost.replay-ppi-uniform.weight\endcsname{$+$0.3}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{113.588}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{114}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{11358.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{$+$11358.8}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{179.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{179}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{17900.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{$+$17900.0}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{-0.013}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$1.3}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$1.3}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{-0.005}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{$-$0.5}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{$-$0.5}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{-0.012}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$1.2}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$1.2}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{-0.008}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{$-$0.8}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.231}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{23.1}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{$+$23.1}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{0.903}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{90.3}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{$+$90.3}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.status\endcsname{ok}
\expandafter\def\csname val@sspro.p2.equal-cost.uniform-fresh.weight\endcsname{0.234}
\expandafter\def\csname cnt@sspro.p2.equal-cost.uniform-fresh.weight\endcsname{0}
\expandafter\def\csname pct@sspro.p2.equal-cost.uniform-fresh.weight\endcsname{23.4}
\expandafter\def\csname ppt@sspro.p2.equal-cost.uniform-fresh.weight\endcsname{$+$23.4}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.acc-macro\endcsname{0.917}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.acc-macro\endcsname{91.7}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.acc-macro\endcsname{$+$91.7}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.mean-requests\endcsname{2.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.mean-requests\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.mean-requests\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.n\endcsname{96}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0.240}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{24.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{$+$24.0}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{0.094}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{9.4}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{$+$9.4}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{0.156}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{15.6}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{$+$15.6}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.acc-macro\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.acc-macro\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.acc-macro\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.mean-requests\endcsname{2.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.mean-requests\endcsname{200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.mean-requests\endcsname{$+$200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.n\endcsname{96}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0.208}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{20.8}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{$+$20.8}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.direct\endcsname{0.760}
\expandafter\def\csname cnt@sspro.p2.execution-layer.direct\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.direct\endcsname{76.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.direct\endcsname{$+$76.0}
\expandafter\def\csname val@sspro.p2.execution-layer.direct-sc3\endcsname{0.812}
\expandafter\def\csname cnt@sspro.p2.execution-layer.direct-sc3\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.direct-sc3\endcsname{81.2}
\expandafter\def\csname ppt@sspro.p2.execution-layer.direct-sc3\endcsname{$+$81.2}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.acc-macro\endcsname{0.917}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.acc-macro\endcsname{91.7}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.acc-macro\endcsname{$+$91.7}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.mean-requests\endcsname{3.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.mean-requests\endcsname{3}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.mean-requests\endcsname{300.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.mean-requests\endcsname{$+$300.0}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.n\endcsname{96}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{0.083}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{8.3}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{$+$8.3}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{0.229}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{22.9}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{$+$22.9}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{0.094}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{9.4}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{$+$9.4}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{0.156}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{15.6}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{$+$15.6}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.acc-macro\endcsname{0.906}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.acc-macro\endcsname{90.6}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.acc-macro\endcsname{$+$90.6}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.mean-requests\endcsname{3.677}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.mean-requests\endcsname{4}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.mean-requests\endcsname{367.7}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.mean-requests\endcsname{$+$367.7}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.n\endcsname{96}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{0.062}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{6.2}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{$+$6.2}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0.240}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{24.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{$+$24.0}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{0.073}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{7.3}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{$+$7.3}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{0.146}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{14.6}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{$+$14.6}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.001}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.1}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{$+$0.1}
\expandafter\def\csname val@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{0.927}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{92.7}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{$+$92.7}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{3.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{3}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{300.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{$+$300.0}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.n\endcsname{96}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.n\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.n\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{0.104}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{10.4}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{$+$10.4}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0.240}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{24.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{$+$24.0}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{0.115}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{11.5}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{$+$11.5}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{0.167}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{16.7}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{$+$16.7}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{0.011}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{1.1}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{$+$1.1}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{0.008}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{0.8}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{$+$0.8}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0.011}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{1.1}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{$+$1.1}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.008}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.8}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{$+$0.8}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname cnt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname pct@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@sspro.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname val@sspro.p2.n-cal\endcsname{48}
\expandafter\def\csname cnt@sspro.p2.n-cal\endcsname{48}
\expandafter\def\csname pct@sspro.p2.n-cal\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.p2.n-cal\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.p2.n-cal-apps\endcsname{6}
\expandafter\def\csname cnt@sspro.p2.n-cal-apps\endcsname{6}
\expandafter\def\csname pct@sspro.p2.n-cal-apps\endcsname{600.0}
\expandafter\def\csname ppt@sspro.p2.n-cal-apps\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.p2.n-test\endcsname{96}
\expandafter\def\csname cnt@sspro.p2.n-test\endcsname{96}
\expandafter\def\csname pct@sspro.p2.n-test\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.p2.n-test\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.p2.n-test-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.p2.n-test-apps\endcsname{12}
\expandafter\def\csname pct@sspro.p2.n-test-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.p2.n-test-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.p2.primary.best-single.cost\endcsname{80.787}
\expandafter\def\csname cnt@sspro.p2.primary.best-single.cost\endcsname{81}
\expandafter\def\csname pct@sspro.p2.primary.best-single.cost\endcsname{8078.7}
\expandafter\def\csname ppt@sspro.p2.primary.best-single.cost\endcsname{$+$8078.7}
\expandafter\def\csname val@sspro.p2.primary.best-single.cost-fraction-of-full\endcsname{0.451}
\expandafter\def\csname cnt@sspro.p2.primary.best-single.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.best-single.cost-fraction-of-full\endcsname{45.1}
\expandafter\def\csname ppt@sspro.p2.primary.best-single.cost-fraction-of-full\endcsname{$+$45.1}
\expandafter\def\csname val@sspro.p2.primary.best-single.score\endcsname{0.913}
\expandafter\def\csname cnt@sspro.p2.primary.best-single.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.best-single.score\endcsname{91.3}
\expandafter\def\csname ppt@sspro.p2.primary.best-single.score\endcsname{$+$91.3}
\expandafter\def\csname val@sspro.p2.primary.best-single.vs-full-recert\endcsname{0.007}
\expandafter\def\csname cnt@sspro.p2.primary.best-single.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.best-single.vs-full-recert\endcsname{0.7}
\expandafter\def\csname ppt@sspro.p2.primary.best-single.vs-full-recert\endcsname{$+$0.7}
\expandafter\def\csname val@sspro.p2.primary.best-single.vs-suspend-all\endcsname{0.153}
\expandafter\def\csname cnt@sspro.p2.primary.best-single.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.best-single.vs-suspend-all\endcsname{15.3}
\expandafter\def\csname ppt@sspro.p2.primary.best-single.vs-suspend-all\endcsname{$+$15.3}
\expandafter\def\csname val@sspro.p2.primary.generic-ppi-source.cost\endcsname{80.787}
\expandafter\def\csname cnt@sspro.p2.primary.generic-ppi-source.cost\endcsname{81}
\expandafter\def\csname pct@sspro.p2.primary.generic-ppi-source.cost\endcsname{8078.7}
\expandafter\def\csname ppt@sspro.p2.primary.generic-ppi-source.cost\endcsname{$+$8078.7}
\expandafter\def\csname val@sspro.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0.451}
\expandafter\def\csname cnt@sspro.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{45.1}
\expandafter\def\csname ppt@sspro.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{$+$45.1}
\expandafter\def\csname val@sspro.p2.primary.generic-ppi-source.score\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p2.primary.generic-ppi-source.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.generic-ppi-source.score\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p2.primary.generic-ppi-source.score\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p2.primary.generic-ppi-source.vs-full-recert\endcsname{-0.021}
\expandafter\def\csname cnt@sspro.p2.primary.generic-ppi-source.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.generic-ppi-source.vs-full-recert\endcsname{$-$2.1}
\expandafter\def\csname ppt@sspro.p2.primary.generic-ppi-source.vs-full-recert\endcsname{$-$2.1}
\expandafter\def\csname val@sspro.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p2.primary.rcr-stratified.cost\endcsname{128.900}
\expandafter\def\csname cnt@sspro.p2.primary.rcr-stratified.cost\endcsname{129}
\expandafter\def\csname pct@sspro.p2.primary.rcr-stratified.cost\endcsname{12890.0}
\expandafter\def\csname ppt@sspro.p2.primary.rcr-stratified.cost\endcsname{$+$12890.0}
\expandafter\def\csname val@sspro.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{0.720}
\expandafter\def\csname cnt@sspro.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{72.0}
\expandafter\def\csname ppt@sspro.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{$+$72.0}
\expandafter\def\csname val@sspro.p2.primary.rcr-stratified.score\endcsname{0.895}
\expandafter\def\csname cnt@sspro.p2.primary.rcr-stratified.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.rcr-stratified.score\endcsname{89.5}
\expandafter\def\csname ppt@sspro.p2.primary.rcr-stratified.score\endcsname{$+$89.5}
\expandafter\def\csname val@sspro.p2.primary.rcr-stratified.vs-full-recert\endcsname{-0.011}
\expandafter\def\csname cnt@sspro.p2.primary.rcr-stratified.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.rcr-stratified.vs-full-recert\endcsname{$-$1.1}
\expandafter\def\csname ppt@sspro.p2.primary.rcr-stratified.vs-full-recert\endcsname{$-$1.1}
\expandafter\def\csname val@sspro.p2.primary.rcr-stratified.vs-suspend-all\endcsname{0.134}
\expandafter\def\csname cnt@sspro.p2.primary.rcr-stratified.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.rcr-stratified.vs-suspend-all\endcsname{13.4}
\expandafter\def\csname ppt@sspro.p2.primary.rcr-stratified.vs-suspend-all\endcsname{$+$13.4}
\expandafter\def\csname val@sspro.p2.primary.replay-ppi-uniform.cost\endcsname{128.787}
\expandafter\def\csname cnt@sspro.p2.primary.replay-ppi-uniform.cost\endcsname{129}
\expandafter\def\csname pct@sspro.p2.primary.replay-ppi-uniform.cost\endcsname{12878.8}
\expandafter\def\csname ppt@sspro.p2.primary.replay-ppi-uniform.cost\endcsname{$+$12878.8}
\expandafter\def\csname val@sspro.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{0.719}
\expandafter\def\csname cnt@sspro.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{71.9}
\expandafter\def\csname ppt@sspro.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{$+$71.9}
\expandafter\def\csname val@sspro.p2.primary.replay-ppi-uniform.score\endcsname{0.885}
\expandafter\def\csname cnt@sspro.p2.primary.replay-ppi-uniform.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.replay-ppi-uniform.score\endcsname{88.5}
\expandafter\def\csname ppt@sspro.p2.primary.replay-ppi-uniform.score\endcsname{$+$88.5}
\expandafter\def\csname val@sspro.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{-0.021}
\expandafter\def\csname cnt@sspro.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{$-$2.1}
\expandafter\def\csname ppt@sspro.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{$-$2.1}
\expandafter\def\csname val@sspro.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{0.125}
\expandafter\def\csname cnt@sspro.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{12.5}
\expandafter\def\csname ppt@sspro.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{$+$12.5}
\expandafter\def\csname val@sspro.p2.primary.uniform-fresh.cost\endcsname{80.787}
\expandafter\def\csname cnt@sspro.p2.primary.uniform-fresh.cost\endcsname{81}
\expandafter\def\csname pct@sspro.p2.primary.uniform-fresh.cost\endcsname{8078.7}
\expandafter\def\csname ppt@sspro.p2.primary.uniform-fresh.cost\endcsname{$+$8078.7}
\expandafter\def\csname val@sspro.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{0.451}
\expandafter\def\csname cnt@sspro.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{45.1}
\expandafter\def\csname ppt@sspro.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{$+$45.1}
\expandafter\def\csname val@sspro.p2.primary.uniform-fresh.score\endcsname{0.891}
\expandafter\def\csname cnt@sspro.p2.primary.uniform-fresh.score\endcsname{1}
\expandafter\def\csname pct@sspro.p2.primary.uniform-fresh.score\endcsname{89.1}
\expandafter\def\csname ppt@sspro.p2.primary.uniform-fresh.score\endcsname{$+$89.1}
\expandafter\def\csname val@sspro.p2.primary.uniform-fresh.vs-full-recert\endcsname{-0.015}
\expandafter\def\csname cnt@sspro.p2.primary.uniform-fresh.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.uniform-fresh.vs-full-recert\endcsname{$-$1.5}
\expandafter\def\csname ppt@sspro.p2.primary.uniform-fresh.vs-full-recert\endcsname{$-$1.5}
\expandafter\def\csname val@sspro.p2.primary.uniform-fresh.vs-suspend-all\endcsname{0.131}
\expandafter\def\csname cnt@sspro.p2.primary.uniform-fresh.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@sspro.p2.primary.uniform-fresh.vs-suspend-all\endcsname{13.1}
\expandafter\def\csname ppt@sspro.p2.primary.uniform-fresh.vs-suspend-all\endcsname{$+$13.1}
\expandafter\def\csname val@sspro.records.audit.answer-echo-via-bash\endcsname{8}
\expandafter\def\csname cnt@sspro.records.audit.answer-echo-via-bash\endcsname{8}
\expandafter\def\csname pct@sspro.records.audit.answer-echo-via-bash\endcsname{800.0}
\expandafter\def\csname ppt@sspro.records.audit.answer-echo-via-bash\endcsname{$+$800.0}
\expandafter\def\csname val@sspro.records.audit.bash-non-echo\endcsname{1}
\expandafter\def\csname cnt@sspro.records.audit.bash-non-echo\endcsname{1}
\expandafter\def\csname pct@sspro.records.audit.bash-non-echo\endcsname{100.0}
\expandafter\def\csname ppt@sspro.records.audit.bash-non-echo\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.records.audit.file-access-attempts-nonexistent\endcsname{0}
\expandafter\def\csname cnt@sspro.records.audit.file-access-attempts-nonexistent\endcsname{0}
\expandafter\def\csname pct@sspro.records.audit.file-access-attempts-nonexistent\endcsname{0.0}
\expandafter\def\csname ppt@sspro.records.audit.file-access-attempts-nonexistent\endcsname{0.0}
\expandafter\def\csname val@sspro.records.audit.file-access-violations\endcsname{1}
\expandafter\def\csname cnt@sspro.records.audit.file-access-violations\endcsname{1}
\expandafter\def\csname pct@sspro.records.audit.file-access-violations\endcsname{100.0}
\expandafter\def\csname ppt@sspro.records.audit.file-access-violations\endcsname{$+$100.0}
\expandafter\def\csname val@sspro.records.audit.harness-meta-tool-calls-only\endcsname{28}
\expandafter\def\csname cnt@sspro.records.audit.harness-meta-tool-calls-only\endcsname{28}
\expandafter\def\csname pct@sspro.records.audit.harness-meta-tool-calls-only\endcsname{2800.0}
\expandafter\def\csname ppt@sspro.records.audit.harness-meta-tool-calls-only\endcsname{$+$2800.0}
\expandafter\def\csname val@sspro.records.audit.read-outside-allowed-existing-file\endcsname{0}
\expandafter\def\csname cnt@sspro.records.audit.read-outside-allowed-existing-file\endcsname{0}
\expandafter\def\csname pct@sspro.records.audit.read-outside-allowed-existing-file\endcsname{0.0}
\expandafter\def\csname ppt@sspro.records.audit.read-outside-allowed-existing-file\endcsname{0.0}
\expandafter\def\csname val@sspro.records.audit.requests-with-unexpected-tools\endcsname{29}
\expandafter\def\csname cnt@sspro.records.audit.requests-with-unexpected-tools\endcsname{29}
\expandafter\def\csname pct@sspro.records.audit.requests-with-unexpected-tools\endcsname{2900.0}
\expandafter\def\csname ppt@sspro.records.audit.requests-with-unexpected-tools\endcsname{$+$2900.0}
\expandafter\def\csname val@sspro.records.audit.requests-with-violations\endcsname{29}
\expandafter\def\csname cnt@sspro.records.audit.requests-with-violations\endcsname{29}
\expandafter\def\csname pct@sspro.records.audit.requests-with-violations\endcsname{2900.0}
\expandafter\def\csname ppt@sspro.records.audit.requests-with-violations\endcsname{$+$2900.0}
\expandafter\def\csname val@sspro.records.fidelity.exact-bytes\endcsname{13821}
\expandafter\def\csname cnt@sspro.records.fidelity.exact-bytes\endcsname{13{,}821}
\expandafter\def\csname pct@sspro.records.fidelity.exact-bytes\endcsname{1382100.0}
\expandafter\def\csname ppt@sspro.records.fidelity.exact-bytes\endcsname{$+$1382100.0}
\expandafter\def\csname val@sspro.records.fidelity.images-checked\endcsname{13821}
\expandafter\def\csname cnt@sspro.records.fidelity.images-checked\endcsname{13{,}821}
\expandafter\def\csname pct@sspro.records.fidelity.images-checked\endcsname{1382100.0}
\expandafter\def\csname ppt@sspro.records.fidelity.images-checked\endcsname{$+$1382100.0}
\expandafter\def\csname val@sspro.records.fidelity.mismatch\endcsname{0}
\expandafter\def\csname cnt@sspro.records.fidelity.mismatch\endcsname{0}
\expandafter\def\csname pct@sspro.records.fidelity.mismatch\endcsname{0.0}
\expandafter\def\csname ppt@sspro.records.fidelity.mismatch\endcsname{0.0}
\expandafter\def\csname val@sspro.records.latency.acquire-box.mean\endcsname{4.860}
\expandafter\def\csname cnt@sspro.records.latency.acquire-box.mean\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.acquire-box.mean\endcsname{486.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-box.mean\endcsname{$+$486.0}
\expandafter\def\csname val@sspro.records.latency.acquire-box.median\endcsname{5.750}
\expandafter\def\csname cnt@sspro.records.latency.acquire-box.median\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.acquire-box.median\endcsname{575.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-box.median\endcsname{$+$575.0}
\expandafter\def\csname val@sspro.records.latency.acquire-box.n\endcsname{1827}
\expandafter\def\csname cnt@sspro.records.latency.acquire-box.n\endcsname{1{,}827}
\expandafter\def\csname pct@sspro.records.latency.acquire-box.n\endcsname{182700.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-box.n\endcsname{$+$182700.0}
\expandafter\def\csname val@sspro.records.latency.acquire-box.p90\endcsname{8.360}
\expandafter\def\csname cnt@sspro.records.latency.acquire-box.p90\endcsname{8}
\expandafter\def\csname pct@sspro.records.latency.acquire-box.p90\endcsname{836.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-box.p90\endcsname{$+$836.0}
\expandafter\def\csname val@sspro.records.latency.acquire-cell.mean\endcsname{5.550}
\expandafter\def\csname cnt@sspro.records.latency.acquire-cell.mean\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.acquire-cell.mean\endcsname{555.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-cell.mean\endcsname{$+$555.0}
\expandafter\def\csname val@sspro.records.latency.acquire-cell.median\endcsname{6.140}
\expandafter\def\csname cnt@sspro.records.latency.acquire-cell.median\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.acquire-cell.median\endcsname{614.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-cell.median\endcsname{$+$614.0}
\expandafter\def\csname val@sspro.records.latency.acquire-cell.n\endcsname{1885}
\expandafter\def\csname cnt@sspro.records.latency.acquire-cell.n\endcsname{1{,}885}
\expandafter\def\csname pct@sspro.records.latency.acquire-cell.n\endcsname{188500.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-cell.n\endcsname{$+$188500.0}
\expandafter\def\csname val@sspro.records.latency.acquire-cell.p90\endcsname{9.120}
\expandafter\def\csname cnt@sspro.records.latency.acquire-cell.p90\endcsname{9}
\expandafter\def\csname pct@sspro.records.latency.acquire-cell.p90\endcsname{912.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-cell.p90\endcsname{$+$912.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual-refine.mean\endcsname{6.200}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual-refine.mean\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual-refine.mean\endcsname{620.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual-refine.mean\endcsname{$+$620.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual-refine.median\endcsname{6.420}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual-refine.median\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual-refine.median\endcsname{642.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual-refine.median\endcsname{$+$642.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual-refine.n\endcsname{496}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual-refine.n\endcsname{496}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual-refine.n\endcsname{49600.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual-refine.n\endcsname{$+$49600.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual-refine.p90\endcsname{8.690}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual-refine.p90\endcsname{9}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual-refine.p90\endcsname{869.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual-refine.p90\endcsname{$+$869.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual.mean\endcsname{4.680}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual.mean\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual.mean\endcsname{468.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual.mean\endcsname{$+$468.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual.median\endcsname{5.520}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual.median\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual.median\endcsname{552.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual.median\endcsname{$+$552.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual.n\endcsname{904}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual.n\endcsname{904}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual.n\endcsname{90400.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual.n\endcsname{$+$90400.0}
\expandafter\def\csname val@sspro.records.latency.acquire-dual.p90\endcsname{8.410}
\expandafter\def\csname cnt@sspro.records.latency.acquire-dual.p90\endcsname{8}
\expandafter\def\csname pct@sspro.records.latency.acquire-dual.p90\endcsname{841.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-dual.p90\endcsname{$+$841.0}
\expandafter\def\csname val@sspro.records.latency.acquire-point.mean\endcsname{5.060}
\expandafter\def\csname cnt@sspro.records.latency.acquire-point.mean\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.acquire-point.mean\endcsname{506.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-point.mean\endcsname{$+$506.0}
\expandafter\def\csname val@sspro.records.latency.acquire-point.median\endcsname{5.380}
\expandafter\def\csname cnt@sspro.records.latency.acquire-point.median\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.acquire-point.median\endcsname{538.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-point.median\endcsname{$+$538.0}
\expandafter\def\csname val@sspro.records.latency.acquire-point.n\endcsname{1112}
\expandafter\def\csname cnt@sspro.records.latency.acquire-point.n\endcsname{1{,}112}
\expandafter\def\csname pct@sspro.records.latency.acquire-point.n\endcsname{111200.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-point.n\endcsname{$+$111200.0}
\expandafter\def\csname val@sspro.records.latency.acquire-point.p90\endcsname{7.750}
\expandafter\def\csname cnt@sspro.records.latency.acquire-point.p90\endcsname{8}
\expandafter\def\csname pct@sspro.records.latency.acquire-point.p90\endcsname{775.0}
\expandafter\def\csname ppt@sspro.records.latency.acquire-point.p90\endcsname{$+$775.0}
\expandafter\def\csname val@sspro.records.latency.direct.mean\endcsname{4.680}
\expandafter\def\csname cnt@sspro.records.latency.direct.mean\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.direct.mean\endcsname{468.0}
\expandafter\def\csname ppt@sspro.records.latency.direct.mean\endcsname{$+$468.0}
\expandafter\def\csname val@sspro.records.latency.direct.median\endcsname{5.380}
\expandafter\def\csname cnt@sspro.records.latency.direct.median\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.direct.median\endcsname{538.0}
\expandafter\def\csname ppt@sspro.records.latency.direct.median\endcsname{$+$538.0}
\expandafter\def\csname val@sspro.records.latency.direct.n\endcsname{1724}
\expandafter\def\csname cnt@sspro.records.latency.direct.n\endcsname{1{,}724}
\expandafter\def\csname pct@sspro.records.latency.direct.n\endcsname{172400.0}
\expandafter\def\csname ppt@sspro.records.latency.direct.n\endcsname{$+$172400.0}
\expandafter\def\csname val@sspro.records.latency.direct.p90\endcsname{7.960}
\expandafter\def\csname cnt@sspro.records.latency.direct.p90\endcsname{8}
\expandafter\def\csname pct@sspro.records.latency.direct.p90\endcsname{796.0}
\expandafter\def\csname ppt@sspro.records.latency.direct.p90\endcsname{$+$796.0}
\expandafter\def\csname val@sspro.records.latency.read.mean\endcsname{5.350}
\expandafter\def\csname cnt@sspro.records.latency.read.mean\endcsname{5}
\expandafter\def\csname pct@sspro.records.latency.read.mean\endcsname{535.0}
\expandafter\def\csname ppt@sspro.records.latency.read.mean\endcsname{$+$535.0}
\expandafter\def\csname val@sspro.records.latency.read.median\endcsname{5.700}
\expandafter\def\csname cnt@sspro.records.latency.read.median\endcsname{6}
\expandafter\def\csname pct@sspro.records.latency.read.median\endcsname{570.0}
\expandafter\def\csname ppt@sspro.records.latency.read.median\endcsname{$+$570.0}
\expandafter\def\csname val@sspro.records.latency.read.n\endcsname{5037}
\expandafter\def\csname cnt@sspro.records.latency.read.n\endcsname{5{,}037}
\expandafter\def\csname pct@sspro.records.latency.read.n\endcsname{503700.0}
\expandafter\def\csname ppt@sspro.records.latency.read.n\endcsname{$+$503700.0}
\expandafter\def\csname val@sspro.records.latency.read.p90\endcsname{8.380}
\expandafter\def\csname cnt@sspro.records.latency.read.p90\endcsname{8}
\expandafter\def\csname pct@sspro.records.latency.read.p90\endcsname{838.0}
\expandafter\def\csname ppt@sspro.records.latency.read.p90\endcsname{$+$838.0}
\expandafter\def\csname val@sspro.records.model-id-match.haiku\endcsname{1924}
\expandafter\def\csname cnt@sspro.records.model-id-match.haiku\endcsname{1{,}924}
\expandafter\def\csname pct@sspro.records.model-id-match.haiku\endcsname{192400.0}
\expandafter\def\csname ppt@sspro.records.model-id-match.haiku\endcsname{$+$192400.0}
\expandafter\def\csname val@sspro.records.model-id-match.opus\endcsname{4042}
\expandafter\def\csname cnt@sspro.records.model-id-match.opus\endcsname{4{,}042}
\expandafter\def\csname pct@sspro.records.model-id-match.opus\endcsname{404200.0}
\expandafter\def\csname ppt@sspro.records.model-id-match.opus\endcsname{$+$404200.0}
\expandafter\def\csname val@sspro.records.model-id-match.sonnet\endcsname{3818}
\expandafter\def\csname cnt@sspro.records.model-id-match.sonnet\endcsname{3{,}818}
\expandafter\def\csname pct@sspro.records.model-id-match.sonnet\endcsname{381800.0}
\expandafter\def\csname ppt@sspro.records.model-id-match.sonnet\endcsname{$+$381800.0}
\expandafter\def\csname val@sspro.records.model-id-mismatches\endcsname{0}
\expandafter\def\csname cnt@sspro.records.model-id-mismatches\endcsname{0}
\expandafter\def\csname pct@sspro.records.model-id-mismatches\endcsname{0.0}
\expandafter\def\csname ppt@sspro.records.model-id-mismatches\endcsname{0.0}
\expandafter\def\csname val@sspro.records.model.haiku\endcsname{2669}
\expandafter\def\csname cnt@sspro.records.model.haiku\endcsname{2{,}669}
\expandafter\def\csname pct@sspro.records.model.haiku\endcsname{266900.0}
\expandafter\def\csname ppt@sspro.records.model.haiku\endcsname{$+$266900.0}
\expandafter\def\csname val@sspro.records.model.opus\endcsname{5302}
\expandafter\def\csname cnt@sspro.records.model.opus\endcsname{5{,}302}
\expandafter\def\csname pct@sspro.records.model.opus\endcsname{530200.0}
\expandafter\def\csname ppt@sspro.records.model.opus\endcsname{$+$530200.0}
\expandafter\def\csname val@sspro.records.model.sonnet\endcsname{5014}
\expandafter\def\csname cnt@sspro.records.model.sonnet\endcsname{5{,}014}
\expandafter\def\csname pct@sspro.records.model.sonnet\endcsname{501400.0}
\expandafter\def\csname ppt@sspro.records.model.sonnet\endcsname{$+$501400.0}
\expandafter\def\csname val@sspro.records.ok-requests\endcsname{9784}
\expandafter\def\csname cnt@sspro.records.ok-requests\endcsname{9{,}784}
\expandafter\def\csname pct@sspro.records.ok-requests\endcsname{978400.0}
\expandafter\def\csname ppt@sspro.records.ok-requests\endcsname{$+$978400.0}
\expandafter\def\csname val@sspro.records.requests\endcsname{12985}
\expandafter\def\csname cnt@sspro.records.requests\endcsname{12{,}985}
\expandafter\def\csname pct@sspro.records.requests\endcsname{1298500.0}
\expandafter\def\csname ppt@sspro.records.requests\endcsname{$+$1298500.0}
\expandafter\def\csname val@sspro.records.status.harness-failed\endcsname{3201}
\expandafter\def\csname cnt@sspro.records.status.harness-failed\endcsname{3{,}201}
\expandafter\def\csname pct@sspro.records.status.harness-failed\endcsname{320100.0}
\expandafter\def\csname ppt@sspro.records.status.harness-failed\endcsname{$+$320100.0}
\expandafter\def\csname val@sspro.records.status.ok\endcsname{9784}
\expandafter\def\csname cnt@sspro.records.status.ok\endcsname{9{,}784}
\expandafter\def\csname pct@sspro.records.status.ok\endcsname{978400.0}
\expandafter\def\csname ppt@sspro.records.status.ok\endcsname{$+$978400.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-box.api-calls\endcsname{3.400}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-box.api-calls\endcsname{3}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-box.api-calls\endcsname{340.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-box.api-calls\endcsname{$+$340.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{17278.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{17{,}279}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{1727890.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{$+$1727890.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{117858.800}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{117{,}859}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{11785880.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{$+$11785880.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-box.input-tokens\endcsname{6.300}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-box.input-tokens\endcsname{6}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-box.input-tokens\endcsname{630.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-box.input-tokens\endcsname{$+$630.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-box.output-tokens\endcsname{503.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-box.output-tokens\endcsname{504}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-box.output-tokens\endcsname{50390.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-box.output-tokens\endcsname{$+$50390.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-box.thinking-tokens\endcsname{164.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-box.thinking-tokens\endcsname{165}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-box.thinking-tokens\endcsname{16490.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-box.thinking-tokens\endcsname{$+$16490.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-cell.api-calls\endcsname{4.400}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-cell.api-calls\endcsname{4}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-cell.api-calls\endcsname{440.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-cell.api-calls\endcsname{$+$440.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{24210.400}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{24{,}210}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{2421040.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{$+$2421040.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{158559.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{158{,}559}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{15855910.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{$+$15855910.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-cell.input-tokens\endcsname{8.400}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-cell.input-tokens\endcsname{8}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-cell.input-tokens\endcsname{840.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-cell.input-tokens\endcsname{$+$840.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-cell.output-tokens\endcsname{865.300}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-cell.output-tokens\endcsname{865}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-cell.output-tokens\endcsname{86530.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-cell.output-tokens\endcsname{$+$86530.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{189.500}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{190}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{18950.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{$+$18950.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{4.700}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{5}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{470.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{$+$470.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{25329.600}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{25{,}330}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{2532960.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{$+$2532960.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{171199.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{171{,}200}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{17119990.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{$+$17119990.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{9.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{9}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{910.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{$+$910.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{965.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{966}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{96590.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{$+$96590.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{199.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{199}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{19910.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{$+$19910.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual.api-calls\endcsname{3.300}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual.api-calls\endcsname{3}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual.api-calls\endcsname{330.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual.api-calls\endcsname{$+$330.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{16066.700}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{16{,}067}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{1606670.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{$+$1606670.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{109385.700}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{109{,}386}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{10938570.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{$+$10938570.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual.input-tokens\endcsname{5.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual.input-tokens\endcsname{6}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual.input-tokens\endcsname{590.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual.input-tokens\endcsname{$+$590.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual.output-tokens\endcsname{492.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual.output-tokens\endcsname{492}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual.output-tokens\endcsname{49210.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual.output-tokens\endcsname{$+$49210.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{166.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{166}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{16610.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{$+$16610.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-point.api-calls\endcsname{3.600}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-point.api-calls\endcsname{4}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-point.api-calls\endcsname{360.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-point.api-calls\endcsname{$+$360.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{20180.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{20{,}181}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{2018090.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{$+$2018090.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{126392.200}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{126{,}392}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{12639220.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{$+$12639220.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-point.input-tokens\endcsname{6.900}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-point.input-tokens\endcsname{7}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-point.input-tokens\endcsname{690.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-point.input-tokens\endcsname{$+$690.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-point.output-tokens\endcsname{496.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-point.output-tokens\endcsname{496}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-point.output-tokens\endcsname{49610.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-point.output-tokens\endcsname{$+$49610.0}
\expandafter\def\csname val@sspro.records.usage-per-request.acquire-point.thinking-tokens\endcsname{147.200}
\expandafter\def\csname cnt@sspro.records.usage-per-request.acquire-point.thinking-tokens\endcsname{147}
\expandafter\def\csname pct@sspro.records.usage-per-request.acquire-point.thinking-tokens\endcsname{14720.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.acquire-point.thinking-tokens\endcsname{$+$14720.0}
\expandafter\def\csname val@sspro.records.usage-per-request.direct.api-calls\endcsname{3.500}
\expandafter\def\csname cnt@sspro.records.usage-per-request.direct.api-calls\endcsname{4}
\expandafter\def\csname pct@sspro.records.usage-per-request.direct.api-calls\endcsname{350.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.direct.api-calls\endcsname{$+$350.0}
\expandafter\def\csname val@sspro.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{18613.300}
\expandafter\def\csname cnt@sspro.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{18{,}613}
\expandafter\def\csname pct@sspro.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{1861330.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{$+$1861330.0}
\expandafter\def\csname val@sspro.records.usage-per-request.direct.cache-read-input-tokens\endcsname{119219.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.direct.cache-read-input-tokens\endcsname{119{,}219}
\expandafter\def\csname pct@sspro.records.usage-per-request.direct.cache-read-input-tokens\endcsname{11921910.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.direct.cache-read-input-tokens\endcsname{$+$11921910.0}
\expandafter\def\csname val@sspro.records.usage-per-request.direct.input-tokens\endcsname{6.500}
\expandafter\def\csname cnt@sspro.records.usage-per-request.direct.input-tokens\endcsname{6}
\expandafter\def\csname pct@sspro.records.usage-per-request.direct.input-tokens\endcsname{650.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.direct.input-tokens\endcsname{$+$650.0}
\expandafter\def\csname val@sspro.records.usage-per-request.direct.output-tokens\endcsname{523.400}
\expandafter\def\csname cnt@sspro.records.usage-per-request.direct.output-tokens\endcsname{523}
\expandafter\def\csname pct@sspro.records.usage-per-request.direct.output-tokens\endcsname{52340.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.direct.output-tokens\endcsname{$+$52340.0}
\expandafter\def\csname val@sspro.records.usage-per-request.direct.thinking-tokens\endcsname{196.200}
\expandafter\def\csname cnt@sspro.records.usage-per-request.direct.thinking-tokens\endcsname{196}
\expandafter\def\csname pct@sspro.records.usage-per-request.direct.thinking-tokens\endcsname{19620.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.direct.thinking-tokens\endcsname{$+$19620.0}
\expandafter\def\csname val@sspro.records.usage-per-request.read.api-calls\endcsname{4.000}
\expandafter\def\csname cnt@sspro.records.usage-per-request.read.api-calls\endcsname{4}
\expandafter\def\csname pct@sspro.records.usage-per-request.read.api-calls\endcsname{400.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.read.api-calls\endcsname{$+$400.0}
\expandafter\def\csname val@sspro.records.usage-per-request.read.cache-creation-input-tokens\endcsname{22441.700}
\expandafter\def\csname cnt@sspro.records.usage-per-request.read.cache-creation-input-tokens\endcsname{22{,}442}
\expandafter\def\csname pct@sspro.records.usage-per-request.read.cache-creation-input-tokens\endcsname{2244170.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.read.cache-creation-input-tokens\endcsname{$+$2244170.0}
\expandafter\def\csname val@sspro.records.usage-per-request.read.cache-read-input-tokens\endcsname{139202.700}
\expandafter\def\csname cnt@sspro.records.usage-per-request.read.cache-read-input-tokens\endcsname{139{,}203}
\expandafter\def\csname pct@sspro.records.usage-per-request.read.cache-read-input-tokens\endcsname{13920270.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.read.cache-read-input-tokens\endcsname{$+$13920270.0}
\expandafter\def\csname val@sspro.records.usage-per-request.read.input-tokens\endcsname{7.500}
\expandafter\def\csname cnt@sspro.records.usage-per-request.read.input-tokens\endcsname{8}
\expandafter\def\csname pct@sspro.records.usage-per-request.read.input-tokens\endcsname{750.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.read.input-tokens\endcsname{$+$750.0}
\expandafter\def\csname val@sspro.records.usage-per-request.read.output-tokens\endcsname{717.100}
\expandafter\def\csname cnt@sspro.records.usage-per-request.read.output-tokens\endcsname{717}
\expandafter\def\csname pct@sspro.records.usage-per-request.read.output-tokens\endcsname{71710.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.read.output-tokens\endcsname{$+$71710.0}
\expandafter\def\csname val@sspro.records.usage-per-request.read.thinking-tokens\endcsname{123.600}
\expandafter\def\csname cnt@sspro.records.usage-per-request.read.thinking-tokens\endcsname{124}
\expandafter\def\csname pct@sspro.records.usage-per-request.read.thinking-tokens\endcsname{12360.0}
\expandafter\def\csname ppt@sspro.records.usage-per-request.read.thinking-tokens\endcsname{$+$12360.0}
\expandafter\def\csname val@sspro.records.usage.api-calls\endcsname{49962}
\expandafter\def\csname cnt@sspro.records.usage.api-calls\endcsname{49{,}962}
\expandafter\def\csname pct@sspro.records.usage.api-calls\endcsname{4996200.0}
\expandafter\def\csname ppt@sspro.records.usage.api-calls\endcsname{$+$4996200.0}
\expandafter\def\csname val@sspro.records.usage.cache-creation-input-tokens\endcsname{271862339}
\expandafter\def\csname cnt@sspro.records.usage.cache-creation-input-tokens\endcsname{271{,}862{,}339}
\expandafter\def\csname pct@sspro.records.usage.cache-creation-input-tokens\endcsname{27186233900.0}
\expandafter\def\csname ppt@sspro.records.usage.cache-creation-input-tokens\endcsname{$+$27186233900.0}
\expandafter\def\csname val@sspro.records.usage.cache-read-input-tokens\endcsname{1745257909}
\expandafter\def\csname cnt@sspro.records.usage.cache-read-input-tokens\endcsname{1{,}745{,}257{,}909}
\expandafter\def\csname pct@sspro.records.usage.cache-read-input-tokens\endcsname{174525790900.0}
\expandafter\def\csname ppt@sspro.records.usage.cache-read-input-tokens\endcsname{$+$174525790900.0}
\expandafter\def\csname val@sspro.records.usage.input-tokens\endcsname{94082}
\expandafter\def\csname cnt@sspro.records.usage.input-tokens\endcsname{94{,}082}
\expandafter\def\csname pct@sspro.records.usage.input-tokens\endcsname{9408200.0}
\expandafter\def\csname ppt@sspro.records.usage.input-tokens\endcsname{$+$9408200.0}
\expandafter\def\csname val@sspro.records.usage.output-tokens\endcsname{8541696}
\expandafter\def\csname cnt@sspro.records.usage.output-tokens\endcsname{8{,}541{,}696}
\expandafter\def\csname pct@sspro.records.usage.output-tokens\endcsname{854169600.0}
\expandafter\def\csname ppt@sspro.records.usage.output-tokens\endcsname{$+$854169600.0}
\expandafter\def\csname val@sspro.records.usage.thinking-tokens\endcsname{2031958}
\expandafter\def\csname cnt@sspro.records.usage.thinking-tokens\endcsname{2{,}031{,}958}
\expandafter\def\csname pct@sspro.records.usage.thinking-tokens\endcsname{203195800.0}
\expandafter\def\csname ppt@sspro.records.usage.thinking-tokens\endcsname{$+$203195800.0}
\expandafter\def\csname val@sspro.tasks.A.n-apps\endcsname{4}
\expandafter\def\csname cnt@sspro.tasks.A.n-apps\endcsname{4}
\expandafter\def\csname pct@sspro.tasks.A.n-apps\endcsname{400.0}
\expandafter\def\csname ppt@sspro.tasks.A.n-apps\endcsname{$+$400.0}
\expandafter\def\csname val@sspro.tasks.A.n-tasks\endcsname{32}
\expandafter\def\csname cnt@sspro.tasks.A.n-tasks\endcsname{32}
\expandafter\def\csname pct@sspro.tasks.A.n-tasks\endcsname{3200.0}
\expandafter\def\csname ppt@sspro.tasks.A.n-tasks\endcsname{$+$3200.0}
\expandafter\def\csname val@sspro.tasks.C.n-apps\endcsname{6}
\expandafter\def\csname cnt@sspro.tasks.C.n-apps\endcsname{6}
\expandafter\def\csname pct@sspro.tasks.C.n-apps\endcsname{600.0}
\expandafter\def\csname ppt@sspro.tasks.C.n-apps\endcsname{$+$600.0}
\expandafter\def\csname val@sspro.tasks.C.n-tasks\endcsname{48}
\expandafter\def\csname cnt@sspro.tasks.C.n-tasks\endcsname{48}
\expandafter\def\csname pct@sspro.tasks.C.n-tasks\endcsname{4800.0}
\expandafter\def\csname ppt@sspro.tasks.C.n-tasks\endcsname{$+$4800.0}
\expandafter\def\csname val@sspro.tasks.T.n-apps\endcsname{12}
\expandafter\def\csname cnt@sspro.tasks.T.n-apps\endcsname{12}
\expandafter\def\csname pct@sspro.tasks.T.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@sspro.tasks.T.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@sspro.tasks.T.n-tasks\endcsname{96}
\expandafter\def\csname cnt@sspro.tasks.T.n-tasks\endcsname{96}
\expandafter\def\csname pct@sspro.tasks.T.n-tasks\endcsname{9600.0}
\expandafter\def\csname ppt@sspro.tasks.T.n-tasks\endcsname{$+$9600.0}
\expandafter\def\csname val@sspro.tasks.n-apps\endcsname{22}
\expandafter\def\csname cnt@sspro.tasks.n-apps\endcsname{22}
\expandafter\def\csname pct@sspro.tasks.n-apps\endcsname{2200.0}
\expandafter\def\csname ppt@sspro.tasks.n-apps\endcsname{$+$2200.0}
\expandafter\def\csname val@sspro.tasks.n-tasks\endcsname{176}
\expandafter\def\csname cnt@sspro.tasks.n-tasks\endcsname{176}
\expandafter\def\csname pct@sspro.tasks.n-tasks\endcsname{17600.0}
\expandafter\def\csname ppt@sspro.tasks.n-tasks\endcsname{$+$17600.0}
\expandafter\def\csname val@summary.all.agree-stable-resid-perskill.max\endcsname{0.081}
\expandafter\def\csname cnt@summary.all.agree-stable-resid-perskill.max\endcsname{0}
\expandafter\def\csname pct@summary.all.agree-stable-resid-perskill.max\endcsname{8.1}
\expandafter\def\csname ppt@summary.all.agree-stable-resid-perskill.max\endcsname{$+$8.1}
\expandafter\def\csname val@summary.all.agree-stable-resid-perskill.min\endcsname{-0.057}
\expandafter\def\csname cnt@summary.all.agree-stable-resid-perskill.min\endcsname{0}
\expandafter\def\csname pct@summary.all.agree-stable-resid-perskill.min\endcsname{$-$5.7}
\expandafter\def\csname ppt@summary.all.agree-stable-resid-perskill.min\endcsname{$-$5.7}
\expandafter\def\csname val@summary.all.agree-stable-resid.max\endcsname{0.018}
\expandafter\def\csname cnt@summary.all.agree-stable-resid.max\endcsname{0}
\expandafter\def\csname pct@summary.all.agree-stable-resid.max\endcsname{1.8}
\expandafter\def\csname ppt@summary.all.agree-stable-resid.max\endcsname{$+$1.8}
\expandafter\def\csname val@summary.all.agree-stable-resid.min\endcsname{-0.013}
\expandafter\def\csname cnt@summary.all.agree-stable-resid.min\endcsname{0}
\expandafter\def\csname pct@summary.all.agree-stable-resid.min\endcsname{$-$1.2}
\expandafter\def\csname ppt@summary.all.agree-stable-resid.min\endcsname{$-$1.2}
\expandafter\def\csname val@summary.all.agree-stable-share.max\endcsname{0.889}
\expandafter\def\csname cnt@summary.all.agree-stable-share.max\endcsname{1}
\expandafter\def\csname pct@summary.all.agree-stable-share.max\endcsname{88.9}
\expandafter\def\csname ppt@summary.all.agree-stable-share.max\endcsname{$+$88.9}
\expandafter\def\csname val@summary.all.agree-stable-share.min\endcsname{0.706}
\expandafter\def\csname cnt@summary.all.agree-stable-share.min\endcsname{1}
\expandafter\def\csname pct@summary.all.agree-stable-share.min\endcsname{70.6}
\expandafter\def\csname ppt@summary.all.agree-stable-share.min\endcsname{$+$70.6}
\expandafter\def\csname val@summary.all.disagree-gap.max\endcsname{0.253}
\expandafter\def\csname cnt@summary.all.disagree-gap.max\endcsname{0}
\expandafter\def\csname pct@summary.all.disagree-gap.max\endcsname{25.3}
\expandafter\def\csname ppt@summary.all.disagree-gap.max\endcsname{$+$25.3}
\expandafter\def\csname val@summary.all.disagree-gap.min\endcsname{0.017}
\expandafter\def\csname cnt@summary.all.disagree-gap.min\endcsname{0}
\expandafter\def\csname pct@summary.all.disagree-gap.min\endcsname{1.7}
\expandafter\def\csname ppt@summary.all.disagree-gap.min\endcsname{$+$1.7}
\expandafter\def\csname val@summary.all.disagree-gap.n\endcsname{6}
\expandafter\def\csname cnt@summary.all.disagree-gap.n\endcsname{6}
\expandafter\def\csname pct@summary.all.disagree-gap.n\endcsname{600.0}
\expandafter\def\csname ppt@summary.all.disagree-gap.n\endcsname{$+$600.0}
\expandafter\def\csname val@summary.all.disagree-gap.n-positive\endcsname{6}
\expandafter\def\csname cnt@summary.all.disagree-gap.n-positive\endcsname{6}
\expandafter\def\csname pct@summary.all.disagree-gap.n-positive\endcsname{600.0}
\expandafter\def\csname ppt@summary.all.disagree-gap.n-positive\endcsname{$+$600.0}
\expandafter\def\csname val@summary.all.disagree-share.max\endcsname{0.182}
\expandafter\def\csname cnt@summary.all.disagree-share.max\endcsname{0}
\expandafter\def\csname pct@summary.all.disagree-share.max\endcsname{18.2}
\expandafter\def\csname ppt@summary.all.disagree-share.max\endcsname{$+$18.2}
\expandafter\def\csname val@summary.all.disagree-share.min\endcsname{0.082}
\expandafter\def\csname cnt@summary.all.disagree-share.min\endcsname{0}
\expandafter\def\csname pct@summary.all.disagree-share.min\endcsname{8.2}
\expandafter\def\csname ppt@summary.all.disagree-share.min\endcsname{$+$8.2}
\expandafter\def\csname val@summary.all.holm-p.max\endcsname{0.165}
\expandafter\def\csname cnt@summary.all.holm-p.max\endcsname{0}
\expandafter\def\csname pct@summary.all.holm-p.max\endcsname{16.5}
\expandafter\def\csname ppt@summary.all.holm-p.max\endcsname{$+$16.5}
\expandafter\def\csname val@summary.all.holm-p.min\endcsname{0.002}
\expandafter\def\csname cnt@summary.all.holm-p.min\endcsname{0}
\expandafter\def\csname pct@summary.all.holm-p.min\endcsname{0.2}
\expandafter\def\csname ppt@summary.all.holm-p.min\endcsname{$+$0.2}
\expandafter\def\csname val@summary.all.loo-comparisons\endcsname{8}
\expandafter\def\csname cnt@summary.all.loo-comparisons\endcsname{8}
\expandafter\def\csname pct@summary.all.loo-comparisons\endcsname{800.0}
\expandafter\def\csname ppt@summary.all.loo-comparisons\endcsname{$+$800.0}
\expandafter\def\csname val@summary.all.loo-min\endcsname{0.000}
\expandafter\def\csname cnt@summary.all.loo-min\endcsname{0}
\expandafter\def\csname pct@summary.all.loo-min\endcsname{0.0}
\expandafter\def\csname ppt@summary.all.loo-min\endcsname{0.0}
\expandafter\def\csname val@summary.all.loo-n-negative\endcsname{0}
\expandafter\def\csname cnt@summary.all.loo-n-negative\endcsname{0}
\expandafter\def\csname pct@summary.all.loo-n-negative\endcsname{0.0}
\expandafter\def\csname ppt@summary.all.loo-n-negative\endcsname{0.0}
\expandafter\def\csname val@summary.all.ni-pass\endcsname{3}
\expandafter\def\csname cnt@summary.all.ni-pass\endcsname{3}
\expandafter\def\csname pct@summary.all.ni-pass\endcsname{300.0}
\expandafter\def\csname ppt@summary.all.ni-pass\endcsname{$+$300.0}
\expandafter\def\csname val@summary.all.ni-settings\endcsname{4}
\expandafter\def\csname cnt@summary.all.ni-settings\endcsname{4}
\expandafter\def\csname pct@summary.all.ni-settings\endcsname{400.0}
\expandafter\def\csname ppt@summary.all.ni-settings\endcsname{$+$400.0}
\expandafter\def\csname val@summary.all.old-decision-ge-rcr\endcsname{3}
\expandafter\def\csname cnt@summary.all.old-decision-ge-rcr\endcsname{3}
\expandafter\def\csname pct@summary.all.old-decision-ge-rcr\endcsname{300.0}
\expandafter\def\csname ppt@summary.all.old-decision-ge-rcr\endcsname{$+$300.0}
\expandafter\def\csname val@summary.all.old-decision-vs-rcr-n\endcsname{4}
\expandafter\def\csname cnt@summary.all.old-decision-vs-rcr-n\endcsname{4}
\expandafter\def\csname pct@summary.all.old-decision-vs-rcr-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.all.old-decision-vs-rcr-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.all.primary-gain.max\endcsname{0.013}
\expandafter\def\csname cnt@summary.all.primary-gain.max\endcsname{0}
\expandafter\def\csname pct@summary.all.primary-gain.max\endcsname{1.3}
\expandafter\def\csname ppt@summary.all.primary-gain.max\endcsname{$+$1.3}
\expandafter\def\csname val@summary.all.primary-gain.min\endcsname{0.001}
\expandafter\def\csname cnt@summary.all.primary-gain.min\endcsname{0}
\expandafter\def\csname pct@summary.all.primary-gain.min\endcsname{0.1}
\expandafter\def\csname ppt@summary.all.primary-gain.min\endcsname{$+$0.1}
\expandafter\def\csname val@summary.all.rcr-cost-fraction.max\endcsname{0.731}
\expandafter\def\csname cnt@summary.all.rcr-cost-fraction.max\endcsname{1}
\expandafter\def\csname pct@summary.all.rcr-cost-fraction.max\endcsname{73.1}
\expandafter\def\csname ppt@summary.all.rcr-cost-fraction.max\endcsname{$+$73.1}
\expandafter\def\csname val@summary.all.rcr-cost-fraction.min\endcsname{0.718}
\expandafter\def\csname cnt@summary.all.rcr-cost-fraction.min\endcsname{1}
\expandafter\def\csname pct@summary.all.rcr-cost-fraction.min\endcsname{71.8}
\expandafter\def\csname ppt@summary.all.rcr-cost-fraction.min\endcsname{$+$71.8}
\expandafter\def\csname val@summary.all.replay-cost-fraction-of-rcr.max\endcsname{0.750}
\expandafter\def\csname cnt@summary.all.replay-cost-fraction-of-rcr.max\endcsname{1}
\expandafter\def\csname pct@summary.all.replay-cost-fraction-of-rcr.max\endcsname{75.0}
\expandafter\def\csname ppt@summary.all.replay-cost-fraction-of-rcr.max\endcsname{$+$75.0}
\expandafter\def\csname val@summary.all.replay-cost-fraction-of-rcr.min\endcsname{0.745}
\expandafter\def\csname cnt@summary.all.replay-cost-fraction-of-rcr.min\endcsname{1}
\expandafter\def\csname pct@summary.all.replay-cost-fraction-of-rcr.min\endcsname{74.5}
\expandafter\def\csname ppt@summary.all.replay-cost-fraction-of-rcr.min\endcsname{$+$74.5}
\expandafter\def\csname val@summary.all.replay-only-ge-rcr\endcsname{4}
\expandafter\def\csname cnt@summary.all.replay-only-ge-rcr\endcsname{4}
\expandafter\def\csname pct@summary.all.replay-only-ge-rcr\endcsname{400.0}
\expandafter\def\csname ppt@summary.all.replay-only-ge-rcr\endcsname{$+$400.0}
\expandafter\def\csname val@summary.all.replay-only-vs-rcr-n\endcsname{4}
\expandafter\def\csname cnt@summary.all.replay-only-vs-rcr-n\endcsname{4}
\expandafter\def\csname pct@summary.all.replay-only-vs-rcr-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.all.replay-only-vs-rcr-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.best-single-above-replay\endcsname{1}
\expandafter\def\csname cnt@summary.best-single-above-replay\endcsname{1}
\expandafter\def\csname pct@summary.best-single-above-replay\endcsname{100.0}
\expandafter\def\csname ppt@summary.best-single-above-replay\endcsname{$+$100.0}
\expandafter\def\csname val@summary.e3.C.n\endcsname{4}
\expandafter\def\csname cnt@summary.e3.C.n\endcsname{4}
\expandafter\def\csname pct@summary.e3.C.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.e3.C.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.e3.C.n-ci-includes-0\endcsname{2}
\expandafter\def\csname cnt@summary.e3.C.n-ci-includes-0\endcsname{2}
\expandafter\def\csname pct@summary.e3.C.n-ci-includes-0\endcsname{200.0}
\expandafter\def\csname ppt@summary.e3.C.n-ci-includes-0\endcsname{$+$200.0}
\expandafter\def\csname val@summary.e4.sspro.max\endcsname{0.104}
\expandafter\def\csname cnt@summary.e4.sspro.max\endcsname{0}
\expandafter\def\csname pct@summary.e4.sspro.max\endcsname{10.4}
\expandafter\def\csname ppt@summary.e4.sspro.max\endcsname{$+$10.4}
\expandafter\def\csname val@summary.e4.sspro.min\endcsname{0.000}
\expandafter\def\csname cnt@summary.e4.sspro.min\endcsname{0}
\expandafter\def\csname pct@summary.e4.sspro.min\endcsname{0.0}
\expandafter\def\csname ppt@summary.e4.sspro.min\endcsname{0.0}
\expandafter\def\csname val@summary.e4.uiv.max\endcsname{0.058}
\expandafter\def\csname cnt@summary.e4.uiv.max\endcsname{0}
\expandafter\def\csname pct@summary.e4.uiv.max\endcsname{5.8}
\expandafter\def\csname ppt@summary.e4.uiv.max\endcsname{$+$5.8}
\expandafter\def\csname val@summary.e4.uiv.min\endcsname{-0.008}
\expandafter\def\csname cnt@summary.e4.uiv.min\endcsname{0}
\expandafter\def\csname pct@summary.e4.uiv.min\endcsname{$-$0.8}
\expandafter\def\csname ppt@summary.e4.uiv.min\endcsname{$-$0.8}
\expandafter\def\csname val@summary.e6.generic-ppi-source.max\endcsname{0.003}
\expandafter\def\csname cnt@summary.e6.generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@summary.e6.generic-ppi-source.max\endcsname{0.3}
\expandafter\def\csname ppt@summary.e6.generic-ppi-source.max\endcsname{$+$0.3}
\expandafter\def\csname val@summary.e6.generic-ppi-source.min\endcsname{-0.001}
\expandafter\def\csname cnt@summary.e6.generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@summary.e6.generic-ppi-source.min\endcsname{$-$0.1}
\expandafter\def\csname ppt@summary.e6.generic-ppi-source.min\endcsname{$-$0.1}
\expandafter\def\csname val@summary.e6.n\endcsname{16}
\expandafter\def\csname cnt@summary.e6.n\endcsname{16}
\expandafter\def\csname pct@summary.e6.n\endcsname{1600.0}
\expandafter\def\csname ppt@summary.e6.n\endcsname{$+$1600.0}
\expandafter\def\csname val@summary.e6.n-ci-includes-0\endcsname{16}
\expandafter\def\csname cnt@summary.e6.n-ci-includes-0\endcsname{16}
\expandafter\def\csname pct@summary.e6.n-ci-includes-0\endcsname{1600.0}
\expandafter\def\csname ppt@summary.e6.n-ci-includes-0\endcsname{$+$1600.0}
\expandafter\def\csname val@summary.e6.replay-only.max\endcsname{-0.002}
\expandafter\def\csname cnt@summary.e6.replay-only.max\endcsname{0}
\expandafter\def\csname pct@summary.e6.replay-only.max\endcsname{$-$0.2}
\expandafter\def\csname ppt@summary.e6.replay-only.max\endcsname{$-$0.2}
\expandafter\def\csname val@summary.e6.replay-only.min\endcsname{-0.023}
\expandafter\def\csname cnt@summary.e6.replay-only.min\endcsname{0}
\expandafter\def\csname pct@summary.e6.replay-only.min\endcsname{$-$2.3}
\expandafter\def\csname ppt@summary.e6.replay-only.min\endcsname{$-$2.3}
\expandafter\def\csname val@summary.e6.replay-ppi-uniform.max\endcsname{0.002}
\expandafter\def\csname cnt@summary.e6.replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@summary.e6.replay-ppi-uniform.max\endcsname{0.2}
\expandafter\def\csname ppt@summary.e6.replay-ppi-uniform.max\endcsname{$+$0.2}
\expandafter\def\csname val@summary.e6.replay-ppi-uniform.min\endcsname{-0.001}
\expandafter\def\csname cnt@summary.e6.replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@summary.e6.replay-ppi-uniform.min\endcsname{$-$0.1}
\expandafter\def\csname ppt@summary.e6.replay-ppi-uniform.min\endcsname{$-$0.1}
\expandafter\def\csname val@summary.e6.uniform-fresh.max\endcsname{0.010}
\expandafter\def\csname cnt@summary.e6.uniform-fresh.max\endcsname{0}
\expandafter\def\csname pct@summary.e6.uniform-fresh.max\endcsname{1.0}
\expandafter\def\csname ppt@summary.e6.uniform-fresh.max\endcsname{$+$1.0}
\expandafter\def\csname val@summary.e6.uniform-fresh.min\endcsname{-0.004}
\expandafter\def\csname cnt@summary.e6.uniform-fresh.min\endcsname{0}
\expandafter\def\csname pct@summary.e6.uniform-fresh.min\endcsname{$-$0.4}
\expandafter\def\csname ppt@summary.e6.uniform-fresh.min\endcsname{$-$0.4}
\expandafter\def\csname val@summary.eqcost.best-single.max\endcsname{0.009}
\expandafter\def\csname cnt@summary.eqcost.best-single.max\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.best-single.max\endcsname{0.9}
\expandafter\def\csname ppt@summary.eqcost.best-single.max\endcsname{$+$0.9}
\expandafter\def\csname val@summary.eqcost.best-single.min\endcsname{-0.015}
\expandafter\def\csname cnt@summary.eqcost.best-single.min\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.best-single.min\endcsname{$-$1.5}
\expandafter\def\csname ppt@summary.eqcost.best-single.min\endcsname{$-$1.5}
\expandafter\def\csname val@summary.eqcost.best-single.n\endcsname{4}
\expandafter\def\csname cnt@summary.eqcost.best-single.n\endcsname{4}
\expandafter\def\csname pct@summary.eqcost.best-single.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.eqcost.best-single.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.eqcost.best-single.n-ci-above-0\endcsname{0}
\expandafter\def\csname cnt@summary.eqcost.best-single.n-ci-above-0\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.best-single.n-ci-above-0\endcsname{0.0}
\expandafter\def\csname ppt@summary.eqcost.best-single.n-ci-above-0\endcsname{0.0}
\expandafter\def\csname val@summary.eqcost.best-single.n-ci-below-0\endcsname{2}
\expandafter\def\csname cnt@summary.eqcost.best-single.n-ci-below-0\endcsname{2}
\expandafter\def\csname pct@summary.eqcost.best-single.n-ci-below-0\endcsname{200.0}
\expandafter\def\csname ppt@summary.eqcost.best-single.n-ci-below-0\endcsname{$+$200.0}
\expandafter\def\csname val@summary.eqcost.generic-ppi-source.max\endcsname{0.005}
\expandafter\def\csname cnt@summary.eqcost.generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.generic-ppi-source.max\endcsname{0.5}
\expandafter\def\csname ppt@summary.eqcost.generic-ppi-source.max\endcsname{$+$0.5}
\expandafter\def\csname val@summary.eqcost.generic-ppi-source.min\endcsname{-0.005}
\expandafter\def\csname cnt@summary.eqcost.generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.generic-ppi-source.min\endcsname{$-$0.5}
\expandafter\def\csname ppt@summary.eqcost.generic-ppi-source.min\endcsname{$-$0.5}
\expandafter\def\csname val@summary.eqcost.generic-ppi-source.n\endcsname{4}
\expandafter\def\csname cnt@summary.eqcost.generic-ppi-source.n\endcsname{4}
\expandafter\def\csname pct@summary.eqcost.generic-ppi-source.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.eqcost.generic-ppi-source.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.eqcost.generic-ppi-source.n-ci-above-0\endcsname{1}
\expandafter\def\csname cnt@summary.eqcost.generic-ppi-source.n-ci-above-0\endcsname{1}
\expandafter\def\csname pct@summary.eqcost.generic-ppi-source.n-ci-above-0\endcsname{100.0}
\expandafter\def\csname ppt@summary.eqcost.generic-ppi-source.n-ci-above-0\endcsname{$+$100.0}
\expandafter\def\csname val@summary.eqcost.generic-ppi-source.n-ci-below-0\endcsname{2}
\expandafter\def\csname cnt@summary.eqcost.generic-ppi-source.n-ci-below-0\endcsname{2}
\expandafter\def\csname pct@summary.eqcost.generic-ppi-source.n-ci-below-0\endcsname{200.0}
\expandafter\def\csname ppt@summary.eqcost.generic-ppi-source.n-ci-below-0\endcsname{$+$200.0}
\expandafter\def\csname val@summary.eqcost.replay-ppi-uniform.max\endcsname{0.010}
\expandafter\def\csname cnt@summary.eqcost.replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.replay-ppi-uniform.max\endcsname{1.0}
\expandafter\def\csname ppt@summary.eqcost.replay-ppi-uniform.max\endcsname{$+$1.0}
\expandafter\def\csname val@summary.eqcost.replay-ppi-uniform.min\endcsname{0.001}
\expandafter\def\csname cnt@summary.eqcost.replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.replay-ppi-uniform.min\endcsname{0.1}
\expandafter\def\csname ppt@summary.eqcost.replay-ppi-uniform.min\endcsname{$+$0.1}
\expandafter\def\csname val@summary.eqcost.replay-ppi-uniform.n\endcsname{4}
\expandafter\def\csname cnt@summary.eqcost.replay-ppi-uniform.n\endcsname{4}
\expandafter\def\csname pct@summary.eqcost.replay-ppi-uniform.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.eqcost.replay-ppi-uniform.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.eqcost.replay-ppi-uniform.n-ci-above-0\endcsname{3}
\expandafter\def\csname cnt@summary.eqcost.replay-ppi-uniform.n-ci-above-0\endcsname{3}
\expandafter\def\csname pct@summary.eqcost.replay-ppi-uniform.n-ci-above-0\endcsname{300.0}
\expandafter\def\csname ppt@summary.eqcost.replay-ppi-uniform.n-ci-above-0\endcsname{$+$300.0}
\expandafter\def\csname val@summary.eqcost.replay-ppi-uniform.n-ci-below-0\endcsname{0}
\expandafter\def\csname cnt@summary.eqcost.replay-ppi-uniform.n-ci-below-0\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.replay-ppi-uniform.n-ci-below-0\endcsname{0.0}
\expandafter\def\csname ppt@summary.eqcost.replay-ppi-uniform.n-ci-below-0\endcsname{0.0}
\expandafter\def\csname val@summary.eqcost.uniform-fresh.max\endcsname{0.001}
\expandafter\def\csname cnt@summary.eqcost.uniform-fresh.max\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.uniform-fresh.max\endcsname{0.1}
\expandafter\def\csname ppt@summary.eqcost.uniform-fresh.max\endcsname{$+$0.1}
\expandafter\def\csname val@summary.eqcost.uniform-fresh.min\endcsname{-0.008}
\expandafter\def\csname cnt@summary.eqcost.uniform-fresh.min\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.uniform-fresh.min\endcsname{$-$0.8}
\expandafter\def\csname ppt@summary.eqcost.uniform-fresh.min\endcsname{$-$0.8}
\expandafter\def\csname val@summary.eqcost.uniform-fresh.n\endcsname{4}
\expandafter\def\csname cnt@summary.eqcost.uniform-fresh.n\endcsname{4}
\expandafter\def\csname pct@summary.eqcost.uniform-fresh.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.eqcost.uniform-fresh.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.eqcost.uniform-fresh.n-ci-above-0\endcsname{0}
\expandafter\def\csname cnt@summary.eqcost.uniform-fresh.n-ci-above-0\endcsname{0}
\expandafter\def\csname pct@summary.eqcost.uniform-fresh.n-ci-above-0\endcsname{0.0}
\expandafter\def\csname ppt@summary.eqcost.uniform-fresh.n-ci-above-0\endcsname{0.0}
\expandafter\def\csname val@summary.eqcost.uniform-fresh.n-ci-below-0\endcsname{2}
\expandafter\def\csname cnt@summary.eqcost.uniform-fresh.n-ci-below-0\endcsname{2}
\expandafter\def\csname pct@summary.eqcost.uniform-fresh.n-ci-below-0\endcsname{200.0}
\expandafter\def\csname ppt@summary.eqcost.uniform-fresh.n-ci-below-0\endcsname{$+$200.0}
\expandafter\def\csname val@summary.expl.agree-notcov.max\endcsname{0.103}
\expandafter\def\csname cnt@summary.expl.agree-notcov.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.agree-notcov.max\endcsname{10.3}
\expandafter\def\csname ppt@summary.expl.agree-notcov.max\endcsname{$+$10.3}
\expandafter\def\csname val@summary.expl.agree-notcov.min\endcsname{0.012}
\expandafter\def\csname cnt@summary.expl.agree-notcov.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.agree-notcov.min\endcsname{1.2}
\expandafter\def\csname ppt@summary.expl.agree-notcov.min\endcsname{$+$1.2}
\expandafter\def\csname val@summary.expl.covered-resid.max\endcsname{0.006}
\expandafter\def\csname cnt@summary.expl.covered-resid.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.covered-resid.max\endcsname{0.6}
\expandafter\def\csname ppt@summary.expl.covered-resid.max\endcsname{$+$0.6}
\expandafter\def\csname val@summary.expl.covered-resid.min\endcsname{-0.031}
\expandafter\def\csname cnt@summary.expl.covered-resid.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.covered-resid.min\endcsname{$-$3.1}
\expandafter\def\csname ppt@summary.expl.covered-resid.min\endcsname{$-$3.1}
\expandafter\def\csname val@summary.expl.disagree-notcov.max\endcsname{0.607}
\expandafter\def\csname cnt@summary.expl.disagree-notcov.max\endcsname{1}
\expandafter\def\csname pct@summary.expl.disagree-notcov.max\endcsname{60.7}
\expandafter\def\csname ppt@summary.expl.disagree-notcov.max\endcsname{$+$60.7}
\expandafter\def\csname val@summary.expl.disagree-notcov.min\endcsname{0.270}
\expandafter\def\csname cnt@summary.expl.disagree-notcov.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.disagree-notcov.min\endcsname{27.0}
\expandafter\def\csname ppt@summary.expl.disagree-notcov.min\endcsname{$+$27.0}
\expandafter\def\csname val@summary.expl.eqcost-simpler-more-accurate\endcsname{4}
\expandafter\def\csname cnt@summary.expl.eqcost-simpler-more-accurate\endcsname{4}
\expandafter\def\csname pct@summary.expl.eqcost-simpler-more-accurate\endcsname{400.0}
\expandafter\def\csname ppt@summary.expl.eqcost-simpler-more-accurate\endcsname{$+$400.0}
\expandafter\def\csname val@summary.expl.err-share-missed.max\endcsname{0.733}
\expandafter\def\csname cnt@summary.expl.err-share-missed.max\endcsname{1}
\expandafter\def\csname pct@summary.expl.err-share-missed.max\endcsname{73.3}
\expandafter\def\csname ppt@summary.expl.err-share-missed.max\endcsname{$+$73.3}
\expandafter\def\csname val@summary.expl.err-share-missed.min\endcsname{0.359}
\expandafter\def\csname cnt@summary.expl.err-share-missed.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.err-share-missed.min\endcsname{35.9}
\expandafter\def\csname ppt@summary.expl.err-share-missed.min\endcsname{$+$35.9}
\expandafter\def\csname val@summary.expl.flag-in-disagree.max\endcsname{1.000}
\expandafter\def\csname cnt@summary.expl.flag-in-disagree.max\endcsname{1}
\expandafter\def\csname pct@summary.expl.flag-in-disagree.max\endcsname{100.0}
\expandafter\def\csname ppt@summary.expl.flag-in-disagree.max\endcsname{$+$100.0}
\expandafter\def\csname val@summary.expl.flag-in-disagree.min\endcsname{0.756}
\expandafter\def\csname cnt@summary.expl.flag-in-disagree.min\endcsname{1}
\expandafter\def\csname pct@summary.expl.flag-in-disagree.min\endcsname{75.6}
\expandafter\def\csname ppt@summary.expl.flag-in-disagree.min\endcsname{$+$75.6}
\expandafter\def\csname val@summary.expl.flag-outside-agree.max\endcsname{1.000}
\expandafter\def\csname cnt@summary.expl.flag-outside-agree.max\endcsname{1}
\expandafter\def\csname pct@summary.expl.flag-outside-agree.max\endcsname{100.0}
\expandafter\def\csname ppt@summary.expl.flag-outside-agree.max\endcsname{$+$100.0}
\expandafter\def\csname val@summary.expl.flag-outside-agree.min\endcsname{0.947}
\expandafter\def\csname cnt@summary.expl.flag-outside-agree.min\endcsname{1}
\expandafter\def\csname pct@summary.expl.flag-outside-agree.min\endcsname{94.7}
\expandafter\def\csname ppt@summary.expl.flag-outside-agree.min\endcsname{$+$94.7}
\expandafter\def\csname val@summary.expl.loo-c.n\endcsname{36}
\expandafter\def\csname cnt@summary.expl.loo-c.n\endcsname{36}
\expandafter\def\csname pct@summary.expl.loo-c.n\endcsname{3600.0}
\expandafter\def\csname ppt@summary.expl.loo-c.n\endcsname{$+$3600.0}
\expandafter\def\csname val@summary.expl.loo-c.rcr-below-replay\endcsname{33}
\expandafter\def\csname cnt@summary.expl.loo-c.rcr-below-replay\endcsname{33}
\expandafter\def\csname pct@summary.expl.loo-c.rcr-below-replay\endcsname{3300.0}
\expandafter\def\csname ppt@summary.expl.loo-c.rcr-below-replay\endcsname{$+$3300.0}
\expandafter\def\csname val@summary.expl.multi-missed-accR.max\endcsname{0.167}
\expandafter\def\csname cnt@summary.expl.multi-missed-accR.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.multi-missed-accR.max\endcsname{16.7}
\expandafter\def\csname ppt@summary.expl.multi-missed-accR.max\endcsname{$+$16.7}
\expandafter\def\csname val@summary.expl.multi-missed-accR.min\endcsname{0.000}
\expandafter\def\csname cnt@summary.expl.multi-missed-accR.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.multi-missed-accR.min\endcsname{0.0}
\expandafter\def\csname ppt@summary.expl.multi-missed-accR.min\endcsname{0.0}
\expandafter\def\csname val@summary.expl.notcov-accF.max\endcsname{0.448}
\expandafter\def\csname cnt@summary.expl.notcov-accF.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-accF.max\endcsname{44.8}
\expandafter\def\csname ppt@summary.expl.notcov-accF.max\endcsname{$+$44.8}
\expandafter\def\csname val@summary.expl.notcov-accF.min\endcsname{0.208}
\expandafter\def\csname cnt@summary.expl.notcov-accF.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-accF.min\endcsname{20.8}
\expandafter\def\csname ppt@summary.expl.notcov-accF.min\endcsname{$+$20.8}
\expandafter\def\csname val@summary.expl.notcov-accR.max\endcsname{0.089}
\expandafter\def\csname cnt@summary.expl.notcov-accR.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-accR.max\endcsname{8.9}
\expandafter\def\csname ppt@summary.expl.notcov-accR.max\endcsname{$+$8.9}
\expandafter\def\csname val@summary.expl.notcov-accR.min\endcsname{0.000}
\expandafter\def\csname cnt@summary.expl.notcov-accR.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-accR.min\endcsname{0.0}
\expandafter\def\csname ppt@summary.expl.notcov-accR.min\endcsname{0.0}
\expandafter\def\csname val@summary.expl.notcov-resid.max\endcsname{0.373}
\expandafter\def\csname cnt@summary.expl.notcov-resid.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-resid.max\endcsname{37.3}
\expandafter\def\csname ppt@summary.expl.notcov-resid.max\endcsname{$+$37.3}
\expandafter\def\csname val@summary.expl.notcov-resid.min\endcsname{0.125}
\expandafter\def\csname cnt@summary.expl.notcov-resid.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-resid.min\endcsname{12.5}
\expandafter\def\csname ppt@summary.expl.notcov-resid.min\endcsname{$+$12.5}
\expandafter\def\csname val@summary.expl.notcov-share.max\endcsname{0.184}
\expandafter\def\csname cnt@summary.expl.notcov-share.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-share.max\endcsname{18.4}
\expandafter\def\csname ppt@summary.expl.notcov-share.max\endcsname{$+$18.4}
\expandafter\def\csname val@summary.expl.notcov-share.min\endcsname{0.037}
\expandafter\def\csname cnt@summary.expl.notcov-share.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.notcov-share.min\endcsname{3.7}
\expandafter\def\csname ppt@summary.expl.notcov-share.min\endcsname{$+$3.7}
\expandafter\def\csname val@summary.expl.perm-p.n\endcsname{6}
\expandafter\def\csname cnt@summary.expl.perm-p.n\endcsname{6}
\expandafter\def\csname pct@summary.expl.perm-p.n\endcsname{600.0}
\expandafter\def\csname ppt@summary.expl.perm-p.n\endcsname{$+$600.0}
\expandafter\def\csname val@summary.expl.perm-p.n-below-05\endcsname{1}
\expandafter\def\csname cnt@summary.expl.perm-p.n-below-05\endcsname{1}
\expandafter\def\csname pct@summary.expl.perm-p.n-below-05\endcsname{100.0}
\expandafter\def\csname ppt@summary.expl.perm-p.n-below-05\endcsname{$+$100.0}
\expandafter\def\csname val@summary.expl.perm-p.other-min\endcsname{0.168}
\expandafter\def\csname cnt@summary.expl.perm-p.other-min\endcsname{0}
\expandafter\def\csname pct@summary.expl.perm-p.other-min\endcsname{16.8}
\expandafter\def\csname ppt@summary.expl.perm-p.other-min\endcsname{$+$16.8}
\expandafter\def\csname val@summary.expl.rcr-lowest-rmse\endcsname{3}
\expandafter\def\csname cnt@summary.expl.rcr-lowest-rmse\endcsname{3}
\expandafter\def\csname pct@summary.expl.rcr-lowest-rmse\endcsname{300.0}
\expandafter\def\csname ppt@summary.expl.rcr-lowest-rmse\endcsname{$+$300.0}
\expandafter\def\csname val@summary.expl.rcr-rmse-settings\endcsname{4}
\expandafter\def\csname cnt@summary.expl.rcr-rmse-settings\endcsname{4}
\expandafter\def\csname pct@summary.expl.rcr-rmse-settings\endcsname{400.0}
\expandafter\def\csname ppt@summary.expl.rcr-rmse-settings\endcsname{$+$400.0}
\expandafter\def\csname val@summary.expl.refine-delta-eta2-text-max\endcsname{7.0}
\expandafter\def\csname val@summary.expl.refine-delta-eta2-text-min\endcsname{0.1}
\expandafter\def\csname val@summary.expl.refine-delta-eta2.max\endcsname{0.070}
\expandafter\def\csname cnt@summary.expl.refine-delta-eta2.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.refine-delta-eta2.max\endcsname{7.0}
\expandafter\def\csname ppt@summary.expl.refine-delta-eta2.max\endcsname{$+$7.0}
\expandafter\def\csname val@summary.expl.refine-delta-eta2.min\endcsname{0.001}
\expandafter\def\csname cnt@summary.expl.refine-delta-eta2.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.refine-delta-eta2.min\endcsname{0.1}
\expandafter\def\csname ppt@summary.expl.refine-delta-eta2.min\endcsname{$+$0.1}
\expandafter\def\csname val@summary.expl.replay-only-lower-rmse-than-rcr\endcsname{3}
\expandafter\def\csname cnt@summary.expl.replay-only-lower-rmse-than-rcr\endcsname{3}
\expandafter\def\csname pct@summary.expl.replay-only-lower-rmse-than-rcr\endcsname{300.0}
\expandafter\def\csname ppt@summary.expl.replay-only-lower-rmse-than-rcr\endcsname{$+$300.0}
\expandafter\def\csname val@summary.expl.replay-only-rmse-n\endcsname{4}
\expandafter\def\csname cnt@summary.expl.replay-only-rmse-n\endcsname{4}
\expandafter\def\csname pct@summary.expl.replay-only-rmse-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.expl.replay-only-rmse-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.expl.replay-pessimistic\endcsname{12}
\expandafter\def\csname cnt@summary.expl.replay-pessimistic\endcsname{12}
\expandafter\def\csname pct@summary.expl.replay-pessimistic\endcsname{1200.0}
\expandafter\def\csname ppt@summary.expl.replay-pessimistic\endcsname{$+$1200.0}
\expandafter\def\csname val@summary.expl.replay-pessimistic-n\endcsname{16}
\expandafter\def\csname cnt@summary.expl.replay-pessimistic-n\endcsname{16}
\expandafter\def\csname pct@summary.expl.replay-pessimistic-n\endcsname{1600.0}
\expandafter\def\csname ppt@summary.expl.replay-pessimistic-n\endcsname{$+$1600.0}
\expandafter\def\csname val@summary.expl.single-missed-accR.max\endcsname{0.048}
\expandafter\def\csname cnt@summary.expl.single-missed-accR.max\endcsname{0}
\expandafter\def\csname pct@summary.expl.single-missed-accR.max\endcsname{4.8}
\expandafter\def\csname ppt@summary.expl.single-missed-accR.max\endcsname{$+$4.8}
\expandafter\def\csname val@summary.expl.single-missed-accR.min\endcsname{0.000}
\expandafter\def\csname cnt@summary.expl.single-missed-accR.min\endcsname{0}
\expandafter\def\csname pct@summary.expl.single-missed-accR.min\endcsname{0.0}
\expandafter\def\csname ppt@summary.expl.single-missed-accR.min\endcsname{0.0}
\expandafter\def\csname val@summary.expl.visual-stratum-ge-agree\endcsname{4}
\expandafter\def\csname cnt@summary.expl.visual-stratum-ge-agree\endcsname{4}
\expandafter\def\csname pct@summary.expl.visual-stratum-ge-agree\endcsname{400.0}
\expandafter\def\csname ppt@summary.expl.visual-stratum-ge-agree\endcsname{$+$400.0}
\expandafter\def\csname val@summary.expl.visual-stratum-n\endcsname{6}
\expandafter\def\csname cnt@summary.expl.visual-stratum-n\endcsname{6}
\expandafter\def\csname pct@summary.expl.visual-stratum-n\endcsname{600.0}
\expandafter\def\csname ppt@summary.expl.visual-stratum-n\endcsname{$+$600.0}
\expandafter\def\csname val@summary.haiku-C-sonnet-T-sign-flips\endcsname{0}
\expandafter\def\csname cnt@summary.haiku-C-sonnet-T-sign-flips\endcsname{0}
\expandafter\def\csname pct@summary.haiku-C-sonnet-T-sign-flips\endcsname{0.0}
\expandafter\def\csname ppt@summary.haiku-C-sonnet-T-sign-flips\endcsname{0.0}
\expandafter\def\csname val@summary.haiku-C-sonnet-T-sign-n\endcsname{8}
\expandafter\def\csname cnt@summary.haiku-C-sonnet-T-sign-n\endcsname{8}
\expandafter\def\csname pct@summary.haiku-C-sonnet-T-sign-n\endcsname{800.0}
\expandafter\def\csname ppt@summary.haiku-C-sonnet-T-sign-n\endcsname{$+$800.0}
\expandafter\def\csname val@summary.old-decision-at-oracle\endcsname{3}
\expandafter\def\csname cnt@summary.old-decision-at-oracle\endcsname{3}
\expandafter\def\csname pct@summary.old-decision-at-oracle\endcsname{300.0}
\expandafter\def\csname ppt@summary.old-decision-at-oracle\endcsname{$+$300.0}
\expandafter\def\csname val@summary.old-decision-at-oracle-n\endcsname{4}
\expandafter\def\csname cnt@summary.old-decision-at-oracle-n\endcsname{4}
\expandafter\def\csname pct@summary.old-decision-at-oracle-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.old-decision-at-oracle-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.old-decision-ties-replay\endcsname{3}
\expandafter\def\csname cnt@summary.old-decision-ties-replay\endcsname{3}
\expandafter\def\csname pct@summary.old-decision-ties-replay\endcsname{300.0}
\expandafter\def\csname ppt@summary.old-decision-ties-replay\endcsname{$+$300.0}
\expandafter\def\csname val@summary.rcr-vs-old-decision.max\endcsname{0.012}
\expandafter\def\csname cnt@summary.rcr-vs-old-decision.max\endcsname{0}
\expandafter\def\csname pct@summary.rcr-vs-old-decision.max\endcsname{1.2}
\expandafter\def\csname ppt@summary.rcr-vs-old-decision.max\endcsname{$+$1.2}
\expandafter\def\csname val@summary.rcr-vs-old-decision.min\endcsname{-0.030}
\expandafter\def\csname cnt@summary.rcr-vs-old-decision.min\endcsname{0}
\expandafter\def\csname pct@summary.rcr-vs-old-decision.min\endcsname{$-$3.0}
\expandafter\def\csname ppt@summary.rcr-vs-old-decision.min\endcsname{$-$3.0}
\expandafter\def\csname val@summary.rcr-vs-old-decision.n\endcsname{4}
\expandafter\def\csname cnt@summary.rcr-vs-old-decision.n\endcsname{4}
\expandafter\def\csname pct@summary.rcr-vs-old-decision.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.rcr-vs-old-decision.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.rcr-vs-old-decision.n-ci-below-0\endcsname{3}
\expandafter\def\csname cnt@summary.rcr-vs-old-decision.n-ci-below-0\endcsname{3}
\expandafter\def\csname pct@summary.rcr-vs-old-decision.n-ci-below-0\endcsname{300.0}
\expandafter\def\csname ppt@summary.rcr-vs-old-decision.n-ci-below-0\endcsname{$+$300.0}
\expandafter\def\csname val@summary.rcr-vs-replay-only.max\endcsname{-0.002}
\expandafter\def\csname cnt@summary.rcr-vs-replay-only.max\endcsname{0}
\expandafter\def\csname pct@summary.rcr-vs-replay-only.max\endcsname{$-$0.2}
\expandafter\def\csname ppt@summary.rcr-vs-replay-only.max\endcsname{$-$0.2}
\expandafter\def\csname val@summary.rcr-vs-replay-only.min\endcsname{-0.030}
\expandafter\def\csname cnt@summary.rcr-vs-replay-only.min\endcsname{0}
\expandafter\def\csname pct@summary.rcr-vs-replay-only.min\endcsname{$-$3.0}
\expandafter\def\csname ppt@summary.rcr-vs-replay-only.min\endcsname{$-$3.0}
\expandafter\def\csname val@summary.rcr-vs-replay-only.n\endcsname{4}
\expandafter\def\csname cnt@summary.rcr-vs-replay-only.n\endcsname{4}
\expandafter\def\csname pct@summary.rcr-vs-replay-only.n\endcsname{400.0}
\expandafter\def\csname ppt@summary.rcr-vs-replay-only.n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.rcr-vs-replay-only.n-ci-below-0\endcsname{3}
\expandafter\def\csname cnt@summary.rcr-vs-replay-only.n-ci-below-0\endcsname{3}
\expandafter\def\csname pct@summary.rcr-vs-replay-only.n-ci-below-0\endcsname{300.0}
\expandafter\def\csname ppt@summary.rcr-vs-replay-only.n-ci-below-0\endcsname{$+$300.0}
\expandafter\def\csname val@summary.replay-only-at-oracle\endcsname{3}
\expandafter\def\csname cnt@summary.replay-only-at-oracle\endcsname{3}
\expandafter\def\csname pct@summary.replay-only-at-oracle\endcsname{300.0}
\expandafter\def\csname ppt@summary.replay-only-at-oracle\endcsname{$+$300.0}
\expandafter\def\csname val@summary.replay-only-ge-perskill-all-budgets\endcsname{4}
\expandafter\def\csname cnt@summary.replay-only-ge-perskill-all-budgets\endcsname{4}
\expandafter\def\csname pct@summary.replay-only-ge-perskill-all-budgets\endcsname{400.0}
\expandafter\def\csname ppt@summary.replay-only-ge-perskill-all-budgets\endcsname{$+$400.0}
\expandafter\def\csname val@summary.replay-only-ge-perskill-budgeted\endcsname{4}
\expandafter\def\csname cnt@summary.replay-only-ge-perskill-budgeted\endcsname{4}
\expandafter\def\csname pct@summary.replay-only-ge-perskill-budgeted\endcsname{400.0}
\expandafter\def\csname ppt@summary.replay-only-ge-perskill-budgeted\endcsname{$+$400.0}
\expandafter\def\csname val@summary.replay-only-ge-perskill-budgeted-n\endcsname{4}
\expandafter\def\csname cnt@summary.replay-only-ge-perskill-budgeted-n\endcsname{4}
\expandafter\def\csname pct@summary.replay-only-ge-perskill-budgeted-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.replay-only-ge-perskill-budgeted-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.sonnet-opus-sign-flips\endcsname{0}
\expandafter\def\csname cnt@summary.sonnet-opus-sign-flips\endcsname{0}
\expandafter\def\csname pct@summary.sonnet-opus-sign-flips\endcsname{0.0}
\expandafter\def\csname ppt@summary.sonnet-opus-sign-flips\endcsname{0.0}
\expandafter\def\csname val@summary.sonnet-opus-sign-n\endcsname{7}
\expandafter\def\csname cnt@summary.sonnet-opus-sign-n\endcsname{7}
\expandafter\def\csname pct@summary.sonnet-opus-sign-n\endcsname{700.0}
\expandafter\def\csname ppt@summary.sonnet-opus-sign-n\endcsname{$+$700.0}
\expandafter\def\csname val@summary.sonnet-opus-zero\endcsname{1}
\expandafter\def\csname cnt@summary.sonnet-opus-zero\endcsname{1}
\expandafter\def\csname pct@summary.sonnet-opus-zero\endcsname{100.0}
\expandafter\def\csname ppt@summary.sonnet-opus-zero\endcsname{$+$100.0}
\expandafter\def\csname val@summary.sspro.gain-vs-medoid.max\endcsname{0.188}
\expandafter\def\csname cnt@summary.sspro.gain-vs-medoid.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.gain-vs-medoid.max\endcsname{18.8}
\expandafter\def\csname ppt@summary.sspro.gain-vs-medoid.max\endcsname{$+$18.8}
\expandafter\def\csname val@summary.sspro.gain-vs-medoid.min\endcsname{0.073}
\expandafter\def\csname cnt@summary.sspro.gain-vs-medoid.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.gain-vs-medoid.min\endcsname{7.3}
\expandafter\def\csname ppt@summary.sspro.gain-vs-medoid.min\endcsname{$+$7.3}
\expandafter\def\csname val@summary.sspro.holm-p.max\endcsname{0.049}
\expandafter\def\csname cnt@summary.sspro.holm-p.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.holm-p.max\endcsname{4.9}
\expandafter\def\csname ppt@summary.sspro.holm-p.max\endcsname{$+$4.9}
\expandafter\def\csname val@summary.sspro.holm-p.min\endcsname{0.002}
\expandafter\def\csname cnt@summary.sspro.holm-p.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.holm-p.min\endcsname{0.2}
\expandafter\def\csname ppt@summary.sspro.holm-p.min\endcsname{$+$0.2}
\expandafter\def\csname val@summary.sspro.p1.C.disagree-minus-agree-stable\endcsname{0.017}
\expandafter\def\csname cnt@summary.sspro.p1.C.disagree-minus-agree-stable\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.C.disagree-minus-agree-stable\endcsname{1.7}
\expandafter\def\csname ppt@summary.sspro.p1.C.disagree-minus-agree-stable\endcsname{$+$1.7}
\expandafter\def\csname val@summary.sspro.p1.full-recert.vs-suspend-all\endcsname{0.120}
\expandafter\def\csname cnt@summary.sspro.p1.full-recert.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.full-recert.vs-suspend-all\endcsname{12.0}
\expandafter\def\csname ppt@summary.sspro.p1.full-recert.vs-suspend-all\endcsname{$+$12.0}
\expandafter\def\csname val@summary.sspro.p1.gain-vs-medoid.max\endcsname{0.188}
\expandafter\def\csname cnt@summary.sspro.p1.gain-vs-medoid.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.gain-vs-medoid.max\endcsname{18.8}
\expandafter\def\csname ppt@summary.sspro.p1.gain-vs-medoid.max\endcsname{$+$18.8}
\expandafter\def\csname val@summary.sspro.p1.gain-vs-medoid.min\endcsname{0.115}
\expandafter\def\csname cnt@summary.sspro.p1.gain-vs-medoid.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.gain-vs-medoid.min\endcsname{11.5}
\expandafter\def\csname ppt@summary.sspro.p1.gain-vs-medoid.min\endcsname{$+$11.5}
\expandafter\def\csname val@summary.sspro.p1.keep-all.vs-suspend-all\endcsname{0.120}
\expandafter\def\csname cnt@summary.sspro.p1.keep-all.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.keep-all.vs-suspend-all\endcsname{12.0}
\expandafter\def\csname ppt@summary.sspro.p1.keep-all.vs-suspend-all\endcsname{$+$12.0}
\expandafter\def\csname val@summary.sspro.p1.old-decision-eq-T-oracle\endcsname{4}
\expandafter\def\csname cnt@summary.sspro.p1.old-decision-eq-T-oracle\endcsname{4}
\expandafter\def\csname pct@summary.sspro.p1.old-decision-eq-T-oracle\endcsname{400.0}
\expandafter\def\csname ppt@summary.sspro.p1.old-decision-eq-T-oracle\endcsname{$+$400.0}
\expandafter\def\csname val@summary.sspro.p1.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname cnt@summary.sspro.p1.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname pct@summary.sspro.p1.old-decision-eq-T-oracle-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.sspro.p1.old-decision-eq-T-oracle-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.sspro.p1.old-decision-minus-rcr\endcsname{0.002}
\expandafter\def\csname cnt@summary.sspro.p1.old-decision-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.old-decision-minus-rcr\endcsname{0.2}
\expandafter\def\csname ppt@summary.sspro.p1.old-decision-minus-rcr\endcsname{$+$0.2}
\expandafter\def\csname val@summary.sspro.p1.old-decision.vs-suspend-all\endcsname{0.120}
\expandafter\def\csname cnt@summary.sspro.p1.old-decision.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.old-decision.vs-suspend-all\endcsname{12.0}
\expandafter\def\csname ppt@summary.sspro.p1.old-decision.vs-suspend-all\endcsname{$+$12.0}
\expandafter\def\csname val@summary.sspro.p1.oracle-on-T.vs-suspend-all\endcsname{0.120}
\expandafter\def\csname cnt@summary.sspro.p1.oracle-on-T.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.oracle-on-T.vs-suspend-all\endcsname{12.0}
\expandafter\def\csname ppt@summary.sspro.p1.oracle-on-T.vs-suspend-all\endcsname{$+$12.0}
\expandafter\def\csname val@summary.sspro.p1.replay-only-cost-fraction-of-rcr\endcsname{0.745}
\expandafter\def\csname cnt@summary.sspro.p1.replay-only-cost-fraction-of-rcr\endcsname{1}
\expandafter\def\csname pct@summary.sspro.p1.replay-only-cost-fraction-of-rcr\endcsname{74.5}
\expandafter\def\csname ppt@summary.sspro.p1.replay-only-cost-fraction-of-rcr\endcsname{$+$74.5}
\expandafter\def\csname val@summary.sspro.p1.replay-only-minus-rcr\endcsname{0.002}
\expandafter\def\csname cnt@summary.sspro.p1.replay-only-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.replay-only-minus-rcr\endcsname{0.2}
\expandafter\def\csname ppt@summary.sspro.p1.replay-only-minus-rcr\endcsname{$+$0.2}
\expandafter\def\csname val@summary.sspro.p1.replay-only.vs-suspend-all\endcsname{0.120}
\expandafter\def\csname cnt@summary.sspro.p1.replay-only.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.replay-only.vs-suspend-all\endcsname{12.0}
\expandafter\def\csname ppt@summary.sspro.p1.replay-only.vs-suspend-all\endcsname{$+$12.0}
\expandafter\def\csname val@summary.sspro.p1.tau-T.max\endcsname{0.177}
\expandafter\def\csname cnt@summary.sspro.p1.tau-T.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.tau-T.max\endcsname{17.7}
\expandafter\def\csname ppt@summary.sspro.p1.tau-T.max\endcsname{$+$17.7}
\expandafter\def\csname val@summary.sspro.p1.tau-T.min\endcsname{0.104}
\expandafter\def\csname cnt@summary.sspro.p1.tau-T.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p1.tau-T.min\endcsname{10.4}
\expandafter\def\csname ppt@summary.sspro.p1.tau-T.min\endcsname{$+$10.4}
\expandafter\def\csname val@summary.sspro.p2.C.disagree-minus-agree-stable\endcsname{0.120}
\expandafter\def\csname cnt@summary.sspro.p2.C.disagree-minus-agree-stable\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.C.disagree-minus-agree-stable\endcsname{12.0}
\expandafter\def\csname ppt@summary.sspro.p2.C.disagree-minus-agree-stable\endcsname{$+$12.0}
\expandafter\def\csname val@summary.sspro.p2.T.disagree-minus-agree-stable\endcsname{0.089}
\expandafter\def\csname cnt@summary.sspro.p2.T.disagree-minus-agree-stable\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.T.disagree-minus-agree-stable\endcsname{8.9}
\expandafter\def\csname ppt@summary.sspro.p2.T.disagree-minus-agree-stable\endcsname{$+$8.9}
\expandafter\def\csname val@summary.sspro.p2.full-recert.vs-suspend-all\endcsname{0.146}
\expandafter\def\csname cnt@summary.sspro.p2.full-recert.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.full-recert.vs-suspend-all\endcsname{14.6}
\expandafter\def\csname ppt@summary.sspro.p2.full-recert.vs-suspend-all\endcsname{$+$14.6}
\expandafter\def\csname val@summary.sspro.p2.gain-vs-medoid.max\endcsname{0.115}
\expandafter\def\csname cnt@summary.sspro.p2.gain-vs-medoid.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.gain-vs-medoid.max\endcsname{11.5}
\expandafter\def\csname ppt@summary.sspro.p2.gain-vs-medoid.max\endcsname{$+$11.5}
\expandafter\def\csname val@summary.sspro.p2.gain-vs-medoid.min\endcsname{0.073}
\expandafter\def\csname cnt@summary.sspro.p2.gain-vs-medoid.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.gain-vs-medoid.min\endcsname{7.3}
\expandafter\def\csname ppt@summary.sspro.p2.gain-vs-medoid.min\endcsname{$+$7.3}
\expandafter\def\csname val@summary.sspro.p2.keep-all.vs-suspend-all\endcsname{0.146}
\expandafter\def\csname cnt@summary.sspro.p2.keep-all.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.keep-all.vs-suspend-all\endcsname{14.6}
\expandafter\def\csname ppt@summary.sspro.p2.keep-all.vs-suspend-all\endcsname{$+$14.6}
\expandafter\def\csname val@summary.sspro.p2.old-decision-eq-T-oracle\endcsname{4}
\expandafter\def\csname cnt@summary.sspro.p2.old-decision-eq-T-oracle\endcsname{4}
\expandafter\def\csname pct@summary.sspro.p2.old-decision-eq-T-oracle\endcsname{400.0}
\expandafter\def\csname ppt@summary.sspro.p2.old-decision-eq-T-oracle\endcsname{$+$400.0}
\expandafter\def\csname val@summary.sspro.p2.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname cnt@summary.sspro.p2.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname pct@summary.sspro.p2.old-decision-eq-T-oracle-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.sspro.p2.old-decision-eq-T-oracle-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.sspro.p2.old-decision-minus-rcr\endcsname{0.011}
\expandafter\def\csname cnt@summary.sspro.p2.old-decision-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.old-decision-minus-rcr\endcsname{1.1}
\expandafter\def\csname ppt@summary.sspro.p2.old-decision-minus-rcr\endcsname{$+$1.1}
\expandafter\def\csname val@summary.sspro.p2.old-decision.vs-suspend-all\endcsname{0.146}
\expandafter\def\csname cnt@summary.sspro.p2.old-decision.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.old-decision.vs-suspend-all\endcsname{14.6}
\expandafter\def\csname ppt@summary.sspro.p2.old-decision.vs-suspend-all\endcsname{$+$14.6}
\expandafter\def\csname val@summary.sspro.p2.oracle-on-T.vs-suspend-all\endcsname{0.146}
\expandafter\def\csname cnt@summary.sspro.p2.oracle-on-T.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.oracle-on-T.vs-suspend-all\endcsname{14.6}
\expandafter\def\csname ppt@summary.sspro.p2.oracle-on-T.vs-suspend-all\endcsname{$+$14.6}
\expandafter\def\csname val@summary.sspro.p2.replay-only-cost-fraction-of-rcr\endcsname{0.745}
\expandafter\def\csname cnt@summary.sspro.p2.replay-only-cost-fraction-of-rcr\endcsname{1}
\expandafter\def\csname pct@summary.sspro.p2.replay-only-cost-fraction-of-rcr\endcsname{74.5}
\expandafter\def\csname ppt@summary.sspro.p2.replay-only-cost-fraction-of-rcr\endcsname{$+$74.5}
\expandafter\def\csname val@summary.sspro.p2.replay-only-minus-rcr\endcsname{0.011}
\expandafter\def\csname cnt@summary.sspro.p2.replay-only-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.replay-only-minus-rcr\endcsname{1.1}
\expandafter\def\csname ppt@summary.sspro.p2.replay-only-minus-rcr\endcsname{$+$1.1}
\expandafter\def\csname val@summary.sspro.p2.replay-only.vs-suspend-all\endcsname{0.146}
\expandafter\def\csname cnt@summary.sspro.p2.replay-only.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.replay-only.vs-suspend-all\endcsname{14.6}
\expandafter\def\csname ppt@summary.sspro.p2.replay-only.vs-suspend-all\endcsname{$+$14.6}
\expandafter\def\csname val@summary.sspro.p2.tau-T.max\endcsname{0.167}
\expandafter\def\csname cnt@summary.sspro.p2.tau-T.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.tau-T.max\endcsname{16.7}
\expandafter\def\csname ppt@summary.sspro.p2.tau-T.max\endcsname{$+$16.7}
\expandafter\def\csname val@summary.sspro.p2.tau-T.min\endcsname{0.125}
\expandafter\def\csname cnt@summary.sspro.p2.tau-T.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.p2.tau-T.min\endcsname{12.5}
\expandafter\def\csname ppt@summary.sspro.p2.tau-T.min\endcsname{$+$12.5}
\expandafter\def\csname val@summary.sspro.pool-change-max-abs-tau\endcsname{0.000}
\expandafter\def\csname cnt@summary.sspro.pool-change-max-abs-tau\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-change-max-abs-tau\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-change-max-abs-tau\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-changes-away\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-changes-away\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-changes-away\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-changes-away\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-changes-matching-T-oracle\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-changes-matching-T-oracle\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-changes-matching-T-oracle\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-changes-matching-T-oracle\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-decision-changes\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-decision-changes\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-decision-changes\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-decision-changes\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-decision-changes-with-public\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-decision-changes-with-public\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-decision-changes-with-public\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-decision-changes-with-public\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-decision-n\endcsname{8}
\expandafter\def\csname cnt@summary.sspro.pool-decision-n\endcsname{8}
\expandafter\def\csname pct@summary.sspro.pool-decision-n\endcsname{800.0}
\expandafter\def\csname ppt@summary.sspro.pool-decision-n\endcsname{$+$800.0}
\expandafter\def\csname val@summary.sspro.pool-decision-n-with-public\endcsname{10}
\expandafter\def\csname cnt@summary.sspro.pool-decision-n-with-public\endcsname{10}
\expandafter\def\csname pct@summary.sspro.pool-decision-n-with-public\endcsname{1000.0}
\expandafter\def\csname ppt@summary.sspro.pool-decision-n-with-public\endcsname{$+$1000.0}
\expandafter\def\csname val@summary.sspro.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{0.000}
\expandafter\def\csname cnt@summary.sspro.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-sign-flips\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-sign-flips\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-sign-flips\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-flips\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-sign-flips-held-on-T\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-sign-flips-held-on-T\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-sign-flips-held-on-T\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-flips-held-on-T\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-sign-flips-held-on-T-with-public\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-sign-flips-held-on-T-with-public\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-sign-flips-held-on-T-with-public\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-flips-held-on-T-with-public\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-sign-flips-with-public\endcsname{0}
\expandafter\def\csname cnt@summary.sspro.pool-sign-flips-with-public\endcsname{0}
\expandafter\def\csname pct@summary.sspro.pool-sign-flips-with-public\endcsname{0.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-flips-with-public\endcsname{0.0}
\expandafter\def\csname val@summary.sspro.pool-sign-n\endcsname{8}
\expandafter\def\csname cnt@summary.sspro.pool-sign-n\endcsname{8}
\expandafter\def\csname pct@summary.sspro.pool-sign-n\endcsname{800.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-n\endcsname{$+$800.0}
\expandafter\def\csname val@summary.sspro.pool-sign-n-with-public\endcsname{10}
\expandafter\def\csname cnt@summary.sspro.pool-sign-n-with-public\endcsname{10}
\expandafter\def\csname pct@summary.sspro.pool-sign-n-with-public\endcsname{1000.0}
\expandafter\def\csname ppt@summary.sspro.pool-sign-n-with-public\endcsname{$+$1000.0}
\expandafter\def\csname val@summary.sspro.rcr-cost-fraction.max\endcsname{0.720}
\expandafter\def\csname cnt@summary.sspro.rcr-cost-fraction.max\endcsname{1}
\expandafter\def\csname pct@summary.sspro.rcr-cost-fraction.max\endcsname{72.0}
\expandafter\def\csname ppt@summary.sspro.rcr-cost-fraction.max\endcsname{$+$72.0}
\expandafter\def\csname val@summary.sspro.rcr-cost-fraction.min\endcsname{0.718}
\expandafter\def\csname cnt@summary.sspro.rcr-cost-fraction.min\endcsname{1}
\expandafter\def\csname pct@summary.sspro.rcr-cost-fraction.min\endcsname{71.8}
\expandafter\def\csname ppt@summary.sspro.rcr-cost-fraction.min\endcsname{$+$71.8}
\expandafter\def\csname val@summary.sspro.tau-T.max\endcsname{0.177}
\expandafter\def\csname cnt@summary.sspro.tau-T.max\endcsname{0}
\expandafter\def\csname pct@summary.sspro.tau-T.max\endcsname{17.7}
\expandafter\def\csname ppt@summary.sspro.tau-T.max\endcsname{$+$17.7}
\expandafter\def\csname val@summary.sspro.tau-T.min\endcsname{0.104}
\expandafter\def\csname cnt@summary.sspro.tau-T.min\endcsname{0}
\expandafter\def\csname pct@summary.sspro.tau-T.min\endcsname{10.4}
\expandafter\def\csname ppt@summary.sspro.tau-T.min\endcsname{$+$10.4}
\expandafter\def\csname val@summary.suspend-all-above-replay\endcsname{1}
\expandafter\def\csname cnt@summary.suspend-all-above-replay\endcsname{1}
\expandafter\def\csname pct@summary.suspend-all-above-replay\endcsname{100.0}
\expandafter\def\csname ppt@summary.suspend-all-above-replay\endcsname{$+$100.0}
\expandafter\def\csname val@summary.uiv.gain-vs-medoid.max\endcsname{-0.007}
\expandafter\def\csname cnt@summary.uiv.gain-vs-medoid.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.gain-vs-medoid.max\endcsname{$-$0.7}
\expandafter\def\csname ppt@summary.uiv.gain-vs-medoid.max\endcsname{$-$0.7}
\expandafter\def\csname val@summary.uiv.gain-vs-medoid.min\endcsname{-0.083}
\expandafter\def\csname cnt@summary.uiv.gain-vs-medoid.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.gain-vs-medoid.min\endcsname{$-$8.3}
\expandafter\def\csname ppt@summary.uiv.gain-vs-medoid.min\endcsname{$-$8.3}
\expandafter\def\csname val@summary.uiv.holm-p.max\endcsname{0.165}
\expandafter\def\csname cnt@summary.uiv.holm-p.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.holm-p.max\endcsname{16.5}
\expandafter\def\csname ppt@summary.uiv.holm-p.max\endcsname{$+$16.5}
\expandafter\def\csname val@summary.uiv.holm-p.min\endcsname{0.002}
\expandafter\def\csname cnt@summary.uiv.holm-p.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.holm-p.min\endcsname{0.2}
\expandafter\def\csname ppt@summary.uiv.holm-p.min\endcsname{$+$0.2}
\expandafter\def\csname val@summary.uiv.p1.C.disagree-minus-agree-stable\endcsname{0.253}
\expandafter\def\csname cnt@summary.uiv.p1.C.disagree-minus-agree-stable\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.C.disagree-minus-agree-stable\endcsname{25.3}
\expandafter\def\csname ppt@summary.uiv.p1.C.disagree-minus-agree-stable\endcsname{$+$25.3}
\expandafter\def\csname val@summary.uiv.p1.full-recert.vs-suspend-all\endcsname{-0.040}
\expandafter\def\csname cnt@summary.uiv.p1.full-recert.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.full-recert.vs-suspend-all\endcsname{$-$4.0}
\expandafter\def\csname ppt@summary.uiv.p1.full-recert.vs-suspend-all\endcsname{$-$4.0}
\expandafter\def\csname val@summary.uiv.p1.gain-vs-medoid.max\endcsname{-0.035}
\expandafter\def\csname cnt@summary.uiv.p1.gain-vs-medoid.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.gain-vs-medoid.max\endcsname{$-$3.5}
\expandafter\def\csname ppt@summary.uiv.p1.gain-vs-medoid.max\endcsname{$-$3.5}
\expandafter\def\csname val@summary.uiv.p1.gain-vs-medoid.min\endcsname{-0.083}
\expandafter\def\csname cnt@summary.uiv.p1.gain-vs-medoid.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.gain-vs-medoid.min\endcsname{$-$8.3}
\expandafter\def\csname ppt@summary.uiv.p1.gain-vs-medoid.min\endcsname{$-$8.3}
\expandafter\def\csname val@summary.uiv.p1.keep-all.vs-suspend-all\endcsname{-0.073}
\expandafter\def\csname cnt@summary.uiv.p1.keep-all.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.keep-all.vs-suspend-all\endcsname{$-$7.3}
\expandafter\def\csname ppt@summary.uiv.p1.keep-all.vs-suspend-all\endcsname{$-$7.3}
\expandafter\def\csname val@summary.uiv.p1.old-decision-eq-T-oracle\endcsname{4}
\expandafter\def\csname cnt@summary.uiv.p1.old-decision-eq-T-oracle\endcsname{4}
\expandafter\def\csname pct@summary.uiv.p1.old-decision-eq-T-oracle\endcsname{400.0}
\expandafter\def\csname ppt@summary.uiv.p1.old-decision-eq-T-oracle\endcsname{$+$400.0}
\expandafter\def\csname val@summary.uiv.p1.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname cnt@summary.uiv.p1.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname pct@summary.uiv.p1.old-decision-eq-T-oracle-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.uiv.p1.old-decision-eq-T-oracle-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.uiv.p1.old-decision-minus-rcr\endcsname{0.030}
\expandafter\def\csname cnt@summary.uiv.p1.old-decision-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.old-decision-minus-rcr\endcsname{3.0}
\expandafter\def\csname ppt@summary.uiv.p1.old-decision-minus-rcr\endcsname{$+$3.0}
\expandafter\def\csname val@summary.uiv.p1.old-decision.vs-suspend-all\endcsname{0.000}
\expandafter\def\csname cnt@summary.uiv.p1.old-decision.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.old-decision.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.p1.old-decision.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.p1.oracle-on-T.vs-suspend-all\endcsname{0.000}
\expandafter\def\csname cnt@summary.uiv.p1.oracle-on-T.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.oracle-on-T.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.p1.oracle-on-T.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.p1.replay-only-cost-fraction-of-rcr\endcsname{0.747}
\expandafter\def\csname cnt@summary.uiv.p1.replay-only-cost-fraction-of-rcr\endcsname{1}
\expandafter\def\csname pct@summary.uiv.p1.replay-only-cost-fraction-of-rcr\endcsname{74.7}
\expandafter\def\csname ppt@summary.uiv.p1.replay-only-cost-fraction-of-rcr\endcsname{$+$74.7}
\expandafter\def\csname val@summary.uiv.p1.replay-only-minus-rcr\endcsname{0.030}
\expandafter\def\csname cnt@summary.uiv.p1.replay-only-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.replay-only-minus-rcr\endcsname{3.0}
\expandafter\def\csname ppt@summary.uiv.p1.replay-only-minus-rcr\endcsname{$+$3.0}
\expandafter\def\csname val@summary.uiv.p1.replay-only.vs-suspend-all\endcsname{0.000}
\expandafter\def\csname cnt@summary.uiv.p1.replay-only.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.replay-only.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.p1.replay-only.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.p1.tau-T.max\endcsname{-0.056}
\expandafter\def\csname cnt@summary.uiv.p1.tau-T.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.tau-T.max\endcsname{$-$5.6}
\expandafter\def\csname ppt@summary.uiv.p1.tau-T.max\endcsname{$-$5.6}
\expandafter\def\csname val@summary.uiv.p1.tau-T.min\endcsname{-0.104}
\expandafter\def\csname cnt@summary.uiv.p1.tau-T.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p1.tau-T.min\endcsname{$-$10.4}
\expandafter\def\csname ppt@summary.uiv.p1.tau-T.min\endcsname{$-$10.4}
\expandafter\def\csname val@summary.uiv.p2.C.disagree-minus-agree-stable\endcsname{0.020}
\expandafter\def\csname cnt@summary.uiv.p2.C.disagree-minus-agree-stable\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.C.disagree-minus-agree-stable\endcsname{2.0}
\expandafter\def\csname ppt@summary.uiv.p2.C.disagree-minus-agree-stable\endcsname{$+$2.0}
\expandafter\def\csname val@summary.uiv.p2.T.disagree-minus-agree-stable\endcsname{0.199}
\expandafter\def\csname cnt@summary.uiv.p2.T.disagree-minus-agree-stable\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.T.disagree-minus-agree-stable\endcsname{19.9}
\expandafter\def\csname ppt@summary.uiv.p2.T.disagree-minus-agree-stable\endcsname{$+$19.9}
\expandafter\def\csname val@summary.uiv.p2.ci-includes-0\endcsname{3}
\expandafter\def\csname cnt@summary.uiv.p2.ci-includes-0\endcsname{3}
\expandafter\def\csname pct@summary.uiv.p2.ci-includes-0\endcsname{300.0}
\expandafter\def\csname ppt@summary.uiv.p2.ci-includes-0\endcsname{$+$300.0}
\expandafter\def\csname val@summary.uiv.p2.ci-n\endcsname{4}
\expandafter\def\csname cnt@summary.uiv.p2.ci-n\endcsname{4}
\expandafter\def\csname pct@summary.uiv.p2.ci-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.uiv.p2.ci-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.uiv.p2.full-recert.vs-suspend-all\endcsname{-0.009}
\expandafter\def\csname cnt@summary.uiv.p2.full-recert.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.full-recert.vs-suspend-all\endcsname{$-$0.9}
\expandafter\def\csname ppt@summary.uiv.p2.full-recert.vs-suspend-all\endcsname{$-$0.9}
\expandafter\def\csname val@summary.uiv.p2.gain-vs-medoid.max\endcsname{-0.007}
\expandafter\def\csname cnt@summary.uiv.p2.gain-vs-medoid.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.gain-vs-medoid.max\endcsname{$-$0.7}
\expandafter\def\csname ppt@summary.uiv.p2.gain-vs-medoid.max\endcsname{$-$0.7}
\expandafter\def\csname val@summary.uiv.p2.gain-vs-medoid.min\endcsname{-0.069}
\expandafter\def\csname cnt@summary.uiv.p2.gain-vs-medoid.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.gain-vs-medoid.min\endcsname{$-$6.9}
\expandafter\def\csname ppt@summary.uiv.p2.gain-vs-medoid.min\endcsname{$-$6.9}
\expandafter\def\csname val@summary.uiv.p2.keep-all.vs-suspend-all\endcsname{-0.024}
\expandafter\def\csname cnt@summary.uiv.p2.keep-all.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.keep-all.vs-suspend-all\endcsname{$-$2.4}
\expandafter\def\csname ppt@summary.uiv.p2.keep-all.vs-suspend-all\endcsname{$-$2.4}
\expandafter\def\csname val@summary.uiv.p2.old-decision-eq-T-oracle\endcsname{1}
\expandafter\def\csname cnt@summary.uiv.p2.old-decision-eq-T-oracle\endcsname{1}
\expandafter\def\csname pct@summary.uiv.p2.old-decision-eq-T-oracle\endcsname{100.0}
\expandafter\def\csname ppt@summary.uiv.p2.old-decision-eq-T-oracle\endcsname{$+$100.0}
\expandafter\def\csname val@summary.uiv.p2.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname cnt@summary.uiv.p2.old-decision-eq-T-oracle-n\endcsname{4}
\expandafter\def\csname pct@summary.uiv.p2.old-decision-eq-T-oracle-n\endcsname{400.0}
\expandafter\def\csname ppt@summary.uiv.p2.old-decision-eq-T-oracle-n\endcsname{$+$400.0}
\expandafter\def\csname val@summary.uiv.p2.old-decision-minus-rcr\endcsname{-0.012}
\expandafter\def\csname cnt@summary.uiv.p2.old-decision-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.old-decision-minus-rcr\endcsname{$-$1.2}
\expandafter\def\csname ppt@summary.uiv.p2.old-decision-minus-rcr\endcsname{$-$1.2}
\expandafter\def\csname val@summary.uiv.p2.old-decision.vs-suspend-all\endcsname{-0.023}
\expandafter\def\csname cnt@summary.uiv.p2.old-decision.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.old-decision.vs-suspend-all\endcsname{$-$2.3}
\expandafter\def\csname ppt@summary.uiv.p2.old-decision.vs-suspend-all\endcsname{$-$2.3}
\expandafter\def\csname val@summary.uiv.p2.oracle-on-T.vs-suspend-all\endcsname{0.000}
\expandafter\def\csname cnt@summary.uiv.p2.oracle-on-T.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.oracle-on-T.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.p2.oracle-on-T.vs-suspend-all\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.p2.replay-only-cost-fraction-of-rcr\endcsname{0.750}
\expandafter\def\csname cnt@summary.uiv.p2.replay-only-cost-fraction-of-rcr\endcsname{1}
\expandafter\def\csname pct@summary.uiv.p2.replay-only-cost-fraction-of-rcr\endcsname{75.0}
\expandafter\def\csname ppt@summary.uiv.p2.replay-only-cost-fraction-of-rcr\endcsname{$+$75.0}
\expandafter\def\csname val@summary.uiv.p2.replay-only-minus-rcr\endcsname{0.004}
\expandafter\def\csname cnt@summary.uiv.p2.replay-only-minus-rcr\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.replay-only-minus-rcr\endcsname{0.4}
\expandafter\def\csname ppt@summary.uiv.p2.replay-only-minus-rcr\endcsname{$+$0.4}
\expandafter\def\csname val@summary.uiv.p2.replay-only.vs-suspend-all\endcsname{-0.007}
\expandafter\def\csname cnt@summary.uiv.p2.replay-only.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.replay-only.vs-suspend-all\endcsname{$-$0.7}
\expandafter\def\csname ppt@summary.uiv.p2.replay-only.vs-suspend-all\endcsname{$-$0.7}
\expandafter\def\csname val@summary.uiv.p2.tau-T.max\endcsname{0.000}
\expandafter\def\csname cnt@summary.uiv.p2.tau-T.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.tau-T.max\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.p2.tau-T.max\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.p2.tau-T.min\endcsname{-0.062}
\expandafter\def\csname cnt@summary.uiv.p2.tau-T.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.p2.tau-T.min\endcsname{$-$6.2}
\expandafter\def\csname ppt@summary.uiv.p2.tau-T.min\endcsname{$-$6.2}
\expandafter\def\csname val@summary.uiv.pool-change-max-abs-tau\endcsname{0.010}
\expandafter\def\csname cnt@summary.uiv.pool-change-max-abs-tau\endcsname{0}
\expandafter\def\csname pct@summary.uiv.pool-change-max-abs-tau\endcsname{1.0}
\expandafter\def\csname ppt@summary.uiv.pool-change-max-abs-tau\endcsname{$+$1.0}
\expandafter\def\csname val@summary.uiv.pool-change-max-abs-tau-pt\endcsname{1.042}
\expandafter\def\csname cnt@summary.uiv.pool-change-max-abs-tau-pt\endcsname{1}
\expandafter\def\csname pct@summary.uiv.pool-change-max-abs-tau-pt\endcsname{104.2}
\expandafter\def\csname ppt@summary.uiv.pool-change-max-abs-tau-pt\endcsname{$+$104.2}
\expandafter\def\csname val@summary.uiv.pool-changes-away\endcsname{3}
\expandafter\def\csname cnt@summary.uiv.pool-changes-away\endcsname{3}
\expandafter\def\csname pct@summary.uiv.pool-changes-away\endcsname{300.0}
\expandafter\def\csname ppt@summary.uiv.pool-changes-away\endcsname{$+$300.0}
\expandafter\def\csname val@summary.uiv.pool-changes-matching-T-oracle\endcsname{2}
\expandafter\def\csname cnt@summary.uiv.pool-changes-matching-T-oracle\endcsname{2}
\expandafter\def\csname pct@summary.uiv.pool-changes-matching-T-oracle\endcsname{200.0}
\expandafter\def\csname ppt@summary.uiv.pool-changes-matching-T-oracle\endcsname{$+$200.0}
\expandafter\def\csname val@summary.uiv.pool-decision-changes\endcsname{5}
\expandafter\def\csname cnt@summary.uiv.pool-decision-changes\endcsname{5}
\expandafter\def\csname pct@summary.uiv.pool-decision-changes\endcsname{500.0}
\expandafter\def\csname ppt@summary.uiv.pool-decision-changes\endcsname{$+$500.0}
\expandafter\def\csname val@summary.uiv.pool-decision-changes-with-public\endcsname{6}
\expandafter\def\csname cnt@summary.uiv.pool-decision-changes-with-public\endcsname{6}
\expandafter\def\csname pct@summary.uiv.pool-decision-changes-with-public\endcsname{600.0}
\expandafter\def\csname ppt@summary.uiv.pool-decision-changes-with-public\endcsname{$+$600.0}
\expandafter\def\csname val@summary.uiv.pool-decision-n\endcsname{8}
\expandafter\def\csname cnt@summary.uiv.pool-decision-n\endcsname{8}
\expandafter\def\csname pct@summary.uiv.pool-decision-n\endcsname{800.0}
\expandafter\def\csname ppt@summary.uiv.pool-decision-n\endcsname{$+$800.0}
\expandafter\def\csname val@summary.uiv.pool-decision-n-with-public\endcsname{10}
\expandafter\def\csname cnt@summary.uiv.pool-decision-n-with-public\endcsname{10}
\expandafter\def\csname pct@summary.uiv.pool-decision-n-with-public\endcsname{1000.0}
\expandafter\def\csname ppt@summary.uiv.pool-decision-n-with-public\endcsname{$+$1000.0}
\expandafter\def\csname val@summary.uiv.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{1.042}
\expandafter\def\csname cnt@summary.uiv.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{1}
\expandafter\def\csname pct@summary.uiv.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{104.2}
\expandafter\def\csname ppt@summary.uiv.pool-sign-flip-max-abs-tau-pt-with-public\endcsname{$+$104.2}
\expandafter\def\csname val@summary.uiv.pool-sign-flips\endcsname{3}
\expandafter\def\csname cnt@summary.uiv.pool-sign-flips\endcsname{3}
\expandafter\def\csname pct@summary.uiv.pool-sign-flips\endcsname{300.0}
\expandafter\def\csname ppt@summary.uiv.pool-sign-flips\endcsname{$+$300.0}
\expandafter\def\csname val@summary.uiv.pool-sign-flips-held-on-T\endcsname{0}
\expandafter\def\csname cnt@summary.uiv.pool-sign-flips-held-on-T\endcsname{0}
\expandafter\def\csname pct@summary.uiv.pool-sign-flips-held-on-T\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.pool-sign-flips-held-on-T\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.pool-sign-flips-held-on-T-with-public\endcsname{0}
\expandafter\def\csname cnt@summary.uiv.pool-sign-flips-held-on-T-with-public\endcsname{0}
\expandafter\def\csname pct@summary.uiv.pool-sign-flips-held-on-T-with-public\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.pool-sign-flips-held-on-T-with-public\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.pool-sign-flips-with-public\endcsname{4}
\expandafter\def\csname cnt@summary.uiv.pool-sign-flips-with-public\endcsname{4}
\expandafter\def\csname pct@summary.uiv.pool-sign-flips-with-public\endcsname{400.0}
\expandafter\def\csname ppt@summary.uiv.pool-sign-flips-with-public\endcsname{$+$400.0}
\expandafter\def\csname val@summary.uiv.pool-sign-n\endcsname{6}
\expandafter\def\csname cnt@summary.uiv.pool-sign-n\endcsname{6}
\expandafter\def\csname pct@summary.uiv.pool-sign-n\endcsname{600.0}
\expandafter\def\csname ppt@summary.uiv.pool-sign-n\endcsname{$+$600.0}
\expandafter\def\csname val@summary.uiv.pool-sign-n-with-public\endcsname{8}
\expandafter\def\csname cnt@summary.uiv.pool-sign-n-with-public\endcsname{8}
\expandafter\def\csname pct@summary.uiv.pool-sign-n-with-public\endcsname{800.0}
\expandafter\def\csname ppt@summary.uiv.pool-sign-n-with-public\endcsname{$+$800.0}
\expandafter\def\csname val@summary.uiv.rcr-cost-fraction.max\endcsname{0.731}
\expandafter\def\csname cnt@summary.uiv.rcr-cost-fraction.max\endcsname{1}
\expandafter\def\csname pct@summary.uiv.rcr-cost-fraction.max\endcsname{73.1}
\expandafter\def\csname ppt@summary.uiv.rcr-cost-fraction.max\endcsname{$+$73.1}
\expandafter\def\csname val@summary.uiv.rcr-cost-fraction.min\endcsname{0.721}
\expandafter\def\csname cnt@summary.uiv.rcr-cost-fraction.min\endcsname{1}
\expandafter\def\csname pct@summary.uiv.rcr-cost-fraction.min\endcsname{72.1}
\expandafter\def\csname ppt@summary.uiv.rcr-cost-fraction.min\endcsname{$+$72.1}
\expandafter\def\csname val@summary.uiv.tau-T.max\endcsname{0.000}
\expandafter\def\csname cnt@summary.uiv.tau-T.max\endcsname{0}
\expandafter\def\csname pct@summary.uiv.tau-T.max\endcsname{0.0}
\expandafter\def\csname ppt@summary.uiv.tau-T.max\endcsname{0.0}
\expandafter\def\csname val@summary.uiv.tau-T.min\endcsname{-0.104}
\expandafter\def\csname cnt@summary.uiv.tau-T.min\endcsname{0}
\expandafter\def\csname pct@summary.uiv.tau-T.min\endcsname{$-$10.4}
\expandafter\def\csname ppt@summary.uiv.tau-T.min\endcsname{$-$10.4}
\expandafter\def\csname val@uiv.p1.catalog.best-single@0.1.mean-over-histories\endcsname{0.790}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@0.1.mean-over-histories\endcsname{79.0}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@0.1.mean-over-histories\endcsname{$+$79.0}
\expandafter\def\csname val@uiv.p1.catalog.best-single@0.1.sd-over-histories\endcsname{0.039}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@0.1.sd-over-histories\endcsname{3.9}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@0.1.sd-over-histories\endcsname{$+$3.9}
\expandafter\def\csname val@uiv.p1.catalog.best-single@0.25.mean-over-histories\endcsname{0.802}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@0.25.mean-over-histories\endcsname{80.2}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@0.25.mean-over-histories\endcsname{$+$80.2}
\expandafter\def\csname val@uiv.p1.catalog.best-single@0.25.sd-over-histories\endcsname{0.033}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@0.25.sd-over-histories\endcsname{3.3}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@0.25.sd-over-histories\endcsname{$+$3.3}
\expandafter\def\csname val@uiv.p1.catalog.best-single@0.5.mean-over-histories\endcsname{0.814}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@0.5.mean-over-histories\endcsname{81.4}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@0.5.mean-over-histories\endcsname{$+$81.4}
\expandafter\def\csname val@uiv.p1.catalog.best-single@0.5.sd-over-histories\endcsname{0.031}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@0.5.sd-over-histories\endcsname{3.1}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@0.5.sd-over-histories\endcsname{$+$3.1}
\expandafter\def\csname val@uiv.p1.catalog.best-single@1.0.mean-over-histories\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@1.0.mean-over-histories\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@1.0.mean-over-histories\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.catalog.full-recert.score\endcsname{0.793}
\expandafter\def\csname cnt@uiv.p1.catalog.full-recert.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.full-recert.score\endcsname{79.3}
\expandafter\def\csname ppt@uiv.p1.catalog.full-recert.score\endcsname{$+$79.3}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{0.795}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{79.5}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{$+$79.5}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{0.790}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{79.0}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{$+$79.0}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0.022}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{2.2}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{$+$2.2}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.024}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{2.4}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{$+$2.4}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{0.793}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{79.3}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{$+$79.3}
\expandafter\def\csname val@uiv.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.catalog.keep-all.score\endcsname{0.760}
\expandafter\def\csname cnt@uiv.p1.catalog.keep-all.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.keep-all.score\endcsname{76.0}
\expandafter\def\csname ppt@uiv.p1.catalog.keep-all.score\endcsname{$+$76.0}
\expandafter\def\csname val@uiv.p1.catalog.old-decision.score\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p1.catalog.old-decision.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.old-decision.score\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p1.catalog.old-decision.score\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p1.catalog.oracle-on-T.score\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p1.catalog.oracle-on-T.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.oracle-on-T.score\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p1.catalog.oracle-on-T.score\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{0.807}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{80.7}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{$+$80.7}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{0.804}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{80.4}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{$+$80.4}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0.019}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{1.9}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{$+$1.9}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{0.799}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{79.9}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{$+$79.9}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.017}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{1.7}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{$+$1.7}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{0.793}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{79.3}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{$+$79.3}
\expandafter\def\csname val@uiv.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.catalog.replay-only.score\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-only.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.replay-only.score\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-only.score\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{0.803}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{80.3}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{$+$80.3}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0.022}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{2.2}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{$+$2.2}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{0.802}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{80.2}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{$+$80.2}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0.023}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{2.3}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{$+$2.3}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{0.810}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{81.0}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{$+$81.0}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{0.793}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{79.3}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{$+$79.3}
\expandafter\def\csname val@uiv.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.catalog.suspend-all.score\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p1.catalog.suspend-all.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.suspend-all.score\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p1.catalog.suspend-all.score\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{0.790}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{79.0}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{$+$79.0}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{0.797}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{79.7}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{$+$79.7}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{0.806}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{80.6}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{$+$80.6}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{0.793}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{79.3}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{$+$79.3}
\expandafter\def\csname val@uiv.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{0.014}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{1.4}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.ci95.1\endcsname{$+$1.4}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.mean\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.mean\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.mean\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{0.422}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{42.2}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{$+$42.2}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0.019}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{1.9}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{$+$1.9}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{1.3}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{$+$1.3}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{-0.047}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$-$4.7}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$-$4.7}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{-0.015}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{$-$1.5}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.ci95.1\endcsname{$-$1.5}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{-0.044}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$-$4.4}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$-$4.4}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.996}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{99.6}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{$+$99.6}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{-0.047}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$4.7}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$4.7}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{-0.015}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{$-$1.5}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.ci95.1\endcsname{$-$1.5}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{-0.044}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$4.4}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$4.4}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0.996}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{99.6}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{$+$99.6}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0.165}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{16.5}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{$+$16.5}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{-0.047}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{$-$4.7}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{$-$4.7}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{-0.015}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{$-$1.5}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{$-$1.5}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{-0.044}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{$-$4.4}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{$-$4.4}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.996}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{99.6}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{$+$99.6}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{123.100}
\expandafter\def\csname cnt@uiv.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{123}
\expandafter\def\csname pct@uiv.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{12310.0}
\expandafter\def\csname ppt@uiv.p1.cost.best-single@0.1.mean-requests-per-skill\endcsname{$+$12310.0}
\expandafter\def\csname val@uiv.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{161.075}
\expandafter\def\csname cnt@uiv.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{161}
\expandafter\def\csname pct@uiv.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{16107.5}
\expandafter\def\csname ppt@uiv.p1.cost.best-single@0.25.mean-requests-per-skill\endcsname{$+$16107.5}
\expandafter\def\csname val@uiv.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{226.300}
\expandafter\def\csname cnt@uiv.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{226}
\expandafter\def\csname pct@uiv.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{22630.0}
\expandafter\def\csname ppt@uiv.p1.cost.best-single@0.5.mean-requests-per-skill\endcsname{$+$22630.0}
\expandafter\def\csname val@uiv.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{356}
\expandafter\def\csname pct@uiv.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.cost.best-single@1.0.mean-requests-per-skill\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.cost.full-recert.mean-requests-per-skill\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.cost.full-recert.mean-requests-per-skill\endcsname{356}
\expandafter\def\csname pct@uiv.p1.cost.full-recert.mean-requests-per-skill\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.cost.full-recert.mean-requests-per-skill\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{123.100}
\expandafter\def\csname cnt@uiv.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{123}
\expandafter\def\csname pct@uiv.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{12310.0}
\expandafter\def\csname ppt@uiv.p1.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{$+$12310.0}
\expandafter\def\csname val@uiv.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{161.075}
\expandafter\def\csname cnt@uiv.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{161}
\expandafter\def\csname pct@uiv.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{16107.5}
\expandafter\def\csname ppt@uiv.p1.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{$+$16107.5}
\expandafter\def\csname val@uiv.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{226.300}
\expandafter\def\csname cnt@uiv.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{226}
\expandafter\def\csname pct@uiv.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{22630.0}
\expandafter\def\csname ppt@uiv.p1.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{$+$22630.0}
\expandafter\def\csname val@uiv.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{356}
\expandafter\def\csname pct@uiv.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{219.150}
\expandafter\def\csname cnt@uiv.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{219}
\expandafter\def\csname pct@uiv.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{21915.0}
\expandafter\def\csname ppt@uiv.p1.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{$+$21915.0}
\expandafter\def\csname val@uiv.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{256.988}
\expandafter\def\csname cnt@uiv.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{257}
\expandafter\def\csname pct@uiv.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{25698.8}
\expandafter\def\csname ppt@uiv.p1.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{$+$25698.8}
\expandafter\def\csname val@uiv.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{322.238}
\expandafter\def\csname cnt@uiv.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{322}
\expandafter\def\csname pct@uiv.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{32223.8}
\expandafter\def\csname ppt@uiv.p1.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{$+$32223.8}
\expandafter\def\csname val@uiv.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{452.250}
\expandafter\def\csname cnt@uiv.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{452}
\expandafter\def\csname pct@uiv.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{45225.0}
\expandafter\def\csname ppt@uiv.p1.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{$+$45225.0}
\expandafter\def\csname val@uiv.p1.cost.replay-only.mean-requests-per-skill\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p1.cost.replay-only.mean-requests-per-skill\endcsname{192}
\expandafter\def\csname pct@uiv.p1.cost.replay-only.mean-requests-per-skill\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.cost.replay-only.mean-requests-per-skill\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{219.100}
\expandafter\def\csname cnt@uiv.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{219}
\expandafter\def\csname pct@uiv.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{21910.0}
\expandafter\def\csname ppt@uiv.p1.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{$+$21910.0}
\expandafter\def\csname val@uiv.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{257.075}
\expandafter\def\csname cnt@uiv.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{257}
\expandafter\def\csname pct@uiv.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{25707.5}
\expandafter\def\csname ppt@uiv.p1.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{$+$25707.5}
\expandafter\def\csname val@uiv.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{322.300}
\expandafter\def\csname cnt@uiv.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{322}
\expandafter\def\csname pct@uiv.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{32230.0}
\expandafter\def\csname ppt@uiv.p1.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{$+$32230.0}
\expandafter\def\csname val@uiv.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{452.250}
\expandafter\def\csname cnt@uiv.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{452}
\expandafter\def\csname pct@uiv.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{45225.0}
\expandafter\def\csname ppt@uiv.p1.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{$+$45225.0}
\expandafter\def\csname val@uiv.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{123.100}
\expandafter\def\csname cnt@uiv.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{123}
\expandafter\def\csname pct@uiv.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{12310.0}
\expandafter\def\csname ppt@uiv.p1.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{$+$12310.0}
\expandafter\def\csname val@uiv.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{161.075}
\expandafter\def\csname cnt@uiv.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{161}
\expandafter\def\csname pct@uiv.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{16107.5}
\expandafter\def\csname ppt@uiv.p1.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{$+$16107.5}
\expandafter\def\csname val@uiv.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{226.300}
\expandafter\def\csname cnt@uiv.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{226}
\expandafter\def\csname pct@uiv.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{22630.0}
\expandafter\def\csname ppt@uiv.p1.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{$+$22630.0}
\expandafter\def\csname val@uiv.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{356}
\expandafter\def\csname pct@uiv.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.1.center-d1\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.1.center-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.1.center-d1\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.1.center-d1\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.1.direct\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.1.direct\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.1.direct\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.1.direct\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.1.dual-d2\endcsname{0.200}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.1.dual-d2\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.1.dual-d2\endcsname{20.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.1.dual-d2\endcsname{$+$20.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.25.center-d1\endcsname{0.350}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.25.center-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.25.center-d1\endcsname{35.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.25.center-d1\endcsname{$+$35.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.25.context-d1\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.25.context-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.25.context-d1\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.25.context-d1\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.25.direct\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.25.direct\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.25.direct\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.25.direct\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.25.dual-d2\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.25.dual-d2\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.25.dual-d2\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.25.dual-d2\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.25.grid2-d3\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.25.grid2-d3\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.25.grid2-d3\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.25.grid2-d3\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.5.center-d1\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.5.center-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.5.center-d1\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.5.center-d1\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.5.direct\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.5.direct\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.5.direct\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.5.direct\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@0.5.dual-d2\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@0.5.dual-d2\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.best-single@0.5.dual-d2\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@0.5.dual-d2\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p1.decide.best-single@1.0.direct\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.best-single@1.0.direct\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.best-single@1.0.direct\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.best-single@1.0.direct\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.128}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{12.8}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$12.8}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.005}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$0.5}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$0.5}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.074}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{7.4}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$7.4}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.023}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{2.3}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$2.3}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.119}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{11.9}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$11.9}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.095}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{9.5}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$9.5}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.017}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{1.7}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$1.7}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.079}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{7.9}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$7.9}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.031}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{3.1}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$3.1}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.070}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{7.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$7.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.052}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{5.2}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$5.2}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.048}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.8}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.8}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.016}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{1.6}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$1.6}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.005}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.5}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$0.5}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.033}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{3.3}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.3}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{-0.003}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$0.3}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$0.3}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.032}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.2}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.2}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.cost.full-recert-fresh\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.cost.full-recert-fresh\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.no-budget-tau.full-recert\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget-tau.old-source\endcsname{-0.073}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.no-budget-tau.old-source\endcsname{$-$7.3}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.no-budget-tau.old-source\endcsname{$-$7.3}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{-0.062}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{$-$6.2}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.no-budget-tau.replay-only\endcsname{$-$6.2}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.center-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.center-d1.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.sigma-used.agree-stable\endcsname{0.137}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.sigma-used.agree-stable\endcsname{13.7}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.sigma-used.agree-stable\endcsname{$+$13.7}
\expandafter\def\csname val@uiv.p1.decide.center-d1.sigma-used.disagree\endcsname{0.497}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.sigma-used.disagree\endcsname{49.7}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.sigma-used.disagree\endcsname{$+$49.7}
\expandafter\def\csname val@uiv.p1.decide.center-d1.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.strata-N.agree-drift\endcsname{7}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.strata-N.agree-drift\endcsname{7}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.strata-N.agree-drift\endcsname{700.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.strata-N.agree-drift\endcsname{$+$700.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.strata-N.agree-stable\endcsname{70}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.strata-N.agree-stable\endcsname{70}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.strata-N.agree-stable\endcsname{7000.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.strata-N.agree-stable\endcsname{$+$7000.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.strata-N.disagree\endcsname{17}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.strata-N.disagree\endcsname{17}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.strata-N.disagree\endcsname{1700.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.strata-N.disagree\endcsname{$+$1700.0}
\expandafter\def\csname val@uiv.p1.decide.center-d1.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname cnt@uiv.p1.decide.center-d1.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname pct@uiv.p1.decide.center-d1.strata-N.parse-fail\endcsname{200.0}
\expandafter\def\csname ppt@uiv.p1.decide.center-d1.strata-N.parse-fail\endcsname{$+$200.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.130}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{13.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$13.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.033}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$3.3}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$3.3}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.035}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{3.5}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$3.5}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.150}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{15.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$15.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.093}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{9.3}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$9.3}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{-0.050}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$5.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$5.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.102}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{10.2}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$10.2}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.088}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{8.8}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$8.8}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{-0.025}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$2.5}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$2.5}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.029}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{2.9}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$2.9}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{-0.015}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.5}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.5}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.047}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{4.7}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.7}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{-0.042}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$4.2}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$4.2}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.059}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{5.9}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$5.9}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{-0.025}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$2.5}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$2.5}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.044}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.4}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.4}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{-0.019}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$1.9}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$1.9}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.150}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{15.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$15.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{-0.026}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.6}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.6}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.034}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.4}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.4}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.cost.full-recert-fresh\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.cost.full-recert-fresh\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.no-budget-tau.full-recert\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget-tau.old-source\endcsname{-0.073}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.no-budget-tau.old-source\endcsname{$-$7.3}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.no-budget-tau.old-source\endcsname{$-$7.3}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.no-budget-tau.replay-only\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget.full-recert\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.context-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.context-d1.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.sigma-used.disagree\endcsname{0.458}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.sigma-used.disagree\endcsname{45.8}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.sigma-used.disagree\endcsname{$+$45.8}
\expandafter\def\csname val@uiv.p1.decide.context-d1.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.strata-N.agree-drift\endcsname{11}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.strata-N.agree-drift\endcsname{11}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.strata-N.agree-drift\endcsname{1100.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.strata-N.agree-drift\endcsname{$+$1100.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.strata-N.agree-stable\endcsname{73}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.strata-N.agree-stable\endcsname{73}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.strata-N.agree-stable\endcsname{7300.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.strata-N.agree-stable\endcsname{$+$7300.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.strata-N.disagree\endcsname{11}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.strata-N.disagree\endcsname{11}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.strata-N.disagree\endcsname{1100.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.strata-N.disagree\endcsname{$+$1100.0}
\expandafter\def\csname val@uiv.p1.decide.context-d1.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname cnt@uiv.p1.decide.context-d1.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.context-d1.strata-N.parse-fail\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.context-d1.strata-N.parse-fail\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{126.250}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{12625.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$12625.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{-0.023}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$-$2.3}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$-$2.3}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.139}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{13.9}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$13.9}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{222.300}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{22230.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$22230.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.076}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{7.6}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$7.6}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222.250}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{22225.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$22225.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{-0.013}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.3}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.3}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.086}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{8.6}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$8.6}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{126.250}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{12625.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$12625.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{-0.005}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$0.5}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$0.5}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.112}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{11.2}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$11.2}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{168.850}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{169}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{16885.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$16885.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.085}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{8.5}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$8.5}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{264.600}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{265}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{26460.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$26460.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.048}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{4.8}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$4.8}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264.850}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{265}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{26485.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$26485.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.067}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{6.7}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.7}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{168.850}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{169}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{16885.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$16885.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.049}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{4.9}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$4.9}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{241.650}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{242}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{24165.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$24165.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.047}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.7}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.7}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{337.450}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{337}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{33745.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$33745.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.035}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{3.5}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$3.5}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{337.650}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{338}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{33765.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$33765.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.036}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{3.6}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.6}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{241.650}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{242}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{24165.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$24165.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{-0.012}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$1.2}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$1.2}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.044}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{4.4}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$4.4}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{387.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{387}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{38700.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$38700.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{483.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{483}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{48300.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$48300.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{483.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{483}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{48300.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$48300.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{387.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{387}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{38700.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$38700.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{291}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{291}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{29100.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.cost.full-recert-fresh\endcsname{$+$29100.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.no-budget-tau.full-recert\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{-0.083}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{$-$8.3}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.no-budget-tau.old-source\endcsname{$-$8.3}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{-0.073}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{$-$7.3}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.no-budget-tau.replay-only\endcsname{$-$7.3}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.sigma-used.agree-drift\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{0.202}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{20.2}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.sigma-used.agree-stable\endcsname{$+$20.2}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.sigma-used.disagree\endcsname{0.640}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.sigma-used.disagree\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.sigma-used.disagree\endcsname{64.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.sigma-used.disagree\endcsname{$+$64.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.strata-N.agree-drift\endcsname{10}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.strata-N.agree-drift\endcsname{10}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.strata-N.agree-drift\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.strata-N.agree-drift\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.strata-N.agree-stable\endcsname{66}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.strata-N.agree-stable\endcsname{66}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.strata-N.agree-stable\endcsname{6600.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.strata-N.agree-stable\endcsname{$+$6600.0}
\expandafter\def\csname val@uiv.p1.decide.dual-d2.strata-N.disagree\endcsname{20}
\expandafter\def\csname cnt@uiv.p1.decide.dual-d2.strata-N.disagree\endcsname{20}
\expandafter\def\csname pct@uiv.p1.decide.dual-d2.strata-N.disagree\endcsname{2000.0}
\expandafter\def\csname ppt@uiv.p1.decide.dual-d2.strata-N.disagree\endcsname{$+$2000.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{134.150}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{134}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{13415.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$13415.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{-0.036}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$-$3.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$-$3.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.111}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{11.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$11.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{230.300}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{230}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{23030.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$23030.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.046}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$4.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$4.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.092}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{9.2}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$9.2}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{230.150}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{230}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{23015.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$23015.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{-0.056}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$5.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$5.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.110}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{11.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$11.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{134.150}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{134}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{13415.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$13415.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{-0.060}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$6.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$6.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.107}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{10.7}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$10.7}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{187.450}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{187}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{18745.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$18745.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{-0.027}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$-$2.7}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$-$2.7}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.076}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{7.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$7.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{283.350}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{283}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{28335.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$28335.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{-0.040}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$4.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$4.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.076}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{7.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$7.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{283.450}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{283}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{28345.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$28345.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{-0.040}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$4.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$4.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.076}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{7.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$7.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{187.450}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{187}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{18745.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$18745.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{-0.046}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$4.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$4.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.049}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{4.9}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$4.9}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{279.550}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{280}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{27955.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$27955.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{-0.041}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$4.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$4.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.048}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{4.8}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$4.8}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{375.500}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{376}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{37550.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$37550.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{-0.026}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$2.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$2.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.033}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{3.3}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$3.3}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{375.550}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{376}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{37555.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$37555.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{-0.039}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$3.9}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$3.9}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.040}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{4.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$4.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{279.550}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{280}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{27955.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$27955.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{0.150}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{15.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$15.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{-0.047}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$4.7}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$4.7}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.031}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{462.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{462}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{46200.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$46200.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{558.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{558}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{55800.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$55800.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{558.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{558}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{55800.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$55800.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{462.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{462}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{46200.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$46200.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{366}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{366}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{36600.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.cost.full-recert-fresh\endcsname{$+$36600.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.no-budget-tau.full-recert\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{-0.146}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{$-$14.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.no-budget-tau.old-source\endcsname{$-$14.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{-0.156}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{$-$15.6}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.no-budget-tau.replay-only\endcsname{$-$15.6}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget.full-recert\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.sigma-used.agree-drift\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.sigma-used.agree-drift\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.sigma-used.agree-drift\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{0.211}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{21.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.sigma-used.agree-stable\endcsname{$+$21.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.sigma-used.disagree\endcsname{0.498}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.sigma-used.disagree\endcsname{49.8}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.sigma-used.disagree\endcsname{$+$49.8}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{0.471}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{47.1}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.sigma-used.parse-fail\endcsname{$+$47.1}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.strata-N.agree-drift\endcsname{8}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.strata-N.agree-drift\endcsname{8}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.strata-N.agree-drift\endcsname{800.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.strata-N.agree-drift\endcsname{$+$800.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{62}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{62}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{6200.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.strata-N.agree-stable\endcsname{$+$6200.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.strata-N.disagree\endcsname{22}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.strata-N.disagree\endcsname{22}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.strata-N.disagree\endcsname{2200.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.strata-N.disagree\endcsname{$+$2200.0}
\expandafter\def\csname val@uiv.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{4}
\expandafter\def\csname cnt@uiv.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{4}
\expandafter\def\csname pct@uiv.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{400.0}
\expandafter\def\csname ppt@uiv.p1.decide.grid2-d3.strata-N.parse-fail\endcsname{$+$400.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{126.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{12600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$12600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.097}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{9.7}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$9.7}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{222.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{22200.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$22200.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.019}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{1.9}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$1.9}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{22200.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$22200.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.200}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{20.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$20.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{-0.026}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.6}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.6}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.067}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{6.7}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.7}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{126.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{12600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$12600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.090}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{9.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$9.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{168}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.061}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{6.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$6.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{264.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{264}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{26400.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$26400.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0.150}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{15.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$15.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{-0.034}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$3.4}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$3.4}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.037}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{3.7}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$3.7}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{26400.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$26400.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.350}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{35.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$35.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{-0.025}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.5}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.5}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.051}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{5.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$5.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{168}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{-0.042}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$4.2}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$-$4.2}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{-0.014}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$1.4}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$1.4}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.034}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{3.4}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$3.4}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{336.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{336}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{33600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$33600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{-0.020}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$2.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$2.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.024}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.4}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.4}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{336.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{336}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{33600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$33600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{-0.024}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.4}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.4}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.035}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.5}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.5}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{480.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{480}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{48000.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$48000.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{480.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{480}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{48000.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$48000.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{288}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{288}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget.full-recert\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.sigma-used.agree-drift\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{0.722}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{72.2}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.sigma-used.disagree\endcsname{$+$72.2}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{6}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{6}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.strata-N.agree-drift\endcsname{$+$600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{76}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{76}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{7600.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.strata-N.agree-stable\endcsname{$+$7600.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{13}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{13}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{1300.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.strata-N.disagree\endcsname{$+$1300.0}
\expandafter\def\csname val@uiv.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname cnt@uiv.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{1}
\expandafter\def\csname pct@uiv.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.decide.zoomclick-d3.strata-N.parse-fail\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.bracket-costs.0\endcsname{226.300}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.bracket-costs.0\endcsname{226}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.bracket-costs.0\endcsname{22630.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.bracket-costs.0\endcsname{$+$22630.0}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.bracket-costs.1\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.bracket-costs.1\endcsname{356}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.bracket-costs.1\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.bracket-costs.1\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{-0.022}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$2.2}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$2.2}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.ci95.1\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.mean\endcsname{-0.015}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.mean\endcsname{$-$1.5}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.mean\endcsname{$-$1.5}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.927}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{92.7}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{$+$92.7}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{0.819}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{81.9}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.score-at-rcr-cost\endcsname{$+$81.9}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.status\endcsname{ok}
\expandafter\def\csname val@uiv.p1.equal-cost.best-single.weight\endcsname{0.236}
\expandafter\def\csname cnt@uiv.p1.equal-cost.best-single.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.best-single.weight\endcsname{23.6}
\expandafter\def\csname ppt@uiv.p1.equal-cost.best-single.weight\endcsname{$+$23.6}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{226.300}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{226}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{22630.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{$+$22630.0}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{356}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0.005}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0.5}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{$+$0.5}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{0.799}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{79.9}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{$+$79.9}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.status\endcsname{ok}
\expandafter\def\csname val@uiv.p1.equal-cost.generic-ppi-source.weight\endcsname{0.236}
\expandafter\def\csname cnt@uiv.p1.equal-cost.generic-ppi-source.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.generic-ppi-source.weight\endcsname{23.6}
\expandafter\def\csname ppt@uiv.p1.equal-cost.generic-ppi-source.weight\endcsname{$+$23.6}
\expandafter\def\csname val@uiv.p1.equal-cost.rcr-cost\endcsname{256.988}
\expandafter\def\csname cnt@uiv.p1.equal-cost.rcr-cost\endcsname{257}
\expandafter\def\csname pct@uiv.p1.equal-cost.rcr-cost\endcsname{25698.8}
\expandafter\def\csname ppt@uiv.p1.equal-cost.rcr-cost\endcsname{$+$25698.8}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{219.100}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{219}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{21910.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{$+$21910.0}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{257.075}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{257}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{25707.5}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{$+$25707.5}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0.183}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{18.3}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{$+$18.3}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{0.802}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{80.2}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{$+$80.2}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.status\endcsname{ok}
\expandafter\def\csname val@uiv.p1.equal-cost.replay-ppi-uniform.weight\endcsname{0.998}
\expandafter\def\csname cnt@uiv.p1.equal-cost.replay-ppi-uniform.weight\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.replay-ppi-uniform.weight\endcsname{99.8}
\expandafter\def\csname ppt@uiv.p1.equal-cost.replay-ppi-uniform.weight\endcsname{$+$99.8}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{226.300}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{226}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{22630.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.bracket-costs.0\endcsname{$+$22630.0}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{356.250}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{356}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{35625.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.bracket-costs.1\endcsname{$+$35625.0}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{0.222}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{22.2}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{$+$22.2}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{0.803}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{80.3}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{$+$80.3}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.status\endcsname{ok}
\expandafter\def\csname val@uiv.p1.equal-cost.uniform-fresh.weight\endcsname{0.236}
\expandafter\def\csname cnt@uiv.p1.equal-cost.uniform-fresh.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p1.equal-cost.uniform-fresh.weight\endcsname{23.6}
\expandafter\def\csname ppt@uiv.p1.equal-cost.uniform-fresh.weight\endcsname{$+$23.6}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.acc-macro\endcsname{0.778}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.acc-macro\endcsname{77.8}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.acc-macro\endcsname{$+$77.8}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.mean-requests\endcsname{2.007}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.mean-requests\endcsname{200.7}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.mean-requests\endcsname{$+$200.7}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.n\endcsname{144}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{-0.118}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{$-$11.8}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{$-$11.8}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{-0.000}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{-0.111}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$11.1}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$11.1}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{-0.056}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{$-$5.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.mean\endcsname{$-$5.6}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.980}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{98.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{$+$98.0}
\expandafter\def\csname val@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.939}
\expandafter\def\csname cnt@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{93.9}
\expandafter\def\csname ppt@uiv.p1.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$93.9}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.acc-macro\endcsname{0.778}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.acc-macro\endcsname{77.8}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.acc-macro\endcsname{$+$77.8}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.mean-requests\endcsname{2.007}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.mean-requests\endcsname{200.7}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.mean-requests\endcsname{$+$200.7}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.n\endcsname{144}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{-0.111}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{$-$11.1}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{$-$11.1}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{-0.104}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$10.4}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$10.4}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{-0.056}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{$-$5.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.mean\endcsname{$-$5.6}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.994}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{99.4}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{$+$99.4}
\expandafter\def\csname val@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.968}
\expandafter\def\csname cnt@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{96.8}
\expandafter\def\csname ppt@uiv.p1.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$96.8}
\expandafter\def\csname val@uiv.p1.execution-layer.direct\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p1.execution-layer.direct\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.direct\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p1.execution-layer.direct\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p1.execution-layer.direct-sc3\endcsname{0.812}
\expandafter\def\csname cnt@uiv.p1.execution-layer.direct-sc3\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.direct-sc3\endcsname{81.2}
\expandafter\def\csname ppt@uiv.p1.execution-layer.direct-sc3\endcsname{$+$81.2}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.acc-macro\endcsname{0.729}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.acc-macro\endcsname{72.9}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.acc-macro\endcsname{$+$72.9}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.mean-requests\endcsname{3.021}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.mean-requests\endcsname{3}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.mean-requests\endcsname{302.1}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.mean-requests\endcsname{$+$302.1}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.n\endcsname{144}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{-0.160}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{$-$16.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{$-$16.0}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{-0.049}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{$-$4.9}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{$-$4.9}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{-0.146}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{$-$14.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{$-$14.6}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{-0.104}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{$-$10.4}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{$-$10.4}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.999}
\expandafter\def\csname cnt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{99.9}
\expandafter\def\csname ppt@uiv.p1.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$99.9}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.acc-macro\endcsname{0.757}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.acc-macro\endcsname{75.7}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.acc-macro\endcsname{$+$75.7}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.mean-requests\endcsname{3.653}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.mean-requests\endcsname{4}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.mean-requests\endcsname{365.3}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.mean-requests\endcsname{$+$365.3}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.n\endcsname{144}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{-0.139}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{$-$13.9}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{$-$13.9}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{-0.125}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$12.5}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$12.5}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{-0.076}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{$-$7.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{$-$7.6}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.996}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{99.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{$+$99.6}
\expandafter\def\csname val@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.986}
\expandafter\def\csname cnt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{98.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$98.6}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{0.778}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{77.8}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.acc-macro\endcsname{$+$77.8}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{3.000}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{3}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{300.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.mean-requests\endcsname{$+$300.0}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.n\endcsname{144}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{-0.111}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{$-$11.1}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{$-$11.1}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{-0.104}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$10.4}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$10.4}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{-0.056}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{$-$5.6}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{$-$5.6}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.987}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{98.7}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{$+$98.7}
\expandafter\def\csname val@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.963}
\expandafter\def\csname cnt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{96.3}
\expandafter\def\csname ppt@uiv.p1.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$96.3}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-generic-ppi-source.max\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-generic-ppi-source.min\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.max\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname cnt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname pct@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p1.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname val@uiv.p1.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p1.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p1.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p1.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p1.n-cal-apps\endcsname{12}
\expandafter\def\csname cnt@uiv.p1.n-cal-apps\endcsname{12}
\expandafter\def\csname pct@uiv.p1.n-cal-apps\endcsname{1200.0}
\expandafter\def\csname ppt@uiv.p1.n-cal-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@uiv.p1.n-test\endcsname{144}
\expandafter\def\csname cnt@uiv.p1.n-test\endcsname{144}
\expandafter\def\csname pct@uiv.p1.n-test\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p1.n-test\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p1.n-test-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p1.n-test-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p1.n-test-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p1.n-test-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p1.primary.best-single.cost\endcsname{161.075}
\expandafter\def\csname cnt@uiv.p1.primary.best-single.cost\endcsname{161}
\expandafter\def\csname pct@uiv.p1.primary.best-single.cost\endcsname{16107.5}
\expandafter\def\csname ppt@uiv.p1.primary.best-single.cost\endcsname{$+$16107.5}
\expandafter\def\csname val@uiv.p1.primary.best-single.cost-fraction-of-full\endcsname{0.452}
\expandafter\def\csname cnt@uiv.p1.primary.best-single.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.best-single.cost-fraction-of-full\endcsname{45.2}
\expandafter\def\csname ppt@uiv.p1.primary.best-single.cost-fraction-of-full\endcsname{$+$45.2}
\expandafter\def\csname val@uiv.p1.primary.best-single.score\endcsname{0.802}
\expandafter\def\csname cnt@uiv.p1.primary.best-single.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.best-single.score\endcsname{80.2}
\expandafter\def\csname ppt@uiv.p1.primary.best-single.score\endcsname{$+$80.2}
\expandafter\def\csname val@uiv.p1.primary.best-single.vs-full-recert\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p1.primary.best-single.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.best-single.vs-full-recert\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p1.primary.best-single.vs-full-recert\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p1.primary.best-single.vs-suspend-all\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.primary.best-single.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.best-single.vs-suspend-all\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.primary.best-single.vs-suspend-all\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.primary.generic-ppi-source.cost\endcsname{161.075}
\expandafter\def\csname cnt@uiv.p1.primary.generic-ppi-source.cost\endcsname{161}
\expandafter\def\csname pct@uiv.p1.primary.generic-ppi-source.cost\endcsname{16107.5}
\expandafter\def\csname ppt@uiv.p1.primary.generic-ppi-source.cost\endcsname{$+$16107.5}
\expandafter\def\csname val@uiv.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0.452}
\expandafter\def\csname cnt@uiv.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{45.2}
\expandafter\def\csname ppt@uiv.p1.primary.generic-ppi-source.cost-fraction-of-full\endcsname{$+$45.2}
\expandafter\def\csname val@uiv.p1.primary.generic-ppi-source.score\endcsname{0.790}
\expandafter\def\csname cnt@uiv.p1.primary.generic-ppi-source.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.generic-ppi-source.score\endcsname{79.0}
\expandafter\def\csname ppt@uiv.p1.primary.generic-ppi-source.score\endcsname{$+$79.0}
\expandafter\def\csname val@uiv.p1.primary.generic-ppi-source.vs-full-recert\endcsname{-0.003}
\expandafter\def\csname cnt@uiv.p1.primary.generic-ppi-source.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.generic-ppi-source.vs-full-recert\endcsname{$-$0.3}
\expandafter\def\csname ppt@uiv.p1.primary.generic-ppi-source.vs-full-recert\endcsname{$-$0.3}
\expandafter\def\csname val@uiv.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{-0.043}
\expandafter\def\csname cnt@uiv.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{$-$4.3}
\expandafter\def\csname ppt@uiv.p1.primary.generic-ppi-source.vs-suspend-all\endcsname{$-$4.3}
\expandafter\def\csname val@uiv.p1.primary.rcr-stratified.cost\endcsname{256.988}
\expandafter\def\csname cnt@uiv.p1.primary.rcr-stratified.cost\endcsname{257}
\expandafter\def\csname pct@uiv.p1.primary.rcr-stratified.cost\endcsname{25698.8}
\expandafter\def\csname ppt@uiv.p1.primary.rcr-stratified.cost\endcsname{$+$25698.8}
\expandafter\def\csname val@uiv.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{0.721}
\expandafter\def\csname cnt@uiv.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{72.1}
\expandafter\def\csname ppt@uiv.p1.primary.rcr-stratified.cost-fraction-of-full\endcsname{$+$72.1}
\expandafter\def\csname val@uiv.p1.primary.rcr-stratified.score\endcsname{0.804}
\expandafter\def\csname cnt@uiv.p1.primary.rcr-stratified.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.rcr-stratified.score\endcsname{80.4}
\expandafter\def\csname ppt@uiv.p1.primary.rcr-stratified.score\endcsname{$+$80.4}
\expandafter\def\csname val@uiv.p1.primary.rcr-stratified.vs-full-recert\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p1.primary.rcr-stratified.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.rcr-stratified.vs-full-recert\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p1.primary.rcr-stratified.vs-full-recert\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p1.primary.rcr-stratified.vs-suspend-all\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p1.primary.rcr-stratified.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.rcr-stratified.vs-suspend-all\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p1.primary.rcr-stratified.vs-suspend-all\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p1.primary.replay-ppi-uniform.cost\endcsname{257.075}
\expandafter\def\csname cnt@uiv.p1.primary.replay-ppi-uniform.cost\endcsname{257}
\expandafter\def\csname pct@uiv.p1.primary.replay-ppi-uniform.cost\endcsname{25707.5}
\expandafter\def\csname ppt@uiv.p1.primary.replay-ppi-uniform.cost\endcsname{$+$25707.5}
\expandafter\def\csname val@uiv.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{0.722}
\expandafter\def\csname cnt@uiv.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{72.2}
\expandafter\def\csname ppt@uiv.p1.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{$+$72.2}
\expandafter\def\csname val@uiv.p1.primary.replay-ppi-uniform.score\endcsname{0.802}
\expandafter\def\csname cnt@uiv.p1.primary.replay-ppi-uniform.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.replay-ppi-uniform.score\endcsname{80.2}
\expandafter\def\csname ppt@uiv.p1.primary.replay-ppi-uniform.score\endcsname{$+$80.2}
\expandafter\def\csname val@uiv.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p1.primary.replay-ppi-uniform.vs-full-recert\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p1.primary.replay-ppi-uniform.vs-suspend-all\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p1.primary.uniform-fresh.cost\endcsname{161.075}
\expandafter\def\csname cnt@uiv.p1.primary.uniform-fresh.cost\endcsname{161}
\expandafter\def\csname pct@uiv.p1.primary.uniform-fresh.cost\endcsname{16107.5}
\expandafter\def\csname ppt@uiv.p1.primary.uniform-fresh.cost\endcsname{$+$16107.5}
\expandafter\def\csname val@uiv.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{0.452}
\expandafter\def\csname cnt@uiv.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{45.2}
\expandafter\def\csname ppt@uiv.p1.primary.uniform-fresh.cost-fraction-of-full\endcsname{$+$45.2}
\expandafter\def\csname val@uiv.p1.primary.uniform-fresh.score\endcsname{0.797}
\expandafter\def\csname cnt@uiv.p1.primary.uniform-fresh.score\endcsname{1}
\expandafter\def\csname pct@uiv.p1.primary.uniform-fresh.score\endcsname{79.7}
\expandafter\def\csname ppt@uiv.p1.primary.uniform-fresh.score\endcsname{$+$79.7}
\expandafter\def\csname val@uiv.p1.primary.uniform-fresh.vs-full-recert\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p1.primary.uniform-fresh.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.uniform-fresh.vs-full-recert\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p1.primary.uniform-fresh.vs-full-recert\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p1.primary.uniform-fresh.vs-suspend-all\endcsname{-0.036}
\expandafter\def\csname cnt@uiv.p1.primary.uniform-fresh.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p1.primary.uniform-fresh.vs-suspend-all\endcsname{$-$3.6}
\expandafter\def\csname ppt@uiv.p1.primary.uniform-fresh.vs-suspend-all\endcsname{$-$3.6}
\expandafter\def\csname val@uiv.p2.catalog.best-single@0.1.mean-over-histories\endcsname{0.830}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@0.1.mean-over-histories\endcsname{83.0}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@0.1.mean-over-histories\endcsname{$+$83.0}
\expandafter\def\csname val@uiv.p2.catalog.best-single@0.1.sd-over-histories\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@0.1.sd-over-histories\endcsname{1.3}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@0.1.sd-over-histories\endcsname{$+$1.3}
\expandafter\def\csname val@uiv.p2.catalog.best-single@0.25.mean-over-histories\endcsname{0.831}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@0.25.mean-over-histories\endcsname{83.1}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@0.25.mean-over-histories\endcsname{$+$83.1}
\expandafter\def\csname val@uiv.p2.catalog.best-single@0.25.sd-over-histories\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@0.25.sd-over-histories\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@0.25.sd-over-histories\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p2.catalog.best-single@0.5.mean-over-histories\endcsname{0.826}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@0.5.mean-over-histories\endcsname{82.6}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@0.5.mean-over-histories\endcsname{$+$82.6}
\expandafter\def\csname val@uiv.p2.catalog.best-single@0.5.sd-over-histories\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@0.5.sd-over-histories\endcsname{1.3}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@0.5.sd-over-histories\endcsname{$+$1.3}
\expandafter\def\csname val@uiv.p2.catalog.best-single@1.0.mean-over-histories\endcsname{0.812}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@1.0.mean-over-histories\endcsname{81.2}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@1.0.mean-over-histories\endcsname{$+$81.2}
\expandafter\def\csname val@uiv.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.catalog.best-single@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.catalog.full-recert.score\endcsname{0.832}
\expandafter\def\csname cnt@uiv.p2.catalog.full-recert.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.full-recert.score\endcsname{83.2}
\expandafter\def\csname ppt@uiv.p2.catalog.full-recert.score\endcsname{$+$83.2}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{0.828}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{82.8}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@0.1.mean-over-histories\endcsname{$+$82.8}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@0.1.sd-over-histories\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{0.826}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{82.6}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@0.25.mean-over-histories\endcsname{$+$82.6}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@0.25.sd-over-histories\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{0.827}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{82.7}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@0.5.mean-over-histories\endcsname{$+$82.7}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@0.5.sd-over-histories\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{0.832}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{83.2}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@1.0.mean-over-histories\endcsname{$+$83.2}
\expandafter\def\csname val@uiv.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.catalog.generic-ppi-source@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.catalog.keep-all.score\endcsname{0.816}
\expandafter\def\csname cnt@uiv.p2.catalog.keep-all.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.keep-all.score\endcsname{81.6}
\expandafter\def\csname ppt@uiv.p2.catalog.keep-all.score\endcsname{$+$81.6}
\expandafter\def\csname val@uiv.p2.catalog.old-decision.score\endcsname{0.818}
\expandafter\def\csname cnt@uiv.p2.catalog.old-decision.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.old-decision.score\endcsname{81.8}
\expandafter\def\csname ppt@uiv.p2.catalog.old-decision.score\endcsname{$+$81.8}
\expandafter\def\csname val@uiv.p2.catalog.oracle-on-T.score\endcsname{0.840}
\expandafter\def\csname cnt@uiv.p2.catalog.oracle-on-T.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.oracle-on-T.score\endcsname{84.0}
\expandafter\def\csname ppt@uiv.p2.catalog.oracle-on-T.score\endcsname{$+$84.0}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{0.826}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{82.6}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@0.1.mean-over-histories\endcsname{$+$82.6}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@0.1.sd-over-histories\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{0.829}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{82.9}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@0.25.mean-over-histories\endcsname{$+$82.9}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@0.25.sd-over-histories\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{0.832}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{83.2}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@0.5.mean-over-histories\endcsname{$+$83.2}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@0.5.sd-over-histories\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{0.832}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{83.2}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@1.0.mean-over-histories\endcsname{$+$83.2}
\expandafter\def\csname val@uiv.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.catalog.rcr-stratified@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.catalog.replay-only.score\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-only.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.replay-only.score\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-only.score\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{0.826}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{82.6}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@0.1.mean-over-histories\endcsname{$+$82.6}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@0.1.sd-over-histories\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{0.828}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{82.8}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@0.25.mean-over-histories\endcsname{$+$82.8}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@0.25.sd-over-histories\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{0.826}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{82.6}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@0.5.mean-over-histories\endcsname{$+$82.6}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@0.5.sd-over-histories\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{0.832}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{83.2}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@1.0.mean-over-histories\endcsname{$+$83.2}
\expandafter\def\csname val@uiv.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.catalog.replay-ppi-uniform@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.catalog.suspend-all.score\endcsname{0.840}
\expandafter\def\csname cnt@uiv.p2.catalog.suspend-all.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.suspend-all.score\endcsname{84.0}
\expandafter\def\csname ppt@uiv.p2.catalog.suspend-all.score\endcsname{$+$84.0}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{0.819}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{81.9}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@0.1.mean-over-histories\endcsname{$+$81.9}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@0.1.sd-over-histories\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{0.821}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{82.1}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@0.25.mean-over-histories\endcsname{$+$82.1}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@0.25.sd-over-histories\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{0.829}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{82.9}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@0.5.mean-over-histories\endcsname{$+$82.9}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@0.5.sd-over-histories\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{0.832}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{1}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{83.2}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@1.0.mean-over-histories\endcsname{$+$83.2}
\expandafter\def\csname val@uiv.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0}
\expandafter\def\csname pct@uiv.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.catalog.uniform-fresh@1.0.sd-over-histories\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{-0.009}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$0.9}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.ci95.0\endcsname{$-$0.9}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{0.006}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{0.6}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.ci95.1\endcsname{$+$0.6}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.mean\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.mean\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.mean\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{0.660}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{66.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-gt0\endcsname{$+$66.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{1.3}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-best-single.p-one-sided-noninferiority-0.01\endcsname{$+$1.3}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{-0.009}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$-$0.9}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.0\endcsname{$-$0.9}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0.006}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{0.6}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).ci95.1\endcsname{$+$0.6}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).lower95-one-sided\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{-0.002}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).mean\endcsname{$-$0.2}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{0.726}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{72.6}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-gt0\endcsname{$+$72.6}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-full-recert-noninferiority(margin -0.01).p-one-sided-noninferiority-0.01\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.0\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.ci95.1\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.lower95-one-sided\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.mean\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-gt0\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-generic-ppi-source.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.ci95.0\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.ci95.1\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{0.005}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{0.5}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.lower95-one-sided\endcsname{$+$0.5}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.mean\endcsname{0.012}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.mean\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.mean\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-gt0\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-old-decision.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{-0.011}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$1.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.ci95.0\endcsname{$-$1.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.ci95.1\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.lower95-one-sided\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.mean\endcsname{-0.004}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.mean\endcsname{$-$0.4}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.mean\endcsname{$-$0.4}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{0.867}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{86.7}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-gt0\endcsname{$+$86.7}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0.049}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{4.9}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-only.p-one-sided-noninferiority-0.01\endcsname{$+$4.9}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.0\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.ci95.1\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.lower95-one-sided\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.mean\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{1.3}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-gt0\endcsname{$+$1.3}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-replay-ppi-uniform.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{-0.027}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{$-$2.7}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.0\endcsname{$-$2.7}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).ci95.1\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{-0.024}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{$-$2.4}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).lower95-one-sided\endcsname{$-$2.4}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{-0.011}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{$-$1.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).mean\endcsname{$-$1.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{0.936}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{93.6}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-gt0\endcsname{$+$93.6}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{0.531}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{53.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-suspend-all(direct).p-one-sided-noninferiority-0.01\endcsname{$+$53.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.0\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.ci95.1\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.lower95-one-sided\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.mean\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0.034}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{3.4}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-gt0\endcsname{$+$3.4}
\expandafter\def\csname val@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.comparisons.rcr-vs-uniform-fresh.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{122.550}
\expandafter\def\csname cnt@uiv.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{123}
\expandafter\def\csname pct@uiv.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{12255.0}
\expandafter\def\csname ppt@uiv.p2.cost.best-single@0.1.mean-requests-per-skill\endcsname{$+$12255.0}
\expandafter\def\csname val@uiv.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{159.637}
\expandafter\def\csname cnt@uiv.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{160}
\expandafter\def\csname pct@uiv.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{15963.7}
\expandafter\def\csname ppt@uiv.p2.cost.best-single@0.25.mean-requests-per-skill\endcsname{$+$15963.7}
\expandafter\def\csname val@uiv.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{223.137}
\expandafter\def\csname cnt@uiv.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{223}
\expandafter\def\csname pct@uiv.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{22313.8}
\expandafter\def\csname ppt@uiv.p2.cost.best-single@0.5.mean-requests-per-skill\endcsname{$+$22313.8}
\expandafter\def\csname val@uiv.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{350}
\expandafter\def\csname pct@uiv.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.cost.best-single@1.0.mean-requests-per-skill\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.cost.full-recert.mean-requests-per-skill\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.cost.full-recert.mean-requests-per-skill\endcsname{350}
\expandafter\def\csname pct@uiv.p2.cost.full-recert.mean-requests-per-skill\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.cost.full-recert.mean-requests-per-skill\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{122.550}
\expandafter\def\csname cnt@uiv.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{123}
\expandafter\def\csname pct@uiv.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{12255.0}
\expandafter\def\csname ppt@uiv.p2.cost.generic-ppi-source@0.1.mean-requests-per-skill\endcsname{$+$12255.0}
\expandafter\def\csname val@uiv.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{159.637}
\expandafter\def\csname cnt@uiv.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{160}
\expandafter\def\csname pct@uiv.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{15963.7}
\expandafter\def\csname ppt@uiv.p2.cost.generic-ppi-source@0.25.mean-requests-per-skill\endcsname{$+$15963.7}
\expandafter\def\csname val@uiv.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{223.137}
\expandafter\def\csname cnt@uiv.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{223}
\expandafter\def\csname pct@uiv.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{22313.8}
\expandafter\def\csname ppt@uiv.p2.cost.generic-ppi-source@0.5.mean-requests-per-skill\endcsname{$+$22313.8}
\expandafter\def\csname val@uiv.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{350}
\expandafter\def\csname pct@uiv.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.cost.generic-ppi-source@1.0.mean-requests-per-skill\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{218.787}
\expandafter\def\csname cnt@uiv.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{219}
\expandafter\def\csname pct@uiv.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{21878.8}
\expandafter\def\csname ppt@uiv.p2.cost.rcr-stratified@0.1.mean-requests-per-skill\endcsname{$+$21878.8}
\expandafter\def\csname val@uiv.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{255.838}
\expandafter\def\csname cnt@uiv.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{256}
\expandafter\def\csname pct@uiv.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{25583.8}
\expandafter\def\csname ppt@uiv.p2.cost.rcr-stratified@0.25.mean-requests-per-skill\endcsname{$+$25583.8}
\expandafter\def\csname val@uiv.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{319.163}
\expandafter\def\csname cnt@uiv.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{319}
\expandafter\def\csname pct@uiv.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{31916.3}
\expandafter\def\csname ppt@uiv.p2.cost.rcr-stratified@0.5.mean-requests-per-skill\endcsname{$+$31916.3}
\expandafter\def\csname val@uiv.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{446.000}
\expandafter\def\csname cnt@uiv.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{446}
\expandafter\def\csname pct@uiv.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{44600.0}
\expandafter\def\csname ppt@uiv.p2.cost.rcr-stratified@1.0.mean-requests-per-skill\endcsname{$+$44600.0}
\expandafter\def\csname val@uiv.p2.cost.replay-only.mean-requests-per-skill\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p2.cost.replay-only.mean-requests-per-skill\endcsname{192}
\expandafter\def\csname pct@uiv.p2.cost.replay-only.mean-requests-per-skill\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.cost.replay-only.mean-requests-per-skill\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{218.550}
\expandafter\def\csname cnt@uiv.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{219}
\expandafter\def\csname pct@uiv.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{21855.0}
\expandafter\def\csname ppt@uiv.p2.cost.replay-ppi-uniform@0.1.mean-requests-per-skill\endcsname{$+$21855.0}
\expandafter\def\csname val@uiv.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{255.637}
\expandafter\def\csname cnt@uiv.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{256}
\expandafter\def\csname pct@uiv.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{25563.8}
\expandafter\def\csname ppt@uiv.p2.cost.replay-ppi-uniform@0.25.mean-requests-per-skill\endcsname{$+$25563.8}
\expandafter\def\csname val@uiv.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{319.137}
\expandafter\def\csname cnt@uiv.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{319}
\expandafter\def\csname pct@uiv.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{31913.8}
\expandafter\def\csname ppt@uiv.p2.cost.replay-ppi-uniform@0.5.mean-requests-per-skill\endcsname{$+$31913.8}
\expandafter\def\csname val@uiv.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{446.000}
\expandafter\def\csname cnt@uiv.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{446}
\expandafter\def\csname pct@uiv.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{44600.0}
\expandafter\def\csname ppt@uiv.p2.cost.replay-ppi-uniform@1.0.mean-requests-per-skill\endcsname{$+$44600.0}
\expandafter\def\csname val@uiv.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{122.550}
\expandafter\def\csname cnt@uiv.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{123}
\expandafter\def\csname pct@uiv.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{12255.0}
\expandafter\def\csname ppt@uiv.p2.cost.uniform-fresh@0.1.mean-requests-per-skill\endcsname{$+$12255.0}
\expandafter\def\csname val@uiv.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{159.637}
\expandafter\def\csname cnt@uiv.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{160}
\expandafter\def\csname pct@uiv.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{15963.7}
\expandafter\def\csname ppt@uiv.p2.cost.uniform-fresh@0.25.mean-requests-per-skill\endcsname{$+$15963.7}
\expandafter\def\csname val@uiv.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{223.137}
\expandafter\def\csname cnt@uiv.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{223}
\expandafter\def\csname pct@uiv.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{22313.8}
\expandafter\def\csname ppt@uiv.p2.cost.uniform-fresh@0.5.mean-requests-per-skill\endcsname{$+$22313.8}
\expandafter\def\csname val@uiv.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{350}
\expandafter\def\csname pct@uiv.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.cost.uniform-fresh@1.0.mean-requests-per-skill\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.1.center-d1\endcsname{0.350}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.1.center-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.1.center-d1\endcsname{35.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.1.center-d1\endcsname{$+$35.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.1.direct\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.1.direct\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.1.direct\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.1.direct\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.1.grid2-d3\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.1.grid2-d3\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.1.grid2-d3\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.1.grid2-d3\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.25.center-d1\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.25.center-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.25.center-d1\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.25.center-d1\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.25.context-d1\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.25.context-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.25.context-d1\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.25.context-d1\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.25.direct\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.25.direct\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.25.direct\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.25.direct\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.25.grid2-d3\endcsname{0.150}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.25.grid2-d3\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.25.grid2-d3\endcsname{15.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.25.grid2-d3\endcsname{$+$15.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.5.center-d1\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.5.center-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.5.center-d1\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.5.center-d1\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.5.context-d1\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.5.context-d1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.5.context-d1\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.5.context-d1\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.5.direct\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.5.direct\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.5.direct\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.5.direct\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@0.5.grid2-d3\endcsname{0.200}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@0.5.grid2-d3\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.best-single@0.5.grid2-d3\endcsname{20.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@0.5.grid2-d3\endcsname{$+$20.0}
\expandafter\def\csname val@uiv.p2.decide.best-single@1.0.center-d1\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.best-single@1.0.center-d1\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.best-single@1.0.center-d1\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.best-single@1.0.center-d1\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.019}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{1.9}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$1.9}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.092}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{9.2}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$9.2}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.040}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{4.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$4.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.075}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{7.5}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$7.5}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.106}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{10.6}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$10.6}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.030}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{3.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$3.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.090}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{9.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$9.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.051}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{5.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$5.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.014}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{1.4}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$1.4}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.038}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{3.8}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$3.8}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.059}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{5.9}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$5.9}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.060}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{6.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$6.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.950}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{95.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$95.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.026}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{2.6}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$2.6}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.026}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.6}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.6}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.020}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{2.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$2.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.022}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{2.2}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$2.2}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.cost.full-recert-fresh\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.cost.full-recert-fresh\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.no-budget-tau.full-recert\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget-tau.old-source\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.no-budget-tau.old-source\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.no-budget-tau.old-source\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.no-budget-tau.replay-only\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.center-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.center-d1.sigma-used.agree-drift\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.sigma-used.agree-drift\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.sigma-used.agree-drift\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.sigma-used.agree-stable\endcsname{0.187}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.sigma-used.agree-stable\endcsname{18.7}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.sigma-used.agree-stable\endcsname{$+$18.7}
\expandafter\def\csname val@uiv.p2.decide.center-d1.sigma-used.disagree\endcsname{0.350}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.sigma-used.disagree\endcsname{35.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.sigma-used.disagree\endcsname{$+$35.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.strata-N.agree-drift\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.strata-N.agree-drift\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.strata-N.agree-drift\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.strata-N.agree-stable\endcsname{87}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.strata-N.agree-stable\endcsname{87}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.strata-N.agree-stable\endcsname{8700.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.strata-N.agree-stable\endcsname{$+$8700.0}
\expandafter\def\csname val@uiv.p2.decide.center-d1.strata-N.disagree\endcsname{8}
\expandafter\def\csname cnt@uiv.p2.decide.center-d1.strata-N.disagree\endcsname{8}
\expandafter\def\csname pct@uiv.p2.decide.center-d1.strata-N.disagree\endcsname{800.0}
\expandafter\def\csname ppt@uiv.p2.decide.center-d1.strata-N.disagree\endcsname{$+$800.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.038}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{3.8}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$3.8}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.114}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{11.4}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$11.4}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.016}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$1.6}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$1.6}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.058}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{5.8}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$5.8}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{212}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{21200.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$21200.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.006}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.6}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$0.6}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.101}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{10.1}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$10.1}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{116}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{11600.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$11600.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.030}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{3.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$3.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.105}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{10.5}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$10.5}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{1.3}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$1.3}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.077}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{7.7}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$7.7}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.024}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{2.4}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$2.4}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.062}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{6.2}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.2}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{144}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.017}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{1.7}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$1.7}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.069}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{6.9}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$6.9}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.011}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{1.1}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$1.1}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.037}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{3.7}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$3.7}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.016}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{1.6}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$1.6}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.028}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.8}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.8}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{192}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.030}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.cost.full-recert-fresh\endcsname{192}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.cost.full-recert-fresh\endcsname{19200.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.cost.full-recert-fresh\endcsname{$+$19200.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.no-budget-tau.full-recert\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget-tau.old-source\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.no-budget-tau.old-source\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.no-budget-tau.old-source\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.no-budget-tau.replay-only\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget.replay-only\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.context-d1.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.context-d1.sigma-used.agree-drift\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.sigma-used.agree-drift\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.sigma-used.agree-drift\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.sigma-used.agree-stable\endcsname{0.132}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.sigma-used.agree-stable\endcsname{13.2}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.sigma-used.agree-stable\endcsname{$+$13.2}
\expandafter\def\csname val@uiv.p2.decide.context-d1.sigma-used.disagree\endcsname{0.490}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.sigma-used.disagree\endcsname{49.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.sigma-used.disagree\endcsname{$+$49.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.strata-N.agree-drift\endcsname{2}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.strata-N.agree-drift\endcsname{2}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.strata-N.agree-drift\endcsname{200.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.strata-N.agree-drift\endcsname{$+$200.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.strata-N.agree-stable\endcsname{84}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.strata-N.agree-stable\endcsname{84}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.strata-N.agree-stable\endcsname{8400.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.strata-N.agree-stable\endcsname{$+$8400.0}
\expandafter\def\csname val@uiv.p2.decide.context-d1.strata-N.disagree\endcsname{10}
\expandafter\def\csname cnt@uiv.p2.decide.context-d1.strata-N.disagree\endcsname{10}
\expandafter\def\csname pct@uiv.p2.decide.context-d1.strata-N.disagree\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p2.decide.context-d1.strata-N.disagree\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{126.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{12600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$12600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.014}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{1.4}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$1.4}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.112}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{11.2}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$11.2}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{222.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{22200.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$22200.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.030}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$3.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.148}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{14.8}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$14.8}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{22200.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$22200.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{-0.016}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.6}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.6}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.116}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{11.6}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$11.6}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{126.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{12600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$12600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{0.900}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{90.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$90.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.030}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{3.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$3.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{168}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.061}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{6.1}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$6.1}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{264.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{264}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{26400.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$26400.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{0.400}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{40.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$40.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.061}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{6.1}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$6.1}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{26400.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$26400.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{-0.008}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$0.8}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.062}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{6.2}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$6.2}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{168}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.006}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.6}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$0.6}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.055}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{5.5}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$5.5}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.350}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{35.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$35.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{-0.011}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$1.1}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$-$1.1}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.028}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{2.8}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$2.8}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{336.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{336}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{33600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$33600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{-0.015}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$1.5}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$1.5}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.034}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{3.4}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$3.4}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{336.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{336}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{33600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$33600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{-0.016}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.6}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.6}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.033}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{3.3}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.3}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{-0.018}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$1.8}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$-$1.8}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{480.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{480}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{48000.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$48000.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{480.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{480}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{48000.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$48000.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.keep-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{288}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.cost.full-recert-fresh\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.no-budget-tau.full-recert\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.no-budget-tau.old-source\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.no-budget-tau.replay-only\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget.full-recert\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget.old-decision\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{0.135}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{13.5}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.sigma-used.agree-stable\endcsname{$+$13.5}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.sigma-used.disagree\endcsname{0.471}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.sigma-used.disagree\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.sigma-used.disagree\endcsname{47.1}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.sigma-used.disagree\endcsname{$+$47.1}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.strata-N.agree-drift\endcsname{4}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.strata-N.agree-drift\endcsname{4}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.strata-N.agree-drift\endcsname{400.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.strata-N.agree-drift\endcsname{$+$400.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.strata-N.agree-stable\endcsname{86}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.strata-N.agree-stable\endcsname{86}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.strata-N.agree-stable\endcsname{8600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.strata-N.agree-stable\endcsname{$+$8600.0}
\expandafter\def\csname val@uiv.p2.decide.dual-d2.strata-N.disagree\endcsname{6}
\expandafter\def\csname cnt@uiv.p2.decide.dual-d2.strata-N.disagree\endcsname{6}
\expandafter\def\csname pct@uiv.p2.decide.dual-d2.strata-N.disagree\endcsname{600.0}
\expandafter\def\csname ppt@uiv.p2.decide.dual-d2.strata-N.disagree\endcsname{$+$600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{132.200}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{132}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{13220.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$13220.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.042}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{4.2}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$4.2}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.136}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{13.6}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$13.6}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{229.150}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{229}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{22915.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$22915.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.300}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{30.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$30.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{-0.029}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$2.9}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$-$2.9}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.096}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{9.6}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$9.6}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{228.200}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{228}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{22820.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$22820.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.121}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{12.1}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$12.1}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{132.200}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{132}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{13220.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$13220.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.035}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{3.5}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$3.5}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.091}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{9.1}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$9.1}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{182.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{183}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{18255.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$18255.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.013}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{1.2}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$1.2}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.069}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{6.9}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$6.9}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{279.350}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{279}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{27935.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$27935.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{-0.002}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$0.2}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$-$0.2}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{278.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{279}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{27855.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$27855.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.006}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0.6}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$+$0.6}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.070}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{7.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$7.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{182.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{183}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{18255.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$18255.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.023}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{2.3}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$2.3}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{268.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{269}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{26855.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$26855.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.035}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{3.5}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$3.5}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{364.650}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{365}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{36465.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$36465.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0.250}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{25.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$25.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{-0.004}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$0.4}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$-$0.4}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.029}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.9}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.9}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{364.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{365}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{36455.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$36455.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.800}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{80.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$80.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.034}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{3.4}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$3.4}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{268.550}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{269}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{26855.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$26855.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.011}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{1.1}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$1.1}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.030}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{3.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$3.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{440.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{440}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{44000.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$44000.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{536.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{536}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{53600.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$53600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{536.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{536}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{53600.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$53600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{440.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{440}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{44000.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$44000.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{344}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{344}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{34400.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.cost.full-recert-fresh\endcsname{$+$34400.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.no-budget-tau.full-recert\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.no-budget-tau.old-source\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{-0.062}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{$-$6.2}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.no-budget-tau.replay-only\endcsname{$-$6.2}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.sigma-used.agree-drift\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.sigma-used.agree-drift\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.sigma-used.agree-drift\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.sigma-used.agree-drift\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{0.100}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{10.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.sigma-used.agree-stable\endcsname{$+$10.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.sigma-used.disagree\endcsname{0.514}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.sigma-used.disagree\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.sigma-used.disagree\endcsname{51.4}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.sigma-used.disagree\endcsname{$+$51.4}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.sigma-used.parse-fail\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.strata-N.agree-drift\endcsname{2}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.strata-N.agree-drift\endcsname{2}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.strata-N.agree-drift\endcsname{200.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.strata-N.agree-drift\endcsname{$+$200.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{77}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{77}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{7700.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.strata-N.agree-stable\endcsname{$+$7700.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.strata-N.disagree\endcsname{15}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.strata-N.disagree\endcsname{15}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.strata-N.disagree\endcsname{1500.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.strata-N.disagree\endcsname{$+$1500.0}
\expandafter\def\csname val@uiv.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname cnt@uiv.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{2}
\expandafter\def\csname pct@uiv.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{200.0}
\expandafter\def\csname ppt@uiv.p2.decide.grid2-d3.strata-N.parse-fail\endcsname{$+$200.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{10}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{1000.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.B\endcsname{$+$1000.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{126.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{12600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.cost-mean\endcsname{$+$12600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-mean\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0.084}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{8.4}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.generic-ppi-source.tau-hat-sd\endcsname{$+$8.4}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{222.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{22200.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.cost-mean\endcsname{$+$22200.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-mean\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0.057}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{5.7}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.rcr-stratified.tau-hat-sd\endcsname{$+$5.7}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{222}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{22200.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.cost-mean\endcsname{$+$22200.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0.450}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{45.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.keep-rate\endcsname{$+$45.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0.014}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{1.4}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.4}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0.092}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{9.2}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.replay-ppi-uniform.tau-hat-sd\endcsname{$+$9.2}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{126.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{126}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{12600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.cost-mean\endcsname{$+$12600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{0.850}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{85.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.keep-rate\endcsname{$+$85.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0.030}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{3.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-mean\endcsname{$+$3.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0.071}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{7.1}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.1.uniform-fresh.tau-hat-sd\endcsname{$+$7.1}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{24}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.B\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{168}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.006}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{0.6}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-mean\endcsname{$+$0.6}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0.062}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{6.2}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.generic-ppi-source.tau-hat-sd\endcsname{$+$6.2}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{264.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{264}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{26400.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.cost-mean\endcsname{$+$26400.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0.500}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{50.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.keep-rate\endcsname{$+$50.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0.015}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{1.5}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-mean\endcsname{$+$1.5}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0.046}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{4.6}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.rcr-stratified.tau-hat-sd\endcsname{$+$4.6}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{264}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{26400.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.cost-mean\endcsname{$+$26400.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{-0.006}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$0.6}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-mean\endcsname{$-$0.6}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0.050}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{5.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.replay-ppi-uniform.tau-hat-sd\endcsname{$+$5.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{168.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{168}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{16800.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.cost-mean\endcsname{$+$16800.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{0.750}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{75.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.keep-rate\endcsname{$+$75.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0.043}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{4.3}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.25.uniform-fresh.tau-hat-sd\endcsname{$+$4.3}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{48}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{4800.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.B\endcsname{$+$4800.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{0.600}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{60.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.keep-rate\endcsname{$+$60.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0.032}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{3.2}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.generic-ppi-source.tau-hat-sd\endcsname{$+$3.2}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{336.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{336}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{33600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.cost-mean\endcsname{$+$33600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{0.550}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{55.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.keep-rate\endcsname{$+$55.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-mean\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0.026}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{2.6}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.rcr-stratified.tau-hat-sd\endcsname{$+$2.6}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{336.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{336}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{33600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.cost-mean\endcsname{$+$33600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{0.650}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{65.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.keep-rate\endcsname{$+$65.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.009}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{0.9}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-mean\endcsname{$+$0.9}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.replay-ppi-uniform.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{240.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{240}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{24000.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.cost-mean\endcsname{$+$24000.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{0.700}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{70.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.keep-rate\endcsname{$+$70.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0.027}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{2.7}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@0.5.uniform-fresh.tau-hat-sd\endcsname{$+$2.7}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.B\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.generic-ppi-source.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{480.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{480}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{48000.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.cost-mean\endcsname{$+$48000.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.rcr-stratified.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{480.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{480}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{48000.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.cost-mean\endcsname{$+$48000.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.replay-ppi-uniform.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{384.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{384}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{38400.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.cost-mean\endcsname{$+$38400.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.infeasible-rate\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{100.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.keep-rate\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-mean\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.budget@1.0.uniform-fresh.tau-hat-sd\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.cost.direct-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.cost.direct-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.cost.direct-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{288}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{288}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{28800.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.cost.full-recert-fresh\endcsname{$+$28800.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.cost.replay-all\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.cost.replay-all\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.cost.replay-all\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0.010}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{1.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.no-budget-tau.full-recert\endcsname{$+$1.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.no-budget-tau.old-source\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{-0.031}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{$-$3.1}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.no-budget-tau.replay-only\endcsname{$-$3.1}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget.full-recert\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget.keep-all\endcsname{KEEP}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget.old-decision\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget.replay-only\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.no-budget.suspend-all\endcsname{SUSPEND}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0.187}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{0}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{18.7}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.sigma-used.agree-stable\endcsname{$+$18.7}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{0.599}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{1}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{59.9}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.sigma-used.disagree\endcsname{$+$59.9}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{85}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{85}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{8500.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.strata-N.agree-stable\endcsname{$+$8500.0}
\expandafter\def\csname val@uiv.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{11}
\expandafter\def\csname cnt@uiv.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{11}
\expandafter\def\csname pct@uiv.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{1100.0}
\expandafter\def\csname ppt@uiv.p2.decide.zoomclick-d3.strata-N.disagree\endcsname{$+$1100.0}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.bracket-costs.0\endcsname{223.137}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.bracket-costs.0\endcsname{223}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.bracket-costs.0\endcsname{22313.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.bracket-costs.0\endcsname{$+$22313.8}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.bracket-costs.1\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.bracket-costs.1\endcsname{350}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.bracket-costs.1\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.bracket-costs.1\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{-0.009}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$0.9}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.ci95.0\endcsname{$-$0.9}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{0.025}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{2.5}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.ci95.1\endcsname{$+$2.5}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.lower95-one-sided\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.mean\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.mean\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.mean\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{0.248}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{24.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-gt0\endcsname{$+$24.8}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.021}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{2.1}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{$+$2.1}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{0.823}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{82.3}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.score-at-rcr-cost\endcsname{$+$82.3}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.status\endcsname{ok}
\expandafter\def\csname val@uiv.p2.equal-cost.best-single.weight\endcsname{0.258}
\expandafter\def\csname cnt@uiv.p2.equal-cost.best-single.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.best-single.weight\endcsname{25.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.best-single.weight\endcsname{$+$25.8}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{223.137}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{223}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{22313.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.0\endcsname{$+$22313.8}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{350}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.bracket-costs.1\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{-0.004}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.0\endcsname{$-$0.4}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0.008}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{0.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.ci95.1\endcsname{$+$0.8}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{-0.003}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.lower95-one-sided\endcsname{$-$0.3}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.mean\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0.322}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{32.2}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-gt0\endcsname{$+$32.2}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{0.828}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{82.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.score-at-rcr-cost\endcsname{$+$82.8}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.status\endcsname{ok}
\expandafter\def\csname val@uiv.p2.equal-cost.generic-ppi-source.weight\endcsname{0.258}
\expandafter\def\csname cnt@uiv.p2.equal-cost.generic-ppi-source.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.generic-ppi-source.weight\endcsname{25.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.generic-ppi-source.weight\endcsname{$+$25.8}
\expandafter\def\csname val@uiv.p2.equal-cost.rcr-cost\endcsname{255.838}
\expandafter\def\csname cnt@uiv.p2.equal-cost.rcr-cost\endcsname{256}
\expandafter\def\csname pct@uiv.p2.equal-cost.rcr-cost\endcsname{25583.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.rcr-cost\endcsname{$+$25583.8}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{255.637}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{256}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{25563.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.0\endcsname{$+$25563.8}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{319.137}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{319}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{31913.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.bracket-costs.1\endcsname{$+$31913.8}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.0\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.ci95.1\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.lower95-one-sided\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.mean\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0.018}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{1.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-gt0\endcsname{$+$1.8}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{0.828}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{82.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.score-at-rcr-cost\endcsname{$+$82.8}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.status\endcsname{ok}
\expandafter\def\csname val@uiv.p2.equal-cost.replay-ppi-uniform.weight\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p2.equal-cost.replay-ppi-uniform.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.replay-ppi-uniform.weight\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p2.equal-cost.replay-ppi-uniform.weight\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{223.137}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{223}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{22313.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.bracket-costs.0\endcsname{$+$22313.8}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{350.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{350}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{35000.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.bracket-costs.1\endcsname{$+$35000.0}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{-0.005}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$0.5}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.0\endcsname{$-$0.5}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0.005}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{0.5}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.ci95.1\endcsname{$+$0.5}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{-0.004}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$0.4}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.lower95-one-sided\endcsname{$-$0.4}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{-0.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{0.559}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{55.9}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-gt0\endcsname{$+$55.9}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.rcr-minus.p-one-sided-noninferiority-0.01\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{0.830}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{1}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{83.0}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.score-at-rcr-cost\endcsname{$+$83.0}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.status\endcsname{ok}
\expandafter\def\csname val@uiv.p2.equal-cost.uniform-fresh.weight\endcsname{0.258}
\expandafter\def\csname cnt@uiv.p2.equal-cost.uniform-fresh.weight\endcsname{0}
\expandafter\def\csname pct@uiv.p2.equal-cost.uniform-fresh.weight\endcsname{25.8}
\expandafter\def\csname ppt@uiv.p2.equal-cost.uniform-fresh.weight\endcsname{$+$25.8}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.acc-macro\endcsname{0.812}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.acc-macro\endcsname{81.2}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.acc-macro\endcsname{$+$81.2}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.mean-requests\endcsname{2.000}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.mean-requests\endcsname{200.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.mean-requests\endcsname{$+$200.0}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.n\endcsname{144}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{-0.069}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{$-$6.9}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.0\endcsname{$-$6.9}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0.007}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{0.7}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.ci95.1\endcsname{$+$0.7}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{-0.062}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$6.2}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$6.2}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{-0.028}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{$-$2.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.mean\endcsname{$-$2.8}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.896}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{89.6}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-gt0\endcsname{$+$89.6}
\expandafter\def\csname val@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.785}
\expandafter\def\csname cnt@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{78.5}
\expandafter\def\csname ppt@uiv.p2.execution-layer.center-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$78.5}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.acc-macro\endcsname{0.840}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.acc-macro\endcsname{84.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.acc-macro\endcsname{$+$84.0}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.mean-requests\endcsname{2.000}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.mean-requests\endcsname{2}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.mean-requests\endcsname{200.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.mean-requests\endcsname{$+$200.0}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.n\endcsname{144}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{-0.028}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.0\endcsname{$-$2.8}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{-0.021}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$2.1}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.lower95-one-sided\endcsname{$-$2.1}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0.000}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.mean\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0.477}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{47.7}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-gt0\endcsname{$+$47.7}
\expandafter\def\csname val@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.216}
\expandafter\def\csname cnt@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{21.6}
\expandafter\def\csname ppt@uiv.p2.execution-layer.context-d1.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$21.6}
\expandafter\def\csname val@uiv.p2.execution-layer.direct\endcsname{0.840}
\expandafter\def\csname cnt@uiv.p2.execution-layer.direct\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.direct\endcsname{84.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.direct\endcsname{$+$84.0}
\expandafter\def\csname val@uiv.p2.execution-layer.direct-sc3\endcsname{0.847}
\expandafter\def\csname cnt@uiv.p2.execution-layer.direct-sc3\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.direct-sc3\endcsname{84.7}
\expandafter\def\csname ppt@uiv.p2.execution-layer.direct-sc3\endcsname{$+$84.7}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.acc-macro\endcsname{0.778}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.acc-macro\endcsname{77.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.acc-macro\endcsname{$+$77.8}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.mean-requests\endcsname{3.000}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.mean-requests\endcsname{3}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.mean-requests\endcsname{300.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.mean-requests\endcsname{$+$300.0}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.n\endcsname{144}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{-0.125}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{$-$12.5}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.0\endcsname{$-$12.5}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.ci95.1\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{-0.111}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{$-$11.1}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.lower95-one-sided\endcsname{$-$11.1}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{-0.062}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{$-$6.2}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.mean\endcsname{$-$6.2}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{0.978}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{97.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-gt0\endcsname{$+$97.8}
\expandafter\def\csname val@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.965}
\expandafter\def\csname cnt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{96.5}
\expandafter\def\csname ppt@uiv.p2.execution-layer.dual-d2.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$96.5}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.acc-macro\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.acc-macro\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.acc-macro\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.mean-requests\endcsname{3.583}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.mean-requests\endcsname{4}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.mean-requests\endcsname{358.3}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.mean-requests\endcsname{$+$358.3}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.n\endcsname{144}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{-0.042}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.0\endcsname{$-$4.2}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{-0.035}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$3.5}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$3.5}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.mean\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.642}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{64.2}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-gt0\endcsname{$+$64.2}
\expandafter\def\csname val@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.430}
\expandafter\def\csname cnt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{43.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.grid2-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$43.0}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{0.833}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{83.3}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.acc-macro\endcsname{$+$83.3}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{3.000}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{3}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{300.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.mean-requests\endcsname{$+$300.0}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.n\endcsname{144}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.n\endcsname{144}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.n\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.n\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{-0.049}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{$-$4.9}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.0\endcsname{$-$4.9}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0.028}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{2.8}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.ci95.1\endcsname{$+$2.8}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{-0.042}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$4.2}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.lower95-one-sided\endcsname{$-$4.2}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{-0.007}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{$-$0.7}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.mean\endcsname{$-$0.7}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{0.571}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{1}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{57.1}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-gt0\endcsname{$+$57.1}
\expandafter\def\csname val@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0.431}
\expandafter\def\csname cnt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{0}
\expandafter\def\csname pct@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{43.1}
\expandafter\def\csname ppt@uiv.p2.execution-layer.zoomclick-d3.tau-vs-direct.p-one-sided-noninferiority-0.01\endcsname{$+$43.1}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{0.004}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{0}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{0.4}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-generic-ppi-source.max\endcsname{$+$0.4}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{0.003}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{0}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{0.3}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-generic-ppi-source.min\endcsname{$+$0.3}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-generic-ppi-source.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-generic-ppi-source.n-negative\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0.002}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{0.2}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.max\endcsname{$+$0.2}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.001}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{0.1}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.min\endcsname{$+$0.1}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname cnt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0}
\expandafter\def\csname pct@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname ppt@uiv.p2.loo.rcr-vs-replay-ppi-uniform.n-negative\endcsname{0.0}
\expandafter\def\csname val@uiv.p2.n-cal\endcsname{96}
\expandafter\def\csname cnt@uiv.p2.n-cal\endcsname{96}
\expandafter\def\csname pct@uiv.p2.n-cal\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.p2.n-cal\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.p2.n-cal-apps\endcsname{12}
\expandafter\def\csname cnt@uiv.p2.n-cal-apps\endcsname{12}
\expandafter\def\csname pct@uiv.p2.n-cal-apps\endcsname{1200.0}
\expandafter\def\csname ppt@uiv.p2.n-cal-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@uiv.p2.n-test\endcsname{144}
\expandafter\def\csname cnt@uiv.p2.n-test\endcsname{144}
\expandafter\def\csname pct@uiv.p2.n-test\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.p2.n-test\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.p2.n-test-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.p2.n-test-apps\endcsname{24}
\expandafter\def\csname pct@uiv.p2.n-test-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.p2.n-test-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.p2.primary.best-single.cost\endcsname{159.637}
\expandafter\def\csname cnt@uiv.p2.primary.best-single.cost\endcsname{160}
\expandafter\def\csname pct@uiv.p2.primary.best-single.cost\endcsname{15963.7}
\expandafter\def\csname ppt@uiv.p2.primary.best-single.cost\endcsname{$+$15963.7}
\expandafter\def\csname val@uiv.p2.primary.best-single.cost-fraction-of-full\endcsname{0.456}
\expandafter\def\csname cnt@uiv.p2.primary.best-single.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.best-single.cost-fraction-of-full\endcsname{45.6}
\expandafter\def\csname ppt@uiv.p2.primary.best-single.cost-fraction-of-full\endcsname{$+$45.6}
\expandafter\def\csname val@uiv.p2.primary.best-single.score\endcsname{0.831}
\expandafter\def\csname cnt@uiv.p2.primary.best-single.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.best-single.score\endcsname{83.1}
\expandafter\def\csname ppt@uiv.p2.primary.best-single.score\endcsname{$+$83.1}
\expandafter\def\csname val@uiv.p2.primary.best-single.vs-full-recert\endcsname{-0.001}
\expandafter\def\csname cnt@uiv.p2.primary.best-single.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.best-single.vs-full-recert\endcsname{$-$0.1}
\expandafter\def\csname ppt@uiv.p2.primary.best-single.vs-full-recert\endcsname{$-$0.1}
\expandafter\def\csname val@uiv.p2.primary.best-single.vs-suspend-all\endcsname{-0.009}
\expandafter\def\csname cnt@uiv.p2.primary.best-single.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.best-single.vs-suspend-all\endcsname{$-$0.9}
\expandafter\def\csname ppt@uiv.p2.primary.best-single.vs-suspend-all\endcsname{$-$0.9}
\expandafter\def\csname val@uiv.p2.primary.generic-ppi-source.cost\endcsname{159.637}
\expandafter\def\csname cnt@uiv.p2.primary.generic-ppi-source.cost\endcsname{160}
\expandafter\def\csname pct@uiv.p2.primary.generic-ppi-source.cost\endcsname{15963.7}
\expandafter\def\csname ppt@uiv.p2.primary.generic-ppi-source.cost\endcsname{$+$15963.7}
\expandafter\def\csname val@uiv.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0.456}
\expandafter\def\csname cnt@uiv.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{45.6}
\expandafter\def\csname ppt@uiv.p2.primary.generic-ppi-source.cost-fraction-of-full\endcsname{$+$45.6}
\expandafter\def\csname val@uiv.p2.primary.generic-ppi-source.score\endcsname{0.826}
\expandafter\def\csname cnt@uiv.p2.primary.generic-ppi-source.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.generic-ppi-source.score\endcsname{82.6}
\expandafter\def\csname ppt@uiv.p2.primary.generic-ppi-source.score\endcsname{$+$82.6}
\expandafter\def\csname val@uiv.p2.primary.generic-ppi-source.vs-full-recert\endcsname{-0.006}
\expandafter\def\csname cnt@uiv.p2.primary.generic-ppi-source.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.generic-ppi-source.vs-full-recert\endcsname{$-$0.6}
\expandafter\def\csname ppt@uiv.p2.primary.generic-ppi-source.vs-full-recert\endcsname{$-$0.6}
\expandafter\def\csname val@uiv.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{-0.014}
\expandafter\def\csname cnt@uiv.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{$-$1.4}
\expandafter\def\csname ppt@uiv.p2.primary.generic-ppi-source.vs-suspend-all\endcsname{$-$1.4}
\expandafter\def\csname val@uiv.p2.primary.rcr-stratified.cost\endcsname{255.838}
\expandafter\def\csname cnt@uiv.p2.primary.rcr-stratified.cost\endcsname{256}
\expandafter\def\csname pct@uiv.p2.primary.rcr-stratified.cost\endcsname{25583.8}
\expandafter\def\csname ppt@uiv.p2.primary.rcr-stratified.cost\endcsname{$+$25583.8}
\expandafter\def\csname val@uiv.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{0.731}
\expandafter\def\csname cnt@uiv.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{73.1}
\expandafter\def\csname ppt@uiv.p2.primary.rcr-stratified.cost-fraction-of-full\endcsname{$+$73.1}
\expandafter\def\csname val@uiv.p2.primary.rcr-stratified.score\endcsname{0.829}
\expandafter\def\csname cnt@uiv.p2.primary.rcr-stratified.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.rcr-stratified.score\endcsname{82.9}
\expandafter\def\csname ppt@uiv.p2.primary.rcr-stratified.score\endcsname{$+$82.9}
\expandafter\def\csname val@uiv.p2.primary.rcr-stratified.vs-full-recert\endcsname{-0.002}
\expandafter\def\csname cnt@uiv.p2.primary.rcr-stratified.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.rcr-stratified.vs-full-recert\endcsname{$-$0.2}
\expandafter\def\csname ppt@uiv.p2.primary.rcr-stratified.vs-full-recert\endcsname{$-$0.2}
\expandafter\def\csname val@uiv.p2.primary.rcr-stratified.vs-suspend-all\endcsname{-0.011}
\expandafter\def\csname cnt@uiv.p2.primary.rcr-stratified.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.rcr-stratified.vs-suspend-all\endcsname{$-$1.1}
\expandafter\def\csname ppt@uiv.p2.primary.rcr-stratified.vs-suspend-all\endcsname{$-$1.1}
\expandafter\def\csname val@uiv.p2.primary.replay-ppi-uniform.cost\endcsname{255.637}
\expandafter\def\csname cnt@uiv.p2.primary.replay-ppi-uniform.cost\endcsname{256}
\expandafter\def\csname pct@uiv.p2.primary.replay-ppi-uniform.cost\endcsname{25563.8}
\expandafter\def\csname ppt@uiv.p2.primary.replay-ppi-uniform.cost\endcsname{$+$25563.8}
\expandafter\def\csname val@uiv.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{0.730}
\expandafter\def\csname cnt@uiv.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{73.0}
\expandafter\def\csname ppt@uiv.p2.primary.replay-ppi-uniform.cost-fraction-of-full\endcsname{$+$73.0}
\expandafter\def\csname val@uiv.p2.primary.replay-ppi-uniform.score\endcsname{0.828}
\expandafter\def\csname cnt@uiv.p2.primary.replay-ppi-uniform.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.replay-ppi-uniform.score\endcsname{82.8}
\expandafter\def\csname ppt@uiv.p2.primary.replay-ppi-uniform.score\endcsname{$+$82.8}
\expandafter\def\csname val@uiv.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{-0.004}
\expandafter\def\csname cnt@uiv.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{$-$0.4}
\expandafter\def\csname ppt@uiv.p2.primary.replay-ppi-uniform.vs-full-recert\endcsname{$-$0.4}
\expandafter\def\csname val@uiv.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{-0.013}
\expandafter\def\csname cnt@uiv.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{$-$1.3}
\expandafter\def\csname ppt@uiv.p2.primary.replay-ppi-uniform.vs-suspend-all\endcsname{$-$1.3}
\expandafter\def\csname val@uiv.p2.primary.uniform-fresh.cost\endcsname{159.637}
\expandafter\def\csname cnt@uiv.p2.primary.uniform-fresh.cost\endcsname{160}
\expandafter\def\csname pct@uiv.p2.primary.uniform-fresh.cost\endcsname{15963.7}
\expandafter\def\csname ppt@uiv.p2.primary.uniform-fresh.cost\endcsname{$+$15963.7}
\expandafter\def\csname val@uiv.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{0.456}
\expandafter\def\csname cnt@uiv.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{45.6}
\expandafter\def\csname ppt@uiv.p2.primary.uniform-fresh.cost-fraction-of-full\endcsname{$+$45.6}
\expandafter\def\csname val@uiv.p2.primary.uniform-fresh.score\endcsname{0.821}
\expandafter\def\csname cnt@uiv.p2.primary.uniform-fresh.score\endcsname{1}
\expandafter\def\csname pct@uiv.p2.primary.uniform-fresh.score\endcsname{82.1}
\expandafter\def\csname ppt@uiv.p2.primary.uniform-fresh.score\endcsname{$+$82.1}
\expandafter\def\csname val@uiv.p2.primary.uniform-fresh.vs-full-recert\endcsname{-0.010}
\expandafter\def\csname cnt@uiv.p2.primary.uniform-fresh.vs-full-recert\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.uniform-fresh.vs-full-recert\endcsname{$-$1.0}
\expandafter\def\csname ppt@uiv.p2.primary.uniform-fresh.vs-full-recert\endcsname{$-$1.0}
\expandafter\def\csname val@uiv.p2.primary.uniform-fresh.vs-suspend-all\endcsname{-0.019}
\expandafter\def\csname cnt@uiv.p2.primary.uniform-fresh.vs-suspend-all\endcsname{0}
\expandafter\def\csname pct@uiv.p2.primary.uniform-fresh.vs-suspend-all\endcsname{$-$1.9}
\expandafter\def\csname ppt@uiv.p2.primary.uniform-fresh.vs-suspend-all\endcsname{$-$1.9}
\expandafter\def\csname val@uiv.records.audit.answer-echo-via-bash\endcsname{5}
\expandafter\def\csname cnt@uiv.records.audit.answer-echo-via-bash\endcsname{5}
\expandafter\def\csname pct@uiv.records.audit.answer-echo-via-bash\endcsname{500.0}
\expandafter\def\csname ppt@uiv.records.audit.answer-echo-via-bash\endcsname{$+$500.0}
\expandafter\def\csname val@uiv.records.audit.bash-non-echo\endcsname{0}
\expandafter\def\csname cnt@uiv.records.audit.bash-non-echo\endcsname{0}
\expandafter\def\csname pct@uiv.records.audit.bash-non-echo\endcsname{0.0}
\expandafter\def\csname ppt@uiv.records.audit.bash-non-echo\endcsname{0.0}
\expandafter\def\csname val@uiv.records.audit.file-access-attempts-nonexistent\endcsname{1}
\expandafter\def\csname cnt@uiv.records.audit.file-access-attempts-nonexistent\endcsname{1}
\expandafter\def\csname pct@uiv.records.audit.file-access-attempts-nonexistent\endcsname{100.0}
\expandafter\def\csname ppt@uiv.records.audit.file-access-attempts-nonexistent\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.records.audit.file-access-violations\endcsname{1}
\expandafter\def\csname cnt@uiv.records.audit.file-access-violations\endcsname{1}
\expandafter\def\csname pct@uiv.records.audit.file-access-violations\endcsname{100.0}
\expandafter\def\csname ppt@uiv.records.audit.file-access-violations\endcsname{$+$100.0}
\expandafter\def\csname val@uiv.records.audit.harness-meta-tool-calls-only\endcsname{35}
\expandafter\def\csname cnt@uiv.records.audit.harness-meta-tool-calls-only\endcsname{35}
\expandafter\def\csname pct@uiv.records.audit.harness-meta-tool-calls-only\endcsname{3500.0}
\expandafter\def\csname ppt@uiv.records.audit.harness-meta-tool-calls-only\endcsname{$+$3500.0}
\expandafter\def\csname val@uiv.records.audit.read-outside-allowed-existing-file\endcsname{0}
\expandafter\def\csname cnt@uiv.records.audit.read-outside-allowed-existing-file\endcsname{0}
\expandafter\def\csname pct@uiv.records.audit.read-outside-allowed-existing-file\endcsname{0.0}
\expandafter\def\csname ppt@uiv.records.audit.read-outside-allowed-existing-file\endcsname{0.0}
\expandafter\def\csname val@uiv.records.audit.requests-with-unexpected-tools\endcsname{36}
\expandafter\def\csname cnt@uiv.records.audit.requests-with-unexpected-tools\endcsname{36}
\expandafter\def\csname pct@uiv.records.audit.requests-with-unexpected-tools\endcsname{3600.0}
\expandafter\def\csname ppt@uiv.records.audit.requests-with-unexpected-tools\endcsname{$+$3600.0}
\expandafter\def\csname val@uiv.records.audit.requests-with-violations\endcsname{36}
\expandafter\def\csname cnt@uiv.records.audit.requests-with-violations\endcsname{36}
\expandafter\def\csname pct@uiv.records.audit.requests-with-violations\endcsname{3600.0}
\expandafter\def\csname ppt@uiv.records.audit.requests-with-violations\endcsname{$+$3600.0}
\expandafter\def\csname val@uiv.records.fidelity.exact-bytes\endcsname{23782}
\expandafter\def\csname cnt@uiv.records.fidelity.exact-bytes\endcsname{23{,}782}
\expandafter\def\csname pct@uiv.records.fidelity.exact-bytes\endcsname{2378200.0}
\expandafter\def\csname ppt@uiv.records.fidelity.exact-bytes\endcsname{$+$2378200.0}
\expandafter\def\csname val@uiv.records.fidelity.images-checked\endcsname{23782}
\expandafter\def\csname cnt@uiv.records.fidelity.images-checked\endcsname{23{,}782}
\expandafter\def\csname pct@uiv.records.fidelity.images-checked\endcsname{2378200.0}
\expandafter\def\csname ppt@uiv.records.fidelity.images-checked\endcsname{$+$2378200.0}
\expandafter\def\csname val@uiv.records.fidelity.mismatch\endcsname{0}
\expandafter\def\csname cnt@uiv.records.fidelity.mismatch\endcsname{0}
\expandafter\def\csname pct@uiv.records.fidelity.mismatch\endcsname{0.0}
\expandafter\def\csname ppt@uiv.records.fidelity.mismatch\endcsname{0.0}
\expandafter\def\csname val@uiv.records.latency.acquire-box.mean\endcsname{5.210}
\expandafter\def\csname cnt@uiv.records.latency.acquire-box.mean\endcsname{5}
\expandafter\def\csname pct@uiv.records.latency.acquire-box.mean\endcsname{521.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-box.mean\endcsname{$+$521.0}
\expandafter\def\csname val@uiv.records.latency.acquire-box.median\endcsname{5.680}
\expandafter\def\csname cnt@uiv.records.latency.acquire-box.median\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.acquire-box.median\endcsname{568.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-box.median\endcsname{$+$568.0}
\expandafter\def\csname val@uiv.records.latency.acquire-box.n\endcsname{2525}
\expandafter\def\csname cnt@uiv.records.latency.acquire-box.n\endcsname{2{,}525}
\expandafter\def\csname pct@uiv.records.latency.acquire-box.n\endcsname{252500.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-box.n\endcsname{$+$252500.0}
\expandafter\def\csname val@uiv.records.latency.acquire-box.p90\endcsname{8.270}
\expandafter\def\csname cnt@uiv.records.latency.acquire-box.p90\endcsname{8}
\expandafter\def\csname pct@uiv.records.latency.acquire-box.p90\endcsname{827.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-box.p90\endcsname{$+$827.0}
\expandafter\def\csname val@uiv.records.latency.acquire-cell.mean\endcsname{6.000}
\expandafter\def\csname cnt@uiv.records.latency.acquire-cell.mean\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.acquire-cell.mean\endcsname{600.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-cell.mean\endcsname{$+$600.0}
\expandafter\def\csname val@uiv.records.latency.acquire-cell.median\endcsname{6.250}
\expandafter\def\csname cnt@uiv.records.latency.acquire-cell.median\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.acquire-cell.median\endcsname{625.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-cell.median\endcsname{$+$625.0}
\expandafter\def\csname val@uiv.records.latency.acquire-cell.n\endcsname{2739}
\expandafter\def\csname cnt@uiv.records.latency.acquire-cell.n\endcsname{2{,}739}
\expandafter\def\csname pct@uiv.records.latency.acquire-cell.n\endcsname{273900.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-cell.n\endcsname{$+$273900.0}
\expandafter\def\csname val@uiv.records.latency.acquire-cell.p90\endcsname{8.890}
\expandafter\def\csname cnt@uiv.records.latency.acquire-cell.p90\endcsname{9}
\expandafter\def\csname pct@uiv.records.latency.acquire-cell.p90\endcsname{889.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-cell.p90\endcsname{$+$889.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual-refine.mean\endcsname{6.210}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual-refine.mean\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual-refine.mean\endcsname{621.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual-refine.mean\endcsname{$+$621.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual-refine.median\endcsname{6.400}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual-refine.median\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual-refine.median\endcsname{640.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual-refine.median\endcsname{$+$640.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual-refine.n\endcsname{881}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual-refine.n\endcsname{881}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual-refine.n\endcsname{88100.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual-refine.n\endcsname{$+$88100.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual-refine.p90\endcsname{8.430}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual-refine.p90\endcsname{8}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual-refine.p90\endcsname{843.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual-refine.p90\endcsname{$+$843.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual.mean\endcsname{5.020}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual.mean\endcsname{5}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual.mean\endcsname{502.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual.mean\endcsname{$+$502.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual.median\endcsname{5.580}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual.median\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual.median\endcsname{558.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual.median\endcsname{$+$558.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual.n\endcsname{1278}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual.n\endcsname{1{,}278}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual.n\endcsname{127800.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual.n\endcsname{$+$127800.0}
\expandafter\def\csname val@uiv.records.latency.acquire-dual.p90\endcsname{8.010}
\expandafter\def\csname cnt@uiv.records.latency.acquire-dual.p90\endcsname{8}
\expandafter\def\csname pct@uiv.records.latency.acquire-dual.p90\endcsname{801.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-dual.p90\endcsname{$+$801.0}
\expandafter\def\csname val@uiv.records.latency.acquire-point.mean\endcsname{5.170}
\expandafter\def\csname cnt@uiv.records.latency.acquire-point.mean\endcsname{5}
\expandafter\def\csname pct@uiv.records.latency.acquire-point.mean\endcsname{517.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-point.mean\endcsname{$+$517.0}
\expandafter\def\csname val@uiv.records.latency.acquire-point.median\endcsname{5.290}
\expandafter\def\csname cnt@uiv.records.latency.acquire-point.median\endcsname{5}
\expandafter\def\csname pct@uiv.records.latency.acquire-point.median\endcsname{529.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-point.median\endcsname{$+$529.0}
\expandafter\def\csname val@uiv.records.latency.acquire-point.n\endcsname{1860}
\expandafter\def\csname cnt@uiv.records.latency.acquire-point.n\endcsname{1{,}860}
\expandafter\def\csname pct@uiv.records.latency.acquire-point.n\endcsname{186000.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-point.n\endcsname{$+$186000.0}
\expandafter\def\csname val@uiv.records.latency.acquire-point.p90\endcsname{7.530}
\expandafter\def\csname cnt@uiv.records.latency.acquire-point.p90\endcsname{8}
\expandafter\def\csname pct@uiv.records.latency.acquire-point.p90\endcsname{753.0}
\expandafter\def\csname ppt@uiv.records.latency.acquire-point.p90\endcsname{$+$753.0}
\expandafter\def\csname val@uiv.records.latency.direct.mean\endcsname{4.860}
\expandafter\def\csname cnt@uiv.records.latency.direct.mean\endcsname{5}
\expandafter\def\csname pct@uiv.records.latency.direct.mean\endcsname{486.0}
\expandafter\def\csname ppt@uiv.records.latency.direct.mean\endcsname{$+$486.0}
\expandafter\def\csname val@uiv.records.latency.direct.median\endcsname{5.270}
\expandafter\def\csname cnt@uiv.records.latency.direct.median\endcsname{5}
\expandafter\def\csname pct@uiv.records.latency.direct.median\endcsname{527.0}
\expandafter\def\csname ppt@uiv.records.latency.direct.median\endcsname{$+$527.0}
\expandafter\def\csname val@uiv.records.latency.direct.n\endcsname{2407}
\expandafter\def\csname cnt@uiv.records.latency.direct.n\endcsname{2{,}407}
\expandafter\def\csname pct@uiv.records.latency.direct.n\endcsname{240700.0}
\expandafter\def\csname ppt@uiv.records.latency.direct.n\endcsname{$+$240700.0}
\expandafter\def\csname val@uiv.records.latency.direct.p90\endcsname{7.710}
\expandafter\def\csname cnt@uiv.records.latency.direct.p90\endcsname{8}
\expandafter\def\csname pct@uiv.records.latency.direct.p90\endcsname{771.0}
\expandafter\def\csname ppt@uiv.records.latency.direct.p90\endcsname{$+$771.0}
\expandafter\def\csname val@uiv.records.latency.read.mean\endcsname{6.100}
\expandafter\def\csname cnt@uiv.records.latency.read.mean\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.read.mean\endcsname{610.0}
\expandafter\def\csname ppt@uiv.records.latency.read.mean\endcsname{$+$610.0}
\expandafter\def\csname val@uiv.records.latency.read.median\endcsname{6.030}
\expandafter\def\csname cnt@uiv.records.latency.read.median\endcsname{6}
\expandafter\def\csname pct@uiv.records.latency.read.median\endcsname{603.0}
\expandafter\def\csname ppt@uiv.records.latency.read.median\endcsname{$+$603.0}
\expandafter\def\csname val@uiv.records.latency.read.n\endcsname{8011}
\expandafter\def\csname cnt@uiv.records.latency.read.n\endcsname{8{,}011}
\expandafter\def\csname pct@uiv.records.latency.read.n\endcsname{801100.0}
\expandafter\def\csname ppt@uiv.records.latency.read.n\endcsname{$+$801100.0}
\expandafter\def\csname val@uiv.records.latency.read.p90\endcsname{8.280}
\expandafter\def\csname cnt@uiv.records.latency.read.p90\endcsname{8}
\expandafter\def\csname pct@uiv.records.latency.read.p90\endcsname{828.0}
\expandafter\def\csname ppt@uiv.records.latency.read.p90\endcsname{$+$828.0}
\expandafter\def\csname val@uiv.records.model-id-match.haiku\endcsname{3532}
\expandafter\def\csname cnt@uiv.records.model-id-match.haiku\endcsname{3{,}532}
\expandafter\def\csname pct@uiv.records.model-id-match.haiku\endcsname{353200.0}
\expandafter\def\csname ppt@uiv.records.model-id-match.haiku\endcsname{$+$353200.0}
\expandafter\def\csname val@uiv.records.model-id-match.opus\endcsname{6636}
\expandafter\def\csname cnt@uiv.records.model-id-match.opus\endcsname{6{,}636}
\expandafter\def\csname pct@uiv.records.model-id-match.opus\endcsname{663600.0}
\expandafter\def\csname ppt@uiv.records.model-id-match.opus\endcsname{$+$663600.0}
\expandafter\def\csname val@uiv.records.model-id-match.sonnet\endcsname{6580}
\expandafter\def\csname cnt@uiv.records.model-id-match.sonnet\endcsname{6{,}580}
\expandafter\def\csname pct@uiv.records.model-id-match.sonnet\endcsname{658000.0}
\expandafter\def\csname ppt@uiv.records.model-id-match.sonnet\endcsname{$+$658000.0}
\expandafter\def\csname val@uiv.records.model-id-mismatches\endcsname{0}
\expandafter\def\csname cnt@uiv.records.model-id-mismatches\endcsname{0}
\expandafter\def\csname pct@uiv.records.model-id-mismatches\endcsname{0.0}
\expandafter\def\csname ppt@uiv.records.model-id-mismatches\endcsname{0.0}
\expandafter\def\csname val@uiv.records.model.haiku\endcsname{4220}
\expandafter\def\csname cnt@uiv.records.model.haiku\endcsname{4{,}220}
\expandafter\def\csname pct@uiv.records.model.haiku\endcsname{422000.0}
\expandafter\def\csname ppt@uiv.records.model.haiku\endcsname{$+$422000.0}
\expandafter\def\csname val@uiv.records.model.opus\endcsname{8038}
\expandafter\def\csname cnt@uiv.records.model.opus\endcsname{8{,}038}
\expandafter\def\csname pct@uiv.records.model.opus\endcsname{803800.0}
\expandafter\def\csname ppt@uiv.records.model.opus\endcsname{$+$803800.0}
\expandafter\def\csname val@uiv.records.model.sonnet\endcsname{7921}
\expandafter\def\csname cnt@uiv.records.model.sonnet\endcsname{7{,}921}
\expandafter\def\csname pct@uiv.records.model.sonnet\endcsname{792100.0}
\expandafter\def\csname ppt@uiv.records.model.sonnet\endcsname{$+$792100.0}
\expandafter\def\csname val@uiv.records.ok-requests\endcsname{16748}
\expandafter\def\csname cnt@uiv.records.ok-requests\endcsname{16{,}748}
\expandafter\def\csname pct@uiv.records.ok-requests\endcsname{1674800.0}
\expandafter\def\csname ppt@uiv.records.ok-requests\endcsname{$+$1674800.0}
\expandafter\def\csname val@uiv.records.requests\endcsname{20179}
\expandafter\def\csname cnt@uiv.records.requests\endcsname{20{,}179}
\expandafter\def\csname pct@uiv.records.requests\endcsname{2017900.0}
\expandafter\def\csname ppt@uiv.records.requests\endcsname{$+$2017900.0}
\expandafter\def\csname val@uiv.records.status.harness-failed\endcsname{2953}
\expandafter\def\csname cnt@uiv.records.status.harness-failed\endcsname{2{,}953}
\expandafter\def\csname pct@uiv.records.status.harness-failed\endcsname{295300.0}
\expandafter\def\csname ppt@uiv.records.status.harness-failed\endcsname{$+$295300.0}
\expandafter\def\csname val@uiv.records.status.missing-in-journal\endcsname{478}
\expandafter\def\csname cnt@uiv.records.status.missing-in-journal\endcsname{478}
\expandafter\def\csname pct@uiv.records.status.missing-in-journal\endcsname{47800.0}
\expandafter\def\csname ppt@uiv.records.status.missing-in-journal\endcsname{$+$47800.0}
\expandafter\def\csname val@uiv.records.status.ok\endcsname{16748}
\expandafter\def\csname cnt@uiv.records.status.ok\endcsname{16{,}748}
\expandafter\def\csname pct@uiv.records.status.ok\endcsname{1674800.0}
\expandafter\def\csname ppt@uiv.records.status.ok\endcsname{$+$1674800.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-box.api-calls\endcsname{3.700}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-box.api-calls\endcsname{4}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-box.api-calls\endcsname{370.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-box.api-calls\endcsname{$+$370.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{19341.200}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{19{,}341}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{1934120.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-box.cache-creation-input-tokens\endcsname{$+$1934120.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{128467.200}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{128{,}467}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{12846720.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-box.cache-read-input-tokens\endcsname{$+$12846720.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-box.input-tokens\endcsname{6.900}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-box.input-tokens\endcsname{7}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-box.input-tokens\endcsname{690.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-box.input-tokens\endcsname{$+$690.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-box.output-tokens\endcsname{529.900}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-box.output-tokens\endcsname{530}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-box.output-tokens\endcsname{52990.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-box.output-tokens\endcsname{$+$52990.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-box.thinking-tokens\endcsname{157.200}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-box.thinking-tokens\endcsname{157}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-box.thinking-tokens\endcsname{15720.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-box.thinking-tokens\endcsname{$+$15720.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-cell.api-calls\endcsname{4.700}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-cell.api-calls\endcsname{5}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-cell.api-calls\endcsname{470.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-cell.api-calls\endcsname{$+$470.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{26031.400}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{26{,}031}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{2603140.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-cell.cache-creation-input-tokens\endcsname{$+$2603140.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{171809.000}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{171{,}809}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{17180900.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-cell.cache-read-input-tokens\endcsname{$+$17180900.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-cell.input-tokens\endcsname{9.100}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-cell.input-tokens\endcsname{9}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-cell.input-tokens\endcsname{910.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-cell.input-tokens\endcsname{$+$910.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-cell.output-tokens\endcsname{964.500}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-cell.output-tokens\endcsname{964}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-cell.output-tokens\endcsname{96450.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-cell.output-tokens\endcsname{$+$96450.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{227.300}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{227}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{22730.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-cell.thinking-tokens\endcsname{$+$22730.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{4.500}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{4}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{450.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual-refine.api-calls\endcsname{$+$450.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{23924.300}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{23{,}924}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{2392430.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual-refine.cache-creation-input-tokens\endcsname{$+$2392430.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{166189.400}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{166{,}189}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{16618940.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual-refine.cache-read-input-tokens\endcsname{$+$16618940.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{8.800}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{9}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{880.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual-refine.input-tokens\endcsname{$+$880.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{978.900}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{979}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{97890.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual-refine.output-tokens\endcsname{$+$97890.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{232.100}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{232}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{23210.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual-refine.thinking-tokens\endcsname{$+$23210.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual.api-calls\endcsname{3.400}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual.api-calls\endcsname{3}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual.api-calls\endcsname{340.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual.api-calls\endcsname{$+$340.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{18315.300}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{18{,}315}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{1831530.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual.cache-creation-input-tokens\endcsname{$+$1831530.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{117034.600}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{117{,}035}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{11703460.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual.cache-read-input-tokens\endcsname{$+$11703460.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual.input-tokens\endcsname{6.300}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual.input-tokens\endcsname{6}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual.input-tokens\endcsname{630.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual.input-tokens\endcsname{$+$630.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual.output-tokens\endcsname{520.200}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual.output-tokens\endcsname{520}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual.output-tokens\endcsname{52020.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual.output-tokens\endcsname{$+$52020.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{166.900}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{167}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{16690.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-dual.thinking-tokens\endcsname{$+$16690.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-point.api-calls\endcsname{3.700}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-point.api-calls\endcsname{4}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-point.api-calls\endcsname{370.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-point.api-calls\endcsname{$+$370.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{20771.100}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{20{,}771}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{2077110.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-point.cache-creation-input-tokens\endcsname{$+$2077110.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{131087.000}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{131{,}087}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{13108700.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-point.cache-read-input-tokens\endcsname{$+$13108700.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-point.input-tokens\endcsname{7.200}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-point.input-tokens\endcsname{7}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-point.input-tokens\endcsname{720.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-point.input-tokens\endcsname{$+$720.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-point.output-tokens\endcsname{510.100}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-point.output-tokens\endcsname{510}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-point.output-tokens\endcsname{51010.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-point.output-tokens\endcsname{$+$51010.0}
\expandafter\def\csname val@uiv.records.usage-per-request.acquire-point.thinking-tokens\endcsname{144.400}
\expandafter\def\csname cnt@uiv.records.usage-per-request.acquire-point.thinking-tokens\endcsname{144}
\expandafter\def\csname pct@uiv.records.usage-per-request.acquire-point.thinking-tokens\endcsname{14440.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.acquire-point.thinking-tokens\endcsname{$+$14440.0}
\expandafter\def\csname val@uiv.records.usage-per-request.direct.api-calls\endcsname{3.500}
\expandafter\def\csname cnt@uiv.records.usage-per-request.direct.api-calls\endcsname{4}
\expandafter\def\csname pct@uiv.records.usage-per-request.direct.api-calls\endcsname{350.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.direct.api-calls\endcsname{$+$350.0}
\expandafter\def\csname val@uiv.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{19131.100}
\expandafter\def\csname cnt@uiv.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{19{,}131}
\expandafter\def\csname pct@uiv.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{1913110.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.direct.cache-creation-input-tokens\endcsname{$+$1913110.0}
\expandafter\def\csname val@uiv.records.usage-per-request.direct.cache-read-input-tokens\endcsname{120525.400}
\expandafter\def\csname cnt@uiv.records.usage-per-request.direct.cache-read-input-tokens\endcsname{120{,}525}
\expandafter\def\csname pct@uiv.records.usage-per-request.direct.cache-read-input-tokens\endcsname{12052540.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.direct.cache-read-input-tokens\endcsname{$+$12052540.0}
\expandafter\def\csname val@uiv.records.usage-per-request.direct.input-tokens\endcsname{6.600}
\expandafter\def\csname cnt@uiv.records.usage-per-request.direct.input-tokens\endcsname{7}
\expandafter\def\csname pct@uiv.records.usage-per-request.direct.input-tokens\endcsname{660.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.direct.input-tokens\endcsname{$+$660.0}
\expandafter\def\csname val@uiv.records.usage-per-request.direct.output-tokens\endcsname{475.600}
\expandafter\def\csname cnt@uiv.records.usage-per-request.direct.output-tokens\endcsname{476}
\expandafter\def\csname pct@uiv.records.usage-per-request.direct.output-tokens\endcsname{47560.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.direct.output-tokens\endcsname{$+$47560.0}
\expandafter\def\csname val@uiv.records.usage-per-request.direct.thinking-tokens\endcsname{147.900}
\expandafter\def\csname cnt@uiv.records.usage-per-request.direct.thinking-tokens\endcsname{148}
\expandafter\def\csname pct@uiv.records.usage-per-request.direct.thinking-tokens\endcsname{14790.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.direct.thinking-tokens\endcsname{$+$14790.0}
\expandafter\def\csname val@uiv.records.usage-per-request.read.api-calls\endcsname{4.500}
\expandafter\def\csname cnt@uiv.records.usage-per-request.read.api-calls\endcsname{4}
\expandafter\def\csname pct@uiv.records.usage-per-request.read.api-calls\endcsname{450.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.read.api-calls\endcsname{$+$450.0}
\expandafter\def\csname val@uiv.records.usage-per-request.read.cache-creation-input-tokens\endcsname{25061.800}
\expandafter\def\csname cnt@uiv.records.usage-per-request.read.cache-creation-input-tokens\endcsname{25{,}062}
\expandafter\def\csname pct@uiv.records.usage-per-request.read.cache-creation-input-tokens\endcsname{2506180.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.read.cache-creation-input-tokens\endcsname{$+$2506180.0}
\expandafter\def\csname val@uiv.records.usage-per-request.read.cache-read-input-tokens\endcsname{163838.800}
\expandafter\def\csname cnt@uiv.records.usage-per-request.read.cache-read-input-tokens\endcsname{163{,}839}
\expandafter\def\csname pct@uiv.records.usage-per-request.read.cache-read-input-tokens\endcsname{16383880.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.read.cache-read-input-tokens\endcsname{$+$16383880.0}
\expandafter\def\csname val@uiv.records.usage-per-request.read.input-tokens\endcsname{8.800}
\expandafter\def\csname cnt@uiv.records.usage-per-request.read.input-tokens\endcsname{9}
\expandafter\def\csname pct@uiv.records.usage-per-request.read.input-tokens\endcsname{880.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.read.input-tokens\endcsname{$+$880.0}
\expandafter\def\csname val@uiv.records.usage-per-request.read.output-tokens\endcsname{878.600}
\expandafter\def\csname cnt@uiv.records.usage-per-request.read.output-tokens\endcsname{879}
\expandafter\def\csname pct@uiv.records.usage-per-request.read.output-tokens\endcsname{87860.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.read.output-tokens\endcsname{$+$87860.0}
\expandafter\def\csname val@uiv.records.usage-per-request.read.thinking-tokens\endcsname{184.800}
\expandafter\def\csname cnt@uiv.records.usage-per-request.read.thinking-tokens\endcsname{185}
\expandafter\def\csname pct@uiv.records.usage-per-request.read.thinking-tokens\endcsname{18480.0}
\expandafter\def\csname ppt@uiv.records.usage-per-request.read.thinking-tokens\endcsname{$+$18480.0}
\expandafter\def\csname val@uiv.records.usage.api-calls\endcsname{83428}
\expandafter\def\csname cnt@uiv.records.usage.api-calls\endcsname{83{,}428}
\expandafter\def\csname pct@uiv.records.usage.api-calls\endcsname{8342800.0}
\expandafter\def\csname ppt@uiv.records.usage.api-calls\endcsname{$+$8342800.0}
\expandafter\def\csname val@uiv.records.usage.cache-creation-input-tokens\endcsname{461347974}
\expandafter\def\csname cnt@uiv.records.usage.cache-creation-input-tokens\endcsname{461{,}347{,}974}
\expandafter\def\csname pct@uiv.records.usage.cache-creation-input-tokens\endcsname{46134797400.0}
\expandafter\def\csname ppt@uiv.records.usage.cache-creation-input-tokens\endcsname{$+$46134797400.0}
\expandafter\def\csname val@uiv.records.usage.cache-read-input-tokens\endcsname{3011023868}
\expandafter\def\csname cnt@uiv.records.usage.cache-read-input-tokens\endcsname{3{,}011{,}023{,}868}
\expandafter\def\csname pct@uiv.records.usage.cache-read-input-tokens\endcsname{301102386800.0}
\expandafter\def\csname ppt@uiv.records.usage.cache-read-input-tokens\endcsname{$+$301102386800.0}
\expandafter\def\csname val@uiv.records.usage.input-tokens\endcsname{162100}
\expandafter\def\csname cnt@uiv.records.usage.input-tokens\endcsname{162{,}100}
\expandafter\def\csname pct@uiv.records.usage.input-tokens\endcsname{16210000.0}
\expandafter\def\csname ppt@uiv.records.usage.input-tokens\endcsname{$+$16210000.0}
\expandafter\def\csname val@uiv.records.usage.output-tokens\endcsname{15014989}
\expandafter\def\csname cnt@uiv.records.usage.output-tokens\endcsname{15{,}014{,}989}
\expandafter\def\csname pct@uiv.records.usage.output-tokens\endcsname{1501498900.0}
\expandafter\def\csname ppt@uiv.records.usage.output-tokens\endcsname{$+$1501498900.0}
\expandafter\def\csname val@uiv.records.usage.thinking-tokens\endcsname{3630144}
\expandafter\def\csname cnt@uiv.records.usage.thinking-tokens\endcsname{3{,}630{,}144}
\expandafter\def\csname pct@uiv.records.usage.thinking-tokens\endcsname{363014400.0}
\expandafter\def\csname ppt@uiv.records.usage.thinking-tokens\endcsname{$+$363014400.0}
\expandafter\def\csname val@uiv.tasks.A.n-apps\endcsname{8}
\expandafter\def\csname cnt@uiv.tasks.A.n-apps\endcsname{8}
\expandafter\def\csname pct@uiv.tasks.A.n-apps\endcsname{800.0}
\expandafter\def\csname ppt@uiv.tasks.A.n-apps\endcsname{$+$800.0}
\expandafter\def\csname val@uiv.tasks.A.n-tasks\endcsname{64}
\expandafter\def\csname cnt@uiv.tasks.A.n-tasks\endcsname{64}
\expandafter\def\csname pct@uiv.tasks.A.n-tasks\endcsname{6400.0}
\expandafter\def\csname ppt@uiv.tasks.A.n-tasks\endcsname{$+$6400.0}
\expandafter\def\csname val@uiv.tasks.C.n-apps\endcsname{12}
\expandafter\def\csname cnt@uiv.tasks.C.n-apps\endcsname{12}
\expandafter\def\csname pct@uiv.tasks.C.n-apps\endcsname{1200.0}
\expandafter\def\csname ppt@uiv.tasks.C.n-apps\endcsname{$+$1200.0}
\expandafter\def\csname val@uiv.tasks.C.n-tasks\endcsname{96}
\expandafter\def\csname cnt@uiv.tasks.C.n-tasks\endcsname{96}
\expandafter\def\csname pct@uiv.tasks.C.n-tasks\endcsname{9600.0}
\expandafter\def\csname ppt@uiv.tasks.C.n-tasks\endcsname{$+$9600.0}
\expandafter\def\csname val@uiv.tasks.T.n-apps\endcsname{24}
\expandafter\def\csname cnt@uiv.tasks.T.n-apps\endcsname{24}
\expandafter\def\csname pct@uiv.tasks.T.n-apps\endcsname{2400.0}
\expandafter\def\csname ppt@uiv.tasks.T.n-apps\endcsname{$+$2400.0}
\expandafter\def\csname val@uiv.tasks.T.n-tasks\endcsname{144}
\expandafter\def\csname cnt@uiv.tasks.T.n-tasks\endcsname{144}
\expandafter\def\csname pct@uiv.tasks.T.n-tasks\endcsname{14400.0}
\expandafter\def\csname ppt@uiv.tasks.T.n-tasks\endcsname{$+$14400.0}
\expandafter\def\csname val@uiv.tasks.n-apps\endcsname{44}
\expandafter\def\csname cnt@uiv.tasks.n-apps\endcsname{44}
\expandafter\def\csname pct@uiv.tasks.n-apps\endcsname{4400.0}
\expandafter\def\csname ppt@uiv.tasks.n-apps\endcsname{$+$4400.0}
\expandafter\def\csname val@uiv.tasks.n-tasks\endcsname{304}
\expandafter\def\csname cnt@uiv.tasks.n-tasks\endcsname{304}
\expandafter\def\csname pct@uiv.tasks.n-tasks\endcsname{30400.0}
\expandafter\def\csname ppt@uiv.tasks.n-tasks\endcsname{$+$30400.0}
\makeatother

